Guiding ChatGPT to Fix Web UI Tests via Explanation-Consistency Checking

The rapid evolution of Web UI incurs time and effort in UI test maintenance. Prior techniques in Web UI test repair focus on locating the target elements on the new Webpage that match the old ones so that the corresponding broken statements can be repaired. These techniques usually rely on prioritizing certain attributes (e.g., XPath) during matching where the similarity of certain attributes is ranked before other attributes, indicating that there may be bias towards certain attributes during matching. To mitigate the bias, we present the first study that investigates the feasibility of using prior Web UI repair techniques for initial matching and then using ChatGPT to perform subsequent matching. Our key insight is that given a list of elements matched by prior techniques, ChatGPT can leverage language understanding to perform subsequent matching and use its code generation model for fixing the broken statements. To mitigate hallucination in ChatGPT, we design an explanation validator that checks if the provided explanation for the matching results is consistent, and provides hints to ChatGPT via a self-correction prompt to further improve its results. Our evaluation on a widely used dataset shows that the ChatGPT-enhanced techniques improve the effectiveness of existing Web test repair techniques. Our study also shares several important insights in improving future Web UI test repair techniques.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> authors.tex <==
\author{Ridwan Shariffdeen}
% \authornote{Both authors contributed equally to the paper}
\authornote{Joint first authors}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
 }
\email{ridwan@comp.nus.edu.sg}

\author{Xiang Gao}
\authornotemark[1]
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }
\email{gaoxiang@comp.nus.edu.sg}

\author{Gregory J. Duck}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }

\email{gregory@comp.nus.edu.sg}


\author{Shin Hwei Tan}
\authornote{corresponding author}
\affiliation{\institution{Southern University of Science and Technology\country{China}}}

\email{tansh3@sustech.edu.cn}

\author{Julia Lawall}
\affiliation{%
 \institution{Inria}
  \country{France}
 }

\email{julia.lawall@inria.fr}


\author{Abhik Roychoudhury}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }
  
\email{abhik@comp.nus.edu.sg}

==> cover.tex <==
% \documentclass[10pt,journal,onecolumn]{IEEEtran}
% \usepackage{color}
% \setlength\parindent{0pt}

% \begin{document}
% First of all, we would like thank all the reviewers for their constructive comments and suggestions. We have revised our submission accordingly. This letter summarises our revisions to the paper and lists our responses to the reviewers' comments. \\
% \hrule
% \vspace{5pt}


% {\color{red}{\underline{Comment 1}}} - \textbf{Explain why gaps larger than a single revision have been used in the experiments, justifying why these cases resemble the actual situations faced by developers.}

% {\color{cyan}{\underline{Response 1}}} - Yes, fixing tests across multi-version changes may not be realistic. In fact, we used single-version changes for the industrial dataset (as shown in Table IV), which is practical in an actual industrial environment.
% As for the open-source dataset, we utilized gaps larger than a single revision just to maintain consistency with the existing dataset (citation 4). So that, we can conduct comparison experiment with prior work.
% Moreover, if UITestFix is proved to be effective in fixing tests across multi-version changes, it should perform even better on single-version changes.
% We elaborated the discussion on dataset at Section VI.
% %Since the test cases we used refer to the existing paper ``An automated model-based approach to repair test suites of evolving web applications'', the selected applications and their versions also used in the paper.
% \newline



% {\color{red}{\underline{Comment 2}}} - \textbf{Report evidence about the benefit of the iterative matching.}

% {\color{cyan}{\underline{Response 2}}} - Thanks for pointing it out. We added an evaluation of the iterative algorithm. Figure 5 presents the number of correctly matched elements during the iterative process. 
% In the first iteration, only 908 elements were correctly matched, while the following three iterations successfully matched 1986, 1988, and 2157 elements. 
% The results indicate that the iterative process enhances the matching accuracy.
% More details have been added to Section VI-A.
% \newline



% {\color{red}{\underline{Comment 3}}} - 
% \textbf{Describe how the instrumentation is done in greater detail.}

% {\color{cyan}{\underline{Response 3}}} - 
% The instrumentation module utilizes aspect-oriented programming (AOP) instrumentation, adapted from VISTA, to instrument Selenium tests. 
% The AOP instrumentation dynamically instruments the invocations of \textit{WebDriver.findElement}, \textit{WebElement.findElement}, \textit{WebElement.click}, and other similar methods used for element locating and performing actions on elements. 
% The inserted code records the trace of actions and corresponding UI status before/after each action, allowing for a detailed analysis of the actions performed.
% We have add more details about instrumentation to Section V.
% \newline



% {\color{red}{\underline{Comment 4}}} - \textbf{Implements the writing improvements pointed out by individual reviewers.}

% {\color{cyan}{\underline{Response 4}}} - Thank all the reviewer for pointing out the writing issues. We revised the paper according to the suggestions and checked the problems in the paper carefully. All the revisions have been highlighted in the new version.
% \newline


% {\color{red}{\underline{Comment 5}}} - \textbf{Address as much as possible all other useful recommendations to improve the paper.}

% {\color{cyan}{\underline{Response 5}}} - We have adapted the reviewer's suggestions on the paper. More details can be found in the response to each reviewer's comments.
% % For example, 
% % % move the section MOTIVATING EXAMPLE to the front of the section BACKGROUND, and 
% % move the section DISCUSSION to the front of the section RELATED WORK and add a Threats to Validity paragraph.
% \newline\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441A}

% {\color{red}{\underline{Comment A-1}}} - \textbf{Whether the authors would allow the research community to access and/or use UITestFix at all, and if so, how?}

% {\color{cyan}{\underline{Response B-1}}} - We regret that we cannot make the core algorithm of UITestFix open source due to it being a proprietary project of a business company. 
% However, to enable the research community to reproduce our results, we have made the general framework of UI element matching and test case repair available at https://anonymous.4open.science/r/Web-UI-Dataset-9645. 
% Although the iterative algorithm has been omitted, the implementations of other tools and datasets are available for use. 
% We have made every effort to ensure that readers who are interested in UITestFix can reproduce our tool and experimental results.
% \newline

% {We have addressed all the writing issues pointed out by Reviewer-A. Thanks!}\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441B}

% {\color{red}{\underline{Comment B-1}}} - \textbf{Confusion about web UI datasets and page selection.}

% % I am also confused about the paper making a selection in terms of Web pages. Shouldn’t be the unit of selection the test cases that must be repaired, regardless of the number of pages used by these tests? Why are there so few pages selected per app?

% {\color{cyan}{\underline{Response B-1}}} - 
% We have two dataset: (1) \textit{UI match dataset} for element matching and (2) \textit{UI test dataset} for test repair.
% % The selection of web pages in the UI match dataset is unrelated to the UI test dataset.
% The selected UI tests may not be restricted to the selected web pages.
% Just as Reviewer-B suggested, we select the test cases that must be repaired, regardless of the number of pages used by these tests.
% We further clarified this in the dataset selection (Section Section VI).
% % The web UI dataset directly tests the algorithm's performance on page matching, corresponding to RQ1-2. 
% % The test data set tests the algorithm's performance in the repair test case, corresponding to RQ3.
% \newline
% % The web pages in the UI match dataset are not derived from the applications under test but are actual web pages. 
% % Due to the limited open-source test cases, the UI match dataset can cover more elements of webpages, which can better illustrate the algorithm's abilities. 
% % Some existing paper(citation 6) also select web page from actual web pages and selects one page from each application. 
% % Our dataset is enhanced from the paper's dataset and thus follows this setting.
% % 不要去说别人也这么做的。这个reviewer应该是误会了两个试验之间的关系，因此应该直接挑明web ui dataset 和 test case没有直接的关系。



% {\color{red}{\underline{Comment B-2}}} - \textbf{Why some elements should be excluded and they cannot be labeled with a special label to be used for the unclear cases?}

% % The paper refers to some elements that have not been labeled and thus have been excluded from the dataset. It is however unclear why they should be excluded and they cannot be labeled with a special label to be used for the unclear cases.}}

% {\color{cyan}{\underline{Response B-2}}} - 
% The labeling process does not only label the change types, but also annotate the matching pairs between the old and new versions, which are then served as the ground truth of element matching.
% We cannot measure the element matching correctness for unclear elements, which are labeled with special labels.
% We elaborated the explanation of labelling in Section VI.
% % The labelled elements in the web UI dataset are ground truth, which is used to count the correct matching rate.
% % Therefore, we only label the elements more sure.
% % In fact, the dataset we collected includes all elements, but only some elements without controversy have been annotated. 
% % Therefore, elements without annotated types can also be directly considered as a special type.
% % 直接说明，标注的数据是用来统计匹配的正确率的，也就是ground truth，所以应该标注清洗准确的元素。
% \newline


% % Some elements pose challenges when it comes to labeling.
% % Take content elements, like items in the Amazon application, for instance.
% % These elements may not have an explicit corresponding relationship in the new version. 
% % Weq have decided to exclude such elements from the labeling process to mitigate potential controversies.

% {\color{red}{\underline{Comment B-3}}} - \textbf{Test cases without assertions have been removed. Why?}

% {\color{cyan}{\underline{Response B-3}}} - 
% The assertion is used as the correctness specification for UITestFix.
% If UI test cases lack assertion statements, the incorrectly fixed test by UITestFix may not fail.
% Assertions could help UITestFix filter out some incorrect patches.
% We elaborated the discussion about test selection in Section VI.
% % We do this mainly for the following reasons:
% % 1) Lack of assertion statements. 
% % UI test cases may execute incorrectly but will not fail.
% % 润色该段落
% %2) Some test cases lacking assertion statements are of poor quality. 
% % For example, there is only one sentence in the test method of TestHomeSearch in AddressBook \textit{driver.findElement(By.xpath("//INPUT[@type='text']")).sendKeys( "Zeeshan");}. 
% % It isn't easy to judge the target of its test.
% % 3) Test cases in cooperative enterprises usually have assertions, so it is a better specification to have assertions.
% \newline\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441C}

% {\color{red}{\underline{Comment C-1}}} - \textbf{Concerns about the impact of flakiness on experimental results.}
% % The consideration for a correctly fixed test case is judged based on the test passing after the fix (while covering the original functionality it tests). I wonder if the authors considered cases of test flakiness across those results. Did you observe any tests that can fail nondeterministically? This can impact the validity of the tests. Even after the fix, if the test fails, it may be due to flakiness.

% {\color{cyan}{\underline{Response C-1}}} - During the experiment, we noticed that some UI test cases have been influenced by flakiness.
% % the problem of causing flakiness.
% To avoid the affect affecting the experimental results, we manually checked the elements performed.
% Repair framework can automatically take screenshots and mark the executed elements.
% When flakiness happens, we will rerun the test case.
% We elaborated the explanation of how to avoid flakiness in the experiment in Section VII. 
% \newline



% {\color{red}{\underline{Comment C-2}}} - \textbf{Concerns about the selection of exception types.}

% % In step one of the actions taken when executing the test of the earlier version, two elements-based exceptions are captured (NoSuchElementException and InvalidElementStateException). Why not include other types of Selenium runtime element exceptions (e.g., ElementClickInterceptedException), as those will also be causing the test to fail? This could also be similarly expanded to include attributes exception (e.g., NoSuch{\color{cyan}{\underline{Response ttributeException)

% {\color{cyan}{\underline{Response C-2}}} -
% We chose these two exception types mainly for the following reasons:
% 1) element-type crashes account for most test case crashes (citation 15), our tools mainly target this exception type. NoSuchElementException and InvalidElementStateException  
% are related to the element exception.
% Some other types of exceptions, such as NoSuchCookieException, are excluded, which are not directly caused by element locator changes, 
% 2)  exceptions extended from the type we catch (e.g., ElementClickInterceptedException) can also be caught.
% We elaborated the discussion about exceptions in Section V.
% % 我们try了多少个方法，这些方法抛出异常的主要类型是xxx
% %java中是否拥有python的那个异常，
% %调查webElement会抛出哪些异常，并且检查是否可能覆盖全。
% \newline



%  {\color{red}{\underline{Comment C-3}}} - \textbf{What do you mean it was ``translated" by researchers?}
% %  ``prior work mainly studied the maintenance of UI tests on open-source web apps with test cases written or translated by researchers" $-->$ 

% {\color{cyan}{\underline{Response C-3}}} - The ``translated" here means to transform the test case written by other Capture–Replay tools to the Selenium.
% The ``translate'' here follows the word in the existing paper (citation 4 P16).
% We elaborated the discussion about the meaning of ``translate'' in the Section I.
% %原来的编程语言是什么。转换成了什么
% % citation 4 P 16 :For our experiments, we used Selenium (The Selenium Project. http://seleniumhq.org/docs/03_webdriver.html/) as the underlying Capture–Replay tool for the experiments as the most-widely used, freely available, Capture–Replay tool. The test scripts of the six case studies were migrated to their Selenium equivalent by the experienced test engineer. This activity is similar to the prior studies of automated web testing (Leotta et al., 2015; Biagiola et al., 2019) that also migrate the test scripts of these six case studies to Selenium. All changes made during migration were syntactic to make the scripts compatible with Selenium Web Driver API. By executing both the original and translated test scripts, we confirmed that both are semantically equivalent and reveal the same number of defects. We also manually checked the conformance of the translated and original test scripts to ensure equivalence.
% \newline


% {\color{red}{\underline{Comment C-4}}} -  
% % "Moreover, UITESTFIX takes an average of 0.8685s to match an element, which we believe is acceptable." --> The paper reported the average time taken to match an element. However, o
% \textbf{P1 - One would like to see how this compares to existing matching techniques like SFTM. Also, why also include the fixed time (with the matching)?}

% {\color{cyan}{\underline{Response C-4}}} -
% % The RQ2 experimental testing was conducted after the web page information was saved locally. The main reason for not directly calculating the repair time is due to concerns about network fluctuations and time errors caused by fragmentation of test cases.
% We have compared this problem in RQ2, UITESTFIX
% and SFTM take a similar time to generate matching results
% (0.97s and 0.87s).
% We have revised the introduction and add the comparison result of two tools.
% More details can be found at RQ2.
% % RQ2已经比较了这个问题，我们工具花了多久，SFTM花了多久。
% % 我们已经修改了intro，more details can be found at RQ2
% \newline


% {\color{red}{\underline{Comment C-5}}} - \textbf{P7 - How many tests are there from each app? Please show the time taken to execute all tests (or estimated time) in ms. Why only 250 industrial test cases?}

% {\color{cyan}{\underline{Response C-5}}} -
% 1) In the latest version, there are 2,869 (52.67\%) tests for industrial $AppA$ and 2,578 (47.33\%) tests for $AppB$.
% 2) The company usually uses multiple machines to execute tests in parallel, which can usually be completed in two or three days.
% 3) It doesn't seem easy to experiment on all tests, and choosing 250 tests can be aligned with the number of tests in the existing work (citation 4).
% On the one hand, we need to run test case on the two versions of the applications, experiment with five algorithms, and check the repair results of each algorithm, which will take much time.
% On the other hand, operating large industrial applications will occupy a lot of resources, so the company only maintains the latest two application versions for testing.
% Therefore, We must finish the experiment before the next version comes.
% We added more details about the number of test cases in the Section VI.
% % , and we believe that 250 tests are large enough to represent the industrial test case dataset.
%  %润色该段落
% \newline



% % "The selected two industrial apps AppA and AppB have 5,839 test cases in total. As it is time-consuming to execute all tests, we randomly select the 250 test cases to execute." --> How many tests are there from each app? Also, if this is time-consuming, please show the time taken to execute all tests (or estimated time) in ms. Why only 250? Was this based on some sort of selection criteria or confidence level? A justification needs to be provided here. Later in the same paragraph, you stated that you had removed 46 further tests from the 250 selected, leaving you with 204 tests. Why didn’t you replace the 46 tests, then? To me, the 250 does not look representative of the >5800 tests available. If you want to select this based on a 95\% confidence level and 5\% confidence interval, then you should have around 360 tests in your selection.


% {\color{red}{\underline{Comment C-6}}} - \textbf{P8 - More detail about what reason for the one test can be fixed by WATER but cannot be fixed by UITESTFIX.}
% % "On the other hand, there is only one test case from the open-source dataset that cannot be fixed by UITESTFIX but fixed by other tools (WATER)." $\rightarrow$ Can you please include more details here on what could be the reason for that? This is an intresting outcome that is worth further discussion.


% {\color{cyan}{\underline{Response C-6}}} -
% The test case, that UITestFix failed to fix, needs to do a series of actions and then click ``add task'' button.
% After the web page update, UITestFix failed to match the ``add task'' button because this button was removed from the original page.
% In contrast,  WATER matches this button with an ``add task'' button from a different page.
% These two buttons are matched by WATER just because they simply have the same text.
% Since the matched ``add task'' button also completes the function of adding tasks and passes the assertion checking, this test is considered to be repaired successfully by WATER.
% We added more details to explain this test case in Section VI.
% % UITextfix fail to match this button,
% % In the app, the ``add task'' buttons appear on two different pages (home page and my task page), and the regions where the ``add task'' buttons are located are significantly different.
% % In the update, the ``add task'' button was moved to a different web page, making the regions where the ``add task'' buttons are located significantly different.
% % This is the reason that UITestFix failed to match the ``add task'' button in different page but the WATER correctly matches this element since it simply measures the similarity of the text.
% % In contrast, WATER correctly matches this element since it simply measures the similarity of the text, which is not changed in the web page update.
% % 没匹配上是因为这个按钮被删除了，但是WATER可以匹配上另一个页面上的。
% % The target of this test case is adding a task.
% % There are two ways to accomplish this function: 
% % 1) Click the ``task' button'' on the main page to jump to the ``My task'' page. 
% % Then click the ``add task'' button on the ``My task'' page to complete this function. 
% % 2) Complete this function by clicking the ``add task'' button of the ``My task'' module on the main page.
% % In the old version, the test case chooses method 1 for testing.
% % In the new version, UITESTFIX cannot match them due to the large difference between the regions where the two ``add task'' buttons are located, but WATER matches them by simply using the text attribute.
% % In the repair result of WATER, 1) the function of test case is completed, and 2) the assertion is passed.
% % So the repair is considered as a successful repair.
% % We consider this test case to be more fortuitous, and we don't describe it too much in the paper.
% % To clarify this situation more clearly, we further add some details to explain this test case in Section VI.
% % This test case is ``AddAndRemoveMultipleTasksTest'' for ``Collabtive'' app.
% % The test case, that UITestFIx failed to fix, needs to click a series of actions and then perform the ``add task'' button.
% % However, WATER chose the ``add task'' button in the different interface.
% % Although the ``add task'' button and the original ``add task'' button differ in the DOM area and neighbouring elements, the add task function can still be completed.
% % Therefore, we still regard it as a successful repair case according to our two repair success criteria (complete the original function and no fail).
% %是哪个元素重复出现了但是结构不同，我们认为这个情况属于偶然情况，可能缺乏进一步探讨的价值。
% % 从什么样子变成了什么样子，然后为什么WATER可以，我们不可以。为什么这个例子是不常见的。




% \vspace{35pt}
% Thank you again for your time and reviews.

% Best regards,

% Authors of paper 441
% \end{document}

==> introduction.tex <==
% \section{Introduction}
% Software Product Line Engineering (SPLE) promotes strategic, well-managed software reuse. In reality, however, reuse might be ad-hoc, often realized via artifact cloning. It has become increasingly common to create a variant software product, fix a defect or to add new feature by copying code fragments from similar context. Porting is particularly common in free and open source software projects, where code changes are ported across different versions of the same software or different projects altogether. Three types of porting can be identified based on the source and the target for the porting task, forward-porting, back-porting and cross-porting. Cross-porting is when the code is transferred between two different projects, while the former is within the same project but different versions. Forward-porting is when a patch is created to an older version and ported to the latest version, while back-porting is the when the patch is created to the latest version and ported back to an older version. Back-porting is usually easier and preferred since the latest API changes serve the purpose of supporting the writing of patches with less errors. When back-porting such code, the missing context and deviations can be taken from the latest version. However, when the patch is written to an old version, it may not fit the latest version and possibly would not behave correctly in the future versions as well. It's quite harder to take the missing pieces from the old kernel, because some of them might be removed with the purpose to discourage some behaviors or to force the developers to recheck some assumptions. 

% Currently backporting is typically done manually by a developer, on a case by case basis. The process of adapting a patch to fit into another context is tedious, time-consuming, error-prone and sometimes resulting in porting errors which cannot be detected at compile time. When developers port code from a reference to a target context, they usually expect the ported code to behave similarly. Chou et al report that a significant portion of operating system bugs come from ported edits~\cite{Chou2001}. Li et al. identify errors in Linux and FreeBSD resulting from developers forgetting to rename identifiers after porting code~\cite{Li2006}. Jiang et al present evidence of porting errors when similar code appears in different contexts~\cite{Jiang2007}. Porting error can also happen when developers evolve ported code differently~\cite{Juergens2009}. 

% Linux is an open-source operating system kernel that is evolving in a rapid rate since 1991. The Linux kernel runs on a multitude of devices ranging from servers to IoT devices. Given the increasing number of devices that depend on the Linux kernel and the rapid rate of evolution of the kernel, raises a challenge for device driver developers to ensure continuous availability of the driver code with the latest version of Linux kernel. One approach current device driver developers employ is to target the current mainline version of the Linux kernel, so that the driver code can be integrated into the Linux kernel distribution itself and maintained by the mainline kernel developers\cite{kernel-doc}. Some users however typically run older versions of the kernel which are considered to be more stable and such driver must be back ported to older kernel versions\cite{backport-framework}. 

% Linux back port project provides a compatibility library to mask the difference between the current mainline and the target stable version, which provides patches that allow a set of 800 drivers to target this compatibility library. Stable kernel version maintainers create these patches either manually or with the use of the transformation tool Coccinelle\cite{coccinelle}. In either case the developer has to determine where changes are needed in the code to back port and how to adapt the changes, which is tedious and error-prone. Thung et al presents a recommendation system that generates a ranked list of candidate transformations for backporting of Linux device drivers\cite{backport-framework}. Although they show a success rate of 68\% out of 100 device drivers, it is limited to transformation of a single line modification which cause a compiler error/warning. They focuse only on modification to an existing single statement which cause a compilation error, whereas a patch could be of multiple lines involving line insertions and deletions as well. Furthermore not all changes which are erroneous trigger any compiler error/warning message\cite{Zhen2018}.


% In this paper we propose a step further towards automating the backporting process by transforming patches from the mainline Linux into stable versions of Linux using a scalable, syntactic transformation learnt from the original mainline patch. Our approach accepts as input a patch in a given Linux version, the older stable Linux version to which the patch should be back ported (target Linux version) and the git repository that stores the changes to the Linux source code. First, our approach analyses the difference made in the original patch of the mainline Linux and extracts a transformation script, locate a similar context in the stable Linux version,  adapt the patch to the target context and apply the patch. The adaptation of the patch from the mainline Linux version into the target stable Linux version requires translation of any namespace differences, accounting the difference of the API calls, importing missing definitions and pruning of unnecessary modification which is not relevant for the target stable Linux version. 

% This paper makes the following contributions:

% \begin{itemize}
% 	\item {We present a technique implemented in a tool for vertical code transplantation that does not require developer to specify the patch location}
% 	\item {We evaluate \toolName ~effectiveness by transplanting 100 patches from mainline Linux kernel into a target stable version. We show that our tool can help developers fix bugs significantly better than manual process}
% \end{itemize}




==> sections/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/abstract.tex <==
\begin{abstract}

The rapid evolution of Web UI incurs time and effort in UI test maintenance. Prior techniques in Web UI test repair focus on locating the target elements on the new Webpage that match the old ones so that the corresponding broken statements can be repaired. These techniques usually rely on prioritizing certain attributes (e.g., XPath) during matching where the similarity of certain attributes is ranked before other attributes, indicating that there may be bias towards certain attributes during matching.
To mitigate the bias, we present the first study that investigates the feasibility of using prior Web UI repair techniques for initial matching and then using ChatGPT to perform subsequent matching. Our key insight is that given a list of elements matched by prior techniques, ChatGPT can leverage language understanding to perform subsequent matching and use its code generation model for fixing the broken statements.
To mitigate hallucination in ChatGPT, we design an explanation validator that checks if the provided explanation for the matching results is consistent, and provides hints to ChatGPT via a self-correction prompt to further improve its results. Our evaluation on a widely used dataset shows that the ChatGPT-enhanced techniques improve the effectiveness of existing Web test repair techniques. Our study also shares several important insights in improving future Web UI test repair techniques.

 %To understand the attribute prioritization in prior techniques, we conduct a study of existing techniques. Our study revealed that there may be bias towards certain attributes during matching.

 %As the attribute prioritization may be bias towards certain attributes, we propose mitigating  
 
% In the field of web UI test repair, the main target of research is the broken statement due to element locator failure. Generally, the element locators fail because the web pages are updated and the attributes of the elements change. Existing researches in repairing element locators focus on how to find elements on the new web page that match the old one so that the corresponding broken statements can be repaired. The main research questions in this article are how to use ChatGPT to handle the element matching and broken statement repairing tasks, and how reliable ChatGPT's results are. The article will answer these research questions and compare ChatGPT's effectiveness with existing repair tools (represented by WATER and VISTA) through experiments. The aim of this article is to investigate how ChatGPT can be utilized to perform well on web GUI script repair tasks inspired by existing technologies, with the expectation that ChatGPT will perform better than WATER and VISTA. Our experiments show that ChatGPT can successfully repair more broken statements than WATER and VISTA.


% \yuanzhang{I will rewrite this para after I've revised the paper.}

% Web UI test cases are used for the automatic testing of \delete{W}\add{w}eb applications. 
% When \add{a} \delete{W}\add{w}eb application is updated, these UI tests should also be updated for regression testing of the new version of \delete{W}\add{w}eb application.
% %However, in regression testing, many test cases will be broken due to the invalid element locators.
% % With the rapid evolution of Web applications, testers need to spend time updating the corresponding UI tests to validate the correctness of these applications. 
% With the rapid evolution, updating UI tests is a tedious and time-consuming task.
% To solve these problem\add{s}, automatically repairing \delete{W}\add{w}eb UI tests has gained increasing attention recently.
% % To better understand the challenges of repairing broken Web UI tests, we perform a case study of the Web UI test maintenance in open-source and an industrial app in \company. 
% % We perform a case study of \openteststudy{} tests in \openstudyapp{} open-source apps and \industryteststudy{} tests in an industrial app. Our study shows the rising demand for test repair and the complexity of the UI tests in our industrial app. Moreover, our study of \totdiff{} diff chunks from \totcommit{} commits revealed that repairing outdated locators is still one of the most commonly used repair types by the tester of the industrial app. Inspired by our study, 
% To repair \delete{W}\add{w}eb UI tests, the most important step is to match the UI elements before and after the \delete{W}\add{w}eb page update.
% Existing work match\add{es} UI elements according to visual information, attributes value, or Document Object Model (DOM) structures.
% However, they either achieve low element matching accuracy or only work on simple UI tests.
% To solve th\delete{o}\add{e}se problems, we proposed \toolName, an approach based on a novel iterative matching algorithm for improving the accuracy of matching UI elements.
% \toolName{} is designed based on two main insights: (1) beyond attribute and DOM structures, the relations between different elements can also guide the matching process, and (2) the matching results of previous iterations could guide the matching of the current iteration.
% % We design \toolName{} based on two key observations: (1) nodes with closer-matched ancestors are more similar, and (2) ancestors with more common leaf nodes are more similar.
% Our evaluation of publicly available datasets and \industryevalapp{} industrial apps shows that \toolName{} outperforms \numbaseline{} existing approaches by achieving more accurate element matching and producing more correct fixes.



\end{abstract}

==> sections/authors.tex <==
\author{Ridwan Shariffdeen}
% \authornote{Both authors contributed equally to the paper}
\authornote{Joint first authors}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
 }
\email{ridwan@comp.nus.edu.sg}

\author{Xiang Gao}
\authornotemark[1]
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }
\email{gaoxiang@comp.nus.edu.sg}

\author{Gregory J. Duck}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }

\email{gregory@comp.nus.edu.sg}


\author{Shin Hwei Tan}
\authornote{corresponding author}
\affiliation{\institution{Southern University of Science and Technology\country{China}}}

\email{tansh3@sustech.edu.cn}

\author{Julia Lawall}
\affiliation{%
 \institution{Inria}
  \country{France}
 }

\email{julia.lawall@inria.fr}


\author{Abhik Roychoudhury}
\affiliation{%
  \institution{National University of Singapore}
  \country{Singapore}
  }
  
\email{abhik@comp.nus.edu.sg}

==> sections/cover.tex <==
% \documentclass[10pt,journal,onecolumn]{IEEEtran}
% \usepackage{color}
% \setlength\parindent{0pt}

% \begin{document}
% First of all, we would like thank all the reviewers for their constructive comments and suggestions. We have revised our submission accordingly. This letter summarises our revisions to the paper and lists our responses to the reviewers' comments. \\
% \hrule
% \vspace{5pt}


% {\color{red}{\underline{Comment 1}}} - \textbf{Explain why gaps larger than a single revision have been used in the experiments, justifying why these cases resemble the actual situations faced by developers.}

% {\color{cyan}{\underline{Response 1}}} - Yes, fixing tests across multi-version changes may not be realistic. In fact, we used single-version changes for the industrial dataset (as shown in Table IV), which is practical in an actual industrial environment.
% As for the open-source dataset, we utilized gaps larger than a single revision just to maintain consistency with the existing dataset (citation 4). So that, we can conduct comparison experiment with prior work.
% Moreover, if UITestFix is proved to be effective in fixing tests across multi-version changes, it should perform even better on single-version changes.
% We elaborated the discussion on dataset at Section VI.
% %Since the test cases we used refer to the existing paper ``An automated model-based approach to repair test suites of evolving web applications'', the selected applications and their versions also used in the paper.
% \newline



% {\color{red}{\underline{Comment 2}}} - \textbf{Report evidence about the benefit of the iterative matching.}

% {\color{cyan}{\underline{Response 2}}} - Thanks for pointing it out. We added an evaluation of the iterative algorithm. Figure 5 presents the number of correctly matched elements during the iterative process. 
% In the first iteration, only 908 elements were correctly matched, while the following three iterations successfully matched 1986, 1988, and 2157 elements. 
% The results indicate that the iterative process enhances the matching accuracy.
% More details have been added to Section VI-A.
% \newline



% {\color{red}{\underline{Comment 3}}} - 
% \textbf{Describe how the instrumentation is done in greater detail.}

% {\color{cyan}{\underline{Response 3}}} - 
% The instrumentation module utilizes aspect-oriented programming (AOP) instrumentation, adapted from VISTA, to instrument Selenium tests. 
% The AOP instrumentation dynamically instruments the invocations of \textit{WebDriver.findElement}, \textit{WebElement.findElement}, \textit{WebElement.click}, and other similar methods used for element locating and performing actions on elements. 
% The inserted code records the trace of actions and corresponding UI status before/after each action, allowing for a detailed analysis of the actions performed.
% We have add more details about instrumentation to Section V.
% \newline



% {\color{red}{\underline{Comment 4}}} - \textbf{Implements the writing improvements pointed out by individual reviewers.}

% {\color{cyan}{\underline{Response 4}}} - Thank all the reviewer for pointing out the writing issues. We revised the paper according to the suggestions and checked the problems in the paper carefully. All the revisions have been highlighted in the new version.
% \newline


% {\color{red}{\underline{Comment 5}}} - \textbf{Address as much as possible all other useful recommendations to improve the paper.}

% {\color{cyan}{\underline{Response 5}}} - We have adapted the reviewer's suggestions on the paper. More details can be found in the response to each reviewer's comments.
% % For example, 
% % % move the section MOTIVATING EXAMPLE to the front of the section BACKGROUND, and 
% % move the section DISCUSSION to the front of the section RELATED WORK and add a Threats to Validity paragraph.
% \newline\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441A}

% {\color{red}{\underline{Comment A-1}}} - \textbf{Whether the authors would allow the research community to access and/or use UITestFix at all, and if so, how?}

% {\color{cyan}{\underline{Response B-1}}} - We regret that we cannot make the core algorithm of UITestFix open source due to it being a proprietary project of a business company. 
% However, to enable the research community to reproduce our results, we have made the general framework of UI element matching and test case repair available at https://anonymous.4open.science/r/Web-UI-Dataset-9645. 
% Although the iterative algorithm has been omitted, the implementations of other tools and datasets are available for use. 
% We have made every effort to ensure that readers who are interested in UITestFix can reproduce our tool and experimental results.
% \newline

% {We have addressed all the writing issues pointed out by Reviewer-A. Thanks!}\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441B}

% {\color{red}{\underline{Comment B-1}}} - \textbf{Confusion about web UI datasets and page selection.}

% % I am also confused about the paper making a selection in terms of Web pages. Shouldn’t be the unit of selection the test cases that must be repaired, regardless of the number of pages used by these tests? Why are there so few pages selected per app?

% {\color{cyan}{\underline{Response B-1}}} - 
% We have two dataset: (1) \textit{UI match dataset} for element matching and (2) \textit{UI test dataset} for test repair.
% % The selection of web pages in the UI match dataset is unrelated to the UI test dataset.
% The selected UI tests may not be restricted to the selected web pages.
% Just as Reviewer-B suggested, we select the test cases that must be repaired, regardless of the number of pages used by these tests.
% We further clarified this in the dataset selection (Section Section VI).
% % The web UI dataset directly tests the algorithm's performance on page matching, corresponding to RQ1-2. 
% % The test data set tests the algorithm's performance in the repair test case, corresponding to RQ3.
% \newline
% % The web pages in the UI match dataset are not derived from the applications under test but are actual web pages. 
% % Due to the limited open-source test cases, the UI match dataset can cover more elements of webpages, which can better illustrate the algorithm's abilities. 
% % Some existing paper(citation 6) also select web page from actual web pages and selects one page from each application. 
% % Our dataset is enhanced from the paper's dataset and thus follows this setting.
% % 不要去说别人也这么做的。这个reviewer应该是误会了两个试验之间的关系，因此应该直接挑明web ui dataset 和 test case没有直接的关系。



% {\color{red}{\underline{Comment B-2}}} - \textbf{Why some elements should be excluded and they cannot be labeled with a special label to be used for the unclear cases?}

% % The paper refers to some elements that have not been labeled and thus have been excluded from the dataset. It is however unclear why they should be excluded and they cannot be labeled with a special label to be used for the unclear cases.}}

% {\color{cyan}{\underline{Response B-2}}} - 
% The labeling process does not only label the change types, but also annotate the matching pairs between the old and new versions, which are then served as the ground truth of element matching.
% We cannot measure the element matching correctness for unclear elements, which are labeled with special labels.
% We elaborated the explanation of labelling in Section VI.
% % The labelled elements in the web UI dataset are ground truth, which is used to count the correct matching rate.
% % Therefore, we only label the elements more sure.
% % In fact, the dataset we collected includes all elements, but only some elements without controversy have been annotated. 
% % Therefore, elements without annotated types can also be directly considered as a special type.
% % 直接说明，标注的数据是用来统计匹配的正确率的，也就是ground truth，所以应该标注清洗准确的元素。
% \newline


% % Some elements pose challenges when it comes to labeling.
% % Take content elements, like items in the Amazon application, for instance.
% % These elements may not have an explicit corresponding relationship in the new version. 
% % Weq have decided to exclude such elements from the labeling process to mitigate potential controversies.

% {\color{red}{\underline{Comment B-3}}} - \textbf{Test cases without assertions have been removed. Why?}

% {\color{cyan}{\underline{Response B-3}}} - 
% The assertion is used as the correctness specification for UITestFix.
% If UI test cases lack assertion statements, the incorrectly fixed test by UITestFix may not fail.
% Assertions could help UITestFix filter out some incorrect patches.
% We elaborated the discussion about test selection in Section VI.
% % We do this mainly for the following reasons:
% % 1) Lack of assertion statements. 
% % UI test cases may execute incorrectly but will not fail.
% % 润色该段落
% %2) Some test cases lacking assertion statements are of poor quality. 
% % For example, there is only one sentence in the test method of TestHomeSearch in AddressBook \textit{driver.findElement(By.xpath("//INPUT[@type='text']")).sendKeys( "Zeeshan");}. 
% % It isn't easy to judge the target of its test.
% % 3) Test cases in cooperative enterprises usually have assertions, so it is a better specification to have assertions.
% \newline\\
% \hrule
% \vspace{5pt}


% \noindent\textbf{Review \#441C}

% {\color{red}{\underline{Comment C-1}}} - \textbf{Concerns about the impact of flakiness on experimental results.}
% % The consideration for a correctly fixed test case is judged based on the test passing after the fix (while covering the original functionality it tests). I wonder if the authors considered cases of test flakiness across those results. Did you observe any tests that can fail nondeterministically? This can impact the validity of the tests. Even after the fix, if the test fails, it may be due to flakiness.

% {\color{cyan}{\underline{Response C-1}}} - During the experiment, we noticed that some UI test cases have been influenced by flakiness.
% % the problem of causing flakiness.
% To avoid the affect affecting the experimental results, we manually checked the elements performed.
% Repair framework can automatically take screenshots and mark the executed elements.
% When flakiness happens, we will rerun the test case.
% We elaborated the explanation of how to avoid flakiness in the experiment in Section VII. 
% \newline



% {\color{red}{\underline{Comment C-2}}} - \textbf{Concerns about the selection of exception types.}

% % In step one of the actions taken when executing the test of the earlier version, two elements-based exceptions are captured (NoSuchElementException and InvalidElementStateException). Why not include other types of Selenium runtime element exceptions (e.g., ElementClickInterceptedException), as those will also be causing the test to fail? This could also be similarly expanded to include attributes exception (e.g., NoSuch{\color{cyan}{\underline{Response ttributeException)

% {\color{cyan}{\underline{Response C-2}}} -
% We chose these two exception types mainly for the following reasons:
% 1) element-type crashes account for most test case crashes (citation 15), our tools mainly target this exception type. NoSuchElementException and InvalidElementStateException  
% are related to the element exception.
% Some other types of exceptions, such as NoSuchCookieException, are excluded, which are not directly caused by element locator changes, 
% 2)  exceptions extended from the type we catch (e.g., ElementClickInterceptedException) can also be caught.
% We elaborated the discussion about exceptions in Section V.
% % 我们try了多少个方法，这些方法抛出异常的主要类型是xxx
% %java中是否拥有python的那个异常，
% %调查webElement会抛出哪些异常，并且检查是否可能覆盖全。
% \newline



%  {\color{red}{\underline{Comment C-3}}} - \textbf{What do you mean it was ``translated" by researchers?}
% %  ``prior work mainly studied the maintenance of UI tests on open-source web apps with test cases written or translated by researchers" $-->$ 

% {\color{cyan}{\underline{Response C-3}}} - The ``translated" here means to transform the test case written by other Capture–Replay tools to the Selenium.
% The ``translate'' here follows the word in the existing paper (citation 4 P16).
% We elaborated the discussion about the meaning of ``translate'' in the Section I.
% %原来的编程语言是什么。转换成了什么
% % citation 4 P 16 :For our experiments, we used Selenium (The Selenium Project. http://seleniumhq.org/docs/03_webdriver.html/) as the underlying Capture–Replay tool for the experiments as the most-widely used, freely available, Capture–Replay tool. The test scripts of the six case studies were migrated to their Selenium equivalent by the experienced test engineer. This activity is similar to the prior studies of automated web testing (Leotta et al., 2015; Biagiola et al., 2019) that also migrate the test scripts of these six case studies to Selenium. All changes made during migration were syntactic to make the scripts compatible with Selenium Web Driver API. By executing both the original and translated test scripts, we confirmed that both are semantically equivalent and reveal the same number of defects. We also manually checked the conformance of the translated and original test scripts to ensure equivalence.
% \newline


% {\color{red}{\underline{Comment C-4}}} -  
% % "Moreover, UITESTFIX takes an average of 0.8685s to match an element, which we believe is acceptable." --> The paper reported the average time taken to match an element. However, o
% \textbf{P1 - One would like to see how this compares to existing matching techniques like SFTM. Also, why also include the fixed time (with the matching)?}

% {\color{cyan}{\underline{Response C-4}}} -
% % The RQ2 experimental testing was conducted after the web page information was saved locally. The main reason for not directly calculating the repair time is due to concerns about network fluctuations and time errors caused by fragmentation of test cases.
% We have compared this problem in RQ2, UITESTFIX
% and SFTM take a similar time to generate matching results
% (0.97s and 0.87s).
% We have revised the introduction and add the comparison result of two tools.
% More details can be found at RQ2.
% % RQ2已经比较了这个问题，我们工具花了多久，SFTM花了多久。
% % 我们已经修改了intro，more details can be found at RQ2
% \newline


% {\color{red}{\underline{Comment C-5}}} - \textbf{P7 - How many tests are there from each app? Please show the time taken to execute all tests (or estimated time) in ms. Why only 250 industrial test cases?}

% {\color{cyan}{\underline{Response C-5}}} -
% 1) In the latest version, there are 2,869 (52.67\%) tests for industrial $AppA$ and 2,578 (47.33\%) tests for $AppB$.
% 2) The company usually uses multiple machines to execute tests in parallel, which can usually be completed in two or three days.
% 3) It doesn't seem easy to experiment on all tests, and choosing 250 tests can be aligned with the number of tests in the existing work (citation 4).
% On the one hand, we need to run test case on the two versions of the applications, experiment with five algorithms, and check the repair results of each algorithm, which will take much time.
% On the other hand, operating large industrial applications will occupy a lot of resources, so the company only maintains the latest two application versions for testing.
% Therefore, We must finish the experiment before the next version comes.
% We added more details about the number of test cases in the Section VI.
% % , and we believe that 250 tests are large enough to represent the industrial test case dataset.
%  %润色该段落
% \newline



% % "The selected two industrial apps AppA and AppB have 5,839 test cases in total. As it is time-consuming to execute all tests, we randomly select the 250 test cases to execute." --> How many tests are there from each app? Also, if this is time-consuming, please show the time taken to execute all tests (or estimated time) in ms. Why only 250? Was this based on some sort of selection criteria or confidence level? A justification needs to be provided here. Later in the same paragraph, you stated that you had removed 46 further tests from the 250 selected, leaving you with 204 tests. Why didn’t you replace the 46 tests, then? To me, the 250 does not look representative of the >5800 tests available. If you want to select this based on a 95\% confidence level and 5\% confidence interval, then you should have around 360 tests in your selection.


% {\color{red}{\underline{Comment C-6}}} - \textbf{P8 - More detail about what reason for the one test can be fixed by WATER but cannot be fixed by UITESTFIX.}
% % "On the other hand, there is only one test case from the open-source dataset that cannot be fixed by UITESTFIX but fixed by other tools (WATER)." $\rightarrow$ Can you please include more details here on what could be the reason for that? This is an intresting outcome that is worth further discussion.


% {\color{cyan}{\underline{Response C-6}}} -
% The test case, that UITestFix failed to fix, needs to do a series of actions and then click ``add task'' button.
% After the web page update, UITestFix failed to match the ``add task'' button because this button was removed from the original page.
% In contrast,  WATER matches this button with an ``add task'' button from a different page.
% These two buttons are matched by WATER just because they simply have the same text.
% Since the matched ``add task'' button also completes the function of adding tasks and passes the assertion checking, this test is considered to be repaired successfully by WATER.
% We added more details to explain this test case in Section VI.
% % UITextfix fail to match this button,
% % In the app, the ``add task'' buttons appear on two different pages (home page and my task page), and the regions where the ``add task'' buttons are located are significantly different.
% % In the update, the ``add task'' button was moved to a different web page, making the regions where the ``add task'' buttons are located significantly different.
% % This is the reason that UITestFix failed to match the ``add task'' button in different page but the WATER correctly matches this element since it simply measures the similarity of the text.
% % In contrast, WATER correctly matches this element since it simply measures the similarity of the text, which is not changed in the web page update.
% % 没匹配上是因为这个按钮被删除了，但是WATER可以匹配上另一个页面上的。
% % The target of this test case is adding a task.
% % There are two ways to accomplish this function: 
% % 1) Click the ``task' button'' on the main page to jump to the ``My task'' page. 
% % Then click the ``add task'' button on the ``My task'' page to complete this function. 
% % 2) Complete this function by clicking the ``add task'' button of the ``My task'' module on the main page.
% % In the old version, the test case chooses method 1 for testing.
% % In the new version, UITESTFIX cannot match them due to the large difference between the regions where the two ``add task'' buttons are located, but WATER matches them by simply using the text attribute.
% % In the repair result of WATER, 1) the function of test case is completed, and 2) the assertion is passed.
% % So the repair is considered as a successful repair.
% % We consider this test case to be more fortuitous, and we don't describe it too much in the paper.
% % To clarify this situation more clearly, we further add some details to explain this test case in Section VI.
% % This test case is ``AddAndRemoveMultipleTasksTest'' for ``Collabtive'' app.
% % The test case, that UITestFIx failed to fix, needs to click a series of actions and then perform the ``add task'' button.
% % However, WATER chose the ``add task'' button in the different interface.
% % Although the ``add task'' button and the original ``add task'' button differ in the DOM area and neighbouring elements, the add task function can still be completed.
% % Therefore, we still regard it as a successful repair case according to our two repair success criteria (complete the original function and no fail).
% %是哪个元素重复出现了但是结构不同，我们认为这个情况属于偶然情况，可能缺乏进一步探讨的价值。
% % 从什么样子变成了什么样子，然后为什么WATER可以，我们不可以。为什么这个例子是不常见的。




% \vspace{35pt}
% Thank you again for your time and reviews.

% Best regards,

% Authors of paper 441
% \end{document}

==> sections/discussion.tex <==
\section{Threats to Validity}
Additional programming languages. Because the experiments in this paper are based on a dataset composed of test cases written in Java, the results are only applicable to the repair of Java test cases. Even though we found ChatGPT would sometimes return repaired statements written in Python under flexible prompts, which means ChatGPT may have the ability in repairing broken statements with other programming languages, we reinforced prompt constraints to let ChatGPT give results in Java due to the limitations of the dataset.
% In the meanwhile, since the scripts test web UI instead of Android UI or others, the result only applies to web UI test repair.

Data leakage. Although the repository where we found the test cases for the old version of web applications did not include corresponding repaired scripts for updated web applications, it is difficult to know whether the data producers labeled the ground truths for these scripts as part of the training data of ChatGPT. However, since web applications update frequently, leading to many new versions already available, the probability that we and the data producers happen to choose the same versions as new versions are low. With a different version being the target version, the repair results might be different and will not cause data leakage. Even if the ground truths are in the training data, its effect may be tiny since it is a very small amount in about 45 TB of training data totally.~\cite{GPT3_data_amount}


Availability. Even though this article only examines the effectiveness of ChatGPT in web UI test repair, it shows the promise of LLMs in this field. Thus, even if ChatGPT cannot be used in the future due to various limitations, it can be replaced by other similar LLMs, such as Codex, which has been proven effective in the area of automotive program repair~\cite{codex}.



% %\subsection{Discussion}

% %In this section, we  present some real examples from our evaluation to understand the capabilities of \toolName.

% % \paragraph{Better than the developer patch.} Backporting patches is an error-prone task, in which developers can make mistakes.
% % In our evaluation, we find that~\toolName performs better than the developer in some cases.
% % For instance, the mainline patch at commit ID 45d73860\footnote{The detail of each commit can be found in https://kernel.googlesource.com/ pub/scm/linux/kernel/git/stable/linux-stable/+/COMMIT\_ID} %\textasciicircum!
% % fixes a bug in a usb driver, in which a delay is added to the function \verb+musb_h_tx_flush_fifo+. However, the developer backported this patch at commit ID 98b91bfa to a different function \verb+musb_host_tx+ in the same file although the original function \verb+musb_h_tx_flush_fifo+ exists in the old version. This patch was eventually reverted at commit ID c8443922 after 42 days.
% % In contrast, \toolName transforms the patch at the correct location. 

% % \paragraph{Semantically equivalent with the developer's patch.}
% % We find instances where~\toolName backports a patch in a syntactically different but semantically equivalent way as the developer.
% % The mainline patch at commit ID 74717b28 fixes a bug in the RTC interface.
% % This patch changes an if-condition by inserting a function call to \verb+ktime_before+.
% % Unfortunately, this function does not exist in v3.2.
% % When this patch was backported to v3.2 (commit ID 69328181), the developer improvised and replaced the function call with a semantically equivalent expression.
% % In contrast, \toolName imports the missing function \verb+ktime_before+ from the mainline to v3.2, resulting in a different, but semantically equivalent patch.


% % \paragraph{Incorrectly backported patch.}
% % We also find instances where the backported patch produced by \toolName has a different behavior from the developer patch.
% % The mainline patch at the commit 7809a611 fixes a regression error by inserting an API call \verb+IS_HASWELL+ with \verb+dev_priv+ as the first argument.
% % The developer who backported the patch to v3.2 in commit 2dd2c68e used a different variable \verb+dev+ as the first argument.
% % However, since the variable \verb+dev_priv+ exists in v3.2, \toolName does not change the argument \verb+dev_priv+ to \verb+dev+.
% % \toolName cannot disambiguate such cases, i.e. to keep the original argument \verb+dev_priv+, or to change it to \verb+dev+.

% % \paragraph{Internal DSL} \toolName's DSL allows expressing transformation rules that can be applied in a flexible way (i.e. for each target version, \toolName can decide whether the flexible predicates should be fixed or relaxed using the synthesis process). \toolName's DSL is only for internal use, to reduce the search space by considering a restricted language, rather than for communication with developers.  In the future, we could consider how to present the transformation rules using a syntax such as that of Coccinelle's DSL~\cite{coccinelle}, which is familiar to kernel developers. Note that the choice of DSL syntax is not a core contribution of this paper.


% \subsection{Threats to Validity}

% %During our exploratory study and evaluation, there are a series of threats that could affect the results.

% \noindent\textbf{External.} 
% Our findings of UI test maintenance focus on Web apps and may not generalize to UI apps (e.g., Java apps and Android apps).
% To ensure the general applicability of our \yz{tool}, we evaluate \toolName using both open datasets and industrial datasets.
% % Moreover, we ensure that the study and the evaluation dataset are different to avoid the problem of overfitting.
% When labelling UI elements in the dataset, two authors of the paper independently label each element, and discuss to resolve any disagreement.
% %label as many elements as possible and filter elements that are 
% %However, some elements are difficult to label.
% %To make the result more accurate, we dropped these elements.
% %To reduce errors caused by manual labeling, these elements in the open-source dataset labeled by one author and checked by another author.

% %\mytool{} may produce inaccurate concept matching if the student program and reference solution solve a programming problem with different algorithms. We mitigate this by following previous work~\cite{yang2019refactory,ahmed2022verifix,gulwani2018automated,wang2018search} to include correct students' programs (i.e., student submissions that pass all test cases) as additional reference solutions.

% % \mytool{} focus on evaluating incorrect student submissions. For 
% % In the future, we plan to extend
% % our approach to handle Object-Oriented Programming concepts. Additional complex features available in Python, such
% % as list comprehensions or lambda functions, are currently not
% % handled since novice students rarely utilize advanced concepts

% \noindent\textbf{Internal.} 
% Our automated tests may have bugs that can affect our reported results.
% We have made our experimental data and improved datasets publicly available to mitigate this threat. 
% %Our implementation of the CFG-based approach~\cite{vujovsevic2013software} may not be as effective as the original implementation for C programs. Nevertheless, as our concept graph uses the same CFG as basis for abstraction, our evaluation that compares the CFG approach and the abstracted CFG (our concept graph) ensures fair comparison of the two approaches.

% %To avoid problem of overfitting, we ensure that the study dataset and the evaluation dataset are different. To reduce the influence of different types of applications and pages on the evaluation results, we collected x pages from a total of x\todo{add exact number} applications, which were collected from open-source datasets and industrial datasets. Even so, it is not possible to evaluate on all types of applications and pages. Therefore, \toolName performs well in the evaluated dataset, but may perform differently in other types of applications.
% %In the process of labeling the dataset, we label as many elements as possible.
% %%However, some elements are difficult to label.
% %To make the result more accurate, we dropped these elements.
% %To reduce errors caused by manual labeling, these elements in the open-source dataset labeled by one author and checked by another author.

% %It is impossible to cover all the functions in the application with the open-source test cases of the existing work\cite{imtiaz2021automated}.
% %Different locator positioning methods will affect the execution of the test case %and affect the evaluation results.
% %To alleviate the impact of this problem, we also use open source test cases from another work on locator robustness research.

% % \paragraph{Limitations of \toolName}
% % Our implementation is based on LLVM/Clang, and thus inherits the limitations of that framework.  
% % %Specifically, while the LLVM/Clang AST preserves information about macros, it elides conditional compilation directives, e.g., \texttt{\#ifdef}s, according to the chosen configuration.
% % %Since handling all combinations of compilation options is not scalable, we try two sets of compilation options 1) set all the compilation directives as \texttt{Y} and 2) set all directives as \texttt{N}.
% % Since handling all combinations of compilation options is not scalable, when compiling the project, we only consider two sets of compilation options (see Section ~\ref{sec:implementation}).
% % This strategy works for most cases, but in some cases, it could result in certain un-compiled blocks of code being unavailable to \toolName, thus leading to incomplete backporting or even failure.
% % To alleviate this limitation, we allow users to specify the values of preprocessor variables according to their working environment. 

==> sections/evaluation.tex <==
\section{Evaluation}

We investigate the effectiveness of the combination of WATER, VISTA, and ChatGPT. First, we compare the results obtained by ChatGPT when using different candidates in matching and repairing: the candidates sorted by similarity based on \emph{XPath} edit distance or the candidates sorted by WATER and VISTA. Then we will compare the effectiveness of ChatGPT with WATER and VISTA. Previously, our experiments only studied the effect of ChatGPT on matching elements. In this chapter, we will study both the effect of matching elements and repairing broken statements based on the selected elements with the baseline of WATER and VISTA.



\subsection{Dataset}
We use an existing dataset~\cite{dataset} containing 5 open-source applications (3 of which are used in the release paper of VISTA). After deleting the repeated tests and the tests without assertion, there are 135 test cases.

Among these 135 scripts, 22 can be executed directly on the new version of the webpage and do not need to be fixed. We categorize these scripts under the "Exempt" column. Additionally, some scripts involve the addition or removal of modules or event, which means they can not be repaired by merely modifying the locator of original statements. Simultaneously, there are test cases that original locator points to the wrong element instead of throwing NoSuchElementException, making it challenging to identify the root cause of the breakage.  These have been marked under the "Irreparable" column. The column \emph{Repairable} shows the remaining 62 test cases, for which we manually labeled the ground truths. The column \emph{Broken Stm} specifies the corresponding number of broken statements within the repairable test cases, which we employ in the subsequent experiment.
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[H]
\caption{The number of test cases and broken statements}
\label{table:dataset}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\hline
\multicolumn{1}{l|}{Applications} &
  \multicolumn{1}{l}{Total} &
  \multicolumn{1}{l}{Exempt} &
  \multicolumn{1}{l}{Irreparable} &
  \multicolumn{1}{l}{Repairable} &
  \multicolumn{1}{l}{Broken Stm} \\ \hline
AddressBook & 16  & 8  & 6  & 2  & 2   \\
Claroline   & 31  & 0  & 4  & 27 & 53  \\
Collabtive  & 18  & 13 & 1  & 4  & 11  \\
MatnsiBt    & 45  & 1  & 19 & 25 & 66  \\
MRBS        & 25  & 0  & 21 & 4  & 7   \\ \hline
Total       & 135 & 22 & 51 & 62 & 139 \\ \hline
\end{tabular}%
}
\end{table}


% \begin{description}[leftmargin=*]
% \item[RQ6:] What is the performance of ChatGPT in the matching and repairing task with different kinds of candidate elements? 

% \item[RQ7:] Does the result of ChatGPT with these two kinds of candidates better than WATER and VISTA?
% \end{description}

\subsection{ChatGPT's Effectiveness on Matching}

The different repaired statements may all turn out to be right, as long as they correctly locate the corresponding updated element, and preserve the original intent of the test statement. In the process of repair, changing the locating strategy can be accepted. For example, even though the original test statement used id to locate the element, the correct repaired statement can use the updated element's \emph{XPath} or name as the locator. But it is important to ensure that the locator uses exact the value of the attribute according to the locating strategy. In addition to this, the test statement will involve operations on the element, such as clicking or sending keys, and this is the part that should not be changed during the repair. Similarly, if the test statement originally wants to assert whether the value of the element is equal to the expected value in order to determine whether the element is correctly located or whether the previous test procedure was wrong, then the original part of the assert statement should not be changed either.


Therefore, we will consider the below aspects to study the effectiveness of ChatGPT's repair result. First, whether ChatGPT has followed the prompt to modify only the locator of the statement, leaving the part of the test statement outside the locator unchanged. Then, we will check if ChatGPT changes the locating strategy. Further, we check whether it repairs the locator correctly, which includes the correct syntax as well as the correct attribute value. For the former, we will check whether the locator is able to locate a specific element. For the latter, we will investigate if ChatGPT correctly uses the attribute information of the element in the prompt to correctly locate the element it has selected. Finally, we check if the element's information corresponds to the given information of its selected element, and if the selected element is the ground truth element.





\subsection{The Effectiveness of ChatGPT with Different Candidate Lists}
\subsubsection{The Effectiveness of Matching}




Figure \ref{ExpResult} shows the effectiveness of ChatGPT with different candidate lists. Overall, it can be seen that ChatGPT performs well in both Stability and Mention Rate, with both exceeding 91\%; while ChatGPT's Correct Rate and Ground Truth Selected Rate also reach the range of 74\% to 86\%. Comparing the effects of different candidate types, it can be found that when using candidates generated by WATER+VISTA, ChatGPT performs better than using candidates generated by Edit Distance on almost all metrics except Correct Rate. Therefore, it can be seen that candidates generated by Edit Distance are more advantageous for ChatGPT's performance.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/content/FormalExpResult.png}
%     \caption{The Effectiveness of ChatGPT with Different Candidate Lists}
%     \label{ExpResult}
% \end{figure}

\subsubsection{The Effectiveness of Repair}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{The matching and repair results of different tools}
\label{table:result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccccc}
\hline
         & VISTA & WATER & XPath & sustech & VISTA+ChatGPT & WATER+ChatGPT & XPath+ChatGPT & Total \\ \hline
Matching & 62    & 78    & 42    & 122     & 51            & 71            & 107           & 132   \\
Repair   & 61    & 78    & 40    & 120     & 51            & 70            & 107           & 132   \\ \hline
\end{tabular}%
}
\end{table*}

% % 插入图片或表格并描述
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
% Candidates Selection &
%   \multicolumn{1}{l}{Total} &
%   \multicolumn{1}{l}{Locating Strategy} &
%   \multicolumn{1}{l}{Locator} &
%   \multicolumn{1}{l}{Others} &
%   \multicolumn{1}{l}{\# of Correct} &
%   \multicolumn{1}{l}{Correct Rate} \\ \midrule
% Edit Distance &
%   327 &
%   246 &
%   247 &
%   324 &
%   246 &
%   75.23\% \\
% WATER+VISTA &
%   327 &
%   268 &
%   230 &
%   323 &
%   230 &
%   70.34\% \\ \bottomrule
% \end{tabular}%
% }
% \caption{The repair result of ChatGPT with different candidate selection algorithms}
%     \label{repair_result1}
% \end{table}
Table \ref{repair_result1} shows the repair results of ChatGPT with different candidate selection algorithms. In each column, the first column \textbf{Candidates Selection} represents the different candidate selection algorithms used, the second column \textbf{Total} is the total number of repairs, the third column \textbf{Locating Strategy} refers to the number of times the locating strategy used during repair is identical to the broken statement, the fourth column \textbf{Locator} refers to the number of repairs where the locator can locate the selected element, the fifth column \textbf{Others} refers to the number of repairs where the part outside the locator can maintain its original meaning, the sixth column \textbf{Number of Correct} refers to the number of repairs where both the locator and the part outside the locator are correct, and the seventh column \textbf{Correct Rate} is obtained by dividing the ``Number of Correct'' by the total number of repairs. 


It can be seen that compared to using candidates generated by WATER+VISTA, ChatGPT has a slight advantage in all indicators except \textbf{Locating Strategy} when using candidates generated by Edit Distance. By comparing the performance of different indicators, it can be found that the number of repairs where the part outside the locator can maintain its original meaning is the largest, with almost no changes. This is because the difficulty of repair mainly lies in repairing the locator, and the correctness of the final repair result mainly depends on whether the locator is repaired correctly. Therefore, the prompt used for ChatGPT only allows it to modify the locator, and ChatGPT basically follows this instruction and does not modify the part outside the locator. If ChatGPT modifies the part outside the locator, it will be considered a failure in this indicator, which will lead to unsuccessful repair results. Besides, the \textbf{Locating Strategy} is also close to the total number of repairs, which indicates that ChatGPT is relatively compliant with the original locating strategy. Finally, it can be observed that the number of repairs where the locator can locate the selected element is relatively small (only 247 and 230 out of a total of 327 repairs), indicating that repairing the locator is more difficult. The Number of Correct is almost equal to it, indicating that the number of correct repairs depends largely on whether the locator can be repaired correctly.



\subsection{The Effectiveness of ChatGPT Compared to WATER and VISTA}
Since ChatGPT is asked three times for each breakage but each breakage only needs one repair result, only when there are two or more correct repair results in three, we will consider ChatGPT repair correctly for this breakage repair.

Different from WATER and VISTA, ChatGPT's correct repair is based on correct selection. WATER and VISTA's repair framework is relatively mature and the repair results are relatively accurate as long as the matching element is found correctly during testing. VISTA has even implemented a crawler function that searches for candidate elements on neighboring pages. If found, test statements are added to reach the page where the candidate element is located, and then the original broken test statements are repaired. 





Table \ref{repair_result2} shows the repair results and average running time of different repair methods. It can be seen that among the four repair methods, only ChatGPT+WATER+VISTA has the longest average running time (66.13 s), almost twice as long as the other methods. Considering that the average time for ChatGPT to select and repair one breakage is only about 3 seconds, the reason why the running time of ChatGPT+WATER+VISTA is the longest is that the process of generating candidates using WATER+VISTA takes up a lot of time. However, in terms of repair effectiveness, compared to using WATER and VISTA alone, using ChatGPT for matching and repairing achieves better results. Among them, ChatGPT+Edit Distance has the best performance, successfully matching and repairing 96 and 91 out of 109 breakages, respectively. On the other hand, using VISTA alone performs the worst, with only 53 breakages successfully matched and repaired out of 109, less than half of the total. However, it should be noted that when repairing with WATER and VISTA alone, the number of correct matches is equal to the number of correct repairs. This means that as long as the matching is correct, the repair can be done correctly, which once again proves that repair framework of WATER and VISTA is relatively mature and the repair results are relatively accurate. When using ChatGPT for repair, whether using candidates generated based on Edit Distance or based on WATER+VISTA, the number of correct repairs is slightly less than the number of correct matches, which is the problem to be discussed next.

\subsection{Analysis of ChatGPT's Repair Failure}
There are several reasons why ChatGPT repairs fail. 

Mismatch is the first main reason for ChatGPT's repair failure because ChatGPT cannot repair the locator correctly with the information of its wrong selected element. Generally, there are two cases of mismatch. One is mismatch from the candidate lists without ground truth elements. In this experiment, the proportion of ground truth contained in the candidates of WATER+VISTA and Edit Distance are 98 and 99 out of 109 separately according to Table \ref{gt}, which means ChatGPT can not have a higher correct repair rate than these. The other is that ChatGPT selects wrongly from a candidate list even though there is a ground truth element in it. And this happens more often when selecting candidates with WATER+VISTA. This is because WATER+VISTA more tends to contain nested elements, such as the parent element and grandparent element of the ground truth element, as candidates. These elements are more likely to have similar attributes but can not replace the ground truth element to be tested, which may interfere ChatGPT's selection. Instead, Edit Distance selects sibling elements with different attributes as candidates more frequently because elements with the same hierarchy have smaller XPath edit distance, thus reducing the number of ChatGPT's mismatch.

Another reason for ChatGPT's failure is that ChatGPT tends to follow locating strategies of the original broken statements, which leads ChatGPT to use relative paths for many of the repairs. However, ChatGPT is not good enough at generating relative paths, causing related repair failure.


By relative paths we mean repairing with ``By.xpath()'', but not with the value of the \emph{XPath} absolute path itself. There are two types of relative paths, the first being the simpler one, where the element itself is located using e.g. ``By.xpath(//*[text()=``text value''])''. However, ChatGPT has had cases of repairing errors where the value of the another attribute was filled in as the value of the text value. This was because ChatGPT wanted to maintain the original positioning as much as possible, i.e. using relative paths. However, if the repair is simply done by other positioning methods like ``By.attribute(``attribute value'')'', it is much less likely to fill in the wrong attribute value. Another type of absolute path is created by first locating the ancestor of an element using the previous relative path, and then splicing the absolute path of the element minus the absolute path of the ancestor element. However, no samples of ChatGPT successfully repairing this type of relative path were found in this experiment.


In addition to this, there were some unexpected failures: ChatGPT selected the correct element, but the result of the repair was wrong. The reason why the repair was wrong when it could have been correct is that ChatGPT thought that the element it selected as the most similar element in the list of candidate elements did not look enough like the correct answer, so ChatGPT did not base the repair entirely on the information of the selected element. And ChatGPT's result based on its prediction of the possible correct answer and its repair seems to be reasonable.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/content/example.png}
    \caption{An example of the unexpected failure}
    \label{failure_example}
\end{figure}

 In the example of Figure \ref{failure_example}, the value of the \emph{href} attribute of the target element on the old page is ``manage\_user\_page.php
'', and the locator for the broken statement testing this element is ``//a[@href=`manage\_user\_page.php']''. ChatGPT repaired it by fixing the locator to ``//a[@href=`/mantisbt-1.2.0/manage\_user\_page.php']'', prefixing the original \emph{href} with the prefix that all candidate elements have. 

The value of the \emph{href} of the element on the old page means that the page jumps to the page ``Manage User'' when the element ``Manage'' is clicked. However, ChatGPT does not know that clicking on the ``Manage'' element on the new page redirects the page to the overview page and requires further clicking on the ``Manage User'' element to reach the same page as before. Because the target page is different, the \emph{href} attribute of the ``Manage'' element was changed to ``/mantisbt-1.2.0/manage\_overview\_page.php'', causing the ChatGPT to get the wrong speculation about the truly matched element. 

This ChatGPT ``self-initiated'' error could have been avoided by strictly restricting ChatGPT to repair the locator according to the given candidate elements. In this example, the correct element was included in the list of candidates and ChatGPT selected it as a match correctly. However, it is important to note that we cannot always guarantee that the correct element is in the list of candidates. Therefore, it is worth considering whether we should allow ChatGPT to guess an element that is more correct than the given candidate according to the effectiveness of the candidates selection algorithm.
















% We evaluate the effectiveness of \toolName in \delete{W}\add{w}eb UI tests repair and answer the following research questions: 


% \begin{description}[leftmargin=*]
% \item[RQ1:] How effective is \toolName in UI element matching compared with existing methods?
% %How effective is \toolName ~in backporting patches? 

% \item[RQ2:] How efficient are different matching methods?

% % \item[\add{RQ3:}]\add{ How efficient is the iterative matching?}

% \item[RQ3:] How effective is \toolName in test case repair compared with existing methods? %How does \toolName compare with existing  tools?
% % \item[\textbf{RQ3}] How does different-based validation compare with screen-based validation in intention validate?
% \end{description}


% \noindent \textbf{Selected baselines:} We compared \toolName with four baselines, including two repair tools (\watertool~\cite{choudhary2011water}, \vistatool~\cite{stocco2018vista}), and two UI element matching algorithms (\webevotool~\cite{shao2021webevo}, and \sftmtool~\cite{brisset2020sftm}). 
% We exclude the model-based tool~\cite{imtiaz2021automated} because the code in the GitHub repository fails to compile due to missing dependencies.
% \watertool is a UI test repair tool that uses the similarity of DOM properties of elements for matching.
% \vistatool is a repair tool that uses image processing and computer vision techniques by comparing visual information in two versions of the apps.
% \webevotool computes both text similarity and image similarity of the elements in two versions of the apps to match elements.
% % \todo{add a short sentence to introduce each tool, algorithm and matching which information}
% The recently proposed algorithm, \sftmtool, assigns attribute scores to all potential matches between nodes in two versions and adjust\add{s} the scores using the parent-child relationships of nodes.
% Similar to \vistatool~\cite{stocco2018vista}, \toolName performs online repair, which fixes broken tests during execution. 
% On the other hand, \watertool~\cite{choudhary2011water} uses an offline mode, which collects information during test execution and repairs after the execution. %, and starts repairing after the execution.
% Therefore, we use the re-implemented version in \vistatool~\cite{stocco2018vista} to evaluate \watertool.
% For all other tools, we use their open-source implementations and parameters. 
% The parameters of \toolName \add{in 
%  Algorithm \ref{alg:iterative_optimization}} include: \add{maximum iterations} $t$=5, \add{attribute similarity weight} $\alpha$=0.7, \add{path similarity weight} $\beta$=1.0, \add{region similarity weight} $\gamma$=2 and \add{similarity threshold} $\theta$=1.2. All these parameters are tuned via grid searches for the best values.

% %\watertool and \vistatool use code open-sourced in the code repository of \vistatool\cite{stocco2018vista}, \webevotool and \sftmtool use their open-sourced code\cite{shao2021webevo,brisset2020sftm} respectively.
% %Similar to Section~\ref{sec:study}, 
% % We evaluate the element matching algorithm of \toolName on two sets of applications: %(1) 5 open-source applications that have been used by existing work~\cite{imtiaz2021automated} (we exclude the industrial application, i.e., University Management System from our experiment as it requires creating an university account), 
% % and (2) two industrial apps ($AppB$ and $AppC$). These two selected industrial apps are big data analysis platforms, which are core products of \company{}.

% %Note that, all evaluations run on the same computers.
% %a Windows computer with a Intel Core i5 processor (1.6GHz) and 12 GB RAM.
% % ~\xiang{how do you select the experimental apps}




% \noindent\textbf{UI Match Dataset}:
% % We utilize further augmented datasets 
% To evaluate the performance of different UI element matching algorithms, we use an extended \webevotool dataset~\cite{shao2021webevo} (EWD).
% The \webevotool dataset include\add{s} 13 web applications in total.
% We excluded the webpages \textit{ClassDojo} and \textit{Home Depot} because they could not be loaded correctly. 
% % Since the Alexa service is closed~\footnote{https://en.wikipedia.org/wiki/Alexa\_Internet\#cite\_note-end\_news-5}, 
% To expand our dataset, we select the Top 15 web apps on Semrush~\cite{semrush} (which presents a ranked list of most visited websites) and remove webpages that overlap with the \webevotool dataset~\cite{shao2021webevo}. 
% We use \textit{Wayback Machine}~\cite{wayback} to obtain the historical webpages. 
% \delete{Totally}\add{In total}, our expanded dataset contains 44 webpages of 22 web apps (with 11 apps from \webevotool and 11 extended apps).

% Moreover, to show the ability of different element matching algorithms on large-scale industrial applications, we also include two industrial apps\delete{(IND)}.
% To \delete{keep anonymous}\add{maintain anonymity}, we omit the application and company name in the paper review process.

% We select two apps \appa{} and \appb{}, two big data analysis platforms, which are two core products of \company{}.
% To ensure sufficient changes are collected for our study of web UI elements evolution, we select webpages which contain\delete{s} sufficient changes. 
% Specifically, we select webpages with more than 20 changed elements.
% In the end, we collected 13 webpages from two industrial app\add{s}.
% The types of selected webpages are diverse, which include home pages, pages for configuring system settings, data pages, and pages with charts.


% Similar to prior work~\cite{shao2021webevo}, we also consider three types of element changes: \textit{Update}, \textit{Add}, and \textit{Delete}.
% % Because test cases usually do actions on leaf node elements, the experiment only considers the labeled leaf node elements.
% % Its data set distribution is as follows:
% % Since \vistatool{} only supports matching leaf nodes, \yz{we only count leaf nodes as UI elements.}
% Table~\ref{table:dataset-stats} shows the statistics of our UI element matching dataset.
% % \yuanzhang{How to label this element}
% In the UI element matching dataset, we try to label all the elements on the pages as much as possible. 
% \textit{The labeling process does not only label the change types, but also annotate the matching pairs between the old and new versions, which are then served as the ground truth of element matching.}
% However, some elements, such as content elements, are difficult to label.
% As a result,
% % \add{However, certain elements pose challenges when it comes to labeling. Take content elements, like items in the Amazon application, for instance. In the new version, these elements may not have an  corresponding relationship. To mitigate potential controversies, }
% we made the decision to exclude them from the labeling process.
% % , so we ignored them.
% Since VISTA only supports matching the innermost elements, to make a fair comparison of the performance of different algorithms, we only consider leaf nodes in our experiment.
% Totally, we labelled 2,522 changed elements.


% \begin{table}[!t]
% \centering
% \small
% \caption{Statistics of our UI match dataset}
% % \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{l|rrrr}\toprule
% Dataset   & Add      & Delete     & Update          & Total      \\\hline\hline
% EWD & 301 & 218 & 1,101  & 1,620 \\
% IND & 170 & 101 & 631  & 902 \\ \hline
% Total &471 &319 &1,732 &2,522 \\
% \bottomrule 
% \end{tabular}%}
% \label{table:dataset-stats}
% \end{table}



% % Table \ref{table:evaluation-application-version} shows the collected information for pages that belong to different types of web applications and different time intervals between original version and modified version.

% % \begin{table}[h]
% % \centering
% % \setlength{\tabcolsep}{2.2pt}
% % \vspace{-3pt}
% % \caption{The version about Web application in evaluation dataset}
% % \vspace{-3pt}
% % \begin{tabular}{ll|cc}\toprule
% % Application & Category &Original Version & Modified Version \\\hline\hline
% % \textit{www.w3school.com} & & 2016.01 & 2019.01\\
% % \textit{www.foodnetwork.com} & & 2018.11 & 2019.11\\
% % \textit{music.douban.com} & & 2014.02 & 2019.02\\
% % \textit{beijing.douban.com} & & 2017.10 & 2019.10\\
% % \textit{book.douban.com} & & 2016.08 & 2019.08\\
% % \textit{movie.douban.com} & & 2014.11 & 2019.11\\
% % \textit{www.amazon.com} & & 2017.08 & 2020.08\\
% % \textit{www.apple.com} & & 2018.02 & 2020.08\\
% % % \textit{www.classdojo.com} & 2017.06.05 & 2020.07.22\\
% % % \textit{www.homedepot.com} & 2019.07.15 & 2020.08.04\\
% % \textit{www.linkedin.com} & & 2019.08 & 2020.08\\
% % \textit{www.usps.com} & & 2018.08 & 2020.08\\
% % \textit{www.xfinity.com} & & 2018.08 & 2020.08\\ \hline
% % \textit{www.bing.com} & &  & \\
% % \textit{www.yahoo.com} & &  2017.02 & 2019.06\\
% % \textit{www.wikipedia.com} & & 2019 & 2022\\
% % \textit{www.paypal.com} & & 2019.03 & 2020.03\\
% % \textit{www.instagram.com} & & 2019.03 & 2021.03\\
% % \textit{www.google.com} & &  & \\
% % \textit{www.fandom.com} & & 2022.03 & 2022.12\\
% % \textit{www.twitter.com} & & 2021.08 & 2022.08\\
% % \textit{www.youtube.com} & & 2022.08 & 2023.02\\
% % \textit{www.facebook.com} & & 2020.08 & 2022.08\\
% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:evaluation-application-version}
% % \end{table}




% % \noindent where columns \textit{Add}, \textit{Delete} and \textit{Update} show the number of inserted, deleted and modified elements when webpages evolve, respectively.

% \noindent\textbf{UI Test Dataset}:
% Since the \webevotool dataset does not have open-source test cases, we choose to evaluate the effectiveness of \toolName using open-source and industrial test datasets.
% For the open-source tests, we use an existing test dataset~\cite{imtiaz2021automated}.
% Specifically, we include all \delete{W}\add{w}eb apps in prior work~\cite{imtiaz2021automated}, except for the \texttt{Password Manager} app because the provided link for this app is no longer available for download.
% %and the versions of five application in section \ref{sec:2-dataset}.
% % The original test cases need to be executed in the specified order because the previous cases will provide data for the later cases.
% For the original test case dataset, we mainly made two modifications,
% (1) remove test cases without assertion statements or repeated test cases, \add{as the assertions are used as the correctness specification for \toolName}, and
% (2) insert necessary UI actions (e.g., login) so that test cases can be executed independently.
% To avoid the problem caused by missing data (such as username does not exist or password is incorrect), we first insert some SQL statements to prepare the data for test execution (e.g., create user\delete{,} and save username/password information into the database).
% The selected two industrial apps \appa{} and \appb{} have 5,839 test cases in total. 
% % As it is time-consuming to execute all tests, .
% \add{Conducting experiment on all the tests is too time-consuming, since executing these tests in parallel will take two or three days in industrial environment. Hence, we randomly select 250 test cases (the number is aligned with the existing work~\cite{imtiaz2021automated}) to execute.}
% \add{We select the test cases that must be repaired, regardless of the number of pages used by these tests.}
% We then exclude 46 tests as they require configuring a specific test environment.
% Table \ref{table:open-source-application-version} shows the original and the modified versions of the selected webpages.
% The open-source dataset, following settings from the provided GitHub repository in the prior work~\cite{imtiaz2021automated}, \add{involves changes across multiple versions.
% Note that\delete{,} fixing tests across multi-version changes may not be realistic.
% Hence, we use single-version changes for the industrial dataset, which is practical in an actual industrial environment.}
% % Yes, . In fact, 
% % As for the open-source dataset, we utilized gaps larger than a single revision just to maintain consistency with the existing dataset (citation 4). So that, we can conduct comparison experiment with prior work.
% % On the other hand, if UITestFix is proved to be effective in fixing tests across multi-version changes, it should perform even better on single-version changes.
% % We elaborated the discussion on dataset at Section VI.

% During the classification of the matching results (RQ1) and the generated fixes (RQ3), two authors of the paper independently analyzed them by inspecting the matched UI elements to check if the matching was correct and if it led to any newly thrown exception. Then, they met and discussed resolving any disagreements.

% \begin{table}[!t]
% \centering
% % \setlength{\tabcolsep}{2.2pt}
% \small
% \caption{The original and modified versions of the selected webpages}
% % \resizebox{0.43\textwidth}{!}{%
% \begin{tabular}{ll|rr}\toprule
% Label & Application & Original Version & Modified Version \\\hline\hline
% I     & AddressBook & 4.0              & 6.1              \\
% II    & Claroline   & 1.10.7           & 1.11.5           \\
% III   & Collabtive  & 0.65             & 1.0              \\
% IV    & MantisBT    & 1.1.8            & 1.2.0            \\
% V     & MRBS        & 1.2.6.1          & 1.4.9            \\
% % \hline
% % \add{VI}    & \add{\appa}      &                  &                  \\
% % \add{VII}   & \add{$AppB$}      &                  &                  \\
% \bottomrule
% \end{tabular}
% \label{table:open-source-application-version}
% \end{table}

% All experiments for the open-source apps are run on a computer with an Intel Core i5 processor (2.3GHz) and 24 GB RAM, whereas the experiments for the industrial apps are conducted on a computer with an Intel Core processor (3.20GHz) and 32GB RAM.
% %windows computer with Intel Core processor(3.20GHz) and 32GB RAM.

% % Therefore, we used only five of these applications.

% % All test cases are written in one class in the original dataset, and the execution order is defined by priority. These test cases share a WebDriver, and when a test case fails to execute, it will affect the execution of other test cases. In addition, case events are heavily dependent on backend data. For example, if the AddProject use case fails, all Project-related use cases may fail.

% % Therefore, to improve the independence between test cases as well as the independence of test cases and data, we made certain modifications to the dataset. During this period, keep the original locators and actions as much as possible. We mainly did the following work:
% % \begin{enumerate}
% %     \item  Separate these test cases from one class into different classes.
% % \item  Add necessary events, such as login.
% % \item  Call SQL statements to prepare data or clean data for test cases.
% % \item  Solve the bugs in the test cases and make certain adjustments to enhance stability.
% % \item  Modify the locator generated by the backend data, such as $//*[@id="add\_btn\_1"]$.
% % \item Delete duplicate, empty, meaningless test cases.
% % \item  Merge some test cases.
% % %, such as adding, deleting, and modifying.
% % \end{enumerate}

% % After modifying test cases, we executed them several times and verified them on different devices. Although we try our best to alleviate the dependencies between test cases, there is no guarantee that they will not affect each other.


% % The final test case dataset distribution is as follows:

% % \begin{table}[h]
% % \centering
% % \setlength{\tabcolsep}{2.2pt}
% % \vspace{-3pt}
% % \caption{Distribution in our test cases dataset}
% % \vspace{-3pt}
% % \begin{tabular}{l|l|c|c|c|c}\toprule
% % Label &Application   & Base Version      & Repair Version     & Cases              \\\hline\hline
% % I &AddressBook & 6.1 & 4.0 & 16  \\
% % II &Collabtive & 0.65 & 1.0 & 18   \\
% % III &Claroline & 1.11.5 & 1.10.7 & 33  \\
% % IV &MantisBT & 1.1.8 & 1.2.0 & 45   \\
% % V &MRBS & 1.2.6.1 & 1.4.9 & 25  \\
% % VI  & Industy & - & - & 0   \\\hline
% % Total&- &- &- & 137\\

% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:dataset-stats-temp}
% % \end{table}


% % 	\begin{table*}[ht!]
% % \centering
% % \vspace{-3pt}
% % \caption{Distribution in our ui match dataset}
% % \vspace{-3pt}
% % \begin{tabular}{l|c|c|c|c}\toprule
% % application   & base version      & repair version     & scripts              \\\hline\hline
% % AddressBook & 165 & 78 & 50  \\
% % Collabtive & 165 & 78 & 50   \\
% % Claroline & 1.11.5 & 1.10.7 & 35  \\
% % mantisbt & 1.1.8 & 1.2.0 & 45   \\
% % mrbs & 0.65 & 1.0 & 25  \\
% % industy & - & - & 500   \\
% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:dataset-3stats}
% % \end{table*}

% % Moreover, we evaluate \toolName in backporting security vulnerabilities by selecting \numCVE patches that fix CVEs using the same criteria.
% % We focus on the CVEs reported during 2014-2019, and made sure that the \numCVE CVE patches are disjoint from the \numSubject patches in our main dataset.

% % All experiments are conducted on a Dell Power Edge R530 with Intel(R) Xeon(R)CPU E5-2660 processor and 64GB RAM. 

% \subsection{[RQ1] Effectiveness on Matching Elements}
% % Because the data set used is static, the inputs and outputs are adjusted to use statically saved data.
% % An algorithm is considered to match correctly when the matched element lies in the labeled element cluster.
% \begin{table*}[!tb]
% \centering
% % \small
% % \resizebox{0.45\textwidth}{!}{%
% % \setlength{\tabcolsep}{2.5pt}
% \caption{Accuracy of UI element matching for all evaluated approaches}
% \label{table:experiment-comparison-match-ui}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc}
% \toprule
% Modified & 
% % \multicolumn{2}{c|} {\texttt{WATER-}} &
% \multicolumn{2}{c|} {\watertool} &
% \multicolumn{2}{c|}{\vistatool} &
% \multicolumn{2}{c|}{\webevotool} &
% \multicolumn{2}{c|}{\sftmtool} &
% % \multicolumn{2}{c|}{\texttt{SFTM+}} &
% \multicolumn{2}{c}{\toolName}\\\cline{2-11}
% Type    & EWD & IND  & EWD & IND   & EWD & IND  & EWD & IND  & EWD & IND  
% % & OD & ID & OD & ID
% \\\hline\hline
% % \multirow{2}{*}{Add} & 9 &28 &25 &8 &31 &  1 & 156 & 133  & \textbf{160} &\textbf{142}\\
% % {}    &  3.06\% & 21.76\% & 8.50\% & 4.71\% &10.51\% & 5.9\%  & 52.88\% & 78.23\% & \textbf{54.23\%} & \textbf{83.53\%}\\\hline
% Add &  4 (1.3\%) & 28 (16.47\%) & 30 (10.0\%) & 8 (4.7\%) & 87 (28.9\%) & 1 (5.9\%) & 162 (53.8\%) & 133 (78.2\%) & \textbf{170 (56.5\%)} & \textbf{142 (83.5\%)} \\ 

% Delete & 11 (5.0\%) & 1(1.0\%) & 49 (22.5\%) & 5 (5.0\%) & 44 (20.2\%) & 0 (0\%) & 100(45.9\%) &32 (31.7\%) & \textbf{111 (50.9\%)} & \textbf{77 (76.2\%)} \\ 

% % \multirow{2}{*}{Delete} & 36 &1 &21 &5 &24 &  0 & \textbf{98} & 32 & 95 &\textbf{77}\\
% % {}    & 16.74\%& 0.99\% & 10.24\% &4.95\% &11.16\% & 0\% & \textbf{45.58\%} & 31.68\% & 44.18\% & \textbf{76.24\%}\\\hline
% % Update & &3 & &
% Update &500(45.4\%) & 344(54.52\%) & 651(59.1\%) &434(68.78\%) &803(72.9\%) &278(44.1\%)  &808(73.4\%) &500(79.2\%) &\textbf{1036(94.1\%)} &\textbf{605(95.88\%)} \\ \hline
%     % \multirow{2}{*}{Update} &536 &344 &711 & 434 &821 &278 & 838 & 500 & \textbf{1074} & \textbf{605}\\
% % {}    & 48.16\% & 52.60\% & 64.52\% & 66.36\% & 73.76\% & 42.51\% & 75.29\% & 76.45\%  & \textbf{96.50\%} & \textbf{92.50\%}\\\hline

% % \multirow{3}{*}{Total}& 581&382& 757&447 & 876&  279 & 1092 & 665 & \textbf{1329}&\textbf{824}\\
% % {}     & 35.79\%&41.30\%& 47.28\% & 48.32\% & 53.97\% & 42.50\% & 67.28\% & 71.89\%  & \textbf{81.89\%} & \textbf{89.08\%}\\
% \multirow{2}{*}{Total} &515(31.8\%) &373(41.35\%) &730(45.1\%) &447(49.6\%) & 934(57.7\%) &279(30.93\%) &1070(66.1\%) &665(73.3\%) &\textbf{1317(81.3\%)} & \textbf{824(91.4\%)} \\
% {}     &\multicolumn{2}{c|} {888 (35.2\%)} & \multicolumn{2}{c|}{1177 (46.7\%)}  & \multicolumn{2}{c|}{1213(48.1\%)} & \multicolumn{2}{c|} {1735 (68.8\%)}    & \multicolumn{2}{c} {\textbf{2141 (84.9\%})} \\ \hline\hline

% AVG Time & \multicolumn{2}{c|}{\textbf{0.0003s}} &  \multicolumn{2}{c|}{7.7623s} &\multicolumn{2}{c|}{0.0799s} &\multicolumn{2}{c|}{0.9726s} &\multicolumn{2}{c}{0.8685s} \\

% % \hline
% % Total& 850(61.10\%)& 570(61.62\%)  & 42  & 82  & 59  & 44  & 43  & 648(70.05\%)    &1160(83.39\%)& 761(82.27\%)& 1254(90.15\%)& 783(84.65\%)\\
% \bottomrule
% \end{tabular}}
% \end{table*}

% Table \ref{table:experiment-comparison-match-ui} summarizes the evaluation results on web element matching.
% For each algorithm, the table lists the correct number and accuracy of different types of changes in the extended WebEvo dataset (EWD) and industrial \add{dataset} (IND) \delete{dataset}.
% The ``Total'' row summarizes the total number of corrects and the overall accuracy of different algorithms.
% % According to the experimental results, \toolName has significantly improved the accuracy of matching elements.
% Overall, \toolName achieves the best result on all types of changes (Add, Delete and Update) for both open-source and industrial datasets.

% More specifically, \toolName is more accurate than all other evaluated tools, with the overall success matching rate being 84.9\%, while the best result of existing tools is only 68.8\%.
% \toolName produces better results than existing tools mainly because our optimization approaches iteratively improve the matching results based on region and path similarity, while other tools produce matching results directly.
% It is worth \add{noting} that tree-based matching algorithms (SFTM, \toolName) have significantly higher accuracy in identifying added and deleted elements than other matching algorithms. 
% % For instance, among 101 deleted elements from the industrial dataset, \toolName successfully matches 77 of them with 31.7\% accuracy, while the accuracy of \watertool, \vistatool, \webevotool and \sftmtool is 1\%, 5\%, 0\%, and , respectively.
% For instance, among 170 added elements from the industrial dataset, \sftmtool successfully matches 133 of them with 78.2\% accuracy, while the accuracy of \watertool, \vistatool, and \webevotool is 16.5\%, 4.7\%, and 5.9\%, respectively.
% \toolName even achieves better results, and its accuracy is 83.5\%.
% This is because the tree-based matching algorithm matches elements by referring to parent-\add{child} relations, which has a stronger ability to identify added and deleted elements.
% In terms \add{of} deleted elements, \toolName outperforms \sftmtool (76.2\% vs 31.7\%) mainly because \toolName can also consider the relations of sibling nodes in the iterative, while \sftmtool only measure the parent-\add{child} relations.





% % \yuanzhang{It seems to require a futher disscussion, and this discussion is difficult to explain the advantages of \toolName. I want to analyze the collected dataset in the front subsection, such as the proportion of the elements with text. Discussing the reasons for the high matching accuracy of existing algorithms and the reasons for the low matching accuracy in this subsection. For example, there is a big difference in the performance of WebEvo on two datasets.}

% % \yuanzhang{We can also discuss the elements that our algorithm fails to match and analyze the reasons behind it. Further conclusions that can be drawn are: 1. The semantic similarity algorithm for statements has little effect. 2. The visual approach has also little effect. In other words, these two information can be completely dispensed with.}




% % The open-source(OS) dataset and industrial(IND) dataset can achieve the correct rate of 96.50\% and 92.50\%, respectively. 
% % The overall change recognition rate has also been greatly improved, reaching an accurate rate of 84.9\%.
% % \toolName has also significantly improved the identification accuracy of \textit{Add} and \textit{Delete} types.
% % Among \textit{Add} types, \toolName correctly identified 302, higher than \sftmtool's 289.
% % Among \textit{Delete} types, \toolName correctly identified 172, higher than \sftmtool's 130.
% % \watertool, \vistatool and \webevotool have poor identification ability on \textit{Add} type and \textit{Delete} type.

% %In addition, the robustness of the algorithm on different pages has been also significantly enhanced. Specifically, for each webpage, the correct element matching rates of \toolName on EWD datasets and industrial datasets are from 60.86\% to 93.25\% and 84.09\% to 91.38\%, respectively. While state-of-the-art \sftmtool are from 28.21\% to 95.45\% and 71.21\% to 93.10\%, respectively. This result indicates that \toolName is less sensitive to different webpages.

% % In addition, we also found that many algorithms tend to get matching results to improve the recognition accuracy of newly added and deleted elements, such as \watertool, \vistatool, and \webevotool. Compared with the \watertool algorithm, the \waterlitetool  algorithm does not significantly decrease the correct rate of matching parts. Still, it substantially increases the correct rate of newly added and deleted elements.
% % At the same time, we also noticed that the text attribute is very effective. Compared with \sftmtool, \sftmplustool has a certain improvement in matching and adding two indicators. Among them, the matching accuracy rate has increased from 73.86\% to 88.61\%. Text information has a high effect on element matching.

% \begin{figure}[!th]
% \centering
%     \includegraphics[width=0.48\textwidth]{images/figure_t_iteration2.pdf}
% \caption{The accuracy rate varies with the number of iterations.}
% \label{fig:figure-t-iteration}
% \end{figure}

% \add{We further evaluate \add{the} effectiveness of the iterative algorithm.
% Figure \ref{fig:figure-t-iteration} presents the number of correctly matched elements during the iterative process. 
% The x-axis shows the number of iterations, while the y-axis displays the count of correctly matched elements. 
% It is evident from the graph that the matching accuracy increases progressively with each iteration. 
% In the first iteration, only 908 elements were correctly matched, while the following three iterations successfully matched 1986, 1988, and 2157 elements. 
% However, after the fourth iteration, there is no significant improvement in the matching accuracy. 
% Therefore, we decided to set the maximum iterations to five. 
% The results indicate that the iterative process significantly enhances the matching accuracy.
% % We also note that the accuracy for the "Add" and "Delete" types decreases as the number of iterations increases, stabilizing after the fifth iteration.
%  % This phenomenon occurs due to the inclusion of path similarity and region similarity during the iterative process, which causes the total similarity to exceed the threshold.
% % As a result, certain elements that were initially similar but were added or deleted are mistakenly identified as matches.
% }


% \subsection{[RQ2] Efficiency on Matching Elements}
% %Apart from matching accuracy, we also evaluated the efficiency of \toolName.
% To compare the efficiency of different algorithms, we calculate the average time taken by each algorithm to generate final matching results.
% We use the saved webpage for matching to avoid inaccuracy caused by the network (e.g., page loading latency).

% The ``AVG Time'' row in Table \ref{table:experiment-comparison-match-ui} shows the average time taken (in seconds) by different algorithms to generate matching results across all webpages. %on the UI match dataset.
% % The average time for all tools except vista is within 1 second.
% Among all evaluated tools, \watertool is the fastest in producing matching results (0.0003s) because it matches elements by computing similarities of DOM properties which is very efficient.
% %Among the evaluated tools, \watertool generates matching results using shortest time (0.0003s), because \watertool match the elements according to the similarity of the DOM properties which is very efficient.
% \webevotool and \vistatool are slower than \watertool since they rely on time-consuming image similarities check.
% \webevotool is much faster than \vistatool since it uses a fast image similarity algorithm (aHash).
% \toolName and \sftmtool take similar time to generate matching results (0.97s and 0.87s).
% Compared to \watertool and \webevotool, \toolName is slower mainly because it requires multiple iterations for optimizing the matching results.
% With improved accuracy, we believe it is acceptable to take $<$1s to generate matching results for each webpage.
% % \yuanzhang{This section feels a bit short and strange. I want to merge this section with the previous one and free up an RQ to explore the changes in matching accuracy of elements during the iteration process.}
% % Compared to \webevotool and \watertool, \sftmtool and \toolName are slower because they output a matched element after matching all elements.
% % These indicate that \toolName is an effective tool.


% % \subsection{\add{[RQ3] Effectiveness on iterative matching}}



 
% \add{
% % Despite this, the accuracy improvement resulting from the "Update" type is more significant compared to the decrease in accuracy for the "Add" and "Delete" types.
% }

% \subsection{[RQ3] Effectiveness on Repairing UI Tests}

% \label{sec:evaltools}
% To fairly compare the capabilities of different algorithms in repairing broken UI tests, we integrated the matching algorithm of \watertool, \vistatool, \webevotool and \sftmtool into our repair framework. We named them \watertool{*}, \vistatool{*}, \webevotool{*} and \sftmtool{*}, respectively.

% \noindent \textbf{Successful repair.} We consider a test case to be successfully fixed if (1) the test passes after the repair and (2) each action in the test has been correctly executed (we verify this by manually comparing the screenshots of the traversed webpages).

% The dataset contains 135 test cases in open-source apps and 204 test cases in industrial apps.
% After excluding 163 non-crashing test cases (which do not need to be repaired) and 10 test cases that cannot be repaired due to the tested modules being removed, we obtained 62 crashing test cases in open-source apps and 104 crashing test cases in industrial apps (166 test cases in total).

% Table \ref{table:experiment-repair-scripts} presents the test case repair results of different algorithms. 
% For each application, the table reports the total number of test cases (Total) and the number of test cases successfully repaired by different algorithms.
% \delete{The c}\add{C}olumn $\Delta$V shows the number of released versions between the original and new versions.
% As shown in Table \ref{table:experiment-repair-scripts}, \toolName achieves the best results across all applications.
% In total, \toolName successfully fixes 113 broken test cases with a repair rate of 68\%, while the best existing tool (i.e. \vistatool{*}) only fixes 73 of them with a repair rate of 44\%.
% Moreover, we observe that the larger $\Delta$V is, the more changes introduced to the new versions since the original version, the more challenging to fix the broken tests.
% For instance, for MRBS, the best tool only fix 4 of 24 broken test cases.


% % Note that, there are 2 test cases of \vistatool and 1 test case of \webevotool is failed repair, which passed but violates the original intention.
% % For example, in the test case ``DeleteUser'' of the MantisBT application, the test case uses \textit{administrator} to determine whether the test case returns a user list webpage.
% % However, each page of MantisBt has \textit{Logged in as: administrator} and \vistatool incorrectly matches the \textit{administrator} element in it.
% % After returning the text of the element, the assert was successfully passed.
% % Such fixes are considered failed repair and are excluded from the number of successful repaired test cases.

% \begin{table}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{1.8pt}
% \caption{UI test repair effectiveness}
% \label{table:experiment-repair-scripts}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{l|rr|rrrrrrr}
% \toprule
% Application & Total & $\Delta$V & \watertool{*} & \vistatool{*} & \webevotool{*} & \sftmtool{*} & \toolName \\ \hline \hline
% AddressBook   &8 &30 & 1&\textbf{2} &0 &\textbf{2} &\textbf{2} \\
% Claroline  &29 &7  & 0 &\textbf{24} &0 &0 &\textbf{24}\\
% Collabtive  &5 &4 & \textbf{3}&1 &2 &0 &\textbf{3}  \\
% MantisBt  &38 &1  &18  &4 &19 &6 &\textbf{24} \\
% MRBS  &24 & 12 & 0 &\textbf{4} &0 &2 &\textbf{4} \\\hline
% \appa{}  & 46 & 1 &36 &33 & 37 &40 & \textbf{43}\\ 
% \appb{} &16 & 1 &6 &5 &6 &11 & \textbf{13}\\ \hline
% Total & 166 & - & 64(39\%) &73(44\%) &64(39\%) &61(37\%) &\textbf{113(68\%)} \\ \hline
% % AVG Time & - & & & & & \\ \hline
% \end{tabular}}
% \end{table}

% % \toolName repaired 57 out of 113 crashed test cases in open-source dataset and repaired 56 of 57 crashed test cases in industrial dataset, higher than other algorithms.


% % To improve the credibility of the experiment, we executed each algorithm more than twice on each use case.
% % Two authors analyze the reasons for the failure of all test case fixes separately and finally summarize the reasons.
% % \yuanzhang{Should I explain why some algorithms perform worse in some applications?}\xiang{yes, you should}
% The number of successful repairs generated by the same approach differs across apps.
% \watertool and \webevotool performed well on MantisBt but did not repair any test cases on Claroline.
% \sftmtool performed well on both \appa{} and \appb{} 
%  but did not work well for the five open-source applications.
% This is mainly due to the different element change types of different applications.
% For instance, on the login webpage of MantisBt, the button with the text ``Enter'' is transformed into the input with the value attribute ``Enter''. 
% \vistatool is weak at distinguishing the elements with text, leading to the ``Enter'' button matched with the ``Log out'' button, resulting in test cases that cannot be repaired.
% % Since the attributes of open source applications (1.63 attributes per element) are less to those of industrial applications (2.23 attributes per element)\yuanzhang{Does this need to be written in RQ1 of study?}, \sftmtool performs significantly better in industrial applications than in open source applications.
% Even so, the repair rate of \toolName on different applications is the same or higher than all existing algorithms, which shows the high robustness of \toolName.

% % In the test case of the Claroline application, the ''Enter'' button on the login page changed from text to the value attribute.
% % The \watertool and \webevotool matches failed and all use cases could not be repaired due to login failure.
% \begin{figure}[htbp]
%     \begin{minipage}[t]{0.5\linewidth}
%         \centering
%                 \includegraphics[width=\textwidth]{images/open_test_venns.pdf}
%         \centerline{(a) Open-source test cases}
%     \end{minipage}%
%     \begin{minipage}[t]{0.5\linewidth}
%         \centering
%                 \includegraphics[width=\textwidth]{images/industry_test_venns.pdf}
%         \centerline{(b) Industry test csaes}
%     \end{minipage}
%     \caption{Distribution of test cases repaired by different algorithms.}
%     \label{fig:venns-test-case}
% \end{figure}
% % \input{sections/discussion}


% Figure \ref{fig:venns-test-case} \delete{compares the} \add{shows a} Venn diagram of repaired test cases of  \watertool{*}, \vistatool{*}, \webevotool{*}, \sftmtool{*} and \toolName{} in the open-source and the industrial test dataset.
% The green, blue, pink, yellow, and orange represent the number of test cases repaired by \watertool{*}, \vistatool{*}, \webevotool{*}, \sftmtool{*} and \toolName{}, respectively.
% There are 8 test cases in the open-source dataset that can only be fixed by \toolName{}, while there are 2 test cases in the industrial dataset that can only be fixed by \toolName{}.
% On the other hand, there is only one test case from the open-source dataset that cannot be fixed by \toolName{} but fixed by other tools (\watertool{}).
% \add{%In this test, two buttons with the same text on different pages can accomplish the same function.
% %\watertool can be matched due to the simple use of text, but \toolName cannot be matched due to consideration of structural information.
% The test case, that \toolName{} failed to fix, needs to click a series of actions and then click an ``add task'' button.
% % In the app, the ``add task'' buttons appear on two different pages (home page and my task page), and the regions where the ``add task'' buttons are located are significantly different.
% % In the update, the ``add task'' button was moved to a different webpage, making the regions where the ``add task'' buttons are located significantly different.
% % This is the reason that \toolName{} failed to match the ``add task'' button.
% % In contrast, WATER correctly matches this element since it simply measures the similarity of the text, which is not changed in the webpage update.
% % This is the reason that UITestFix failed to match the ``add task'' button in different page but the WATER correctly matches this element since it simply measures the similarity of the text.
% After the webpage update, \toolName failed to match the ``add task'' button because this button was removed from the original page.
% In contrast,  \watertool matches this button with an ``add task'' button from a different page.
% These two buttons are matched by \watertool just because they simply have the same text.
% Since the matched ``add task'' button also completes the function of adding tasks and passes the assertion checking, this test is considered to be repaired successfully by \watertool.
% This situation happens relatively rarely (only once in the experiment).}
% We also noticed that some test cases could only be correctly fixed by a specific algorithm other than \toolName{}.
% For example, in the open-source test cases, there are 27 test cases that can only be fixed by \vistatool{} and \toolName{}, while in the industrial dataset, there are 6 test cases that can only be fixed by \sftmtool{} and \toolName{}.
% This means that although different algorithms have their own advantages, \toolName{} has a stronger ability to fix test cases.




% To better understand the capability of \toolName{} for future improvement, we manually analyze the 53 broken test cases which \toolName{} fails to repair. 
% Specifically, for each case, we categorize the reason behind the test failure by comparing the correct repair with the algorithm's repair results.
% % , and manually investigating the root cause of failures.
% %   by inspecting the program location in the broken tests where the crash occurs.
% Figure \ref{fig:evluation-error-analysis} shows the distribution of the six reasons behind the failure of \toolName.
% \begin{enumerate}
%     \item \textit{Add Action.} Add Action denotes that an action needs to be added to repair the test.
%     \item \textit{Delete Action.} Delete Action denotes that an action needs to be deleted to repair the test.
%     \item \textit{Modify Assert.} Modify Assert means that the expected value of the assertion needs to be updated in the test.
%     \item \textit{Branch Statement.}
%     Some test cases use some branch statements to enhance the stability of test cases, such as using if-else statements to handle 
%     the empty table data and the case of the table data not being empty.
%     % different situations with data. 
%     The branch statements executed in the new version may not have been executed in the old version, causing the inability to repair the test case in the new version due to the lack of action information. 
%     We label this reason of failure as Branch Statement.
%     % We labeled a crashing event as Branch Event when the event was not executed in the old version but in the new version, \toolName fails to repair the event due to the lack of event information.
%     \item \textit{Propagated Breakages}~\cite{whydowe}. 
%     Propagated Breakages refer to the scenario where the element is pointing to an incorrect element using the original locator without throwing \add{an} immediate exception but triggers a subsequent crash.
%     \item \textit{Incorrect Match.} The test case can be fixed by relocation, but the algorithm matches incorrectly or cannot find the matched element.
% \end{enumerate}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.48\textwidth]{images/evluation-error-analysis.pdf}
% \caption{Reasons behind the repair failures of \toolName.}
% \label{fig:evluation-error-analysis}
% \end{figure}

% As only 7 of them are caused by Incorrect Match (13.21\%), and \toolName can repair 113 (94.16\%) test cases requiring locator fixes, \add{and} this shows that \toolName performs well in repairing broken locators.
% This indicates that for the relocation type of repairs, \toolName already has a strong capability.
% Therefore, in the future, we will focus on the remaining types of repair failures.
% % We left repairing other types of failures as future work.


% % \begin{figure}[t]
% % \centering
% %     \includegraphics[width=0.48\textwidth]{images/industry_test_venns.pdf}
% % \caption{Reasons behind the repair failures of \toolName.}
% % \label{img:industry-test-venns}
% % \end{figure}









==> sections/introduction.tex <==
% \section{Introduction}
% Software Product Line Engineering (SPLE) promotes strategic, well-managed software reuse. In reality, however, reuse might be ad-hoc, often realized via artifact cloning. It has become increasingly common to create a variant software product, fix a defect or to add new feature by copying code fragments from similar context. Porting is particularly common in free and open source software projects, where code changes are ported across different versions of the same software or different projects altogether. Three types of porting can be identified based on the source and the target for the porting task, forward-porting, back-porting and cross-porting. Cross-porting is when the code is transferred between two different projects, while the former is within the same project but different versions. Forward-porting is when a patch is created to an older version and ported to the latest version, while back-porting is the when the patch is created to the latest version and ported back to an older version. Back-porting is usually easier and preferred since the latest API changes serve the purpose of supporting the writing of patches with less errors. When back-porting such code, the missing context and deviations can be taken from the latest version. However, when the patch is written to an old version, it may not fit the latest version and possibly would not behave correctly in the future versions as well. It's quite harder to take the missing pieces from the old kernel, because some of them might be removed with the purpose to discourage some behaviors or to force the developers to recheck some assumptions. 

% Currently backporting is typically done manually by a developer, on a case by case basis. The process of adapting a patch to fit into another context is tedious, time-consuming, error-prone and sometimes resulting in porting errors which cannot be detected at compile time. When developers port code from a reference to a target context, they usually expect the ported code to behave similarly. Chou et al report that a significant portion of operating system bugs come from ported edits~\cite{Chou2001}. Li et al. identify errors in Linux and FreeBSD resulting from developers forgetting to rename identifiers after porting code~\cite{Li2006}. Jiang et al present evidence of porting errors when similar code appears in different contexts~\cite{Jiang2007}. Porting error can also happen when developers evolve ported code differently~\cite{Juergens2009}. 

% Linux is an open-source operating system kernel that is evolving in a rapid rate since 1991. The Linux kernel runs on a multitude of devices ranging from servers to IoT devices. Given the increasing number of devices that depend on the Linux kernel and the rapid rate of evolution of the kernel, raises a challenge for device driver developers to ensure continuous availability of the driver code with the latest version of Linux kernel. One approach current device driver developers employ is to target the current mainline version of the Linux kernel, so that the driver code can be integrated into the Linux kernel distribution itself and maintained by the mainline kernel developers\cite{kernel-doc}. Some users however typically run older versions of the kernel which are considered to be more stable and such driver must be back ported to older kernel versions\cite{backport-framework}. 

% Linux back port project provides a compatibility library to mask the difference between the current mainline and the target stable version, which provides patches that allow a set of 800 drivers to target this compatibility library. Stable kernel version maintainers create these patches either manually or with the use of the transformation tool Coccinelle\cite{coccinelle}. In either case the developer has to determine where changes are needed in the code to back port and how to adapt the changes, which is tedious and error-prone. Thung et al presents a recommendation system that generates a ranked list of candidate transformations for backporting of Linux device drivers\cite{backport-framework}. Although they show a success rate of 68\% out of 100 device drivers, it is limited to transformation of a single line modification which cause a compiler error/warning. They focuse only on modification to an existing single statement which cause a compilation error, whereas a patch could be of multiple lines involving line insertions and deletions as well. Furthermore not all changes which are erroneous trigger any compiler error/warning message\cite{Zhen2018}.


% In this paper we propose a step further towards automating the backporting process by transforming patches from the mainline Linux into stable versions of Linux using a scalable, syntactic transformation learnt from the original mainline patch. Our approach accepts as input a patch in a given Linux version, the older stable Linux version to which the patch should be back ported (target Linux version) and the git repository that stores the changes to the Linux source code. First, our approach analyses the difference made in the original patch of the mainline Linux and extracts a transformation script, locate a similar context in the stable Linux version,  adapt the patch to the target context and apply the patch. The adaptation of the patch from the mainline Linux version into the target stable Linux version requires translation of any namespace differences, accounting the difference of the API calls, importing missing definitions and pruning of unnecessary modification which is not relevant for the target stable Linux version. 

% This paper makes the following contributions:

% \begin{itemize}
% 	\item {We present a technique implemented in a tool for vertical code transplantation that does not require developer to specify the patch location}
% 	\item {We evaluate \toolName ~effectiveness by transplanting 100 patches from mainline Linux kernel into a target stable version. We show that our tool can help developers fix bugs significantly better than manual process}
% \end{itemize}




==> sections/macro.tex <==
\newcommand{\watertool}{\textsc{Water}}
\newcommand{\edtool}{\textsc{Edit Dis}}
%\newcommand{\watertool}{\textsc{WATER}\xspace}
\newcommand{\waterlitetool}{\textsc{WATER-}\xspace}

\newcommand{\vistatool}{\textsc{Vista}}
\newcommand{\webevotool}{\textsc{WebEvo}\xspace}
\newcommand{\sftmtool}{\textsc{SFTM}\xspace}
\newcommand{\sftmplustool}{\textsc{SFTM+}\xspace}
\newcommand{\uitestfix}{\textsc{UITestFix}\xspace}


\newcommand{\timeout}{30}
\newcommand{\codephage}{$CodePhage^I$}
\newcommand{\toolAPR}{$F1X$}
\newcommand{\patchAPR}{$P_{F1X}$}
\newcommand{\sumID}{24}
\newcommand{\numfix}{20}
\newcommand{\numcone}{eight}%c1 
\newcommand{\numctwo}{11}%c2
\newcommand{\numCodePhage}{19}
\newcommand{\percentbackport}{8}
\newcommand{\numversions}{47}
\newcommand{\numstudy}{46}%TODO: change this

% Result
\newcommand{\acc}{75.1\%\xspace}

\newcommand{\numCVE}{30\xspace}
\newcommand{\numCorrectCVE}{21\xspace}
\newcommand{\precision}{86\%\xspace}
\newcommand{\recall}{82\%\xspace}

%TODO: shinhwei use this
\newcommand{\industryteststudy}{2,534}
\newcommand{\openteststudy}{173}
\newcommand{\openstudyapp}{five}
\newcommand{\industryevalapp}{two}
\newcommand{\totdiff}{28,828}
\newcommand{\totcommit}{1611}%1611 commits
\newcommand{\numbaseline}{four}
\newcommand{\cluster}{grouping}
\newcommand{\clusterb}{Grouping}

%Patches that can be formulated as validation check 
%\newcommand{\numClass}{four} %TODO: how many classes of vulnerabilities our subject cover?
\newcommand{\numScapel}{four} %TODO: how many we compare with muscapel

\newcommand{\probName}{propagation}
%\newtheorem{definition}{Definition}
\newcommand{\numSub}{14}
%\newcommand{\toolName}{Crochet}
% \newcommand{\toolName}{\textsc{UITestFix}\xspace}
\newcommand{\toolName}{\textsc{ChatGPT}\xspace}
% \newcommand{\company}{\textsc{BigCompanyA}\xspace}
\newcommand{\company}{\textsc{Huawei}\xspace}
\newcommand{\appa}{FabricInsight}
\newcommand{\appb}{CampusInsight}


\newcommand{\testDatasetA}{TestDataset2\xspace}
\newcommand{\testDatasetB}{TestDataset1\xspace}


\newcommand{\sydittool}{\textsc{Sydit}\xspace}
\newcommand{\msydittool}{\textsc{Sydit*}\xspace}
\newcommand{\refazer}{\textsc{Refazer}\xspace}
\newcommand{\genpat}{\textsc{GenPat}\xspace}



\newcommand{\erratumtool}{\textsc{Erratum}\xspace}
\newcommand{\guidertool}{\textsc{GUIDER}\xspace}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\newcommand{\toolScapel}{$\mu$SCALPEL}
\newcommand{\jasper}{JasPer}
\newcommand{\avgiterations}{six}
\newcommand{\numClass}{five}
\newcommand{\studyversion}{45}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\numdefects}{13}
\newcommand{\Plus}{\mathord{\begin{tikzpicture}[baseline=0ex, line width=0.5, scale=0.06]\draw (1,0) -- (1,2);
\draw (0,1) -- (2,1);
\end{tikzpicture}}}
\newcommand{\Minus}{\mathord{\begin{tikzpicture}[baseline=0ex, line width=0.5, scale=0.06]
\draw (0,1) -- (2,1);
\end{tikzpicture}}}

% Manual line number specifying macro
% Save the original way of printing the number
\let\othelstnumber=\thelstnumber
\def\createlinenumber#1#2{
    \edef\thelstnumber{%
        \unexpanded{%
            \ifnum#1=\value{lstnumber}\relax
              #2%
            \else}%
        \expandafter\unexpanded\expandafter{\thelstnumber\othelstnumber\fi}%
    }
    \ifx\othelstnumber=\relax\else
      \let\othelstnumber\relax
    \fi
}

% \newmdenv[innerlinewidth=0.5pt, roundcorner=4pt,linecolor=mycolor,innerleftmargin=6pt,
% innerrightmargin=6pt,innertopmargin=6pt,innerbottommargin=6pt]{mybox}

\newtcbox{\mybox}[1][breakable]{on line, enlarge top by=10pt, enlarge bottom by=10pt,
     boxsep=8pt, boxrule=2pt, size=small, arc=1mm}
     
     
\newcommand{\triple}[3]{\{#1\}~#2~\{#3\}}

\newcommand{\nbc}[3]{
    {\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
    {\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}
}

\lstset{
captionpos=b,
showspaces=false,
showstringspaces=false,
breaklines=true,
frame=tb,framerule=0.1pt,
keywordstyle=\ttfamily\bfseries,
commentstyle=\ttfamily\textit,
escapechar=\^,
%frame=single,
texcl=true
language=Java,
basicstyle=\ttfamily\footnotesize,
numbers=left,
stepnumber=1,
breakatwhitespace=false,
linewidth=0.45\textwidth,
xleftmargin=0.5cm,
escapeinside={(*@}{@*)}
}


%\usepackage{xcolor}
\definecolor{main-color}{rgb}{0.6627, 0.7176, 0.7764}
\definecolor{string-color}{rgb}{0.3333, 0.5254, 0.345}
\definecolor{key-color}{rgb}{0.8, 0.47, 0.196}
\lstdefinestyle{mystyle}
{
    language = Java,
    basicstyle = {\ttfamily \color{main-color}},
    stringstyle = {\color{string-color}},
    keywordstyle = {\color{key-color}},
    keywordstyle = [2]{\color{lime}},
    keywordstyle = [3]{\color{yellow}},
    keywordstyle = [4]{\color{teal}},
    morekeywords = [3]{<<, >>},
    morekeywords = [4]{++},
    basicstyle=\ttfamily\scriptsize,
    commentstyle=\color{blue}\ttfamily,
    morecomment=[f][\lstbg{red!20}]-,
    morecomment=[f][\lstbg{green!20}]+,
    morecomment=[f][\lstbg{yellow!20}]++,
    morecomment=[f][\lstbg{yellow!20}]--,
    morecomment=[f][\textit]{@@},
    texcl=false
}

%\usepackage{color, colortbl}
\definecolor{grey}{rgb}{0.7,0.7,0.7}

%diff
\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
  basicstyle=\ttfamily\scriptsize,,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\lstbg{yellow!20}]++,
  morecomment=[f][\textit]{@@},
  texcl=false
}

\newcommand{\abhik}[1]{\nbc{AR}{#1}{black}}
\newcommand{\ridwan}[1]{\nbc{RS}{#1}{purple}}
\newcommand{\xiang}[1]{\nbc{GX}{#1}{cyan}}
\newcommand{\shinhwei}[1]{\nbc{ST}{#1}{blue}}
\newcommand\sh[1]{\textcolor{blue}{#1}}
\newcommand{\yuanzhang}[1]{\nbc{YZ}{#1}{red}}
\newcommand{\yz}[1]{\textcolor{red}{#1}}
\newcommand{\zhuolin}[1]{\nbc{ZL}{#1}{orange}}
\newcommand{\zl}[1]{\textcolor{orange}{#1}}

\newcommand{\gjd}[1]{\nbc{GJD}{#1}{red}}
\newcommand{\ignore}[1]{}


% \newcommand{\add}[1]{\textcolor{blue}{#1}}
%\newcommand{\modify}[1]{\textcolor{red}{\st{#1}}}
\newcommand{\delete}[1]{\sout{#1}}
\newcommand{\add}[1]{#1}

==> sections/overview.tex <==
\section{Motivating Example}

TODO

% \label{sec:overview}


% \begin{figure}
% \begin{subfigure}[t]{0.45\textwidth}
% \centering
% \includegraphics[width=\textwidth]{images/matchexample2.pdf}
% \caption{MRBS Web apps of version 1.2.6.1 and 1.4.9, and part of the broken DeleteNegativeAreaTest.}
% \label{fig:picMRNS}
% \end{subfigure}
% \lstset{escapeinside={!@}{@!}}
% \begin{subfigure}[t]{0.45\textwidth}
% \begin{lstlisting}
% <tr>
%   <td !@\textcolor{red}{class="banner" bgcolor="\#C0E0FF" align="CENTER"}@!>
%         <a href="admin.php?day=28;month=01">Admin</a>
%    </td>... </tr>
% \end{lstlisting}
% \caption{The simplified HTML code of the banner in version 1.2.6.1\add{.}}
% \label{fig:old_version_MRBS}
% \end{subfigure}
% \lstset{escapeinside={!@}{@!}}
% \begin{subfigure}[t]{0.48\textwidth}
% \begin{lstlisting}
% <tr>
%  <td>
%     <a href="admin.php?day=28;month=01;!@\textcolor{blue}{area=888;room=409}@!">Rooms</a>
%  </td>...</tr>
% \end{lstlisting}
% \caption{The simplified HTML code of banner in version 1.4.9\add{.}}
% \label{fig:new_version_MRBS}
% \end{subfigure}
% \caption{Motivating example of MRBS webpage\add{.}}
% \label{fig:match-example}
% \end{figure}

% In this section, we use an example of \add{an} open-source app MRBS in the test 
%  cases dataset~\cite{imtiaz2021automated} 
% % \st{ (we did not use the industrial app to remain anonymous) }
%  to explain the shortcomings of existing approaches~\cite{choudhary2011water,stocco2018vista,shao2021webevo,brisset2020sftm}, and how \toolName fix\add{es} the broken test by matching elements.


% Figure \ref{fig:match-example} shows the screenshots of the MRBS app for version\add{s} 1.2.6.1 and 1.4.9, the simplified HTML code, and one simplified test.
% The broken test (\textit{DeleteNegativeAreaTest}) was manually translated to the Selenium test by the authors of prior work~\cite{imtiaz2021automated}. It contains three events: \circled{1} \textit{click} \add{the} ``Log in'' button, \circled{2} \textit{sleep}, and \circled{3} \textit{click} \add{the} ``Admin'' button.
% In Figure \ref{fig:old_version_MRBS}, we use $e_o^{Admin}$ to denote the old element with text \textit{Admin} and $e_o^{ban}$ to represent the old element with tag \textit{tr}, which is a banner. 
% Similarly, in Figure \ref{fig:new_version_MRBS}, we use $e_n^{Rooms}$ to represent the element with text \textit{Rooms} and $e_n^{ban}$ to represent the element with tag \textit{tr}.
% When \add{MRBS} evolved from 1.2.6.1 to 1.4.9, its view and attributes of elements changed drastically.
% For instance, the text of $e_o^{Admin}$ changed from ``\textit{Admin}'' to ``\textit{Rooms}'', 
% the background color of $e_o^{Admin}$ was changed from blue to dark blue, which caused the visual change, 
% % none of its attribute tokens is unique, 
% the attribute of $e_o^{Admin}$ was extended with ``\texttt{area=888;room=409}'',
% and all the attributes of the ancestors of $e_o^{Admin}$ (i.e., $e_o^{ban}$) were removed.
% % In the version 1.4.9, the locator of ``Log in'' button is ``//*[@id=``logon\_submit'']/input'' and the locator of ``Admin'' button is ``//a[text()=`Admin']''.
% The changes cause \textit{DeleteNegativeAreaTest} to fail in the new version.
% From the motivation example, we can obtain the following observations:
% %does not work anymore on the new version.

% % Most of exist matched methods\cite{stocco2018vista,choudhary2011water,shao2021webevo} failed in the action1, because there are two button with text \textit{Log In} and only SFTM\cite{brisset2020sftm} can use structural information to distinguish them.
% % Let us focus on the element of action 3 as an example.
% % Note that, the webpages that the $O_{Admin}$ and $N_{Rooms}$ jumps to have the same funtion, which contain four functions, \textit{Area}, \textit{Rooms}, \textit{Add Area} and \textit{Add Rooms}.


% %\noindent\textbf{Observation1: A element matching depends on other elements being matched first.} \yz{
% Existing approaches usually match elements by matching either their attributes~\cite{choudhary2011water}, visual information~\cite{stocco2018vista}, or both~\cite{shao2021webevo}. 
% % The significant changes on $e_o^{Admin}$ cause existing approaches to produce incorrect matching results.
% Due to the changes in the attributes and visual information, the similarity between $e^{Admin}_o$ and $e^{Rooms}_n$ is low. 
% Algorithms based on text information~\cite{choudhary2011water}, visual information~\cite{stocco2018vista}, or both~\cite{shao2021webevo} fail to match \add{$e_o^{Admin}$ with $e_n^{Rooms}$}.
% % these algorithms cannot correctly match elements $e_o^{Admin}$ and $e_n^{Rooms}$.
% % Specifically, as the text and attribute changes, matching strategies that rely solely on text or attribute matching~\cite{choudhary2011water} fail to match $e^o_{Admin}$ with $e^n_{Rooms}$.
% % Due to the visual changes, matching strategies relying on visual information (e.g., \vistatool~\cite{stocco2018vista}) also fail to match $e^o_{Admin}$ and $e^n_{Rooms}$.
% The SFTM algorithm~\cite{brisset2020sftm}, which matches attributes of the parent nodes and child nodes for similarity propagation, also fails to match $e_o^{Admin}$ with $e_n^{Rooms}$ because (1) the similarity score based on attribute matching is quite low due to the changes in attributes, and (2) the parent node of $e_o^{Admin}$ do not share common attribute tokens with the parent nodes of $e_n^{Rooms}$.

% By investigating this example, we have the following observation: \textit{an element matching could depend on its neighboring elements that have been matched.}
% In this example, there are multiple elements located in the banner $e_o^{ban}$, including the ``Help'' button, ``Admin'' button, ``Report'' button\delete{ and etc}.
% % so similar to the surrounding elements, they are used to jump to a target page. 
% % The shared attribute ``admin.php'' of $e_o^{Admin}$ and $e_n^{Rooms}$ implies that the target pages is consistent.
% Through the word ``admin.php'' also appears elsewhere on the page, %$e_o^{ban}$ and $e_n^{ban}$ can 
% the elements around $e_n^{Admin}$, e.g., the ``Help'' button of the old and new version which can be easily matched, can be used to distinguish $e_n^{Admin}$ with the ``admin.php'' elements located somewhere else. 
% %and help $e_o^{Admin}$ and $e_n^{Rooms}$ match correctly.
% % the matching of $e_o^{Admin}$ and $e_n^{Rooms}$ will depend on their parent elements $e_o^{ban}$ and $e_n^{ban}$ being able to match correctly and assist in their matching.
% It indicates that element matching could also be guided by the matching results of other elements.

% % \textbf{Observation2: Different types of elements have different meanings.} 

% % \yz{
% % Since the webpage is actually a DOM tree, functional elements such as the buttons that users usually contact are mainly elements at the bottom of the tree.
% % Other elements are used as containers of these functional elements and displayed to users in the form of regions.
% % Elements can therefore be divided into functional type elements and region type elements.
% % In Figure 1, elements with the ``tr'' tag represent the banner region, while elements with the ``td'' and ``a'' tags represent the ``Admin'' button.
% % The meaning of these two types of elements affects each other.
% % The meaning of the banner element depends on the meaning of the buttons located in it.
% % The meaning of the button is also limited by the region it locates in.
% % The similar element may express different meanings in different regions.
% % Existing tools simply calculate similarity based on text or visual information, ignoring the true meanings of elements of different types.
% % }


%  % The first step of fixing the given test is identifying the matched elements in the old and new versions.
% % parts of simplified DOM structures of \textit{Xfinity} home page in version 2018 and version 2020.
% % In this example, some representative elements are marked with blue labels, i.e., \texttt{O1}, \texttt{O2}, \texttt{O3} for version 2018, and \texttt{N1}, \texttt{N2}, \texttt{N3} for version 2020.
% % Let us take element \texttt{O3} as an example.
% % When \textit{Xfinity} evolved from 2018 to 2020, (1) the text of element \texttt{O3} was changed from ``\textit{TV}'' to ``\textit{TV \& Streaming}'', which also caused the visual changes, (2) the attribute of \texttt{O3} has also changed from \textit{"class": "shop-deals\_\_lob-name"} to \textit{"class": "x-heading-group3"}, (3) the DOM structure around \texttt{O3} was also changed, and there are no similar attributes between its parents.
% %First of all, its text has changed from \textit{TV} to \textit{TV\&Streaming}, which also caused the visual changes.
% %Second, its attribute has also changed from \textit{"class": "shop-deals\_\_lob-name"} to \textit{"class": "x-heading-group3"}.
% %Finally, the DOM structure around it also has obvious changes, and there are no similar attributes between its parents.
% % Specifically, changes in attributes and visual changes affect the accuracy of existing approaches.

% % The content in the red label means that the element is matched in \textit{ith} iteration by \toolName.

% %The DOM structure changes, and the fact that parent node does not share similar attributes make it difficult for approaches based on SFTM~\cite{brisset2020sftm} to use the attributes of the parent nodes for similarity propagation.
% %difficult for SFTM~\cite{brisset2020sftm} hard to use the attributes of their parent nodes for similarity propagation.
% %Therefore, none of these methods correctly matches $O7$.

% From the observations, we could measure the similarity of elements based on the following ideas.
% \begin{itemize}[leftmargin=*]
%     \item \textbf{\add{I1:} Elements with closer matched ancestor\add{s} are more similar.}
%     For any element $e_o$ in the old version and any node $e_n$ in the new version, if they have the matched ancestor (e.g., banner), we consider $e_o$ and $e_n$ to be structurally similar.
%     If the matched ancestor is closer to $e_o$ and $e_n$ (e.g., the \delete{right side} \add{child element} of the banner), $e_o$ and $e_n$ are more likely to match due to higher structural similarity.
    
%     \item \textbf{\add{I2:} Ancestors with more common leaf elements are more similar.}
%     For two ancestors (non-leaf elements), if most of their leaf elements match, they are likely to be matched.
%     For example, if most of the buttons in the banner before and after the version updates match, these banners tend to be matched.
    
%     \item \textbf{\add{I3:} Matching element\add{s} by multiple iterations.}
%     Different from existing approaches that rely on pre-defined similarity metrics in one single step, we could perform an iterative approach for matching.
%     In each iteration, a matching result is calculated.
%     The next iteration will recalculate the similarity based on the matching result and also update the matching result.
%     % we could perform matching via multiple iterations.
%     During the iterations, the higher-confident matching results could help to increase the similarity of the lower-confident matched elements through multiple iterations of matching.
% \end{itemize}



% % \noindent\textbf{Key Idea 2. Design similarity based on the type of elements.}
% % From observation 2, we have designed new similarities according to the features of different types elements.
% % Specifically, they are designed based on the two insights below:

% % Our main intuitions are (1) when the webpage evolves, certain elements are very likely to remain in the same region, e.g., $e^o_{Admin}$ remains in the same location (the middle banner); (2) the higher-confident matching results could help to increase the matching score for the lower-confident matched elements through multiple iterations of matching.
% % In other words, the matching result of subsequent iterations is determined by existing matching results.

% \emph{How does \toolName match these elements?}
% In the first iteration, \toolName{} has matched elements with high initial similarities (e.g., the element with text \textit{Help}). 
% % guide \toolName to match the correct elements.
% In the second iteration, the structural similarities of $e_o^{ban}$ and $e_n^{ban}$ are increased because the leaf nodes in the region represented by $e_o^{ban}$, i.e., the element with text \add{``}Help\add{''}, are matched in the first iteration.
% Then, in the third iteration, because the $e_o^{Admin}$ is contained in $e_o^{ban}$ and $e_n^{Rooms}$ is contained in $e_n^{ban}$, and $e_o^{ban}$ are matched with $e_n^{ban}$, the structural similarity between $e_o^{Admin}$ and $e_n^{Rooms}$ are increased.
% After the three iterations, the similarity between $e_o^{Admin}$ and $e_n^{Rooms}$ is larger than the threshold $\theta$, so they can be matched.
% This example shows the advantages of \toolName:
% (1) when attributes change significantly, using the matching results to calculate the structural similarity can enhance the accuracy of the matching;
% (2) in the process of multiple iterations, the elements in the previous iteration could guide the matching of the remaining elements.
% In some cases, the wrongly matched elements can even be corrected during the iterative process (not shown in this example). 

% % For instance, \watertool wrongly match the element of action 1 in above example\todo{modify} and match action 3 in wrong page. 
% %Sometimes the wrong matched elements are corrected during the iteration process, which is not shown in this example.
% With the matching results, \toolName will then repair the broken UI test by changing the locators of event \circled{1} and event \circled{3}.
% Specifically, \toolName updates the locator of the ``Log in'' button from ``/html/body/form/input[3]'' to ``//*[@id=``logon\_submit'']/input'', and the locator of ``Admin'' button from ``//a[text()=`Admin']'' to ``//a[text()=`Rooms']''.
% %Incorrect matching leads to propagated errors due the repair phase.\todo{this is strange}
% %For instance, the MRBS has two ``Log in'' buttons in the \textit{Login} page and \watertool incorrectly match the ``Log in'' button related to event 1 with another ``Log in'' button, which results in incorrect fix.


% % (1) Before execution, \toolName will instrument the test case, and will complete the information gathering and repairing in the instrumented code.
% % (2) In the version 1.2.6.1, \toolName will processing and save the webpage DOM infomation before each action executed.
% % (2) In the version 1.4.9, \toolName will try to check whether the element exist in this webpage, and use the matched locator to replace the original locator if the element is not exist. 

% % The XPath path of these elements and text of partial elements has changed.
% % These elements have only a small amount of attributes.
% % To describe elements more simply, we use $o5$ to represent element 5 in version 2018 and $n5$ to represent element 5 in version 2022, the same to other elements.
% % $o5$ is an element used to display data, and it is difficult to match the corresponding element.
% % The data of this type of element is likely to change during the version change process, which causes both the visual and text information of the element to change.
% % Unfortunately, $o5$ has only the attribute \textit{dir="Itr"} in addition to the text.
% % And $o4$, which is the parent element of $o5$, has only one text attribute that changes.
% % This makes $o5$ potentially difficult to match by itself or its parent.

% % When manually matching these elements, the following steps are usually taken.
% % First, the matching results of $o2$ and $o4$ are obtained, because they have a high degree of similarity with the $n2$ and $n4$.
% % Next, we can infer that the areas where the $o2$ and $o4$ are located match the areas where the $n2$ and $n4$ are located.
% % In fact, we knows that $o1$ matches element $n1$ and element $o4$ matches element $n4$ in this step.
% % Finally, both $o5$ and $n5$ are in the matching area and them have similar text styles, so it is judged that the $o5$ and $n5$ match.

% % How does \toolName match these elements?
% % First, match $o1$ and $n1$ through the equality of id attributes.
% % In the first round of iteration, $o2$ matches $n2$ and $o4$ matches $n4$ because the element's own similar attribute and the structural similarity enhanced by the match of $o1$ and $n1$.
% % In the second round of iteration, $o3$ and $n3$ are matched because their structural similarity is enhanced by the match result in the previous iteration.
% % During the third iteration, $o5$ and $n5$ are matched because the match of $o3$ and $n3$ enhances the structural similarity of o5 and n5.




% % \begin{figure}[!t]
% % \begin{subfigure}{0.43\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{images/structrue-example-left3.pdf}
% % \caption{DOM tree of v2018.} 
% %  \label{img:structrue-example-left}
% % \end{subfigure}
% % \begin{subfigure}{0.55\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{images/structrue-example-right3.pdf}
% % \caption{DOM tree of v2020.} 
% %  \label{img:structrue-example-right}
% % \end{subfigure}
% % \caption{Element matching example for \textit{Xfinity} home page.}
% %   \label{fig:matching-example-Xfinity}
% % \end{figure}
% % \begin{figure}[htbp]
% % \centering

% % \begin{minipage}{0.24\textwidth}
% % \centering
% % \includegraphics[width=1\textwidth]{images/structrue-example-left.jpg}
% % \caption{
% %  .} 
% %  \label{img:structrue-example-left}
% % \end{minipage}1

% % \begin{minipage}{0.24\textwidth}
% % \centering
% % \includegraphics[width=1\textwidth]{images/structure-example-right.jpg}
% % \caption{11} 
% % \label{img:structrue-example-right}
% % \end{minipage}

% % \end{figure}


% % \begin{figure*}[!th]
% % \vspace{-5pt}
% %   \centering
% %       \centering
% %       \includegraphics[width=0.9\textwidth]{images/ourapproach.jpg}
% %   \vspace{-5pt}
% %   \caption{Overview of our approach}
% %   \label{fig:overview}
% % \vspace{-5pt}
% % \end{figure*}
% % Our match method generally follows the following steps
% % \begin{enumerate}
% %     \item Preprocessing. Filtering non-displayable elements and  merging elements representing a function.
% %     \item Pre-matching. Match the elements with id first, and the matched elements will not change in the subsequent process.
% %     \item Similarity initialization. Construct the initial similarity matrix by attribute. 
% %     \item Iterative optimization. 
% %     In each iteration, our method will use the current matching result to recalculate a new similarity, and then use the new similarity to obtain an optimized matching result.
% % \end{enumerate}


% % After we get the matching result, we can verify the repaired result through the difference-based intent verification stage.



==> sections/sections/acknowledgements.tex <==
\section{Acknowledgements}
%TODO
% We appreciate the anonymous reviewers for their valuable comments and suggestions to improve our paper.
%We greatly appreciate the suggestions and effort provided by my MS thesis advisor, Shin Hwei Tan.Additionally, 
We greatly appreciate the effort of
Yuanzhang Lin for his help in annotating the ground truth fixes.
This work is supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) Discovery Grants (RGPIN-2024-04301). %Huawei (GUI Automation Testing Technology Collaboration Project - Automated Repair of Test Cases for adapting to UI changes), and the National Natural Science Foundation of China (Grant No. 62202026, 62141209).

==> sections/sections/backkground.tex <==
\section{Background And Related Work}
In this section, we introduce related work on test repair to provide a background on existing approaches.

%\subsection{Automatic UI test case repair.}
\noindent\textbf{Automatic UI test repair.}
Unlike traditional unit tests, UI tests are typically used to validate the functionality of particular UI application components through simulated user interactions such as button clicks.~\cite{water}.
% 可能需要更好地解释一下Web UI测试用例是什么，但是这里突然插入一段代码有些奇怪，如果有motivation可以结合就更好了。
%However, 
When a UI application evolves, the corresponding UI tests may crash, leading to significant effort required to manually fix these broken tests.  
Several techniques have been proposed for UI test maintenance~\cite{
water,vista,UITESTFIX,ATOM,CHATEM,sitar,theory_repair,Vifer,color,WTSR}.
Most of these techniques focus on maintaining UI tests for mobile applications~\cite{ATOM,CHATEM,xu2021guider,METER,Vifer}, Web applications~\cite{water,vista,color,UITESTFIX,WTSR} or desktop applications~\cite{sitar,theory_repair}.
% \todo{put all test repair for android apps in this}
% 讲述一下与APR的差距，重点在于信息从UI上获取。
%The key source of information for fixing UI tests usually originated from the old and new versions of the UI of the application under test.
Prior Web UI test repair techniques~\cite{water,vista,UITESTFIX} typically (1) execute the test, (2) extract information from the Webpage based on various attributes~\cite{water} or visual information~\cite{vista} of Web elements, (3) use various matching algorithms, and (4) update the locator of the matched element in the UI test to fix the broken test.

Model-based approaches~\cite{ATOM,CHATEM,sitar,theory_repair,dataset} build a model of the application under test and modify the event flow to fix tests.
% 我还没验证一下theory_repair的修复策略，但看zhuolin的描述是model-based
Meanwhile, several heuristic-based approaches~\cite{water,vista,UITESTFIX} relocate elements with UI matching algorithms and update broken tests via replacement of the matched elements.
As heuristic-based approaches without building a model are more practical for large-scale applications, our paper mainly evaluates these approaches.
A recent approach~\cite{Vifer} first matches elements of two versions of Android apps using various similarity metrics (e.g., semantic embedding
similarity, and layout similarity
based on node embeddings of the GUI layout tree), and then repairs the tests by updating broken locators.
 %and cannot be compiled,. %does not have open source code due to corporate copyright reasons, and other unopen source work~\cite{WTSR}UITESTFIX~\cite{UITESTFIX} does not have open source code due to corporate copyright reasons, and other unopen source work~\cite{WTSR} has also not been included in the baseline.
%Since the code provided in the paper lacks dependencies and cannot be compiled, we exclude the model-based tool~\cite{imtiaz2021automated} from the baseline.
% \yz{Some existing work~\cite{UITESTFIX,WTSR} has not been used as a baseline because its source code has not been open sourced.}
% Hang et al.~\cite{theory_repair} focus on the issue of mending dysfunctional workflows in GUI applications,
% but their approach does not specifically target the repair of actual tests and we do so.
% These approaches typically build a model (e.g., an event flow graph) to finish the task.  but obtaining an accurate application model in the real world is not easy, so we did not consider these tools as baselines in this paper.

\noindent\textbf{UI element matching.} Given an element from an old version web, UI element matching aims to find the corresponding element in the new version.
UI element matching has been applied to several domains (e.g., test reuse~\cite{10.1145/3460319.3464827,khalili2024semantic}, automated compatibility testing~\cite{CdDiff}, and automated maintenance of UI tests).
While several techniques exist for UI element matching, only a few are suitable for our evaluation.
This paper evaluates classic UI test repair tools \watertool{}~\cite{water} and \vistatool{}~\cite{vista}, which match elements based on attribute information and visual information, respectively. 
Existing repair work mainly relies on strategies based on element information~\cite{water,vista}, or simply combining machine learning algorithms with repair tools~\cite{Vifer}.
COLOR~\cite{color} and GUIDER~\cite{xu2021guider} use a combination of attribute and visual information for matching.
However, COLOR only returns updated locators instead of repairing broken tests while GUIDER focuses on Android test repair. 
% As our goal is to study UI test repair, we did not compare with tools~\cite{shao2021webevo,sftm2023} that perform matching without repair.
Due to the differences between UI tests and existing APR work~\cite{xia2023automated}, we may not be able to directly use prior APR approaches to repair UI tests. %\yz{toolName} technology to apply large models to the repair of UI test cases.
Unlike prior approaches, we explore the feasibility of using prior test repair approaches to obtain an initial ranked list of elements and use ChatGPT to perform subsequent matching.

Instead of fixing broken Web UI tests, several approaches focus on improving the robustness of the element.
\emph{Robula+} ~\cite{robula2} focuses on generating robust XPath locators because the authors' study found that XPath locators are sometimes the only option. \emph{Robula+} checks whether an element or its ancestors possess unique attributes from a predefined whitelist (e.g., id, name, class). If multiple attributes are found, it chooses the attribute with the highest priority to refine the XPath, thereby enhancing its robustness. 
Expanding on this, subsequent work ~\cite{robula3} recommends multiple locator generators voting on the outcome, favoring reliable generators. 
% which generates locators to see if an attribute uniquely locates an element based on a predefined attribute priority.
% They also later proposed using multiple locator generators to further increase the robustness~\cite{robula3}. 
% They determine the final result by having different locator generators vote, where they give higher weight to more reliable locator generators like \emph{Robula+}. 
%Due to legacy tests, it is costly to change all locators to robust ones. Moreover, some attributes (e.g., ID, name, data-*) may be absent for a UI element. %As acknowledged in prior work that aims to improve robustness of locators~\cite{robula3}, ``XPath locators are sometimes the only option'', indicating the needs to repair broken locators (possibly with XPath locators) instead of improving the robustness.
Our design of the experiment is similar in essence with \emph{Robula+}, letting ChatGPT make a selection among multiple candidates. However, our emphasis is on fixing broken locators instead of improving the robustness of the locators.
While enhancing the robustness of locators is outside the scope of this paper, it could be worthwhile future work to explore LLM-based approaches for generating robust locators. %we have not considered making the repaired locators more robust now, which may be a part of our future work.
% \watertool{} is one of the earliest Web UI test repair tool that focuses on structural changes and content changes related to Document Object Model (DOM) tree. 
% \noindent\textbf{Modify Assertion}
% Daniel and his team have conducted research on similar problems~\cite{update_assert1,update_assert2}, but their work has focused on areas other than web application testing.
%\noindent \textbf{UI element matching.}
%\noindent \textbf{Automatic UI test case repair.}

\noindent\textbf{LLMs in software maintenance.}
% ChatGPT trained with billions of parameters becomes prospect in the field of automatic program repair. 
LLMs such as ChatGPT have been applied for various software maintenance tasks ~\cite{msrrepair1,msrgpt,to2023better,Feldt2023aa,sobania2023analysis,fan2023automated}, including related tasks such as (1) test generation~\cite{Feldt2023aa,codamosa,yu2023llm,hu2023augmenting,el2024using,li2023nuances}, Android UI testing~\cite{10172490,feng2023prompting}, predicting flaky tests~\cite{9866550}, and (2) automated program repair~\cite{sobania2023analysis,fan2023automated,msrrepair1,multilingual}. ChatGPT is a transformer-based chatbot developed by OpenAI that helps developers create conversational AI applications~\cite{chatgpt_intro}.
%ChatGPT is designed to assist with various tasks, such as answering questions, providing explanations, generating text, and engaging in conversations. 
Our proposed approach uses ChatGPT for (1) Web UI element matching, (2) providing explanations for the selected elements, and (3) repairing broken statements in tests.  %A recent study revealed that the bug fixing performance of ChatGPT is competitive with existing program repair approaches and providing hints in form of the expected output for a certain input or an observed error message can further increase the bug fixing performance~\cite{sobania2023analysis}. 
To improve code-related generation for LLM-based approaches, a recent approach was proposed using knowledge gained during the pre-training and fine-tuning stage to augment training data and their results show
significant improvement for code summarization and code generation~\cite{to2023better}. Similar to this approach, our proposed workflow also uses the experience gained during the selection of UI elements (i.e., inconsistency in the previous explanation generated by ChatGPT) to improve the UI matching results.
Different from the aforementioned work, this paper focuses on using ChatGPT for solving the Web UI test repair problem that aims to perform UI test update by fixing broken UI element locators. 
To the best of our knowledge, our study also presents the first attempt that investigates and improves the quality of explanations provided by ChatGPT by designing an explanation validator to check the reliability of the explanation to improve the effectiveness of UI matching and test repair. 
%ChatGPT not only shows strong capabilities in the field of UI testing~\cite{Feldt2023aa,tang2023chatgpt}, but also has good performance in program automatic repair~\cite{sobania2023analysis,fan2023automated}. However, the Web UI test repair problem is different from these tasks as it mainly involves Web element matching where accurate matching results will usually lead to the correct repairs being generated.  


% Its dataset concludes tests cases in different programming languages, their bug reports and some solutions, which makes ChatGPT able to addressing various issues in the field of computer science, such as automated code repair and test case generation.

%Several studies have used large language models like ChatGPT to assist in several software maintenance tasks (e.g., testing ~\cite{Feldt2023aa} and repair~\cite{sobania2023analysis,fan2023automated}). 









%existing studies performance of ChatGPT in testing and repair 
%Its categories contain the third kind of change, \yuanzhang{What are the first two changes?} blind changes, which means the changes that are difficult for testers to find and solve directly. So WATER does not consider this kind of reason for broken tests. 

%\watertool{} is a tool that focuses on structural changes and content changes related to the DOM tree.  Its categories contain the third kind of change, \yuanzhang{What are the first two changes?} blind changes, which means the changes that are difficult for testers to find and solve directly. So WATER does not consider this kind of reason for broken tests. 

% To identify structural changes and content changes, \watertool{} collects data about each node of the DOM tree
% before repairing, including \emph{id}, \emph{XPath}, \emph{class}, and other attributes. 
% Then, \watertool{} uses the similarity \cite{similarity_aid} of five attributes \emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, and \emph{name} as the basis for selecting matching elements.

% At the same time, if the \emph{tagName} of the candidate element is not the same as that of the target element, it is considered a mismatch.
% This is because \watertool{} believes that there are few updates to the \emph{tagName} on the webpage.
% But in reality, is present (the example of input becoming form or vice versa), so elements with different \emph{tagName} should not be removed from the list of candidate elements list.

% Its repair process can be concluded as searching for the matched elements in the DOM tree by calculating and comparing the similarities. 
% It uses Levenshtein Distance \cite{edit_distance} to calculate the similarity between the elements' attributes. But it does not take visual information into account.

% Additionally, \watertool{} also checks for data obsolescence. 
% For example, if the expected value in the assert statement should be updated when the page is updated, \watertool{} will detect it and suggest to testers a repair result. 


%\subsection{VISTA}
% \noindent\textbf{\vistatool.}
% Compared to \watertool, \vistatool{} combines computer vision and local crawling with the visual information from executing the test cases, which provides test cases’ automatic repair.
% Since the GUI of web applications is often modified to accommodate the latest trends in appearance and style. These changes can make image matching difficult.

% To solve this problem, \vistatool{} uses Feature Detection for Template Absence and Presence.
% The main idea is to find some key points in the image and store the neighborhood information of these key points as the description of the template \cite{template_matching}.
% Then, after finding the descriptors of the key points in the reference image, the algorithm tries to match two sets of descriptors (one from the template and the other from the reference image) and see how many descriptors match.
% For feature detection, a combination of SIFT \cite{sift1}\cite{sift2} and FAST \cite{fast1} \cite{fast2} algorithms is used. Because these two detectors can detect complementary feature points.
% The element is considered as a possible match if at least 70\% of the key points match.
% Then, the Fast Normalized Cross Correlation algorithm of the open-source computer vision library OpenCV \cite{openCV}is then used for template matching and its results are considered the best matching position.



% For repair, \vistatool{} traces the process and captures
% screenshots for future comparison when testing the old version of a webpage.
% Then, when using these benchmarks on a new version, \vistatool{} will first verify whether
% the case can find the corresponding web element.
% No matter whether the finding is successful or not, \vistatool{} will do a visual search to
% verify whether the result is right, or find if the web element exists on the current
% page.


% If the result is incorrect, \vistatool{} will recognize it as a web UI update. However,
% if the element does not exist on this page, \vistatool{} will do the next step: local crawling.
% Local crawling means that \vistatool{} will try to find this web element on neighboring
% pages by doing a visual search again. If the element is found, \vistatool{} will store the \emph{XPath}
% of reaching that page and add it to the benchmarks as a statement. Else it will consider
% the element as removed and suggest deleting this statement.

% For each test case, the flow chart is in the Figure \ref{Visual test repair process} below:


% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/content/vista.png}
%     \caption{Visual test repair process}
%     \label{Visual test repair process}
% \end{figure}


% But VISTA has low performance on non-visual changes, which is its disadvantage.


% \yz{...In this paper, we hope to use these features of ChatGPT to improve the repair capabilities of UI test cases.}




% Prior study \cite{test_generate} studied the performance of LLMs in generating test cases. He concluded that with the help of LLMs, testers can generate valid, accurate, and complete (covering all scenarios) test cases more easily and efficiently. 
% Prior study \cite{APR} used Generative Pre-trained Transformaer (GPT-2) in Automated Program Repair (APR) and got accuracy 17.25\%. He concluded that if the models trained with more parameters, the results might be better.
% Therefore, in this research, we aim to investigate whether ChatGPT, a large language model trained by OpenAI, can do better than existing web UI test repair tools VISTA and WATER. 
% ChatGPT has demonstrated remarkable capabilities in various natural language processing tasks and has the potential to analyze and understand the context of web UI test cases better than existing tools. 
% Therefore, we plan to compare the performance of ChatGPT with VISTA and WATER in terms of repairing web UI test cases for a set of web applications. 
% We will evaluate the accuracy of repairs suggested by each tool, the time required to suggest repairs and the scalability of the tools for larger test suites.
% The results of this research can provide insights into the potential of using state-of-the-art language models for web UI test repair and help improve the quality and efficiency of automated testing for web applications.






% We denote a web element as $e$.
% When the web application is updated, test cases may fail due to the inability to locate element $e$ in the updated version.
% The automated UI test repair tool fixes the test case by relocating the element $e$ through the element matching algorithm.
% % Element matching algorithms are also commonly used to identify changes in the interface.
% Specifically, for an element $e_o$ in the old version, the element matching algorithm needs to find the corresponding element $e_n$ in the new version page, and the match result can be denoted as $\{e_o \mapsto e_n\}$.
% If there is no matching result for $e_o$, it will be considered a deleted element.
% Similarly, when there is no match result for $e_n$, it will be considered as an added element.


% % \noindent\textbf{Study on breakages.}


% \paragraph{\textbf{Existing element match method}} 
% The element matching algorithm has been proposed for many years.
% The element matching algorithm can be mainly divided into two categories,  element-based, and tree-based approaches.
% For the element-based approach, the matching algorithm takes the old version element $e_o$ and the element list ${E}_n$ of the new version as input and outputs the matching result $\{e_o \mapsto e_n\} \mathtt{where} \ e_n \in {E}_n$.
% Existing approaches check the similarity of elements by measuring the similarity of elements' attribute\add{s}, e.g., \watertool{}~\cite{choudhary2011water}, elements' vision information, e.g., \vistatool{}~\cite{stocco2018vista}, and the combination of attributes and vision, e.g., \webevotool{}~\cite{shao2021webevo}.
% % The attribute-based algorithm \watertool{}~\cite{choudhary2011water}, the vision-based algorithm \vistatool{}~\cite{stocco2018vista}, and the combination of text and vision algorithm \webevotool{}~\cite{shao2021webevo} all belong to this category.
% While the DOM tree-based algorithm takes the old version Dom tree $\mathcal{T}_o$ and the new version DOM tree $\mathcal{T}_n$ as input\add{s}, and outputs the matching result $\mathcal{M}$, which includes all matching relationships $\{e_o \mapsto e_n | e_o \in \mathcal{T}_o \wedge e_n \in \mathcal{T}_n\}$.
% The tree-based method can determine the final matching result \add{by considering the relationship between elements.}\delete{from the perspective of all elements.}
% The \sftmtool{} is the tree-based matching method, which has shown good matching results.

% % \noindent\textbf{Non-leaf node and leaf node.}







% \paragraph{\textbf{Existing repair framework}}
% Existing repair frameworks can be divided into  offline mode and online  mode.
% In \add{the} offline mode, such as \watertool{}~\cite{choudhary2011water}, information is collected during the execution and repairs are made after the execution. 
% In online mode, such as \vistatool{}~\cite{stocco2018vista}, information is collected\add{,} and repairs are made at the runtime.
% Compared with offline mode, online mode can fix multiple breakages in a single run.
% To support online repair, \vistatool{} utilizes Java Parser and regular expressions to parse the test cases into a list of $\langle$locator, action, parameters$\rangle$\delete{, and t}\add{.T}hen \add{it} executes each action according \delete{at}\add{to} the sequences \add{of the list}.
% When an element of \add{the} new version is failed to \add{be} localized, \vistatool{} automatically fix\add{es} the locator and execute\add{s} the broken action again.
% However, due to complex test scenarios and free coding styles, \vistatool{}  may not be able to parse test cases using regular expressions, hence causing repair failures.
% For example, test cases written by the page-object design pattern~\cite{leotta2013improving} are difficult to parse \add{by} using regular expressions.

% \paragraph{\textbf{Definition of successful repair and successful match}}
% % After a web UI test case tests a certain functionality of the interface, it
% To test a certain functionality, developers usually use assertion to determine if the execution result of the test case is correct.
% Therefore, a correctly fixed test case should meet two criteria: (1) the test execution can cover the original functionality, and (2) the test case assertion passes.
% In terms of successful element matching, due to element nesting, there may be more than one element implementing a certain function \delete{in}\add{on} a webpage.
% Different algorithms' strategies may produce different and correct matching results, i.e., match one element to different elements that represent the same function.
% As these elements implement \add{the} same functionality, we consider the matching results of the elements to be a many-to-many relationship.


% % \noindent\textbf{Static repair and dynamic repair.}





==> sections/sections/conclusion.tex <==

\section{Conclusions}
This paper presents the first feasibility study that evaluates the effectiveness of
using prior Web UI repair techniques for initial matching and then using ChatGPT to perform subsequent matching to mitigate the bias in prioritization of attributes of prior approaches. To reduce hallucination in ChatGPT, we introduce an explanation validator that checks the consistency of the provided explanation, and gives hints to ChatGPT via a self-correction prompt to further improve its results. Our evaluation on a widely used dataset shows that the combinations with ChatGPT improve the effectiveness of prior techniques. Our study also reveals several findings and implications. As an initial study that focuses on LLM-based Web test repair, we hope that our study could shed light in improving future Web UI test repair approaches.

% \noindent \textbf{Data availability. }The data and code are available at:~\cite{reproducibility}. 

% https://anonymous.4open.science/r/ChatGPTUITestRepair-7169.

% In summary, ChatGPT does a better job of matching Web UI elements and repairs relevant broken statements more correctly than WATER and VISTA.
% We first explored the results of WATER and VISTA and where they could be improved. The results show that WATER is better at breakages caused by non-structural information changes while VISTA is better at breakages caused by structural information changes.

% We then explored the reliability of ChatGPT's handling of the Web UI test case repair task. We split the task into two sub-blocks, matching elements and repairing broken test statements where elements' locators fail.

% Our first part of experimental results show that ChatGPT is basically consistent in its responses in the matching task, tending to answer the same result in three repetitions of the prompt. It was also more compliant with the instructions specified in the prompt as to which perspective to consider from. Even though its explanations of why it selects an element need improvement, it has a relatively high proportion of the ground truth element selected. Non-structural information allows ChatGPT to get better results than structural information.


% Our second experimental results show that filtering candidate elements according to the Text Editing Distance of \emph{XPath} gives ChatGPT best results and efficiency. In comparison, filtering candidate elements with WATER and VISTA also gives ChatGPT higher correct matching and repair rate than using WATER or VISTA without ChatGPT, but the overall efficiency of this repair approach is lower considering the complexity of the algorithm used to filter candidate elements.
% It is worth noting that ChatGPT also prefers to use the original locating strategy of broken statements in the repair process. This helps to maintain the original code style of the test case writer more than WATER and VISTA, which use a fixed repair pattern.


% To better understand the challenges of repairing broken UI tests, we perform a case study of Web UI test maintenance in open-source and industrial apps.~\xiang{remove study and extend the conclusion a little bit}
% Our study shows that the rising demand for test repair and the complexity of the UI tests in industrial apps pose additional challenges for Web UI test repair in industrial setting. 
% Inspired by our study,
% In recent years, the automatic repair of web UI test cases has gained widespread attention.
% However, existing methods do not fully utilize structural information, resulting in lower accuracy when matching elements with significant changes.
% In this paper, we proposed \toolName, an approach based on a novel iterative matching algorithm for fixing broken UI tests.
% \toolName can use the existing matching results to update the similarity and adjust it during the iteration process. 
% Therefore, it can use high-similarity elements to help match low-similarity elements.
% Our evaluation of publicly available and industrial datasets shows that \toolName{} outperforms \numbaseline{} prior approaches in producing more accurate matching and correct repairs. 
% We analyzed the test cases in which \toolName failed to repair, and the results showed that \toolName could repair 94.16\% of the test cases that only require relocation.






%In future, we plan to extend \toolName{} to repair UI events, and further improve its accuracy and efficiency.
% \begin{tcolorbox}[left=1pt,right=1pt,top=0pt,bottom=0pt]
% Dataset and tool: \href{https://anonymous.4open.science/r/Web-UI-Dataset-B856}{https://anonymous.4open.science/r/Web-UI-Dataset-B856}. 
% \end{tcolorbox}
%Due to the popularity and importance of the Linux kernel, it could be worthwhile for the program repair community to evaluate efficacy of repair techniques on Linux. We have made an open-source release of \toolName to accelerate this process. %A docker image of our tool is publicly available\footnote{https://hub.docker.com/repository/docker/rshariffdeen/fixmorph} as well.
 
%ecause it is a largWeb UI test maintenancee-scale widely used codebase. The sheer complexity of the patches, the diversity of the transformations involved, and the absence of test cases as specification pose additional challenges for patch backporting. Due to the popularity and importance of the Linux kernel, it could be worthwhile for the program repair community to evaluate efficacy of repair techniques on Linux. We have made an open-source release of \toolName to accelerate this process. %A docker image of our tool is publicly available\footnote{https://hub.docker.com/repository/docker/rshariffdeen/fixmorph} as well. 
 
%We conducted our research in a responsible fashion {\em without} introducing any unverified patches into the Linux kernel. In our envisioned workflow, the patches are generated by our tool \toolName as a first step; they need to be vetted thoroughly by the human developer in charge of the process before getting introduced into the code-base of Linux versions.

% At a technical level, this paper studies a different problem from automated program repair. Instead of trying to generate fixes or search for fixes, it tries to transplant a {\em known} fix into other program versions --- the automated patch transplantation problem \cite{PatchWeave}. This work attempts to show the promise of automated transplantation of patches on the Linux kernel code-base, thereby demonstrating the practical promise of such techniques. Apart from automating software maintenance tasks, such patch transplantation is of significant practical value for reducing exposure to security vulnerabilities. With the attack surface moving to edge devices (which may be running older versions of Linux), propagating patches to old Linux versions can be a meaningful security enhancement aid.



==> sections/sections/dataset.tex <==
\section{Experimental Setup}
\noindent\textbf{Dataset.}
We use an existing dataset~\cite{dataset} to evaluate the effectiveness of Web test repair approaches. We use this dataset because (1) it is the only publicly available dataset for Web UI test repair, and (2) it has been widely used in prior evaluations of Web UI test repair approaches~\cite{UITESTFIX,dataset}. The dataset contains Java Selenium UI tests from five open-source real-world Web applications (and VISTA~\cite{vista} used 3 of them). All of these open-source applications are hosted in Sourceforge (except for MantisBT that is hosted in GitHub~\cite{mantisbt}). We follow the same filtering process of a prior evaluation~\cite{UITESTFIX} to remove duplicated tests and non-broken tests. Subsequently, we obtained 62 test cases containing 139 broken statements as our dataset. Each test script contains 1 to 6 broken statements, with an average of 70 lines of code per script. 


\noindent\textbf{Baselines selection.} We evaluated three approaches (\watertool{}, \vistatool{}, \edtool{}) that are widely used in prior studies of Web UI test repair. 
Similar to prior study~\cite{UITESTFIX}, we exclude the model-based tool~\cite{dataset} as the provided code leads to compilation errors due to missing dependencies. We did not compare against several approaches~\cite{UITESTFIX, WTSR} as their matching algorithms are not publicly available so we could not evaluate their effectiveness in both matching and repair.

\noindent\textbf{Comparison with recent approaches.} %\todo{check if want to remove this}
%As our idea is to enhance prior techniques with subsequent matching using ChatGPT, 
To assess the effectiveness of our approaches, we also evaluate two recent approaches: \webevotool~\cite{shao2021webevo}, which employs DOM tree-based change detection, history-based semantic structure change detection, and semantics-based visual search to match elements; and \sftmtool{}~\cite{sftm2023}, which uses TD-IDF to calculate the initial similarity score on tokenized attributes and iteratively refines the matching based on the DOM structure.
% (\webevotool~\cite{shao2021webevo} and \sftmtool{}~\cite{sftm2023}). \webevotool uses DOM tree based change detection, history-based semantic structure change detection, and semantics-based visual search to match elements. 
% In our experiments, we used the version of WebEvo implemented by \cite{UITESTFIX}, which includes only the third stage. % \noindent\textbf{SFTM:} It
% \sftmtool{} uses TD-IDF to calculate the initial similarity score on the tokenized \emph{XPath}, \emph{tagName}, and other attributes, then propagates the similarity scores iteratively to refine the matching based on the DOM structure. 
%WebEvo uses DOM tree based change detection, history-based semantic structure change detection, and semantics-based visual search to iteratively match elements. SFTM uses a similarity-based approach and propagated the similarity scores iteratively to refine the matching between nodes. 
We did not combine these approaches with ChatGPT due to budget constraints.

We used the implementations of \watertool, \vistatool, \webevotool, \sftmtool{} from \uitestfix\cite{UITESTFIX} for evaluation, which includes the re-implemented \watertool{} by \vistatool\cite{vista}, and open-source implementations for the other tools.
%We did not compare with
%\noindent\textbf{Comparison with other matching algorithms.}
%Theoretically, 
%Tools that perform UI matching (e.g., WebEvo~\cite{shao2021webevo} and SFTM~\cite{sftm2023} can be used for guiding repair but
%we exclude these tools as we focus on UI test repair approaches. Moreover, WebEvo and SFTM already contain rematching processes that iteratively enhance their matching result, so we chose not to combine ChatGPT with them for additional matching refinements.
%\todo{add reasons for not comparing with WebEvo and SFTM or remove these reasons} 
%Specifically, WebEvo employs Dom tree based change detaction, history based semantic structure change detection, and semantics-based visual search to iteratively match elements.
%SFTM uses similarity-based approach and propagated the similarity scores iteratively to refine the matching between tree nodes.

%We did not compare against the model-based tool in prior work~\cite{dataset} as the provided source code fails to compile due to missing dependencies. 


\noindent\textbf{Preparing ground truth dataset.} As our evaluation dataset ~\cite{dataset, UITESTFIX} only has tests for the old versions of apps, and the test fixes are unavailable, we need to manually label the ground truths for the matching UI elements for the new versions. %, and (2) construct the ground truth for the repaired statements.
Specifically, two annotators independently labeled ground truths for each UI element located in the broken statement in the dataset for the three individual baselines (\watertool,\vistatool,\edtool). The annotators are graduate students with over one year of experience in relevant research of Web UI test repair. For 12 cases out of 3*139=417 cases (139 for each of the 3 individual baselines), the annotators had disagreements and met to resolve. 
% (Cohen's Kappa=0.94 which indicates almost perfect agreement). 

%\noindent\textbf{Checking repair.}
%In our experiment, we use the ground truths to make sure that all candidates are collected from the correct page. Each broken statement is independent and would not happen. \todo{xzl: perfect locallization}
% We use an existing dataset~\cite{dataset} containing 5 open-source Web applications (3 of which are used in the experiment of VISTA~\cite{vista}). After removing duplicated tests and tests without assertion, there are 135 test cases. Among these 135 scripts, 22 can be executed successfully on the new version of the webpage and do not need to be repair so we excluded these 22 scripts (``Excluded'' column). Additionally, some scripts involve the addition or removal of modules or event, which means they can not be repaired by merely modifying the locator of original statements. Simultaneously, there are test cases that original locator points to the wrong element instead of throwing NoSuchElementException or InalidElementStateException, making it challenging to identify the root cause of the breakage.  These have been marked under the ``Irreparable'' column. The column \emph{Repairable} shows the remaining 62 test cases, for which we manually labeled the ground truths. The column \emph{Broken Stm} specifies the corresponding number of broken statements within the repairable test cases, which we employ in the subsequent experiment. For 12 cases, the first two authors meet to resolve the disagreement.

% \begin{table}[!t]
% \centering
% % \setlength{\tabcolsep}{2.2pt}
% \small
% \vspace{-3pt}
% \caption{The original and modified versions of the selected webpages for the open-source apps}
% \vspace{-3pt}
% \resizebox{0.43\textwidth}{!}{%
% \begin{tabular}{ll|rr}\toprule
% Label & Application & Original Version & Modified Version \\\hline\hline
% I     & AddressBook & 4.0              & 6.1              \\
% II    & Claroline   & 1.10.7           & 1.11.5           \\
% III   & Collabtive  & 0.65             & 1.0              \\
% IV    & MantisBT    & 1.1.8            & 1.2.0            \\
% V     & MRBS        & 1.2.6.1          & 1.4.9            \\ 
% \bottomrule
% \end{tabular}}
% \vspace{-3pt}
% \label{table:open-source-application-version}
% \vspace{-5pt}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


Table \ref{table:open-source-application-version} shows the old and updated versions of the open-source Web apps in our dataset. The ``$\Delta$V'' column denotes the number of versions between them where a greater number means more significant UI changes, posing more challenges to matching and repair tasks. The ``Test'' column denotes the number of tests for each app, whereas the ``Broken Stmt'' denotes the number of broken statements per app. Our experiment assumes each broken statement is independent so that we can measure the effectiveness of ChatGPT in fixing each broken statement. This assumption is similar to
prior evaluations~\cite{dearrepair,lutellier2020coconut} of learning-based automated repair techniques where the correct fault location is provided. %(perfect localization) .

%\sh{TODO: add the number of test scripts and broken statements for each versions} \todo{lqs: do we need to describe more? }
% “” ``''

All experiments are run on a computer with an Intel Core i5 processor (\SI{1.6}{GHz}) and \SI{12}{GB} RAM. For the experiments related to ChatGPT, we use the API of gpt-3.5-turbo model (which was the latest at the time of our experiments) and set the temperature to 0.8 as used in prior work~\cite{fan2023automated}. 
%is renamed to gpt-3.5-turbo-0613, but deprecated on 2024.6, so we can't find it on the webpage

% Our experiment with ChatGPT costs USD 10.96 in total (which uses 8,429 API requests, and 7,178,802 tokens).
% Zhuolin: delete this because these data excludes the experiment of ChatGPT only

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[H]
% \caption{The number of test cases and broken statements}
% \label{table:dataset}
% \resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{l|rrrrr}
% \hline
% \multicolumn{1}{l|}{Applications} &
%   \multicolumn{1}{l}{Total} &
%   \multicolumn{1}{l}{Excluded} &
%   \multicolumn{1}{l}{Irreparable} &
%   \multicolumn{1}{l}{Repairable} &
%   \multicolumn{1}{l}{Broken Stm} \\ \hline
% AddressBook & 16  & 8  & 6  & 2  & 2   \\
% Claroline   & 31  & 0  & 4  & 27 & 53  \\
% Collabtive  & 18  & 13 & 1  & 4  & 11  \\
% MatnsiBt    & 45  & 1  & 19 & 25 & 66  \\
% MRBS        & 25  & 0  & 21 & 4  & 7   \\ \hline
% Total       & 135 & 22 & 51 & 62 & 139 \\ \hline
% \end{tabular}%
% }
% \end{table}

% Since this is a project of business company, because of the copyright issues, we are not allowed to open source the code for \toolName{}.
% % We open sourced our datasets and experimental results.
% To make our results to be replicated, our dataset and experimental data are available at {\\ \href{https://anonymous.4open.science/r/Web-UI-Dataset-9645}{https://anonymous.4open.science/r/Web-UI-Dataset-9645}}. 
% \yuanzhang{Can I open source the code of the elements match experiment framework without our algorithm?}


% \begin{table}[]
% \centering
% % \setlength{\tabcolsep}{2.2pt}
% \small

%\caption{The old and updated versions of the selected webpages for the open-source apps}
% \caption{Statistics of open-source Web apps in our dataset}
% \label{table:open-source-application-version}
% %\vspace{-6pt}
% \resizebox{0.9\linewidth}{!}{%
% \begin{tabular}{l|rrr|rr}
% \hline
% Application &
%   \multicolumn{1}{c}{$\Delta$V} &
%   \multicolumn{1}{c}{Old Version} &
%   \multicolumn{1}{c|}{Updated Version} &
%   \multicolumn{1}{c}{Tests} &
%   \multicolumn{1}{c}{Broken Stmt} \\ \hline
% AddressBook & 8  & 4.0       & 6.1    & 2  & 2  \\
% Claroline   & 29 & 1.10.7  & 1.11.5 & 27 & 53 \\
% Collabtive  & 5  & 0.65    & 1      & 4  & 11 \\
% MantisBT    & 38 & 1.1.8   & 1.2.0  & 25 & 66 \\
% MRBS        & 24 & 1.2.6.1 & 1.4.9  & 4  & 7  \\ \hline
% \end{tabular}%
% }
% \vspace{-6pt}
% \end{table}

\begin{table}[]
\centering
% \setlength{\tabcolsep}{2.2pt}
\small

%\caption{The old and updated versions of the selected webpages for the open-source apps}
\caption{Statistics of open-source Web apps in our dataset}
\label{table:open-source-application-version}
%\vspace{-6pt}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l|rrr|rr}
\hline
Application & \multicolumn{1}{c}{$\Delta$V} & \multicolumn{1}{c}{Old Version} & \multicolumn{1}{c|}{Updated Version} & \multicolumn{1}{c}{Tests} & \multicolumn{1}{c}{Broken Stmt} \\ \hline
AddressBook & 8                             & 4.0                             & 6.1                                  & 2                         & 2                               \\
Claroline   & 29                            & 1.10.7                          & 1.11.5                               & 27                        & 53                              \\
Collabtive  & 5                             & 0.65                            & 1                                    & 4                         & 11                              \\
MantisBT    & 38                            & 1.1.8                           & 1.2.0                                & 25                        & 66                              \\
MRBS        & 24                            & 1.2.6.1                         & 1.4.9                                & 4                         & 7                               \\ \hline
Avg/Total   & 21                            & -                               & -                                    & 62                        & 139                             \\ \hline
\end{tabular}
}
\end{table}

==> sections/sections/discussion.tex <==
\section{Threats to Validity}
Additional programming languages. Because the experiments in this paper are based on a dataset composed of test cases written in Java, the results are only applicable to the repair of Java test cases. Even though we found ChatGPT would sometimes return repaired statements written in Python under flexible prompts, which means ChatGPT may have the ability in repairing broken statements with other programming languages, we reinforced prompt constraints to let ChatGPT give results in Java due to the limitations of the dataset.
% In the meanwhile, since the scripts test web UI instead of Android UI or others, the result only applies to web UI test repair.

Data leakage. Although the repository where we found the test cases for the old version of web applications did not include corresponding repaired scripts for updated web applications, it is difficult to know whether the data producers labeled the ground truths for these scripts as part of the training data of ChatGPT. However, since web applications update frequently, leading to many new versions already available, the probability that we and the data producers happen to choose the same versions as new versions are low. With a different version being the target version, the repair results might be different and will not cause data leakage. Even if the ground truths are in the training data, its effect may be tiny since it is a very small amount in about 45 TB of training data totally.~\cite{GPT3_data_amount}


Availability. Even though this article only examines the effectiveness of ChatGPT in web UI test repair, it shows the promise of LLMs in this field. Thus, even if ChatGPT cannot be used in the future due to various limitations, it can be replaced by other similar LLMs, such as Codex, which has been proven effective in the area of automotive program repair~\cite{codex}.



% %\subsection{Discussion}

% %In this section, we  present some real examples from our evaluation to understand the capabilities of \toolName.

% % \paragraph{Better than the developer patch.} Backporting patches is an error-prone task, in which developers can make mistakes.
% % In our evaluation, we find that~\toolName performs better than the developer in some cases.
% % For instance, the mainline patch at commit ID 45d73860\footnote{The detail of each commit can be found in https://kernel.googlesource.com/ pub/scm/linux/kernel/git/stable/linux-stable/+/COMMIT\_ID} %\textasciicircum!
% % fixes a bug in a usb driver, in which a delay is added to the function \verb+musb_h_tx_flush_fifo+. However, the developer backported this patch at commit ID 98b91bfa to a different function \verb+musb_host_tx+ in the same file although the original function \verb+musb_h_tx_flush_fifo+ exists in the old version. This patch was eventually reverted at commit ID c8443922 after 42 days.
% % In contrast, \toolName transforms the patch at the correct location. 

% % \paragraph{Semantically equivalent with the developer's patch.}
% % We find instances where~\toolName backports a patch in a syntactically different but semantically equivalent way as the developer.
% % The mainline patch at commit ID 74717b28 fixes a bug in the RTC interface.
% % This patch changes an if-condition by inserting a function call to \verb+ktime_before+.
% % Unfortunately, this function does not exist in v3.2.
% % When this patch was backported to v3.2 (commit ID 69328181), the developer improvised and replaced the function call with a semantically equivalent expression.
% % In contrast, \toolName imports the missing function \verb+ktime_before+ from the mainline to v3.2, resulting in a different, but semantically equivalent patch.


% % \paragraph{Incorrectly backported patch.}
% % We also find instances where the backported patch produced by \toolName has a different behavior from the developer patch.
% % The mainline patch at the commit 7809a611 fixes a regression error by inserting an API call \verb+IS_HASWELL+ with \verb+dev_priv+ as the first argument.
% % The developer who backported the patch to v3.2 in commit 2dd2c68e used a different variable \verb+dev+ as the first argument.
% % However, since the variable \verb+dev_priv+ exists in v3.2, \toolName does not change the argument \verb+dev_priv+ to \verb+dev+.
% % \toolName cannot disambiguate such cases, i.e. to keep the original argument \verb+dev_priv+, or to change it to \verb+dev+.

% % \paragraph{Internal DSL} \toolName's DSL allows expressing transformation rules that can be applied in a flexible way (i.e. for each target version, \toolName can decide whether the flexible predicates should be fixed or relaxed using the synthesis process). \toolName's DSL is only for internal use, to reduce the search space by considering a restricted language, rather than for communication with developers.  In the future, we could consider how to present the transformation rules using a syntax such as that of Coccinelle's DSL~\cite{coccinelle}, which is familiar to kernel developers. Note that the choice of DSL syntax is not a core contribution of this paper.


% \subsection{Threats to Validity}

% %During our exploratory study and evaluation, there are a series of threats that could affect the results.

% \noindent\textbf{External.} 
% Our findings of UI test maintenance focus on Web apps and may not generalize to UI apps (e.g., Java apps and Android apps).
% To ensure the general applicability of our \yz{tool}, we evaluate \toolName using both open datasets and industrial datasets.
% % Moreover, we ensure that the study and the evaluation dataset are different to avoid the problem of overfitting.
% When labelling UI elements in the dataset, two authors of the paper independently label each element, and discuss to resolve any disagreement.
% %label as many elements as possible and filter elements that are 
% %However, some elements are difficult to label.
% %To make the result more accurate, we dropped these elements.
% %To reduce errors caused by manual labeling, these elements in the open-source dataset labeled by one author and checked by another author.

% %\mytool{} may produce inaccurate concept matching if the student program and reference solution solve a programming problem with different algorithms. We mitigate this by following previous work~\cite{yang2019refactory,ahmed2022verifix,gulwani2018automated,wang2018search} to include correct students' programs (i.e., student submissions that pass all test cases) as additional reference solutions.

% % \mytool{} focus on evaluating incorrect student submissions. For 
% % In the future, we plan to extend
% % our approach to handle Object-Oriented Programming concepts. Additional complex features available in Python, such
% % as list comprehensions or lambda functions, are currently not
% % handled since novice students rarely utilize advanced concepts

% \noindent\textbf{Internal.} 
% Our automated tests may have bugs that can affect our reported results.
% We have made our experimental data and improved datasets publicly available to mitigate this threat. 
% %Our implementation of the CFG-based approach~\cite{vujovsevic2013software} may not be as effective as the original implementation for C programs. Nevertheless, as our concept graph uses the same CFG as basis for abstraction, our evaluation that compares the CFG approach and the abstracted CFG (our concept graph) ensures fair comparison of the two approaches.

% %To avoid problem of overfitting, we ensure that the study dataset and the evaluation dataset are different. To reduce the influence of different types of applications and pages on the evaluation results, we collected x pages from a total of x\todo{add exact number} applications, which were collected from open-source datasets and industrial datasets. Even so, it is not possible to evaluate on all types of applications and pages. Therefore, \toolName performs well in the evaluated dataset, but may perform differently in other types of applications.
% %In the process of labeling the dataset, we label as many elements as possible.
% %%However, some elements are difficult to label.
% %To make the result more accurate, we dropped these elements.
% %To reduce errors caused by manual labeling, these elements in the open-source dataset labeled by one author and checked by another author.

% %It is impossible to cover all the functions in the application with the open-source test cases of the existing work\cite{imtiaz2021automated}.
% %Different locator positioning methods will affect the execution of the test case %and affect the evaluation results.
% %To alleviate the impact of this problem, we also use open source test cases from another work on locator robustness research.

% % \paragraph{Limitations of \toolName}
% % Our implementation is based on LLVM/Clang, and thus inherits the limitations of that framework.  
% % %Specifically, while the LLVM/Clang AST preserves information about macros, it elides conditional compilation directives, e.g., \texttt{\#ifdef}s, according to the chosen configuration.
% % %Since handling all combinations of compilation options is not scalable, we try two sets of compilation options 1) set all the compilation directives as \texttt{Y} and 2) set all directives as \texttt{N}.
% % Since handling all combinations of compilation options is not scalable, when compiling the project, we only consider two sets of compilation options (see Section ~\ref{sec:implementation}).
% % This strategy works for most cases, but in some cases, it could result in certain un-compiled blocks of code being unavailable to \toolName, thus leading to incomplete backporting or even failure.
% % To alleviate this limitation, we allow users to specify the values of preprocessor variables according to their working environment. 

==> sections/sections/evaluation.tex <==
\section{Evaluation}

We investigate the effectiveness of the combination of WATER, VISTA, and ChatGPT. First, we compare the results obtained by ChatGPT when using different candidates in matching and repairing: the candidates sorted by similarity based on \emph{XPath} edit distance or the candidates sorted by WATER and VISTA. Then we will compare the effectiveness of ChatGPT with WATER and VISTA. Previously, our experiments only studied the effect of ChatGPT on matching elements. In this chapter, we will study both the effect of matching elements and repairing broken statements based on the selected elements with the baseline of WATER and VISTA.



\subsection{Dataset}
We use an existing dataset~\cite{dataset} containing 5 open-source applications (3 of which are used in the release paper of VISTA). After deleting the repeated tests and the tests without assertion, there are 135 test cases.

Among these 135 scripts, 22 can be executed directly on the new version of the webpage and do not need to be fixed. We categorize these scripts under the "Exempt" column. Additionally, some scripts involve the addition or removal of modules or event, which means they can not be repaired by merely modifying the locator of original statements. Simultaneously, there are test cases that original locator points to the wrong element instead of throwing NoSuchElementException, making it challenging to identify the root cause of the breakage.  These have been marked under the "Irreparable" column. The column \emph{Repairable} shows the remaining 62 test cases, for which we manually labeled the ground truths. The column \emph{Broken Stm} specifies the corresponding number of broken statements within the repairable test cases, which we employ in the subsequent experiment.
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[H]
\caption{The number of test cases and broken statements}
\label{table:dataset}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\hline
\multicolumn{1}{l|}{Applications} &
  \multicolumn{1}{l}{Total} &
  \multicolumn{1}{l}{Exempt} &
  \multicolumn{1}{l}{Irreparable} &
  \multicolumn{1}{l}{Repairable} &
  \multicolumn{1}{l}{Broken Stm} \\ \hline
AddressBook & 16  & 8  & 6  & 2  & 2   \\
Claroline   & 31  & 0  & 4  & 27 & 53  \\
Collabtive  & 18  & 13 & 1  & 4  & 11  \\
MatnsiBt    & 45  & 1  & 19 & 25 & 66  \\
MRBS        & 25  & 0  & 21 & 4  & 7   \\ \hline
Total       & 135 & 22 & 51 & 62 & 139 \\ \hline
\end{tabular}%
}
\end{table}


% \begin{description}[leftmargin=*]
% \item[RQ6:] What is the performance of ChatGPT in the matching and repairing task with different kinds of candidate elements? 

% \item[RQ7:] Does the result of ChatGPT with these two kinds of candidates better than WATER and VISTA?
% \end{description}

\subsection{ChatGPT's Effectiveness on Matching}

The different repaired statements may all turn out to be right, as long as they correctly locate the corresponding updated element, and preserve the original intent of the test statement. In the process of repair, changing the locating strategy can be accepted. For example, even though the original test statement used id to locate the element, the correct repaired statement can use the updated element's \emph{XPath} or name as the locator. But it is important to ensure that the locator uses exact the value of the attribute according to the locating strategy. In addition to this, the test statement will involve operations on the element, such as clicking or sending keys, and this is the part that should not be changed during the repair. Similarly, if the test statement originally wants to assert whether the value of the element is equal to the expected value in order to determine whether the element is correctly located or whether the previous test procedure was wrong, then the original part of the assert statement should not be changed either.


Therefore, we will consider the below aspects to study the effectiveness of ChatGPT's repair result. First, whether ChatGPT has followed the prompt to modify only the locator of the statement, leaving the part of the test statement outside the locator unchanged. Then, we will check if ChatGPT changes the locating strategy. Further, we check whether it repairs the locator correctly, which includes the correct syntax as well as the correct attribute value. For the former, we will check whether the locator is able to locate a specific element. For the latter, we will investigate if ChatGPT correctly uses the attribute information of the element in the prompt to correctly locate the element it has selected. Finally, we check if the element's information corresponds to the given information of its selected element, and if the selected element is the ground truth element.





\subsection{The Effectiveness of ChatGPT with Different Candidate Lists}
\subsubsection{The Effectiveness of Matching}




Figure \ref{ExpResult} shows the effectiveness of ChatGPT with different candidate lists. Overall, it can be seen that ChatGPT performs well in both Stability and Mention Rate, with both exceeding 91\%; while ChatGPT's Correct Rate and Ground Truth Selected Rate also reach the range of 74\% to 86\%. Comparing the effects of different candidate types, it can be found that when using candidates generated by WATER+VISTA, ChatGPT performs better than using candidates generated by Edit Distance on almost all metrics except Correct Rate. Therefore, it can be seen that candidates generated by Edit Distance are more advantageous for ChatGPT's performance.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/content/FormalExpResult.png}
%     \caption{The Effectiveness of ChatGPT with Different Candidate Lists}
%     \label{ExpResult}
% \end{figure}

\subsubsection{The Effectiveness of Repair}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{The matching and repair results of different tools}
\label{table:result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccccc}
\hline
         & VISTA & WATER & XPath & sustech & VISTA+ChatGPT & WATER+ChatGPT & XPath+ChatGPT & Total \\ \hline
Matching & 62    & 78    & 42    & 122     & 51            & 71            & 107           & 132   \\
Repair   & 61    & 78    & 40    & 120     & 51            & 70            & 107           & 132   \\ \hline
\end{tabular}%
}
\end{table*}

% % 插入图片或表格并描述
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
% Candidates Selection &
%   \multicolumn{1}{l}{Total} &
%   \multicolumn{1}{l}{Locating Strategy} &
%   \multicolumn{1}{l}{Locator} &
%   \multicolumn{1}{l}{Others} &
%   \multicolumn{1}{l}{\# of Correct} &
%   \multicolumn{1}{l}{Correct Rate} \\ \midrule
% Edit Distance &
%   327 &
%   246 &
%   247 &
%   324 &
%   246 &
%   75.23\% \\
% WATER+VISTA &
%   327 &
%   268 &
%   230 &
%   323 &
%   230 &
%   70.34\% \\ \bottomrule
% \end{tabular}%
% }
% \caption{The repair result of ChatGPT with different candidate selection algorithms}
%     \label{repair_result1}
% \end{table}
Table \ref{repair_result1} shows the repair results of ChatGPT with different candidate selection algorithms. In each column, the first column \textbf{Candidates Selection} represents the different candidate selection algorithms used, the second column \textbf{Total} is the total number of repairs, the third column \textbf{Locating Strategy} refers to the number of times the locating strategy used during repair is identical to the broken statement, the fourth column \textbf{Locator} refers to the number of repairs where the locator can locate the selected element, the fifth column \textbf{Others} refers to the number of repairs where the part outside the locator can maintain its original meaning, the sixth column \textbf{Number of Correct} refers to the number of repairs where both the locator and the part outside the locator are correct, and the seventh column \textbf{Correct Rate} is obtained by dividing the ``Number of Correct'' by the total number of repairs. 


It can be seen that compared to using candidates generated by WATER+VISTA, ChatGPT has a slight advantage in all indicators except \textbf{Locating Strategy} when using candidates generated by Edit Distance. By comparing the performance of different indicators, it can be found that the number of repairs where the part outside the locator can maintain its original meaning is the largest, with almost no changes. This is because the difficulty of repair mainly lies in repairing the locator, and the correctness of the final repair result mainly depends on whether the locator is repaired correctly. Therefore, the prompt used for ChatGPT only allows it to modify the locator, and ChatGPT basically follows this instruction and does not modify the part outside the locator. If ChatGPT modifies the part outside the locator, it will be considered a failure in this indicator, which will lead to unsuccessful repair results. Besides, the \textbf{Locating Strategy} is also close to the total number of repairs, which indicates that ChatGPT is relatively compliant with the original locating strategy. Finally, it can be observed that the number of repairs where the locator can locate the selected element is relatively small (only 247 and 230 out of a total of 327 repairs), indicating that repairing the locator is more difficult. The Number of Correct is almost equal to it, indicating that the number of correct repairs depends largely on whether the locator can be repaired correctly.



\subsection{The Effectiveness of ChatGPT Compared to WATER and VISTA}
Since ChatGPT is asked three times for each breakage but each breakage only needs one repair result, only when there are two or more correct repair results in three, we will consider ChatGPT repair correctly for this breakage repair.

Different from WATER and VISTA, ChatGPT's correct repair is based on correct selection. WATER and VISTA's repair framework is relatively mature and the repair results are relatively accurate as long as the matching element is found correctly during testing. VISTA has even implemented a crawler function that searches for candidate elements on neighboring pages. If found, test statements are added to reach the page where the candidate element is located, and then the original broken test statements are repaired. 





Table \ref{repair_result2} shows the repair results and average running time of different repair methods. It can be seen that among the four repair methods, only ChatGPT+WATER+VISTA has the longest average running time (66.13 s), almost twice as long as the other methods. Considering that the average time for ChatGPT to select and repair one breakage is only about 3 seconds, the reason why the running time of ChatGPT+WATER+VISTA is the longest is that the process of generating candidates using WATER+VISTA takes up a lot of time. However, in terms of repair effectiveness, compared to using WATER and VISTA alone, using ChatGPT for matching and repairing achieves better results. Among them, ChatGPT+Edit Distance has the best performance, successfully matching and repairing 96 and 91 out of 109 breakages, respectively. On the other hand, using VISTA alone performs the worst, with only 53 breakages successfully matched and repaired out of 109, less than half of the total. However, it should be noted that when repairing with WATER and VISTA alone, the number of correct matches is equal to the number of correct repairs. This means that as long as the matching is correct, the repair can be done correctly, which once again proves that repair framework of WATER and VISTA is relatively mature and the repair results are relatively accurate. When using ChatGPT for repair, whether using candidates generated based on Edit Distance or based on WATER+VISTA, the number of correct repairs is slightly less than the number of correct matches, which is the problem to be discussed next.

\subsection{Analysis of ChatGPT's Repair Failure}
There are several reasons why ChatGPT repairs fail. 

Mismatch is the first main reason for ChatGPT's repair failure because ChatGPT cannot repair the locator correctly with the information of its wrong selected element. Generally, there are two cases of mismatch. One is mismatch from the candidate lists without ground truth elements. In this experiment, the proportion of ground truth contained in the candidates of WATER+VISTA and Edit Distance are 98 and 99 out of 109 separately according to Table \ref{gt}, which means ChatGPT can not have a higher correct repair rate than these. The other is that ChatGPT selects wrongly from a candidate list even though there is a ground truth element in it. And this happens more often when selecting candidates with WATER+VISTA. This is because WATER+VISTA more tends to contain nested elements, such as the parent element and grandparent element of the ground truth element, as candidates. These elements are more likely to have similar attributes but can not replace the ground truth element to be tested, which may interfere ChatGPT's selection. Instead, Edit Distance selects sibling elements with different attributes as candidates more frequently because elements with the same hierarchy have smaller XPath edit distance, thus reducing the number of ChatGPT's mismatch.

Another reason for ChatGPT's failure is that ChatGPT tends to follow locating strategies of the original broken statements, which leads ChatGPT to use relative paths for many of the repairs. However, ChatGPT is not good enough at generating relative paths, causing related repair failure.


By relative paths we mean repairing with ``By.xpath()'', but not with the value of the \emph{XPath} absolute path itself. There are two types of relative paths, the first being the simpler one, where the element itself is located using e.g. ``By.xpath(//*[text()=``text value''])''. However, ChatGPT has had cases of repairing errors where the value of the another attribute was filled in as the value of the text value. This was because ChatGPT wanted to maintain the original positioning as much as possible, i.e. using relative paths. However, if the repair is simply done by other positioning methods like ``By.attribute(``attribute value'')'', it is much less likely to fill in the wrong attribute value. Another type of absolute path is created by first locating the ancestor of an element using the previous relative path, and then splicing the absolute path of the element minus the absolute path of the ancestor element. However, no samples of ChatGPT successfully repairing this type of relative path were found in this experiment.


In addition to this, there were some unexpected failures: ChatGPT selected the correct element, but the result of the repair was wrong. The reason why the repair was wrong when it could have been correct is that ChatGPT thought that the element it selected as the most similar element in the list of candidate elements did not look enough like the correct answer, so ChatGPT did not base the repair entirely on the information of the selected element. And ChatGPT's result based on its prediction of the possible correct answer and its repair seems to be reasonable.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/content/example.png}
    \caption{An example of the unexpected failure}
    \label{failure_example}
\end{figure}

 In the example of Figure \ref{failure_example}, the value of the \emph{href} attribute of the target element on the old page is ``manage\_user\_page.php
'', and the locator for the broken statement testing this element is ``//a[@href=`manage\_user\_page.php']''. ChatGPT repaired it by fixing the locator to ``//a[@href=`/mantisbt-1.2.0/manage\_user\_page.php']'', prefixing the original \emph{href} with the prefix that all candidate elements have. 

The value of the \emph{href} of the element on the old page means that the page jumps to the page ``Manage User'' when the element ``Manage'' is clicked. However, ChatGPT does not know that clicking on the ``Manage'' element on the new page redirects the page to the overview page and requires further clicking on the ``Manage User'' element to reach the same page as before. Because the target page is different, the \emph{href} attribute of the ``Manage'' element was changed to ``/mantisbt-1.2.0/manage\_overview\_page.php'', causing the ChatGPT to get the wrong speculation about the truly matched element. 

This ChatGPT ``self-initiated'' error could have been avoided by strictly restricting ChatGPT to repair the locator according to the given candidate elements. In this example, the correct element was included in the list of candidates and ChatGPT selected it as a match correctly. However, it is important to note that we cannot always guarantee that the correct element is in the list of candidates. Therefore, it is worth considering whether we should allow ChatGPT to guess an element that is more correct than the given candidate according to the effectiveness of the candidates selection algorithm.
















% We evaluate the effectiveness of \toolName in \delete{W}\add{w}eb UI tests repair and answer the following research questions: 


% \begin{description}[leftmargin=*]
% \item[RQ1:] How effective is \toolName in UI element matching compared with existing methods?
% %How effective is \toolName ~in backporting patches? 

% \item[RQ2:] How efficient are different matching methods?

% % \item[\add{RQ3:}]\add{ How efficient is the iterative matching?}

% \item[RQ3:] How effective is \toolName in test case repair compared with existing methods? %How does \toolName compare with existing  tools?
% % \item[\textbf{RQ3}] How does different-based validation compare with screen-based validation in intention validate?
% \end{description}


% \noindent \textbf{Selected baselines:} We compared \toolName with four baselines, including two repair tools (\watertool~\cite{choudhary2011water}, \vistatool~\cite{stocco2018vista}), and two UI element matching algorithms (\webevotool~\cite{shao2021webevo}, and \sftmtool~\cite{brisset2020sftm}). 
% We exclude the model-based tool~\cite{imtiaz2021automated} because the code in the GitHub repository fails to compile due to missing dependencies.
% \watertool is a UI test repair tool that uses the similarity of DOM properties of elements for matching.
% \vistatool is a repair tool that uses image processing and computer vision techniques by comparing visual information in two versions of the apps.
% \webevotool computes both text similarity and image similarity of the elements in two versions of the apps to match elements.
% % \todo{add a short sentence to introduce each tool, algorithm and matching which information}
% The recently proposed algorithm, \sftmtool, assigns attribute scores to all potential matches between nodes in two versions and adjust\add{s} the scores using the parent-child relationships of nodes.
% Similar to \vistatool~\cite{stocco2018vista}, \toolName performs online repair, which fixes broken tests during execution. 
% On the other hand, \watertool~\cite{choudhary2011water} uses an offline mode, which collects information during test execution and repairs after the execution. %, and starts repairing after the execution.
% Therefore, we use the re-implemented version in \vistatool~\cite{stocco2018vista} to evaluate \watertool.
% For all other tools, we use their open-source implementations and parameters. 
% The parameters of \toolName \add{in 
%  Algorithm \ref{alg:iterative_optimization}} include: \add{maximum iterations} $t$=5, \add{attribute similarity weight} $\alpha$=0.7, \add{path similarity weight} $\beta$=1.0, \add{region similarity weight} $\gamma$=2 and \add{similarity threshold} $\theta$=1.2. All these parameters are tuned via grid searches for the best values.

% %\watertool and \vistatool use code open-sourced in the code repository of \vistatool\cite{stocco2018vista}, \webevotool and \sftmtool use their open-sourced code\cite{shao2021webevo,brisset2020sftm} respectively.
% %Similar to Section~\ref{sec:study}, 
% % We evaluate the element matching algorithm of \toolName on two sets of applications: %(1) 5 open-source applications that have been used by existing work~\cite{imtiaz2021automated} (we exclude the industrial application, i.e., University Management System from our experiment as it requires creating an university account), 
% % and (2) two industrial apps ($AppB$ and $AppC$). These two selected industrial apps are big data analysis platforms, which are core products of \company{}.

% %Note that, all evaluations run on the same computers.
% %a Windows computer with a Intel Core i5 processor (1.6GHz) and 12 GB RAM.
% % ~\xiang{how do you select the experimental apps}




% \noindent\textbf{UI Match Dataset}:
% % We utilize further augmented datasets 
% To evaluate the performance of different UI element matching algorithms, we use an extended \webevotool dataset~\cite{shao2021webevo} (EWD).
% The \webevotool dataset include\add{s} 13 web applications in total.
% We excluded the webpages \textit{ClassDojo} and \textit{Home Depot} because they could not be loaded correctly. 
% % Since the Alexa service is closed~\footnote{https://en.wikipedia.org/wiki/Alexa\_Internet\#cite\_note-end\_news-5}, 
% To expand our dataset, we select the Top 15 web apps on Semrush~\cite{semrush} (which presents a ranked list of most visited websites) and remove webpages that overlap with the \webevotool dataset~\cite{shao2021webevo}. 
% We use \textit{Wayback Machine}~\cite{wayback} to obtain the historical webpages. 
% \delete{Totally}\add{In total}, our expanded dataset contains 44 webpages of 22 web apps (with 11 apps from \webevotool and 11 extended apps).

% Moreover, to show the ability of different element matching algorithms on large-scale industrial applications, we also include two industrial apps\delete{(IND)}.
% To \delete{keep anonymous}\add{maintain anonymity}, we omit the application and company name in the paper review process.

% We select two apps \appa{} and \appb{}, two big data analysis platforms, which are two core products of \company{}.
% To ensure sufficient changes are collected for our study of web UI elements evolution, we select webpages which contain\delete{s} sufficient changes. 
% Specifically, we select webpages with more than 20 changed elements.
% In the end, we collected 13 webpages from two industrial app\add{s}.
% The types of selected webpages are diverse, which include home pages, pages for configuring system settings, data pages, and pages with charts.


% Similar to prior work~\cite{shao2021webevo}, we also consider three types of element changes: \textit{Update}, \textit{Add}, and \textit{Delete}.
% % Because test cases usually do actions on leaf node elements, the experiment only considers the labeled leaf node elements.
% % Its data set distribution is as follows:
% % Since \vistatool{} only supports matching leaf nodes, \yz{we only count leaf nodes as UI elements.}
% Table~\ref{table:dataset-stats} shows the statistics of our UI element matching dataset.
% % \yuanzhang{How to label this element}
% In the UI element matching dataset, we try to label all the elements on the pages as much as possible. 
% \textit{The labeling process does not only label the change types, but also annotate the matching pairs between the old and new versions, which are then served as the ground truth of element matching.}
% However, some elements, such as content elements, are difficult to label.
% As a result,
% % \add{However, certain elements pose challenges when it comes to labeling. Take content elements, like items in the Amazon application, for instance. In the new version, these elements may not have an  corresponding relationship. To mitigate potential controversies, }
% we made the decision to exclude them from the labeling process.
% % , so we ignored them.
% Since VISTA only supports matching the innermost elements, to make a fair comparison of the performance of different algorithms, we only consider leaf nodes in our experiment.
% Totally, we labelled 2,522 changed elements.


% \begin{table}[!t]
% \centering
% \small
% \caption{Statistics of our UI match dataset}
% % \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{l|rrrr}\toprule
% Dataset   & Add      & Delete     & Update          & Total      \\\hline\hline
% EWD & 301 & 218 & 1,101  & 1,620 \\
% IND & 170 & 101 & 631  & 902 \\ \hline
% Total &471 &319 &1,732 &2,522 \\
% \bottomrule 
% \end{tabular}%}
% \label{table:dataset-stats}
% \end{table}



% % Table \ref{table:evaluation-application-version} shows the collected information for pages that belong to different types of web applications and different time intervals between original version and modified version.

% % \begin{table}[h]
% % \centering
% % \setlength{\tabcolsep}{2.2pt}
% % \vspace{-3pt}
% % \caption{The version about Web application in evaluation dataset}
% % \vspace{-3pt}
% % \begin{tabular}{ll|cc}\toprule
% % Application & Category &Original Version & Modified Version \\\hline\hline
% % \textit{www.w3school.com} & & 2016.01 & 2019.01\\
% % \textit{www.foodnetwork.com} & & 2018.11 & 2019.11\\
% % \textit{music.douban.com} & & 2014.02 & 2019.02\\
% % \textit{beijing.douban.com} & & 2017.10 & 2019.10\\
% % \textit{book.douban.com} & & 2016.08 & 2019.08\\
% % \textit{movie.douban.com} & & 2014.11 & 2019.11\\
% % \textit{www.amazon.com} & & 2017.08 & 2020.08\\
% % \textit{www.apple.com} & & 2018.02 & 2020.08\\
% % % \textit{www.classdojo.com} & 2017.06.05 & 2020.07.22\\
% % % \textit{www.homedepot.com} & 2019.07.15 & 2020.08.04\\
% % \textit{www.linkedin.com} & & 2019.08 & 2020.08\\
% % \textit{www.usps.com} & & 2018.08 & 2020.08\\
% % \textit{www.xfinity.com} & & 2018.08 & 2020.08\\ \hline
% % \textit{www.bing.com} & &  & \\
% % \textit{www.yahoo.com} & &  2017.02 & 2019.06\\
% % \textit{www.wikipedia.com} & & 2019 & 2022\\
% % \textit{www.paypal.com} & & 2019.03 & 2020.03\\
% % \textit{www.instagram.com} & & 2019.03 & 2021.03\\
% % \textit{www.google.com} & &  & \\
% % \textit{www.fandom.com} & & 2022.03 & 2022.12\\
% % \textit{www.twitter.com} & & 2021.08 & 2022.08\\
% % \textit{www.youtube.com} & & 2022.08 & 2023.02\\
% % \textit{www.facebook.com} & & 2020.08 & 2022.08\\
% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:evaluation-application-version}
% % \end{table}




% % \noindent where columns \textit{Add}, \textit{Delete} and \textit{Update} show the number of inserted, deleted and modified elements when webpages evolve, respectively.

% \noindent\textbf{UI Test Dataset}:
% Since the \webevotool dataset does not have open-source test cases, we choose to evaluate the effectiveness of \toolName using open-source and industrial test datasets.
% For the open-source tests, we use an existing test dataset~\cite{imtiaz2021automated}.
% Specifically, we include all \delete{W}\add{w}eb apps in prior work~\cite{imtiaz2021automated}, except for the \texttt{Password Manager} app because the provided link for this app is no longer available for download.
% %and the versions of five application in section \ref{sec:2-dataset}.
% % The original test cases need to be executed in the specified order because the previous cases will provide data for the later cases.
% For the original test case dataset, we mainly made two modifications,
% (1) remove test cases without assertion statements or repeated test cases, \add{as the assertions are used as the correctness specification for \toolName}, and
% (2) insert necessary UI actions (e.g., login) so that test cases can be executed independently.
% To avoid the problem caused by missing data (such as username does not exist or password is incorrect), we first insert some SQL statements to prepare the data for test execution (e.g., create user\delete{,} and save username/password information into the database).
% The selected two industrial apps \appa{} and \appb{} have 5,839 test cases in total. 
% % As it is time-consuming to execute all tests, .
% \add{Conducting experiment on all the tests is too time-consuming, since executing these tests in parallel will take two or three days in industrial environment. Hence, we randomly select 250 test cases (the number is aligned with the existing work~\cite{imtiaz2021automated}) to execute.}
% \add{We select the test cases that must be repaired, regardless of the number of pages used by these tests.}
% We then exclude 46 tests as they require configuring a specific test environment.
% Table \ref{table:open-source-application-version} shows the original and the modified versions of the selected webpages.
% The open-source dataset, following settings from the provided GitHub repository in the prior work~\cite{imtiaz2021automated}, \add{involves changes across multiple versions.
% Note that\delete{,} fixing tests across multi-version changes may not be realistic.
% Hence, we use single-version changes for the industrial dataset, which is practical in an actual industrial environment.}
% % Yes, . In fact, 
% % As for the open-source dataset, we utilized gaps larger than a single revision just to maintain consistency with the existing dataset (citation 4). So that, we can conduct comparison experiment with prior work.
% % On the other hand, if UITestFix is proved to be effective in fixing tests across multi-version changes, it should perform even better on single-version changes.
% % We elaborated the discussion on dataset at Section VI.

% During the classification of the matching results (RQ1) and the generated fixes (RQ3), two authors of the paper independently analyzed them by inspecting the matched UI elements to check if the matching was correct and if it led to any newly thrown exception. Then, they met and discussed resolving any disagreements.

% \begin{table}[!t]
% \centering
% % \setlength{\tabcolsep}{2.2pt}
% \small
% \caption{The original and modified versions of the selected webpages}
% % \resizebox{0.43\textwidth}{!}{%
% \begin{tabular}{ll|rr}\toprule
% Label & Application & Original Version & Modified Version \\\hline\hline
% I     & AddressBook & 4.0              & 6.1              \\
% II    & Claroline   & 1.10.7           & 1.11.5           \\
% III   & Collabtive  & 0.65             & 1.0              \\
% IV    & MantisBT    & 1.1.8            & 1.2.0            \\
% V     & MRBS        & 1.2.6.1          & 1.4.9            \\
% % \hline
% % \add{VI}    & \add{\appa}      &                  &                  \\
% % \add{VII}   & \add{$AppB$}      &                  &                  \\
% \bottomrule
% \end{tabular}
% \label{table:open-source-application-version}
% \end{table}

% All experiments for the open-source apps are run on a computer with an Intel Core i5 processor (2.3GHz) and 24 GB RAM, whereas the experiments for the industrial apps are conducted on a computer with an Intel Core processor (3.20GHz) and 32GB RAM.
% %windows computer with Intel Core processor(3.20GHz) and 32GB RAM.

% % Therefore, we used only five of these applications.

% % All test cases are written in one class in the original dataset, and the execution order is defined by priority. These test cases share a WebDriver, and when a test case fails to execute, it will affect the execution of other test cases. In addition, case events are heavily dependent on backend data. For example, if the AddProject use case fails, all Project-related use cases may fail.

% % Therefore, to improve the independence between test cases as well as the independence of test cases and data, we made certain modifications to the dataset. During this period, keep the original locators and actions as much as possible. We mainly did the following work:
% % \begin{enumerate}
% %     \item  Separate these test cases from one class into different classes.
% % \item  Add necessary events, such as login.
% % \item  Call SQL statements to prepare data or clean data for test cases.
% % \item  Solve the bugs in the test cases and make certain adjustments to enhance stability.
% % \item  Modify the locator generated by the backend data, such as $//*[@id="add\_btn\_1"]$.
% % \item Delete duplicate, empty, meaningless test cases.
% % \item  Merge some test cases.
% % %, such as adding, deleting, and modifying.
% % \end{enumerate}

% % After modifying test cases, we executed them several times and verified them on different devices. Although we try our best to alleviate the dependencies between test cases, there is no guarantee that they will not affect each other.


% % The final test case dataset distribution is as follows:

% % \begin{table}[h]
% % \centering
% % \setlength{\tabcolsep}{2.2pt}
% % \vspace{-3pt}
% % \caption{Distribution in our test cases dataset}
% % \vspace{-3pt}
% % \begin{tabular}{l|l|c|c|c|c}\toprule
% % Label &Application   & Base Version      & Repair Version     & Cases              \\\hline\hline
% % I &AddressBook & 6.1 & 4.0 & 16  \\
% % II &Collabtive & 0.65 & 1.0 & 18   \\
% % III &Claroline & 1.11.5 & 1.10.7 & 33  \\
% % IV &MantisBT & 1.1.8 & 1.2.0 & 45   \\
% % V &MRBS & 1.2.6.1 & 1.4.9 & 25  \\
% % VI  & Industy & - & - & 0   \\\hline
% % Total&- &- &- & 137\\

% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:dataset-stats-temp}
% % \end{table}


% % 	\begin{table*}[ht!]
% % \centering
% % \vspace{-3pt}
% % \caption{Distribution in our ui match dataset}
% % \vspace{-3pt}
% % \begin{tabular}{l|c|c|c|c}\toprule
% % application   & base version      & repair version     & scripts              \\\hline\hline
% % AddressBook & 165 & 78 & 50  \\
% % Collabtive & 165 & 78 & 50   \\
% % Claroline & 1.11.5 & 1.10.7 & 35  \\
% % mantisbt & 1.1.8 & 1.2.0 & 45   \\
% % mrbs & 0.65 & 1.0 & 25  \\
% % industy & - & - & 500   \\
% % \bottomrule
% % \end{tabular}
% % \vspace{-3pt}
% % \label{table:dataset-3stats}
% % \end{table*}

% % Moreover, we evaluate \toolName in backporting security vulnerabilities by selecting \numCVE patches that fix CVEs using the same criteria.
% % We focus on the CVEs reported during 2014-2019, and made sure that the \numCVE CVE patches are disjoint from the \numSubject patches in our main dataset.

% % All experiments are conducted on a Dell Power Edge R530 with Intel(R) Xeon(R)CPU E5-2660 processor and 64GB RAM. 

% \subsection{[RQ1] Effectiveness on Matching Elements}
% % Because the data set used is static, the inputs and outputs are adjusted to use statically saved data.
% % An algorithm is considered to match correctly when the matched element lies in the labeled element cluster.
% \begin{table*}[!tb]
% \centering
% % \small
% % \resizebox{0.45\textwidth}{!}{%
% % \setlength{\tabcolsep}{2.5pt}
% \caption{Accuracy of UI element matching for all evaluated approaches}
% \label{table:experiment-comparison-match-ui}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc}
% \toprule
% Modified & 
% % \multicolumn{2}{c|} {\texttt{WATER-}} &
% \multicolumn{2}{c|} {\watertool} &
% \multicolumn{2}{c|}{\vistatool} &
% \multicolumn{2}{c|}{\webevotool} &
% \multicolumn{2}{c|}{\sftmtool} &
% % \multicolumn{2}{c|}{\texttt{SFTM+}} &
% \multicolumn{2}{c}{\toolName}\\\cline{2-11}
% Type    & EWD & IND  & EWD & IND   & EWD & IND  & EWD & IND  & EWD & IND  
% % & OD & ID & OD & ID
% \\\hline\hline
% % \multirow{2}{*}{Add} & 9 &28 &25 &8 &31 &  1 & 156 & 133  & \textbf{160} &\textbf{142}\\
% % {}    &  3.06\% & 21.76\% & 8.50\% & 4.71\% &10.51\% & 5.9\%  & 52.88\% & 78.23\% & \textbf{54.23\%} & \textbf{83.53\%}\\\hline
% Add &  4 (1.3\%) & 28 (16.47\%) & 30 (10.0\%) & 8 (4.7\%) & 87 (28.9\%) & 1 (5.9\%) & 162 (53.8\%) & 133 (78.2\%) & \textbf{170 (56.5\%)} & \textbf{142 (83.5\%)} \\ 

% Delete & 11 (5.0\%) & 1(1.0\%) & 49 (22.5\%) & 5 (5.0\%) & 44 (20.2\%) & 0 (0\%) & 100(45.9\%) &32 (31.7\%) & \textbf{111 (50.9\%)} & \textbf{77 (76.2\%)} \\ 

% % \multirow{2}{*}{Delete} & 36 &1 &21 &5 &24 &  0 & \textbf{98} & 32 & 95 &\textbf{77}\\
% % {}    & 16.74\%& 0.99\% & 10.24\% &4.95\% &11.16\% & 0\% & \textbf{45.58\%} & 31.68\% & 44.18\% & \textbf{76.24\%}\\\hline
% % Update & &3 & &
% Update &500(45.4\%) & 344(54.52\%) & 651(59.1\%) &434(68.78\%) &803(72.9\%) &278(44.1\%)  &808(73.4\%) &500(79.2\%) &\textbf{1036(94.1\%)} &\textbf{605(95.88\%)} \\ \hline
%     % \multirow{2}{*}{Update} &536 &344 &711 & 434 &821 &278 & 838 & 500 & \textbf{1074} & \textbf{605}\\
% % {}    & 48.16\% & 52.60\% & 64.52\% & 66.36\% & 73.76\% & 42.51\% & 75.29\% & 76.45\%  & \textbf{96.50\%} & \textbf{92.50\%}\\\hline

% % \multirow{3}{*}{Total}& 581&382& 757&447 & 876&  279 & 1092 & 665 & \textbf{1329}&\textbf{824}\\
% % {}     & 35.79\%&41.30\%& 47.28\% & 48.32\% & 53.97\% & 42.50\% & 67.28\% & 71.89\%  & \textbf{81.89\%} & \textbf{89.08\%}\\
% \multirow{2}{*}{Total} &515(31.8\%) &373(41.35\%) &730(45.1\%) &447(49.6\%) & 934(57.7\%) &279(30.93\%) &1070(66.1\%) &665(73.3\%) &\textbf{1317(81.3\%)} & \textbf{824(91.4\%)} \\
% {}     &\multicolumn{2}{c|} {888 (35.2\%)} & \multicolumn{2}{c|}{1177 (46.7\%)}  & \multicolumn{2}{c|}{1213(48.1\%)} & \multicolumn{2}{c|} {1735 (68.8\%)}    & \multicolumn{2}{c} {\textbf{2141 (84.9\%})} \\ \hline\hline

% AVG Time & \multicolumn{2}{c|}{\textbf{0.0003s}} &  \multicolumn{2}{c|}{7.7623s} &\multicolumn{2}{c|}{0.0799s} &\multicolumn{2}{c|}{0.9726s} &\multicolumn{2}{c}{0.8685s} \\

% % \hline
% % Total& 850(61.10\%)& 570(61.62\%)  & 42  & 82  & 59  & 44  & 43  & 648(70.05\%)    &1160(83.39\%)& 761(82.27\%)& 1254(90.15\%)& 783(84.65\%)\\
% \bottomrule
% \end{tabular}}
% \end{table*}

% Table \ref{table:experiment-comparison-match-ui} summarizes the evaluation results on web element matching.
% For each algorithm, the table lists the correct number and accuracy of different types of changes in the extended WebEvo dataset (EWD) and industrial \add{dataset} (IND) \delete{dataset}.
% The ``Total'' row summarizes the total number of corrects and the overall accuracy of different algorithms.
% % According to the experimental results, \toolName has significantly improved the accuracy of matching elements.
% Overall, \toolName achieves the best result on all types of changes (Add, Delete and Update) for both open-source and industrial datasets.

% More specifically, \toolName is more accurate than all other evaluated tools, with the overall success matching rate being 84.9\%, while the best result of existing tools is only 68.8\%.
% \toolName produces better results than existing tools mainly because our optimization approaches iteratively improve the matching results based on region and path similarity, while other tools produce matching results directly.
% It is worth \add{noting} that tree-based matching algorithms (SFTM, \toolName) have significantly higher accuracy in identifying added and deleted elements than other matching algorithms. 
% % For instance, among 101 deleted elements from the industrial dataset, \toolName successfully matches 77 of them with 31.7\% accuracy, while the accuracy of \watertool, \vistatool, \webevotool and \sftmtool is 1\%, 5\%, 0\%, and , respectively.
% For instance, among 170 added elements from the industrial dataset, \sftmtool successfully matches 133 of them with 78.2\% accuracy, while the accuracy of \watertool, \vistatool, and \webevotool is 16.5\%, 4.7\%, and 5.9\%, respectively.
% \toolName even achieves better results, and its accuracy is 83.5\%.
% This is because the tree-based matching algorithm matches elements by referring to parent-\add{child} relations, which has a stronger ability to identify added and deleted elements.
% In terms \add{of} deleted elements, \toolName outperforms \sftmtool (76.2\% vs 31.7\%) mainly because \toolName can also consider the relations of sibling nodes in the iterative, while \sftmtool only measure the parent-\add{child} relations.





% % \yuanzhang{It seems to require a futher disscussion, and this discussion is difficult to explain the advantages of \toolName. I want to analyze the collected dataset in the front subsection, such as the proportion of the elements with text. Discussing the reasons for the high matching accuracy of existing algorithms and the reasons for the low matching accuracy in this subsection. For example, there is a big difference in the performance of WebEvo on two datasets.}

% % \yuanzhang{We can also discuss the elements that our algorithm fails to match and analyze the reasons behind it. Further conclusions that can be drawn are: 1. The semantic similarity algorithm for statements has little effect. 2. The visual approach has also little effect. In other words, these two information can be completely dispensed with.}




% % The open-source(OS) dataset and industrial(IND) dataset can achieve the correct rate of 96.50\% and 92.50\%, respectively. 
% % The overall change recognition rate has also been greatly improved, reaching an accurate rate of 84.9\%.
% % \toolName has also significantly improved the identification accuracy of \textit{Add} and \textit{Delete} types.
% % Among \textit{Add} types, \toolName correctly identified 302, higher than \sftmtool's 289.
% % Among \textit{Delete} types, \toolName correctly identified 172, higher than \sftmtool's 130.
% % \watertool, \vistatool and \webevotool have poor identification ability on \textit{Add} type and \textit{Delete} type.

% %In addition, the robustness of the algorithm on different pages has been also significantly enhanced. Specifically, for each webpage, the correct element matching rates of \toolName on EWD datasets and industrial datasets are from 60.86\% to 93.25\% and 84.09\% to 91.38\%, respectively. While state-of-the-art \sftmtool are from 28.21\% to 95.45\% and 71.21\% to 93.10\%, respectively. This result indicates that \toolName is less sensitive to different webpages.

% % In addition, we also found that many algorithms tend to get matching results to improve the recognition accuracy of newly added and deleted elements, such as \watertool, \vistatool, and \webevotool. Compared with the \watertool algorithm, the \waterlitetool  algorithm does not significantly decrease the correct rate of matching parts. Still, it substantially increases the correct rate of newly added and deleted elements.
% % At the same time, we also noticed that the text attribute is very effective. Compared with \sftmtool, \sftmplustool has a certain improvement in matching and adding two indicators. Among them, the matching accuracy rate has increased from 73.86\% to 88.61\%. Text information has a high effect on element matching.

% \begin{figure}[!th]
% \centering
%     \includegraphics[width=0.48\textwidth]{images/figure_t_iteration2.pdf}
% \caption{The accuracy rate varies with the number of iterations.}
% \label{fig:figure-t-iteration}
% \end{figure}

% \add{We further evaluate \add{the} effectiveness of the iterative algorithm.
% Figure \ref{fig:figure-t-iteration} presents the number of correctly matched elements during the iterative process. 
% The x-axis shows the number of iterations, while the y-axis displays the count of correctly matched elements. 
% It is evident from the graph that the matching accuracy increases progressively with each iteration. 
% In the first iteration, only 908 elements were correctly matched, while the following three iterations successfully matched 1986, 1988, and 2157 elements. 
% However, after the fourth iteration, there is no significant improvement in the matching accuracy. 
% Therefore, we decided to set the maximum iterations to five. 
% The results indicate that the iterative process significantly enhances the matching accuracy.
% % We also note that the accuracy for the "Add" and "Delete" types decreases as the number of iterations increases, stabilizing after the fifth iteration.
%  % This phenomenon occurs due to the inclusion of path similarity and region similarity during the iterative process, which causes the total similarity to exceed the threshold.
% % As a result, certain elements that were initially similar but were added or deleted are mistakenly identified as matches.
% }


% \subsection{[RQ2] Efficiency on Matching Elements}
% %Apart from matching accuracy, we also evaluated the efficiency of \toolName.
% To compare the efficiency of different algorithms, we calculate the average time taken by each algorithm to generate final matching results.
% We use the saved webpage for matching to avoid inaccuracy caused by the network (e.g., page loading latency).

% The ``AVG Time'' row in Table \ref{table:experiment-comparison-match-ui} shows the average time taken (in seconds) by different algorithms to generate matching results across all webpages. %on the UI match dataset.
% % The average time for all tools except vista is within 1 second.
% Among all evaluated tools, \watertool is the fastest in producing matching results (0.0003s) because it matches elements by computing similarities of DOM properties which is very efficient.
% %Among the evaluated tools, \watertool generates matching results using shortest time (0.0003s), because \watertool match the elements according to the similarity of the DOM properties which is very efficient.
% \webevotool and \vistatool are slower than \watertool since they rely on time-consuming image similarities check.
% \webevotool is much faster than \vistatool since it uses a fast image similarity algorithm (aHash).
% \toolName and \sftmtool take similar time to generate matching results (0.97s and 0.87s).
% Compared to \watertool and \webevotool, \toolName is slower mainly because it requires multiple iterations for optimizing the matching results.
% With improved accuracy, we believe it is acceptable to take $<$1s to generate matching results for each webpage.
% % \yuanzhang{This section feels a bit short and strange. I want to merge this section with the previous one and free up an RQ to explore the changes in matching accuracy of elements during the iteration process.}
% % Compared to \webevotool and \watertool, \sftmtool and \toolName are slower because they output a matched element after matching all elements.
% % These indicate that \toolName is an effective tool.


% % \subsection{\add{[RQ3] Effectiveness on iterative matching}}



 
% \add{
% % Despite this, the accuracy improvement resulting from the "Update" type is more significant compared to the decrease in accuracy for the "Add" and "Delete" types.
% }

% \subsection{[RQ3] Effectiveness on Repairing UI Tests}

% \label{sec:evaltools}
% To fairly compare the capabilities of different algorithms in repairing broken UI tests, we integrated the matching algorithm of \watertool, \vistatool, \webevotool and \sftmtool into our repair framework. We named them \watertool{*}, \vistatool{*}, \webevotool{*} and \sftmtool{*}, respectively.

% \noindent \textbf{Successful repair.} We consider a test case to be successfully fixed if (1) the test passes after the repair and (2) each action in the test has been correctly executed (we verify this by manually comparing the screenshots of the traversed webpages).

% The dataset contains 135 test cases in open-source apps and 204 test cases in industrial apps.
% After excluding 163 non-crashing test cases (which do not need to be repaired) and 10 test cases that cannot be repaired due to the tested modules being removed, we obtained 62 crashing test cases in open-source apps and 104 crashing test cases in industrial apps (166 test cases in total).

% Table \ref{table:experiment-repair-scripts} presents the test case repair results of different algorithms. 
% For each application, the table reports the total number of test cases (Total) and the number of test cases successfully repaired by different algorithms.
% \delete{The c}\add{C}olumn $\Delta$V shows the number of released versions between the original and new versions.
% As shown in Table \ref{table:experiment-repair-scripts}, \toolName achieves the best results across all applications.
% In total, \toolName successfully fixes 113 broken test cases with a repair rate of 68\%, while the best existing tool (i.e. \vistatool{*}) only fixes 73 of them with a repair rate of 44\%.
% Moreover, we observe that the larger $\Delta$V is, the more changes introduced to the new versions since the original version, the more challenging to fix the broken tests.
% For instance, for MRBS, the best tool only fix 4 of 24 broken test cases.


% % Note that, there are 2 test cases of \vistatool and 1 test case of \webevotool is failed repair, which passed but violates the original intention.
% % For example, in the test case ``DeleteUser'' of the MantisBT application, the test case uses \textit{administrator} to determine whether the test case returns a user list webpage.
% % However, each page of MantisBt has \textit{Logged in as: administrator} and \vistatool incorrectly matches the \textit{administrator} element in it.
% % After returning the text of the element, the assert was successfully passed.
% % Such fixes are considered failed repair and are excluded from the number of successful repaired test cases.

% \begin{table}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{1.8pt}
% \caption{UI test repair effectiveness}
% \label{table:experiment-repair-scripts}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{l|rr|rrrrrrr}
% \toprule
% Application & Total & $\Delta$V & \watertool{*} & \vistatool{*} & \webevotool{*} & \sftmtool{*} & \toolName \\ \hline \hline
% AddressBook   &8 &30 & 1&\textbf{2} &0 &\textbf{2} &\textbf{2} \\
% Claroline  &29 &7  & 0 &\textbf{24} &0 &0 &\textbf{24}\\
% Collabtive  &5 &4 & \textbf{3}&1 &2 &0 &\textbf{3}  \\
% MantisBt  &38 &1  &18  &4 &19 &6 &\textbf{24} \\
% MRBS  &24 & 12 & 0 &\textbf{4} &0 &2 &\textbf{4} \\\hline
% \appa{}  & 46 & 1 &36 &33 & 37 &40 & \textbf{43}\\ 
% \appb{} &16 & 1 &6 &5 &6 &11 & \textbf{13}\\ \hline
% Total & 166 & - & 64(39\%) &73(44\%) &64(39\%) &61(37\%) &\textbf{113(68\%)} \\ \hline
% % AVG Time & - & & & & & \\ \hline
% \end{tabular}}
% \end{table}

% % \toolName repaired 57 out of 113 crashed test cases in open-source dataset and repaired 56 of 57 crashed test cases in industrial dataset, higher than other algorithms.


% % To improve the credibility of the experiment, we executed each algorithm more than twice on each use case.
% % Two authors analyze the reasons for the failure of all test case fixes separately and finally summarize the reasons.
% % \yuanzhang{Should I explain why some algorithms perform worse in some applications?}\xiang{yes, you should}
% The number of successful repairs generated by the same approach differs across apps.
% \watertool and \webevotool performed well on MantisBt but did not repair any test cases on Claroline.
% \sftmtool performed well on both \appa{} and \appb{} 
%  but did not work well for the five open-source applications.
% This is mainly due to the different element change types of different applications.
% For instance, on the login webpage of MantisBt, the button with the text ``Enter'' is transformed into the input with the value attribute ``Enter''. 
% \vistatool is weak at distinguishing the elements with text, leading to the ``Enter'' button matched with the ``Log out'' button, resulting in test cases that cannot be repaired.
% % Since the attributes of open source applications (1.63 attributes per element) are less to those of industrial applications (2.23 attributes per element)\yuanzhang{Does this need to be written in RQ1 of study?}, \sftmtool performs significantly better in industrial applications than in open source applications.
% Even so, the repair rate of \toolName on different applications is the same or higher than all existing algorithms, which shows the high robustness of \toolName.

% % In the test case of the Claroline application, the ''Enter'' button on the login page changed from text to the value attribute.
% % The \watertool and \webevotool matches failed and all use cases could not be repaired due to login failure.
% \begin{figure}[htbp]
%     \begin{minipage}[t]{0.5\linewidth}
%         \centering
%                 \includegraphics[width=\textwidth]{images/open_test_venns.pdf}
%         \centerline{(a) Open-source test cases}
%     \end{minipage}%
%     \begin{minipage}[t]{0.5\linewidth}
%         \centering
%                 \includegraphics[width=\textwidth]{images/industry_test_venns.pdf}
%         \centerline{(b) Industry test csaes}
%     \end{minipage}
%     \caption{Distribution of test cases repaired by different algorithms.}
%     \label{fig:venns-test-case}
% \end{figure}
% % \input{sections/discussion}


% Figure \ref{fig:venns-test-case} \delete{compares the} \add{shows a} Venn diagram of repaired test cases of  \watertool{*}, \vistatool{*}, \webevotool{*}, \sftmtool{*} and \toolName{} in the open-source and the industrial test dataset.
% The green, blue, pink, yellow, and orange represent the number of test cases repaired by \watertool{*}, \vistatool{*}, \webevotool{*}, \sftmtool{*} and \toolName{}, respectively.
% There are 8 test cases in the open-source dataset that can only be fixed by \toolName{}, while there are 2 test cases in the industrial dataset that can only be fixed by \toolName{}.
% On the other hand, there is only one test case from the open-source dataset that cannot be fixed by \toolName{} but fixed by other tools (\watertool{}).
% \add{%In this test, two buttons with the same text on different pages can accomplish the same function.
% %\watertool can be matched due to the simple use of text, but \toolName cannot be matched due to consideration of structural information.
% The test case, that \toolName{} failed to fix, needs to click a series of actions and then click an ``add task'' button.
% % In the app, the ``add task'' buttons appear on two different pages (home page and my task page), and the regions where the ``add task'' buttons are located are significantly different.
% % In the update, the ``add task'' button was moved to a different webpage, making the regions where the ``add task'' buttons are located significantly different.
% % This is the reason that \toolName{} failed to match the ``add task'' button.
% % In contrast, WATER correctly matches this element since it simply measures the similarity of the text, which is not changed in the webpage update.
% % This is the reason that UITestFix failed to match the ``add task'' button in different page but the WATER correctly matches this element since it simply measures the similarity of the text.
% After the webpage update, \toolName failed to match the ``add task'' button because this button was removed from the original page.
% In contrast,  \watertool matches this button with an ``add task'' button from a different page.
% These two buttons are matched by \watertool just because they simply have the same text.
% Since the matched ``add task'' button also completes the function of adding tasks and passes the assertion checking, this test is considered to be repaired successfully by \watertool.
% This situation happens relatively rarely (only once in the experiment).}
% We also noticed that some test cases could only be correctly fixed by a specific algorithm other than \toolName{}.
% For example, in the open-source test cases, there are 27 test cases that can only be fixed by \vistatool{} and \toolName{}, while in the industrial dataset, there are 6 test cases that can only be fixed by \sftmtool{} and \toolName{}.
% This means that although different algorithms have their own advantages, \toolName{} has a stronger ability to fix test cases.




% To better understand the capability of \toolName{} for future improvement, we manually analyze the 53 broken test cases which \toolName{} fails to repair. 
% Specifically, for each case, we categorize the reason behind the test failure by comparing the correct repair with the algorithm's repair results.
% % , and manually investigating the root cause of failures.
% %   by inspecting the program location in the broken tests where the crash occurs.
% Figure \ref{fig:evluation-error-analysis} shows the distribution of the six reasons behind the failure of \toolName.
% \begin{enumerate}
%     \item \textit{Add Action.} Add Action denotes that an action needs to be added to repair the test.
%     \item \textit{Delete Action.} Delete Action denotes that an action needs to be deleted to repair the test.
%     \item \textit{Modify Assert.} Modify Assert means that the expected value of the assertion needs to be updated in the test.
%     \item \textit{Branch Statement.}
%     Some test cases use some branch statements to enhance the stability of test cases, such as using if-else statements to handle 
%     the empty table data and the case of the table data not being empty.
%     % different situations with data. 
%     The branch statements executed in the new version may not have been executed in the old version, causing the inability to repair the test case in the new version due to the lack of action information. 
%     We label this reason of failure as Branch Statement.
%     % We labeled a crashing event as Branch Event when the event was not executed in the old version but in the new version, \toolName fails to repair the event due to the lack of event information.
%     \item \textit{Propagated Breakages}~\cite{whydowe}. 
%     Propagated Breakages refer to the scenario where the element is pointing to an incorrect element using the original locator without throwing \add{an} immediate exception but triggers a subsequent crash.
%     \item \textit{Incorrect Match.} The test case can be fixed by relocation, but the algorithm matches incorrectly or cannot find the matched element.
% \end{enumerate}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.48\textwidth]{images/evluation-error-analysis.pdf}
% \caption{Reasons behind the repair failures of \toolName.}
% \label{fig:evluation-error-analysis}
% \end{figure}

% As only 7 of them are caused by Incorrect Match (13.21\%), and \toolName can repair 113 (94.16\%) test cases requiring locator fixes, \add{and} this shows that \toolName performs well in repairing broken locators.
% This indicates that for the relocation type of repairs, \toolName already has a strong capability.
% Therefore, in the future, we will focus on the remaining types of repair failures.
% % We left repairing other types of failures as future work.


% % \begin{figure}[t]
% % \centering
% %     \includegraphics[width=0.48\textwidth]{images/industry_test_venns.pdf}
% % \caption{Reasons behind the repair failures of \toolName.}
% % \label{img:industry-test-venns}
% % \end{figure}









==> sections/sections/intro.tex <==
\section{Introduction}

When developers change the user interfaces (UI) of a Web application due to rapidly changing requirements, the corresponding Web UI tests need to be manually updated for test maintenance.  %is essential for ensuring their quality and reliability. 
% \delete{The test cases locate web elements and execute actions on them instead of manual actions to test whether the related functions work correctly.}
%While web apps update frequently and expeditiously, testers commonly utilize existing UI test cases for regression testing purposes. 
%Several approaches have been proposed for repairing broken Web UI tests~\cite{GUITAR, regression}. by %by matching Web UI elements and fixing the outdated locators~\cite{GUITAR, regression}. 
% \delete{Otherwise, the existing test cases will fail on the updated web apps.
% According to a study of Adobe’s Acrobat Reader, 74\% of its test cases failed between two successive versions~\cite{fail_rate}.
% Another study also shows that a simple single GUI change can cause 30\% to 70\% of system test cases to fail ~\cite{fail_rate2}.}
To reduce manual efforts in repairing broken Web UI tests, several automated approaches have been proposed
 in academia and industry to automatically fix broken Web UI test cases caused by software evolution
~\cite{water,vista,UITESTFIX}. The key step in the automated repair of Web UI tests is to modify the broken statements containing outdated element locators by matching the element $e_{old}$ in the old version of a Web application with the element $e_{new}$ in the new version ~\cite{whydowe}. 
Prior Web UI test repair techniques mostly rely on a set of Document Object Model (DOM) attributes (e.g., identifiers and XPath)~\cite{water} or visual information~\cite{vista} %or Document Object Model (DOM) structures~\cite{sftm2023} 
to determine whether the two elements $e_{old}$ and $e_{new}$ match. 
These techniques extract and compute the similarity of this information to select the most similar element as the result of the matching.
% \delete{If no elements on the new web app has higher similarity than the threshold, no match is considered. }


% As there can be many attributes of a Web UI element which can be used for matching,

Due to numerous attributes available for matching Web UI elements, these techniques may prioritize certain attributes. For example, \watertool{} \cite{water}, a classical Web UI test repair technique, applies a multi-step matching process using different attributes. First, it searches for identical elements by matching five attributes (\emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, \emph{name}). If unsuccessful, it then finds similar DOM nodes using additional attributes. Specifically, it identifies elements with the same \emph{tagname}, %based on the assumption that ``it was unusual for a node to change its tagname during evolution''~\cite{water},
and computes their similarity scores %normalized Levenshtein distance 
% between the XPaths
between $e_{old}$ and $e_{new}$ 
% considering \emph{XPath} and other attributes (e.g., screen position), %of a DOM node)
%  and computes a similarity score 
 with the weighted sum of \emph{XPath} and other attributes where it prioritizes \emph{XPath} similarity based on the heuristic that \emph{XPath} of nodes ``should be very similar across versions''~\cite{water}. As the prioritization and the predefined order on matching these attributes are usually based on heuristic of the tool developers, \emph{the matching algorithm may not accurately reflect the evolution of the Web element}, causing inaccuracy during matching, and subsequently failing to repair the broken statement. Hence, it is important to understand the attribute prioritization used by prior test repair approaches. %Meanwhile, other techniques try to combine several~\cite{color} attributes.   
 Meanwhile, prior learning-based techniques show promising results in combining different types of information for repairing broken Android GUI tests (e.g., combining word and layout embeddings~\cite{Vifer}, or fusing GUI structure and visual information~\cite{xu2021guider}). The richer representation used by these learning-based techniques has been shown to enhance the accuracy of the UI matching step.     

To solve the aforementioned %element matching 
problems of Web UI test repair and to hinge on a richer representation in learning-based approach, 
%we propose using ChatGPT to enhance Web UI test repair.
we present the \emph{first study} of understanding the attribute prioritization and enhancing traditional Web UI test repair approaches with LLMs like ChatGPT. %to solve the aforementioned problem in prior techniques. 
Our use of ChatGPT is motivated by the promising results shown in prior studies for solving related software maintenance tasks, (e.g., test generation~\cite{Feldt2023aa}, and automated program repair~\cite{sobania2023analysis,fan2023automated}). %, and the fact that it has been trained on billions of open-source software artifacts which include various forms of information and test code. 
However, the Web UI test repair problem differs from these tasks as it mainly involves Web element matching where accurate matching results typically lead to the correct repairs. Specifically, our study evaluates the effectiveness of integrating ChatGPT into two representative Web test repair techniques (\watertool{} and \vistatool{} \cite{vista}). To further evaluate the heuristic used in \watertool{} that prioritizes XPath similarity, we also design a simplified variant of \watertool{} that performs matching using only Levenshtein edit distance between XPaths of the old element $e_{old}$ and the new element $e_{new}$ (we call this approach \emph{\edtool}). Our study focuses on Java Selenium tests which are commonly used by Java Web applications. 

% The key insight of our study is that \emph{we can improve the overall matching results by first using existing Web test repair approaches to obtain an initial list of candidate matched elements (which may be biased by the prioritization used by a particular technique), and then use ChatGPT to perform global matching to further select the best matched element in the new version}. 

The key insights of our approach are twofold: (1) we first rely on traditional Web UI test repair approaches to obtain an initial list of candidate matched elements (which may be biased by the prioritization used by the approach), and then use ChatGPT to perform subsequent matching to further select the best matched element in the candidate list, and (2) as ChatGPT may suffer from the hallucination problem~\cite{Feldt2023aa}, we design our prompt based on OpenAI's official documentation by asking ChatGPT to generate an explanation along with each selection. To mitigate hallucination, we propose an \emph{explanation validator} that automatically checks for the consistency of the explanation, and instruct ChatGPT to self-correct the initial selection based on detected inconsistent explanation.
% ask ChatGPT for any incorrect explanation to provide a chance for it to self-correct the initial selection.


Our study %of \watertool{},\vistatool{}, and \edtool{} with ChatGPT 
aims to 
answer the following questions: 
\begin{description}[leftmargin=*]
\item[RQ1:] Can ChatGPT help improve the accuracy of Web element matching of prior Web test repair approaches? %with ChatGPT, can the combination help in improving the accuracy of Web element matching?
%\item[RQ1:] If we combine prior Web test repair approaches with ChatGPT, can the combination help in improving the accuracy of Web element matching?


\item[RQ2:] What is the effectiveness of ChatGPT in repairing broken Selenium statements for Web test repair? %If we combine existing approaches with ChatGPT, can ChatGPT help in Web test repair? 

%When ChatGPT explains about the element matching result, what is the quality of the explanation?

\item[RQ3:] When ChatGPT explains the result of the element matching, what is the quality of the explanation?

\item[RQ4:] Can our proposed explanation validator guide ChatGPT in self-correction to improve the matching and repair results?

%With history matching results, will ChatGPT perform better in web UI element matching?

%\item[RQ4:] What is the effectiveness of repaired result of ChatGPT according to its matching result?
\end{description}

 %as it only prioritizes based on single attribute (XPath). 

%Meanwhile, existing works use a threshold to determine whether two elements share sufficient similarity. 
%\yz{However, the differences between webpages can be large or small, which makes it difficult to use a certain threshold to match elements. 
%Furthermore, our experiments show that according to existing tools, correctly matched elements do not always have the highest similarity. 
%This results in the low accuracy of existing tools.

% \delete{Some of the tools only focus on matching instead of repairing.
% For example, WEBEVO~\cite{webevo} utilizes historical webpages to identify matching elements.
% Its primary purpose is to monitor changes on websites and report them to developers and testers.
% It does not involve automatic repairs. 
% And we will research on the tools that also complete the auto repair part after matching element. 
% WATER~\cite{water} and VISTA~\cite{vista} are commonly employed tools that can repair test cases directly in the domain of automated test repair.
% Researchers frequently utilize these two tools for comparative analysis of their own proposed solutions.
% WATER and VISTA use different techniques to suggest repairs for broken web UI test cases. VISTA proposes a visual analysis of the application to detect the root causes of test breakages and suggests potential repair to the testers, while WATER uses differential testing to compare the behavior of the test case on two successive versions of the web application and suggests repairs based on the differences between the two executions. Leotta et al~\cite{dom_visual} conducted research on the expenses related to building and sustaining test suites, including both DOM and visual tests~\cite{visual1}, for web applications. He concluded that DOM-based locators are generally more reliable than visual locators, and it is more cost-effective to develop and improve DOM-based test cases from scratch. Additionally, DOM-based test cases take less time to execute. However, depending on the particular characteristics of the web application being tested and its anticipated changes, visual locators may be the better option in some instances (such as when the visual appearance is more stable than the structure).}

% \delete{Therefore, each of the two localization methods has its strengths. 
% In this paper, we aim to investigate the effectiveness of the DOM-based repair tool WATER and the visual-based repair tool VISTA, and explore ways to improve them.} 




%we first leverage existing work~\cite{water, vista} to filter candidate elements on webpages. Then, the filtered elements are presented to ChatGPT for selection. The core idea of our approach is...

%Our feasibility study aims to answer the following question: 
%\begin{description}[leftmargin=*]
%\item[RQ1:] If we combine existing approaches with ChatGPT, can ChatGPT help in web UI element matching?

%\item[RQ2:] When ChatGPT explains about the element matching result, what is the quality of the explanation?

%\item[RQ3:] With history matching results, will ChatGPT perform better in web UI element matching?

%\item[RQ4:] What is the effectiveness of repaired result of ChatGPT according to its matching result?
%\end{description}



\noindent\textbf{\textit{Contributions.}} Our contributions are summarised as follows:
\begin{description}[leftmargin=*]
    \item[Study:] We present the first study of understanding attribute prioritization and enhancing traditional test repair approaches with ChatGPT for Web UI test repair. Our findings include: (1) prior test repair tools have preferences towards certain attributes (e.g., XPath), %(1) as \watertool{} and \vistatool{} performs selection of the best matched element using their predefined heuristics, these techniques could usually select the best matched element rather effectively, whereas the combination with ChatGPT may even lead to a performance decrease in Web element matching,
(2) the combination with ChatGPT helps improve the matching accuracy of all evaluated approaches; 
(3) to our surprise, although \edtool{} performs the worst individually, its combination with ChatGPT outperforms all the evaluated approaches in element matching and repair; (4) the repair effectiveness of all evaluated approaches
is generally similar to the matching ones but there is one case where the repair performance decreases; %, which shows the limitations of evaluated approaches; 
(5) our proposed workflow of checking for explanation consistency and generating self-correct prompt as hint to ChatGPT could further improve the effectiveness for certain combinations (e.g., \watertool{}+ChatGPT).
    \item[Technique:] We proposed a novel Web UI test repair technique that uses traditional Web test repair approaches for initial matching and then uses ChatGPT for \emph{subsequent matching} (uses all attributes of each UI element to perform another matching) to further improve the matching accuracy. Instead of prioritizing certain attributes in prior approaches (Table \ref{tab:attribute}), the subsequent matching steps use all attributes. To combat the hallucination problem in ChatGPT, we also design an explanation validator that automatically checks for the consistency of the generated explanation to guide %to provide a mechanism for 
    self-correction.  %similarity calculating strategy to make ChatGPT perform better in matching and repair tasks.
    % UI test repair dataset contains 308 reproducible UI tests.
    \item[Evaluation:] We evaluate three baseline approaches (\watertool{}, \vistatool{}, \edtool{}), their combinations with ChatGPT, and two recent approaches (\webevotool and \sftmtool). Our evaluation on a widely used dataset~\cite{dataset} shows that the proposed workflow further improves the effectiveness of prior approaches in Web UI element matching and test repair.
    % \item[Data Availability] To advance future research in test repair, we made our scripts and data available at \url{https://anonymous.4open.science/r/ChatGPTWebUITestRepair-0D95/}.
    
    % \item[Availability:] The dataset, scripts and experimental data are available at: https://anonymous.4open.science/r/ChatGPTUITestRepair-7169. 
    %\item[ChatGPT's mistakes:] We analyzed the patterns of mistakes made by ChatGPT during test repair.
    %\item We found out the role of context in prompts for ChatGPT.
%     in (1) element matching, and (2) test repair.
%     Compared to existing tools' best results (68.8\%), \toolName achieves 84.9\% element matching accuracy. %, much higher than existing tools' best results (68.8\%).
% For test repair, \toolName successfully fixes 113 out of 166 tests, while the best existing tool only fixes 73 tests.
    %We evaluate \toolName on open-source and industrial datasets. Our evaluation shows that \toolName outperforms \numbaseline{} prior approaches.
    % \item To facilitate future research on \delete{W}\add{w}eb UI element matching and repair, we relabeled and augmented an open-source UI element matching dataset, which contains 1,620 label\add{l}ed UI elements. Our dataset and results are available at \href{https://anonymous.4open.science/r/Web-UI-Dataset-9645}{https://anonymous.4open.science/r/Web-UI-Dataset-9645}.
\end{description}






% scripts before 9.15, (appear in final paper)

% Web apps are characterized by rapid updates.
% Existing UI test cases are often used as regression tests to ensure the update does not affect original program behaviors.
% However, during app evolution, developers may modify attributes in \delete{W}\add{w}eb elements, causing the corresponding UI test cases to be broken on the new versions.
% %that perform actions (e.g., click) on the modified elements to be broken. %due to the outdated locators. % in UI test cases also become fragile.
% To make existing test cases executable on the updated version, testers need to manually (1) execute new test cases, (2) locate the bug, and (3) fix it, e.g., modify the element locator of test cases.
% %based on the latest version of the Web application. 
% Updating broken UI tests manually \delete{are} \add{is} time-consuming and labor-intensive.
% In recent years, several techniques have been proposed in academia and industry to automatically fix broken UI test cases caused by app evolution~\cite{waterfull,stocco2018vista,brisset2022erratum,imtiaz2021automated,10.1007/978-3-030-74296-6_29_WTSR}.



% To automatically fix broken web UI tests, one of the most important steps is to repair its outdated element locator.
% Existing approaches fix element locators by matching the UI elements before and after update using either visual information~\cite{stocco2018vista,shao2021webevo}, attributes~\cite{choudhary2011water} (e.g., identifier name), or Document Object Model (DOM) structures~\cite{brisset2020sftm, brisset2022erratum}.
% More specifically, those approaches (1) collect the visual image, attributes, and DOM structure of each element before and after the \delete{W}\add{w}eb page update, (2) compare the similarity of each pair of elements using similarity metrics, (3) if the similarity of two elements is greater than a threshold, they are identified as matched elements.
% UI test repair tools can then fix the broken locators of UI tests according to element matching results.

% However, existing approaches still have some limitations.
% First, their accuracy in matching UI elements is still quite low.
% For instance, as shown in our evaluation (Section~\ref{sec:evaluation}), the state-of-the-art UI element matching tool \sftmtool achieves 68.8\% accuracy, and the UI repair tool \vistatool only achieves 46.7\% accuracy.
% The low element matching accuracy will then significantly decrease the effectiveness of automated UI test repair techniques.
% Second, prior work mainly studied the maintenance of UI tests on open-source web apps with test cases written or translated \add{(migrate test cases from other Capture–Replay tools to Selenium)} by researchers.
% The manually written or translated test cases are usually short and simple.
% % \yz{No existing work has studied the real UI test maintenance of practical and large-scale industrial web apps.}

% Moreover, designing a robust framework that can repair complex industrial UI tests is challenging.
% For instance, \vistatool~\cite{stocco2018vista}, a state-of-the-art repair framework, failed to repair our provided industrial tests correctly because (1) industrial webpage tests have many control-flow branches, but \vistatool only supports tests with a single control flow, and (2) industrial tests usually adopt Page Object design pattern for improving test maintenance~\cite{leotta2013improving}, but \vistatool{} parses and extracts statements using regular expressions, (3) industrial web tests may invoke additional APIs on top of Selenium APIs to expand its functionality but \vistatool{} only supports specific Selenium APIs.
% %these APIs have not been instrumented. %and improve its stability 

% % However, these approaches still need to fully utilize structural information, such as the relative positions of elements and the relations with neighbouring elements, which may help to improve matching accuracy.\xiang{todo}

% To solve the above problem, we propose a general framework \toolName, for automatically fixing the UI tests of practical and large-scale \delete{W}\add{w}eb applications.
% The core technique of \toolName is a novel iterative element-matching approach that fully utilizes the DOM structure information.
% The main insight is that the relative positions of elements and the relations with neighboring elements may help to improve matching accuracy.
% To capture such information, we propose \textit{path similarity} and \textit{region similarity} to measure the similarity of elements according to their relations.
% In an iterative process, \toolName first matches the elements that are more likely to be matched with high confidence, and then current matching results could guide the element matching in the following iterations.
% More specifically, the workflow of \toolName is as follows: (1) it first simplifies the DOM structure by grouping related elements of webpages; (2) calculates the similarity according to id, attribute, DOM structure and etc.; (3) relies on the \textit{iterative matching} algorithm to continuously recalculate the similarity and rematch the elements in multiple iterations to improve the matching accuracy.
% Based on our matching algorithm, we implemented the repair framework for automatically fixing broken web UI tests. 
% % To solve the second challenge of designing a robust repair framework,
% \toolName{} is a robust repair framework that includes a dynamic repair component that can parse and repair the UI tests of all kinds of \delete{W}\add{w}eb applications. 

%   %To solve the first challenge, we also %in industrial scenarios.
% %To evaluate \toolName, we labeled a webpage dataset including 2,522 web elements changes and 166 broken test cases.


% We evaluate \toolName on a set of open source applications and industrial applications.
% In terms of element matching, \toolName correctly matched 2,141 (81.9\%) elements, which increased the correct rate by 16.1\% compared with the best result of existing tool \sftmtool (68.8\%).
% Moreover, \toolName{} \add{  and \sftmtool take similar time to generate
% matching results (0.97s and 0.87s)}, 
% \delete{ takes an average of 0.8685s to match an element} which we believe is acceptable.
% To compare the repairability of \toolName with existing work, 
% we integrate the four element matching baseline approaches (\watertool~\cite{choudhary2011water}, \vistatool~\cite{stocco2018vista}, \webevotool~\cite{shao2021webevo}, and \sftmtool~\cite{brisset2020sftm}) into our repair framework (note that the existing tools do not support the \delete{W}\add{w}eb applications used in our evaluations).
% % to allow them to run correctly on all evaluated apps.
% % We integrate this repair component into the four baselines (\watertool~\cite{choudhary2011water}, \vistatool~\cite{stocco2018vista}, \webevotool~\cite{shao2021webevo}, and \sftmtool~\cite{brisset2020sftm}) to allow them to run correctly on all evaluated apps.
% Evaluation results show that \toolName can fix 113 (68\%) test cases, much higher than the 73 test cases (44\%) of the best existing tools. 
% Our results indicate that \toolName can match more complex element changes and has a higher matching accuracy rate and test case repair rate.


% \noindent\textbf{\textit{Contributions}} Our contributions are summarised as follows:
% \begin{itemize}[leftmargin=*]
%     \item We propose\add{d} \delete{iterative matching, }a novel element matching algorithm that can match UI elements more accurately by matching elements in multiple iterations. %using DOM structure information.
%     \item We proposed \textit{path similarity} and \textit{region similarity} to measure the similarity of elements according to their relations.
%     % UI test repair dataset contains 308 reproducible UI tests.
%     \item We design and implement a UI test repair framework, \toolName{}, and evaluate it by comparing it against four state-of-the-art baselines. Evaluation results show that \toolName outperforms existing techniques.
% %     in (1) element matching, and (2) test repair.
% %     Compared to existing tools' best results (68.8\%), \toolName achieves 84.9\% element matching accuracy. %, much higher than existing tools' best results (68.8\%).
% % For test repair, \toolName successfully fixes 113 out of 166 tests, while the best existing tool only fixes 73 tests.
%     %We evaluate \toolName on open-source and industrial datasets. Our evaluation shows that \toolName outperforms \numbaseline{} prior approaches.
%     \item To facilitate future research on \delete{W}\add{w}eb UI element matching and repair, we relabeled and augmented an open-source UI element matching dataset, which contains 1,620 label\add{l}ed UI elements. Our dataset and results are available at \href{https://anonymous.4open.science/r/Web-UI-Dataset-9645}{https://anonymous.4open.science/r/Web-UI-Dataset-9645}.
% \end{itemize}



% script that didn't appear in final paper of lyz 


% \sftmtool{} algorithm\cite{brisset2020sftm}, which utilizes structural information and attributes for matching.  propose to use flexible tree matching to fix broken locators in test case.
%Erratum\cite{brisset2022erratum}  propose to use flexible tree matching to fix broken locators in test case.
% However, simply using the relationship between parent and child nodes for similarity propagation makes the algorithm unstable.
% Hence, how to utilize the relationships between elements to help relocate webpage elements need to be further investigated.
% Moreover, 
% These evaluated web apps are much simpler than industrial web apps, and their tests are not usually available.
% To the best of our knowledge, only two web apps have available UI test cases~\cite{imtiaz2021automated,leotta2014visual}. \yuanzhang{change in tone.}
% Other studies focus on the webpage dataset~\cite{brisset2022erratum,shao2021webevo} collected from Wayback Machine~\cite{wayback}, but those webpages also do not have available tests.


% To automatically repair broken web tests, the first challenge lies in improving the accuracy of element matching. 
% Although existing approaches~\cite{choudhary2011water,stocco2018vista,shao2021webevo,brisset2020sftm} have demonstrated promising results in fixing broken tests for open-source apps, it is unclear how they perform in industrial apps.
% %when applying them to industrial scenarios, there is still room for improvement.
% % Due to a large number of test cases in the industry and the large number of events per test case, incorrectly fixing one event results in the failure of repair the whole test case.
% %successful repair means saving a lot of human resources, while repair failure will also consume a lot of material resources. 
% As the core step of the repair process, the element matching algorithm determines the accuracy of generated repairs. As our goal is to design a practical tool for repairing broken UI tests to meet the high accuracy requirement of \company{}, improving the element matching accuracy is essential. %still one of the most important tasks.
%Improving the element matching accuracy is still one of the most important and challenging tasks.



% Since web applications are displayed to users with a graphical interface, automated UI testing for web applications is essential.
%While the exact number of web applications keeps changing every second, there are over 1 billion sites on the world wide web. Web applications are playing increasingly important roles in our daily life, hence, testing web application become essential. Since web applications are displayed to users with a graphical interface, testing them is usually conducted via UI testing. Specifically, testers write test cases to simulate the communication between users and the Web application by executing some UI events. Each event locates an element through the locator and performs related operations on the element, such as click, input, etc. By monitoring the reaction of web applications, testers could verify their functional correctness.

% Testers write test cases to verify the functional correctness of web applications by using some UI test automation tools.
% These test cases simulate the process of users communicating with the Web application by executing some UI events.
% Each event locates an element through the locator and performs related operations on the element, such as click, input, etc.

%~\xiang{@Yuanzhang, add some citations here}.
%XPath (a path used to locate web element)
%Program transformation inference has many potential use cases such as systematic editing of multiple locations in the same codebase~\cite{Kim2009,lase}, porting commits across multiple instantiations of the same project (i.e. across forks)~\cite{Ray2012, Ray2013}, fixing recurring bugs using pattern-based transformations~\cite{Kim2006, Gao2015, Nguyen2010}, adapting API changes~\cite{Li2015, wang2016} and refactoring code~\cite{william19190}. However propagating changes from one repository to another related repository is still a major challenge~\cite{Ray2012} and a necessary requirement in software security. Such porting tasks are necessary to keep the software up-to-date and secure without breaking existing functionality~\cite{Chou2001}. In this paper, we focus on backporting patches in the Linux kernel. A key challenge in backporting code from one version to another is the evolution of the patch from the original, such that the evolved patch fixes the issue in the target version. Evolving a patch is not limited to namespace translation but also pruning irrelevant changes and adding supplementary changes which are missing for the required fix. 

%  to generalize the transformation to a suitable level such that it doesn't decrease precision and to specialize to a suitable level that doesn't decrease recall. 


% limitation: lack of labeled dataset 
% accurate 

% The Linux kernel is one of the most important software projects in the landscape of systems today. Its core functionality is used by a multitude of devices, ranging from servers to IoT devices. To support users with different feature/stability requirements, multiple versions of the Linux kernel are actively maintained. 
% When introducing a bug-fixing patch\footnote{Patch generally refer to a change to source files, i.e. to modify, add and delete lines.} to the mainline version, maintainers should backport the patches to old stable versions to keep them up-to-date. The increasing number of devices that depend on the Linux kernel and the rapid rate of evolution of the kernel raise a challenge for maintainers to ensure the continuous availability of the kernel code with the latest patches~\cite{ferdian2016}. 

% Although the mainline version of the Linux kernel shares a common codebase with older versions, they typically diverge over time as different features and fixes are added to the latest branch. As a result, when a bug is patched in the mainline version, 
% the patch is often not directly applicable to another version.
% Given a patch created for the latest version, backporting involves identifying the correct patch location and adapting the patch to an older version. Backporting is typically done manually by a developer, on a case-by-case basis. The manual process of backporting is error-prone and there is usually a long delay in publishing the backported patch. This becomes critical when we consider security patches.
% as they have a significant impact on the system security of Linux kernel. 

% \yuanzhang{todo:change this}To understand the importance and challenges of backporting patches, we first conduct an empirical study on the Linux kernel versions spanning 2011-19.
% We found that (1) 51,663 patches have been backported from the mainline to old versions, representing around 8\% of all the commits to the mainline version, and (2) the backporting process typically took more than one month.
% Moreover, backporting patches is not simple copy and paste, as it may involve changing patch locations, changing the namespace (the variable or function names used in different versions), and modifying the code logic and structure.
% These findings indicate that automatically backporting patches is important but challenging.


% Several existing tools have explored automated maintenance of UI test cases.
% For instance, \watertool~\cite{choudhary2011water} uses the attributes retained by elements or the similarity between attributes to calculate element similarity and recommend candidate elements for inpainting. 
% \vistatool~\cite{stocco2018vista} uses template matching to repair test cases from a visual point of view. 
% When there is no matching result on the page, it will call Crawljax\cite{crawljax2012Invariant-Based,Crawljax2012}~\xiang{explain this tool} to crawl the surrounding pages and find whether the candidate elements appear on these pages. 
% A set of visual and text-based algorithms is designed in \webevotool~\cite{shao2021webevo} to obtain the matching results of elements. 
% In \sftmtool~\cite{brisset2020sftm}, based on the calculation of similarity by attributes, a similarity propagation algorithm is proposed to combine DOM structure information.

% Some existing tools~\cite{choudhary2011water,stocco2018vista,shao2021webevo} use the element's own information, such as visual or attribute information, to relocate the element. 
% These methods did not fully use the relationship between DOM nodes, making it difficult to distinguish elements with similar information, thus generating a large number of false positives.
% Erratum\cite{brisset2022erratum} began to use other node attributes to assist matching. 
% However, simply using the relationship between parent and child nodes for similarity propagation makes the algorithm  perform unstably. Hence, utilizing the relationships between elements as efficiently as possible can significantly help relocate webpage elements.
% ~\xiang{@Yuanzhang, this para is not good, you need to present those tools in high-level instead of giving so many details. You also need to highlight the limitations of those tools.}

% \shinhwei{Visual vs. DOM-Based Web Locators: An Empirical Study}


%like \vistatool~\cite{stocco2018vista}

%the repair framework of the industrial UI tests should consider three important characteristics. 

%First, industrial webpage tests have many control-flow branches, but most existing tools only support analyzing tests with a single control flow. Second, industrial tests usually adopt Page Object Design pattern~\cite{shorturl}, meaning that we cannot parse and execute statements through regular expressions like \vistatool~\cite{stocco2018vista}. Third, the industrial web tests may carry out secondary development of Selenium to expand its functions and improve its stability. These features lead to the fact that the test case has the characteristics of complex control flow and rich event methods in the industrial situation. 
%Instead of using existing repair framework for parsing and executing open-source webpages, the repair framework of the industrial UI tests should consider three important characteristics. 


%To automatically repair broken UI tests, the first challenge lies in designing a robust framework that can analyze complex industrial tests. First, industrial webpage tests have many control-flow branches, but most existing tools only support test cases with a single control flow.  Second, industrial tests usually adopt Page Object Design pattern~\cite{shorturl}, meaning that we cannot parse and execute statements through regular expressions like \vistatool~\cite{stocco2018vista}. Third, the industrial web tests may carry out secondary development of Selenium to expand its functions and improve its stability.  These features lead to the fact that the test case has the characteristics of complex control flow and rich event methods in the industrial situation.  Instead of using existing repair framework for parsing and executing open-source webpages, the repair framework of the industrial UI tests should consider three important characteristics. 
%Compared to designing a repair framework for simple open-source webpages, the repair framework of the industrial UI test cases should consider all these characteristics.

% We found that (1) the actual version changes in the industry are similar to \textcolor{blue}{the open-source webpages dataset colleted by Fei Shao etc.  }\cite{shao2021webevo} \xiang{which collected data sets}, and we think that the page change data sets can be collected through existing methods. (2) The change rate of text elements in leaf nodes is low, and text information is vital to the element-matching process~\xiang{what is leaf node, why do you study text information}.
% (3) the number of locator changes varies with version changes~\xiang{what is locator}. \yuanzhang{Many papers use the term locator\cite{brisset2022erratum,imtiaz2021automated,stocco2018vista}, but no one gives a specific explanation. I think that a locator is used to locate a web element on one page, like XPath or CSS selector. So if one tool only repairs a locator, the problem is also named a locator repair problem.\cite{brisset2022erratum}}
% In some time, many locator changes will consume many human resources. (4) Since the industry adopts the PageFactory mode~\xiang{what is PageFactory}, the proportion of the actual locator that needs to be modified is reduced. (5) In actual scenarios, changes in events and assertions also have potential research value.



% Unfortunately, existing tools mainly study the maintenance of UI tests on open-source dataset or even artificial dataset.
% We observed that in the current paper, as far as we know, the open-source test case dataset\cite{imtiaz2021automated} are usually quite small.
% This is mainly because obtaining open-source data sets for the automatic maintenance of web application UI test cases is difficult.
% Hence, some works collect data sets of webpage changes from Wayback machines\cite{shao2021webevo,brisset2022erratum}.
% Besides, some work even write web UI test cases by themselves\cite{imtiaz2021automated,whydowe}.
% However, no existing work has studied the UI test maintenance of industrial web application.

% Since obtaining open-source data sets for the automatic maintenance of web application UI test cases, these existing works all use the data sets collected by themselves. 
% Some works mainly collect data sets of webpage changes from Wayback machines\cite{shao2021webevo,brisset2022erratum}. Others use automated tools such as Selenium IDE or write web UI test cases by themselves\cite{imtiaz2021automated,whydowe}.
% We observed that in the current paper, as far as we know, the only open-source test case dataset\cite{imtiaz2021automated}, there are still some differences between its implementation and the implementation of the industry.

% Due to the need for industry-wide research on web UI testing cases, we want to know the actual industry situation. 
% To better understand the page changes and the maintenance of real test cases of industrial apps, we first collected the page changes on a \company{}'s product, and their commits to the test cases from 2021-04 to 2022-10, leading to a total of 2534 tests from an ICT Web platform web app.
% By analysing this large-scale industrial dataset, we found that the change ratio for the property of UI elements in industrial webpages is higher than for open-source webpages.
% The industrial tests, with 157.3 events per test, are much more complex than manually written tests for open-source apps, with 14.7 events per test.
% Our study of \totdiff{} diff chunks from \totcommit{} revealed that developers usually fix broken tests by updating the locator, adding/deleting/modifying events, modifying assertions, and fixing events related to page loading. Compared to tests written for open-source apps, fixing industrial tests pose additional challenges.
%Fixing industrial tests is much more challenging than test cases written for open-source applications.

% \textcolor{blue}{We found that though the actual version changes in the industry are 
% similar to the open-source webpages dataset collected by Fei Shao etc.\cite{shao2021webevo}, 
% the fixes of the test cases are also different from the existing research\cite{whydowe,shao2021webevo}, which use the test cases written by themselves as dataset.
% On the one hand, the proportion of locator-related commits has dropped to only 8.4\%. This is because Page Object Designed Model is usually used in industrial UI test cases. This pattern creates an object repository for web elements, which reduces repeated code in test cases and increases maintainability. Page Object Design pattern makes repeated locator changes that only need to be modified once, alleviating the crash caused by locator changes. But there are still a considerable number of commits about locator change.
% On the other hand, there are still some commits related to the event type and assert type, but less attention is paid to them.
% These findings suggest that the automated maintenance of UI test cases is of great interest in the industry. However, the existing open-source datasets and the actual situation in the industry may be different, so it is vital to start research on UI test cases for industrial applications.}\xiang{still not good. let me first modify other sections}


% \yuanzhang{I feel that the current challenges are vague, so I would like to rewrite the challenges as follows:}
% \begin{enumerate}
%     \item \yz{The current algorithm has low robustness. The existing algorithm match elements based on the similarity of elements. When the elements change significantly, the similarity will be low. At this time, the algorithm often cannot correctly match the target element. If the threshold is simply reduced, added or deleted elements will be incorrectly matched. If the threshold is simply increased, it will not be possible to match the elements with low similarity.}
%     \item \yz{The repair frame.}
% \end{enumerate}

% \yuanzhang{.}




%Our analysis shows that the main reason for repair failure is that \toolName does not support fixing test by adding/deleting events. %which is the main reason causing repair failure.
%Adding/deleting events is left as future work.

% that can adapt to changes in webpage structure and implemented a repair tool named \toolName.
% We propose a Web element matching algorithm that has higher matching accuracy and robustness.
% First, we simplify the DOM structure of the page by clustering the DOM structure of webpage.
% Then, id similarity, attribute similarity and text similarity are used to calculate the initial similarity.
% The iterative optimization use path similarity, region similarity and initial similarity to recalculate the similarity and rematch the elements in each iteration.
% Finally, after getting the final match result, \toolName uses the match result to generate a patch and replaces the original element with the element found by new locator to continue executing the event.

% We implement our approach in a tool named \toolName---i.e., a tool for maintaining Web \textsc{UI test} cases through automated \textsc{fix}es.
% First, we constructed a webpage dataset and label 2526 elements.
% We compared existing tools with \toolName, and the 96.70\% matching accuracy of \toolName is much higher than other tools. 
% Next, we verified the repair capabilities of different algorithms on the industrial and open-source test case datasets. 
% The experimental results show that \toolName has the highest repair rate of xxx .




==> sections/sections/methodology.tex <==
\section{Methodology}
%\todo{update the figure}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]
    %, height=4in]
    {figures/content/workflow_new.pdf}
    \caption{Our proposed workflow of Web UI test repair}
    \label{workflow}
    \vspace{-6pt}
\end{figure}

Figure~\ref{workflow} shows the workflow of our approach. First, our approach extracts information from the target element on the old Webpage based on the broken statement and all elements on the new Webpage. 
Then, it uses a test repair tool (\watertool{}, \vistatool{} or \edtool{}) to rank the elements on the new Webpage, and selects top-ranked ones for ChatGPT to perform further element matching. 
Our approach then instructs ChatGPT to select the matching element and explain its choice by mentioning the most similar attributes it considers. 
Based on the generated explanation, our explanation validator calculates the consistency of the explanation. 
As the accuracy of UI matching cannot be automatically validated without checking if the broken statement has been repaired correctly, our approach generates the repair prompt for ChatGPT to proceed with the repair by instructing ChatGPT to fix the broken statement based on its selected element.
% Then, we manually validate the repair result by checking correctness of the matching element, repaired locator, and assertion (if present).
If the repair fails with explanation consistency (EC) less than 1, our approach generates a self-correctness prompt, our approach asks ChatGPT to provide another answer based on the inconsistencies in its original explanation. Finally, we obtain the repaired broken statement from ChatGPT. Due to the randomness of ChatGPT, we rerun the matching and repair process four times, and check if at least one correct repair occurs among the four runs, following the prior study~\cite{sobania2023analysis}. 
% After self-correction, we use explanation validator to check the answer again, and select the improved results as matching results. Finally, based on the matches, ChatGPT proceeds to repair the broken statement according to the repair prompt and outputs repaired statement. Due to the randomness of ChatGPT, we rerun the matching and repair four times, and use the best results across the four runs, following the procedure in prior study~\cite{sobania2023analysis}.

%Moreover, we instruct ChatGPT to provide explanations for its matching results. After ChatGPT generates the initial explanation, we use our explanation validator to check for the explanation consistency. If the explanation consistency is less than or equal to 0.5, we prompt ChatGPT for self-correction. In this process, it selects the matched element and reiterates the explanation. If the selection differs from the previous one, ChatGPT is instructed to perform another repair.

% Figure~\ref{workflow} shows the overall workflow of 




\subsection{Prompt Design of Repair and Self-Correction Prompt}
We interact with ChatGPT via the API of the gpt-3.5-turbo model~\cite{gpt3}. %~\footnote{https://platform.openai.com/docs/api-reference}. 
For optimal results, we design our prompt based on the official OpenAI documentations, including: (1) the official ChatGPT API Guide~\cite{rule_role}
% , (2) OpenAI GPT best practices, 
and 
(2) OpenAI six strategies for achieving better results~\cite{rules}. Table~\ref{table:prompt} shows for each sentence of the prompt (the ``Prompt Content'' column), the corresponding rule (the ``Rule in OpenAI official documentation'' column) that inspires the design. The ChatGPT API Guide emphasizes the importance of system instructions in providing high-level guidance for conversations so we use system instructions to design the Web UI test repair context part by telling ChatGPT that (1) it is a web UI test repair tool, and (2) outlining the steps for fixing a broken statement.%\todo{the following are duplicated in the table. remove all duplication and only have one example rules, add all other citations to the table}

% According to the ``Split complex tasks into simpler subtasks'' best practice~\cite{split_tasks}, we divide the test repair task into two subtasks: (1) matching and (2) repair. 
% % \todo{what does it mean by in content with id=2?}
% in content with \yz{PID}=2. For the matching task, since ChatGPT requires element information to repair a broken UI test statement, we then instruct ChatGPT to match the suitable element for repair according to the given candidate element lists.

% Based on the ``Include details in your query to get more relevant answers'' tactic~\cite{rules},
% we also provide a specific instance of the desired output format by asking ChatGPT to give a short explanation for each of its selection. 
%This enables ChatGPT to emulate the example in generating responses, particularly beneficial for analysing the output, which is adheres to the ``Provide examples'' strategy.

% \todo{check if this is really the third content} 
% p4?
Due to token limits, we summarize ChatGPT's matched elements' information from previous dialogues to guide subsequent repair, aligning with the tactic ``For dialogue applications that require very long conversations, summarize or filter previous dialogue.''~\cite{rules}.
% In the content of id=4, we outline explicit steps for the repair task: firstly, ChatGPT is prompted to select the matching element—a step already accomplished when utilizing this part of content. Following this, we provide the element information based on its matching result. Subsequently, we instruct ChatGPT to use the selected element's information for repairing the broken statement. We also strengthen that ChatGPT should only focus on locators and outdated assertions when repairing statement to prevent ChatGPT from changing original test intent of test statements.
Following the rule ``Use delimiters to clearly indicate distinct parts of the input''~\cite{rules}, we use colons to separate labels from respective contents, and curly braces to separate the information of each element, helping ChatGPT distinguish the input. %in the input part.
% This aids ChatGPT in recognizing the information content of elements and the broken statement. 
Table~\ref{table:prompt} shows our prompt patterns and the applied rules.
The complete prompt generation rules are:
\begin{description}[leftmargin=*]
  \item \textbf{Matching Prompt:} Context{[}p1, p2, p3{]} + Input{[}p8{]}
  \item \textbf{Repair Prompt:} Context{[}p1, p4, p5{]} + Input{[}p9{]}
  \item \textbf{Self-Correction Prompt:} Context{[}p6,  p7{]}
\end{description}


%Note that ``Target element'' refer to the old element on the old Webpage. ``Candidate elements'' are potential matching elements on the new Webpage.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%\setlength{\tabcolsep}{3pt} % Default value: 6pt
\begin{table*}[h]
\centering
\caption{The patterns of prompt and generation rules}
\label{table:prompt}
\resizebox{0.9\linewidth}{!}{%
\begin{threeparttable}
\centering

\begin{tabular}{lp{2.4cm}p{9.1cm}}
\hline
\multicolumn{1}{l|}{\textbf{PID}} &
  \multicolumn{1}{l|}{\textbf{Rule in OpenAI's official documentation}} &
  \textbf{Prompt Content} \\ \hline
\multicolumn{3}{c}{\textbf{Web UI test repair context patterns: Context}} \\ \hline
\multicolumn{1}{l|}{p1} &
  \multicolumn{1}{l|}{Use system instruction to give high level instructions~\cite{rule_role}} &
  You are a web UI test script repair tool. \\ \hline
\multicolumn{1}{l|}{p2} &
  \multicolumn{1}{l|}{Split complex tasks into simpler subtasks~\cite{split_tasks}} &
  To repair the broken statement, you need to choose the element most similar to the target element from the given candidate element list.\\ %firstly. \\
\multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  Give me your selected element's numericId and a brief explanation containing the attributes that are most similar to the target element. \\ \hline
\multicolumn{1}{l|}{p3} &
  \multicolumn{1}{l|}{Provide examples~\cite{rules}} &
  Your answer should follow the format of this example: \\
\multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  ‘‘The most similar element's numericId: 1. Because they share the most similar attributes: id, xpath, text.’’ \\ \hline
\multicolumn{1}{l|}{p4} &
  \multicolumn{1}{l|}{Summarize or filter previous dialogue~\cite{rules}} &
  To repair the broken statement, you chose the element \textit{selected element} as the most similar to the target element from the given candidate element list. \\ \hline
\multicolumn{1}{l|}{p5} &
  \multicolumn{1}{l|}{Specify the steps required to complete a task~\cite{rules}} &
  Now based on your selected element, update the locator and outdated assertion of the broken statement. Give the result of repaired statement. \\ \hline
\multicolumn{1}{l|}{p6} &
  \multicolumn{1}{l|}{Use delimiters to clearly indicate distinct parts} &
  This is a previous prompt: \textit{Matching Prompt} \\
\multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{of the input~\cite{rules}} &
  This is your previous answer: \textit{Corresponding Answer} \\ \hline
\multicolumn{1}{l|}{p7} &
  \multicolumn{1}{l|}{} &
  But your explanation for attributes \textit{attributes} are inconsistent with your selection and this will influence the correctness of your answer. Please answer again. \\ \hline
\multicolumn{3}{c}{\textbf{Input pattern: Input}} \\ \hline
\multicolumn{1}{l|}{p8} &
  \multicolumn{1}{l|}{Use delimiters to clearly indicate distinct parts} &
  Target element: \{\textit{target element}\} \\
\multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{of the input~\cite{rules}} &
  Candidate elements: \{\textit{candidate element 1}\}, \{\textit{candidate element 2}\} ... \\ \hline
\multicolumn{1}{l|}{p9} &
  \multicolumn{1}{l|}{} &
  Broken statement: \textit{broken statement} \\ \hline
% \multicolumn{3}{c}{\textbf{Prompt generation rules}}
\end{tabular}%
% }
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{table*}[h]
% \resizebox{\textwidth}{!}{%
% \begin{threeparttable}
% \centering
% \caption{The patterns of prompt and generation rules\shinhwei{TODO: add citation for each rule}}
% \label{table:prompt}
% %
% \begin{tabular}{lll}
% \hline
% \multicolumn{1}{l|}{PID} &
%   \multicolumn{1}{l|}{Rule in OpenAI's official documentation} &
%  Prompt Content \\ \hline
% \multicolumn{3}{c}{Web UI test repair context patterns: Context} \\ \hline
% \multicolumn{1}{l|}{p1} &
%   \multicolumn{1}{l|}{Use system instruction to give high level instructions} &
%   You are a web UI test script repair tool. \\ \hline
% \multicolumn{1}{l|}{p2} &
%   \multicolumn{1}{l|}{Split complex tasks into simpler subtasks~\cite{split_tasks}} &
%   To repair the broken statement, you need to choose the element most similar to the target element from the given candidate element list firstly. \\
% \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   Give me your selected element's numericId and \textbf{a brief explanation containing the attributes that are most similar to the target element}.\\
% \multicolumn{1}{l|}{p3} &
%   \multicolumn{1}{l|}{Provide examples} &
%   Your answer should follow the format of this example: \\
% \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   ‘‘The most similar element's numericId: 1. \textbf{Because they share the most similar attributes: id, xpath, text.}’’\\ \hline
% \multicolumn{1}{l|}{p4} &
%   \multicolumn{1}{l|}{Summarize or filter previous dialogue} &
%   To repair the broken statement, you chose the element \textless{}selected element\textgreater as the most similar to the target element from the given candidate element list. \\ \hline
% \multicolumn{1}{l|}{p5} &
%   \multicolumn{1}{l|}{Specify the steps required to complete a task} &
%   Now based on your selected element, update the locator and outdated assertion of the broken statement. Give the result of repaired statement.\\ \hline
% \multicolumn{1}{l|}{p6} &
%   \multicolumn{1}{l|}{} &
%   This is a previous prompt: <Matching Prompt>\\
% \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   But your explanation for attributes <attributes> are inconsistent with your selection and this will influence the correctness of your answer. Please answer again.\\ \hline
% \multicolumn{3}{c}{Input pattern: Input} \\ \hline
% \multicolumn{1}{l|}{p6} &
%   \multicolumn{1}{l|}{Use delimiters to clearly indicate distinct parts} &
%   Target element: \textless{}target element\textgreater{} \\
% \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{of the input} &
%   Candidate elements: \textless{}candidate element list\textgreater{} \\ \hline
% \multicolumn{1}{l|}{p7} &
%   \multicolumn{1}{l|}{} &
%   Broken statement: \textless{}broken statement\textgreater{} \\ \hline
% \multicolumn{1}{l|}{p8} &
%   \multicolumn{1}{l|}{} &
%   Previous prompt: \textless{}Matching Prompt\textgreater{} \\
% \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   Your previous answers: \textless{}answer for the prompt\textgreater{} \\ \hline
% %\multicolumn{3}{c}{Prompt generation rules} \\ \hline
% %\multicolumn{1}{l|}{Matching Prompt} &  Context{[}p1,p2{]} + Input{[}p5{]} &
%    % \\
% %\multicolumn{1}{l|}{Repair Prompt} &
% %  Context{[}p1,p3,p4{]} + Input{[}p6{]} &
%    % \\
% %\multicolumn{1}{l|}{Self-Correction Prompt} &
% %  Context{[}p3, p5{]} +  Input{[}p8{]} &
% %   \\ \hline
% \multicolumn{3}{c}{\textbf{Prompt generation rules}} \\

% \end{tabular}%


%}


% \begin{tablenotes}
%    %\textbf{Prompt generation rules}
% 	%\item[*] 
% % \item \textbf{Prompt generation rules}\\ \hline
%  \item \textbf{Matching Prompt:} Context{[}p1, p2, p3{]} + Input{[}p8{]}]
%   \item \textbf{Repair Prompt:} Context{[}p1, p4, p5{]} + Input{[}p9{]}
%     \item \textbf{Self-Correction Prompt:} Context{[}p6,  p7{]}%\shinhwei{the input seems to be incorrect, please recheck all the generation rules}\\
% %\multicolumn{1}{l|}{Matching Prompt} &  Context{[}p1,p2{]} + Input{[}p5{]} &  \\
% %\multicolumn{1}{l|}{Repair Prompt} &  Context{[}p1,p3,p4{]} + Input{[}p6{]} &  \\
%     %\multicolumn{1}{l|}{Self-Correction Prompt} & Context{[}p3, p5{]} +  Input{[}p8{]} &\\

% \end{tablenotes}
\end{threeparttable}}
\end{table*}



\subsection{Information Extraction and Attribute Prioritization}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% \todo{separate detailed info to another table. add how element information is selected}
% done

%In this section, we would introduce the detail of how we get and select the candidate elements' information.


% \todo{which tool used for extraction? We use ...to extract information. ... extract information about attributes .., and added the isLeaf.....}
% done

\begin{table*}[ht]
\caption{Extracted attributes and the tools that use them. The superscript number indicates the priority of an attribute.}%for the last column indicates the priority of an attribute for a tool.}
%\setlength{\tabcolsep}{1pt}
\centering
\renewcommand{\arraystretch}{1.0}
\vspace{-3pt}
\label{tab:attribute}
\footnotesize
%\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{|l|p{9.2cm}|l|}
\hline
Attribute & Description (Example for an element) & Used by Tools \\ \hline
id &  Unique identifier for an element (userName)   & $\watertool^{E1}$ ,$\uitestfix^{E1}$
\\ \hline
name &  Name for an element (submit)  &  $\watertool^{E5}$\\\hline 
 class& Class name for an element (button) &$\watertool^{E3}$
\\\hline 
XPath & Path of an element in the DOM tree %(/html[1]/body[1]/div[1]/div[4]/form[1]/input[1])
(/html[1]/body[1]/div[1]/form[1]/
input[1])
&  $\watertool^{E2,L7}$, $\edtool^{L1}$, $\uitestfix^{T2}$\\ \hline
text & Textual information of an element (Enter)  &   $\uitestfix^{L3}$
\\ \hline
tagName & Name of the HTML tag (input)   &  $\watertool^{E6}$, $\uitestfix^{T2}$
\\\hline\hline 
% href& The content of a hyperlink () & \\ \hline
linkText & The text content of a hyperlink (Logout)  &  $\watertool^{E4}$ 
\\ \hline
x & X-coordinate for an element (66) &  $\watertool^8$
\\ \hline
y & Y-coordinate for an element (183)  &  $\watertool^8$
\\ \hline
width & Width of an element (48)  &  $\vistatool^{P1}$, $\watertool^8$
\\ \hline
height & Height of an element (21)  &  $\vistatool^{P1}$, $\watertool^8$
\\ \hline
isLeaf & True if the element is a leaf node of the DOM tree, and false otherwise (true)  &  $\uitestfix^4$ \\ \hline
\end{tabular}
%}

\begin{tablenotes}

\footnotesize
\item{1} The superscript `E' means the tool checks
whether the candidate element’s attribute is exactly the same as
the target element.
\item{2} The superscript `L' indicates the tool uses Levenshtein Distance
to calculate the similarity.
\item{3} The superscript `T' means that the tool uses TF-IDF
to calculate the similarity.
\item{4} The superscript `P' means that the tool calculates the similarity of images, where the width and height of the images affect the calculation. 
%\item{4} The number in superscript indicates the priority of the attribute. 
% \item{5} We refer to the version of \webevotool, \sftmtool implemented in prior work~\cite{UITESTFIX} to determine the priority of attributes. %in them.
\item{5} We refer to the \textbf{VISUAL} mode of \vistatool{}~\cite{vista} for \vistatool{}'s priority, \textbf{DOM} mode of \vistatool{}~\cite{vista} for \watertool{}'s priority. %\sh{TODO:check if you want to put the paper version of vista or another version and make sure that it is consistent} 
\end{tablenotes}
\end{table*}

To extract Web element information, we use an existing component in
 UITESTFIX~\cite{UITESTFIX} to extract relevant information for each element. Specifically, it retrieves the HTML source code of the target Webpage via a Web browser, then uses \emph{Jsoup} library~\cite{jsoup} to extract the Web elements' information in it. 
Note that we did not evaluate UITESTFIX's performance with other tools due to the unavailability of its matching algorithm.
% in background section we have explained about this
%Specifically, w
We extract information from several attributes: \emph{id}, \emph{name}, \textit{class}, \emph{XPath}, \emph{text}, \emph{tagName}, \emph{linkText}, \emph{x}, \emph{y}, \emph{width}, \emph{height}, and \emph{isLeaf}.  

\noindent\textbf{Understanding attribute prioritization.} To gain a better understanding of the attribute prioritization used in prior techniques, we read the original paper and the implementation of each technique (if available).
Table~\ref{tab:attribute} shows the attributes and the priorities used by prior Web UI matching and repair approaches. The first two columns of Table ~\ref{tab:attribute} show the descriptions and examples of the attributes. The column ``Used by Tools'' shows if prior approaches 
 $\watertool$, $\vistatool$, $\edtool$, or $\uitestfix$ %$\webevotool$, or $\sftmtool$ 
consider these attributes when matching elements and how these tools use them. 
We observe from Table \ref{tab:attribute} that \emph{XPath} is the most commonly used attribute in all approaches. \vistatool{} uses the fewest DOM attributes because it focuses on the image template matching algorithm. Two attributes (ie, \emph{width} and \emph{height}) are used to represent the size of the element. Meanwhile, \watertool{} and \uitestfix{} exclude these two attributes. \watertool{} uses the greatest number of attributes, including \emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, \emph{name}, \emph{tagName}, \emph{x} and \emph{y}. \uitestfix also uses four other attributes, of which \emph{text} and \emph{isLeaf} are not used by \watertool. \emph{isLeaf} is used by \uitestfix toiteratively refining the similarity tthroughugh the DOM structure.

%The number means the priority of consideration. The letter ``E''/``L'' represents the matching algorithm used. 
% \emph{E} means the tool judges whether the candidate element's attribute is exactly the same as the target element. \emph{L} indicates the tool use Levenshtein Distance algorithm to consider the similarity.
% The \emph{id} is typically a unique identifier if it is defined for the element. The \emph{XPath} is the path to the element in the DOM tree, consisting of the element itself and each ancestor element's \emph{tagName} and their index among their siblings. The \emph{text} is the element's own textual information. The \emph{linkText} is the text information of the element's link if there is one. Sometimes the value of \emph{linkText} is equal to the value of \emph{href} attribute. The coordinate \emph{x}, \emph{y} represents the element's position on the entire screen. The \emph{isLeaf} indicates whether the element is a leaf node in the DOM tree. Among these attributes, \emph{id}, \emph{XPath}, \emph{linkText}, \emph{name}, \emph{tagName}, \emph{x}, and \emph{y} are also considered by WATER when matching elements.
% \todo{change the description of this paragraph, and add the calculation of location and size}
% done (describe in table note)
%As the implementation of water is not publicly available, we refer to the vista implementation of water for deriving this priority.\todo{remove?}
% Additionally, WATER also uses \emph{clickable}, \emph{visible}, \emph{zindex}, and \emph{hash} attributes of elements when calculating similarity. However, it gives less weight to the similarity of these attributes, and UITESTFIX does not extract the element information, so we do not add the values of these attributes to the element information provided to ChatGPT.
\subsection{Candidate Selection}

To address token limits, we provide ChatGPT with a list of 10 top-ranked candidate elements from the matching results of prior approaches (\watertool{},\vistatool{}, \edtool{}). We only chose 10 elements due to (1) the model's 4096-token limitation, and (2) the lengthy %the rich 
information of each element's 12 attributes. %and considering the length of elements' information, we decide to set the size as 10. We accomplished this by filtering out 10 potentially matching elements from the numerous extracted elements as candidates for ChatGPT's selection.
%As the gpt-3.5-turbo model that we use has a limitation of 4096 tokens, and considering the length of elements' information, we decide to set the size as 10. We accomplished this by filtering out 10 potentially matching elements from the numerous extracted elements as candidates for ChatGPT's selection.
%We use three bases for the pre-selection and compare their effectiveness. 
We briefly introduce the three approaches below:
%The first two approaches is to select the top 10 elements with the highest similarity using the similarity calculation of \vistatool{} and \watertool{}.
\begin{description}[leftmargin=*]
\item[\vistatool{}:] \vistatool{} uses Fast Normalized Cross Correlation algorithm~\cite{openCV} to calculate the template matching results, defining the position and size of the matching area by the element's \emph{x}, \emph{y}, \emph{width}, and \emph{height}. It returns a list where elements of a particular screen position are ranked in descending order based on their similarity scores. Instead of returning only the top 1 element in the original version of \vistatool, we modify \vistatool{} to retrieve the top 10 elements %based on the matching %point coordinates 
as candidates for further matching.
% The original version of \vistatool{} only identifies one matching element in the new version (i.e., the best match) so we modify it to produce more candidate elements.
%However, it can only give one top-ranked result instead of expected candidate number of results.Therefore
% Specifically, we use the best match and the nine elements with highest similarity scores as candidates from \vistatool{}.
\item[\watertool{}:]

% first finds whether there are candidate elements that have the same \emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, or \emph{name} to the target elements. If so,  \watertool{} add them into the candidate list. Then \watertool{} ranks the elements on the new Webpage according to their similarity score. 
% If there are candidates with same first scores, \watertool{} calculates the second score with \emph{tagName}, \emph{coordinates}, \emph{clickable}, \emph{visible}, \emph{zindex} (the screen stack order of the element), \emph{hash} (checksum of the textual information of the element).
As shown in Table~\ref{tab:attribute}, \watertool{} first checks if any candidate elements share the same \emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, or \emph{name} as the target elements. and returns the first match. If none are found, \watertool{} calculates similarity score for candidates with the same \emph{tagName} as the target element, and returns the first one exceeding the threshold. The score combines the Levenshtein distance of their \emph{XPath}, and the equivalence of their size and position based on \emph{x}, \emph{y}, \emph{width}, and \emph{height} with a small tolerance for variation.
% and the second part checks whether they share the same value of properties \emph{coordinates}, \emph{clickable}, \emph{visible}, \emph{zindex} (the screen stack order of the element), \emph{hash} (checksum of the textual information of the element). 
Notably, \watertool{} gives a greater weight (0.9) to the \emph{XPath} similarity because its authors assume that matched elements have similar \emph{XPaths} after the version update. We modify \watertool{} to return a de-duplicated list of 10 unique candidates instead of a single match.

% (we de-duplicate to ensure that all elements in the list are unique) to the candidate list 
% %with deduplication 
% until the size of the list reaches 10. %maintaining consistency with modifying other part.

\item[\edtool{}:] 
Inspired by the idea of prioritizing XPath similarity in \watertool{}, we design a simplified matching algorithm to only consider the XPath similarity. Similar to \watertool{}, we use Levenshtein distance~\cite{edit_distance} to measure the difference between \emph{XPaths}. Levenshtein distance %is an algorithm within the text edit distance category that 
measures the minimum number of insertions, deletions, and substitutions needed to transform one string into another.  
Greater distance means that the two elements are less similar. This algorithm has also been used in Web testing (e.g., detecting conflicting and outdated data on Webpages~\cite{levenshtein}). %For instance, prior work~\cite{levenshtein} have used the Levenshtein distance algorithm to detect conflicting and outdated data on Webpages. 
This variant returns the top 10 elements ranked in descending order based on their XPath similarities.
%We will refer to this candidates selection method as \edtool{} in the following. 
\end{description}
% \noindent\textbf{Iterative Matching Approaches:} As our idea is to enhance prior techniques with subsequent matching using ChatGPT, we also compare with two UI matching approaches that perform subsequent matching (i.e., WebEvo~\cite{shao2021webevo} and SFTM~\cite{sftm2023}). 







\subsection{Explanation Validator}
\label{sec:evalidate}
%As shown in the highlighted text in Table \ref{table:prompt}\todo{What is the highlighted text? please change the table or this sentence}, 
As shown in the ``Prompt Content'' column in Table~\ref{table:prompt},
we instruct ChatGPT to generate an explanation to describe the attributes used for selecting the best matched element. Our intuition is that \emph{if the provided explanation is consistent, then the selection is more likely to be correct} (and repair is more likely to be successfully generated with correct matches). Based on this intuition, we designed an explanation validator to check if ChatGPT's explanation is consistent with the actual selection. Specifically, for each attribute $a$ mentioned in the explanation, our explanation validator calculates the following to determine the most similar element for the consistency calculation $cons(a_i, R)$ where $cons(a_i, R)$=1 if the most similar element is selected:%The specific calculation logic is as follows:  \todo{this part can be changed to a itemize to make it clearer}

\begin{description}[leftmargin=*]
  \item[Screen position:] We use Euclidean distance to compute position-related attributes (e.g., x and y coordinates). We select the element with the minimum distance as the most similar.
  \item[Size:] We use the product of width and height, and consider the one with the smallest size difference as the most similar.
  \item[isLeaf:] We check if the \emph{isLeaf} values (true or false) are same. 
  \item[Other attributes:] We use Levenshtein edit distance %\todo{is this the Levenshtein edit distance? if yes, use same term as before} edit distance 
  to measure similarity, with lower values indicating higher similarity.
  % with the smallest distance considered as the most similar.
\end{description}

% Firstly, compute the similarity table\todo{what is similarity table? similarity score? similarity matrix?} by assessing the similarity between the attributes of each element in the candidates list and those of the target element for each match. Specifically,  we utilize\todo{refer to the blog about not using more syllabus than you should, and change "utilize"} Euclidean distance for location attributes (x and y coordinates), choosing the element with the minimum distance as the most similar. For size attribute, we calculate the product of width and height, and consider the element with the smallest size difference as the most similar. For other attributes, we use text edit distance to measure similarity, with the smallest edit distance considered as the most similar. 
In the cases where multiple candidate elements and the target element share the same similarity for a particular attribute, we will retain the results of multiple candidate elements and consider the explanation given by ChatGPT to be consistent if either one of these candidate elements has selected. %the results preserve multiple candidate elements.



\begin{definition}[Explanation Consistency (EC)]
\vspace{-5pt}
\label{def:ec}
Given the \emph{target element} $t$ (the element in the old version of the Webpage to be matched), the selection result $R$ and an explanation $e$ where $e$ mentioned one or more attributes $A=a_1,a_2,...,a_n$, we calculate the \emph{Explanation Consistency (EC)} of $e$ by computing 
% cons($a_i, R$) for each attribute $a_i$ where $cons(a_i, R)$ checks whether each attribute $a_i$ of $R$ is most similar to that of the target element $t$ ($cons(a_i, R)$=1 if the most similar element based on $a_$ is selected in $R$, and $cons(a_i, R)$=0
%  otherwise. 
 cons($a_i, R$) for each attribute $a_i$ where $cons(a_i, R)$ checks whether each attribute $a_i$ of $R$ is most similar to that of the target element $t$ ($cons(a_i, R)$=1 if the most similar element based on $a\_{i}$ is selected in $R$, and $cons(a_i, R)$=0 otherwise).

% where cons($a_i, R$) checks whether $R$ selects the most similar element based on the attribute $a_i$ ($cons(a_i, R)$=1 if the most similar element based on $a_$ is selected in $R$, and $cons(a_i, R)$=0 
%  otherwise). 


\[
\small
EC(e)=\frac{\sum_{i=1}^{n} cons(a_i\in A, R)}{|A|}
\]
%\vspace{-6pt}
\end{definition}

Def. ~\ref{def:ec} presents the definition for Explanation Consistency (EC). 
For each explanation generated by ChatGPT, our explanation validator checks whether the attributes mentioned in the explanation that are similar between the selected element and the target element are consistent with the calculated values of all mentioned attributes. If the calculated values for all mentioned attributes are consistent, then our explanation validator considers the provided explanation as \emph{consistent} across all mentioned attributes ($EC$=1).


% We developed an automated script to determine whether $a$ is consistent with the actual circumstances. The specific logic is as follows: the script calculates the similarity of each attribute of each element in the Candidates List to the corresponding attribute of the target element. Specifically, the script considers the distance between two points in terms of x and y coordinates as the minimum for the location attribute to be most similar. Similarly, for the size attribute, the script calculates the size based on width and height. For all other attributes, the attributes which have the minimum edit distance is considered the most similar. Subsequently, the script obtains a list of elements that are most similar to the target element on each attribute and checks if the element selected by XXX is included in this list. If it is, then it is considered that the explanation about attribute $a$ is consistent with the actual circumstances. We assessed the accuracy of this automated script through manual sampling. For each of the three Candidates Lists, we randomly selected 15 broken statements out of the total 139, manually verifying whether the automated script made any errors. According to the statistics, among the 45 sampled broken statements, only one exhibited a script misjudgment in one attribute. Specifically, it incorrectly identified the text attribute as "[ \^ ]" being most similar to "My Account." The rest of the evaluations were error-free, reliably reflecting whether \$a\$ is consistent with the actual circumstances. 
%我们开发了一个自动判断脚本来判断whether $a$ is consistent with the actual circumstances。具体逻辑如下：这个脚本计算Candidates List中每个元素的各个属性与目标元素对应属性的相似程度，具体来说，两个元素的x和y计算出location的两点间距离最小即最相似，通过width和height计算出的size最像则最相似，而其他所有属性都是编辑距离最小即最相似。然后，脚本得出在各个属性上与目标元素最像的元素列表，并判断XXX选择的元素是否包含在这个列表中，如果在，则视为 the explanation about attribute $a$ is consistent with the actual circumstances。我们对这种通过脚本自动判断的方法的准确率进行了人工抽样检测，对基于三种Candidates Lists各自的139条broken statement各自随机抽取15条，来人工检查这种自动脚本判断是否有错。经统计，在抽取的45条broken statement中，只有1条的1个attribute发生了脚本判断错误，将text这一属性为"[ ^ ]"的与"My Account"判断为最相似，其余都没有问题，能可靠地反映whether $a$ is consistent with the actual circumstances。




% \subsection{Selecting Candidates with Algorithm of WATER and VISTA}
%  % The prerequisite for ChatGPT to pick the correct element from a candidate list is that the list contains the correct element. Therefore, we try to improve the algorithm of sorting candidate elements to achieve the prerequisite better before we start.
 
% % As we wanted to investigate how existing technologies could be combined with ChatGPT to achieve better results, we tried to 

% In the second candidate selection approach, we use both the algorithms of WATER and VISTA to calculate the similarity between the elements on the new page and the target elements\yuanzhang{s?} on the old page, and then 
% % filter
% use the top 10 most similar elements as candidates.

% We selected the five most similar elements selected by WATER and VISTA individually as the results.
% If there are duplicate elements, we would remove the duplication and select the next most similar element or elements, keeping the final candidate list at 10. \yuanzhang{Make sure this sentence is correct}
% We will refer to this candidates selection method as WATER+VISTA in the following.

% In the complete\yuanzhang{original?} similarity algorithm of WATER, it uses \emph{id}, \emph{XPath}, \emph{class}, \emph{linkText}, and \emph{name} to calculate the first score. 
% If there are candidates with same first scores, WATER calculate the second score with \emph{tagName}, \emph{coordinates}, \emph{clickable}, \emph{visible}, \emph{zindex} (the screen stack order of the element), \emph{hash} (checksum of the textual information of the element).
% \yuanzhang{So shouldn’t you introduce what you changed here?}

% VISTA originally uses SIFT\yuanzhang{cite?} and FAST\yuanzhang{cite?} algorithms and to get the similarity scores to judge whether there is a matched element on the new Webpage. 
% If so, VISTA use Fast Normalized Cross Correlation algorithm\yuanzhang{cite?} to calculate the final result.
% The final best matched result\yuanzhang{There is no explanation for best matched.} is independent from the similarity scores calculated before.
% However, it can only give one result instead of expected candidate number of results.
% Therefore, we use the best match and the four elements\yuanzhang{There seems to be no explanation as to why there are 4. Is it because there are 5 for water and 5 for vista?} with highest similarity scores as candidates from VISTA.


% \subsection{Analysis of the Candidates Selection Methods}

% The prerequisite for ChatGPT to select the matched element correctly is that the given candidate lists contain ground truth elements. Therefore, we analyzed whether each candidate list contain the ground truth. If the ground truth is included in the candidate list, we record its ranking and make statistics.

% \todo{add rank table and analysis}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table}[h]
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  Candidates Selection &
%   \multicolumn{1}{l}{Top 1} &
%   \multicolumn{1}{l}{Top 3} &
%   \multicolumn{1}{l}{Top 5} &
%   \multicolumn{1}{l}{Top 7} &
%   \multicolumn{1}{l}{Top 9} &
%   \multicolumn{1}{l}{Total} \\ \midrule
% Edit Distance &
%   38 &
%   53 &
%   71 &
%   72 &
%   89 &
%   99 \\
% WATER+VISTA &
%   46 &
%   50 &
%   52 &
%   98 &
%   98 &
%   98 \\ \bottomrule
% \end{tabular}%
% }
% \caption{The statistics of ground truth elements' rankings in two candidates selection methods }
%     \label{gt}
% \end{table}

% Table \ref{gt} shows the statistics of ground truth elements' rankings in two candidates selection methods. The first column indicates the candidates selection methods. \textbf{Top n} means how many ground truth elements are contained in the first \textbf{n} elements of the candidate list. Notice that the first 5 elements are selected by WATER and the first element in the list is considered the most similar one by WATER. Accordingly, the sixth element is the most similar one judged by VISTA (after removing the duplicate elements). Therefore, WATER+VISTA selects more ground truth elements within the top 1 and top 7 meaning that VISTA and WATER excel in selecting ground truth elements as the most similar ones. However, when we consider within the top 10 (Total), XPath Edit Distance includes more ground truth elements. The two selection methods are likely to perform better with a larger candidate list size, but due to the limitation of the input length of ChatGPT, we set the candidate list size as 10.














% \label{sec:method}
% % In this section, we present our matching method, which includes four steps: preprocessing, initializing the similarity and interactively optimizing the match results.

% Figure \ref{fig:method-overview} shows the overall workflow of \toolName. 
% \toolName{} contains several components: \cluster, similarity metrics, iterative matching\delete{,} and dynamic repair. 
% When the element cannot be found by the original locator causing a crash, \toolName takes the current Webpage and the corresponding Webpage in the old version as input, and then obtains the patch via \cluster, calculating similarity\delete{,} and iterative matching.
% After replacing the broken locator with the correct one, the test can continue its execution where subsequently broken locators are fixed until the end of execution.

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.48\textwidth]{images/method-overview.pdf}
% \caption{The workflow of \toolName.}
% \label{fig:method-overview}
% \end{figure}

% \subsection{\clusterb}

% \label{sec:preprocess}
% % In fact, the number of elements on the page exceeds the number of actual functions on the Webpage, which increases the complexity of DOM structure.
% % And the invalid elements, which does not display, affect the matching process of valid elements.

% % There are 12 elements in total, but there are actually only three functional modules: (1) the entire module, (2) the ``Home'' text module, and (3) the ``House'' icon module.
% % Duplicate elements and invalid elements cause the number of page elements to exceed the actual functional modules, which not only increase the matching duration but also affect the matching result.



% To automatically fix broken UI test cases, the first step is to match the elements from old and new versions.
% However, if we use the original DOM as input directly, the following problems will arise:
% (1) the number of elements on Webpages is usually quite high, which increases the complexity of element matching;
% (2) there are a lot of invisible elements, which may also affect the matching accuracy of visible elements;
% % \yz{(2) complex implementation structures can make the structure more prone to changes,
% (3) unable to distinguish which elements represent regions and which elements represent functionality (e.g., button).

% \begin{figure}[t!]
% \centering

% \begin{subfigure}[t]{0.45\textwidth}
% \small
% \begin{lstlisting}
% (*@\color{blue}{1.}@*)<ytd-guide-entry-renderer class="..." active="">
% (*@\color{blue}{2.}@*)  <a id="endpoint" class="yt-simple-endpoint">
% (*@\color{blue}{3.}@*)    <tp-yt-paper-item class="style-scope">
% (*@\color{blue}{4.}@*)      <yt-icon class="guide-icon">
% (*@\color{blue}{5.}@*)        <svg viewBox="0 0 24 24">
% (*@\color{blue}{6.}@*)          <g class="style-scope yt-icon">
% (*@\color{blue}{7.}@*)            <path d="M4,3Z"></path></g></svg>
%         </yt-icon>
% (*@\color{blue}{8.}@*)      <yt-formated-string>Home</yt-formated-string>
% (*@\color{blue}{9.}@*)      <yt-img-shadow hidden=""></yt-img-shadow>
% (*@\color{blue}{10.}@*)     <yt-icon class="guide-entry-badge"></yt-icon>
% (*@\color{blue}{11.}@*)     <span class="guide-entry-count"></span>
% (*@\color{blue}{12.}@*)     <div id="newness-dot"></div></a> </ytd-...>
% \end{lstlisting}
% \caption{A simplified HTML code of Youtube's Home button}
% \label{fig:youtube_html}
% \end{subfigure}
% \begin{subfigure}[t]{0.48\textwidth}
% % \vspace{3pt}

% \centering
%       \includegraphics[width=0.8\textwidth]{images/element_merge_example.pdf}
%   \caption{A gourping process for the YouTube's Home button\add{.}}
%   \label{fig:element_merge_example}
% \end{subfigure}
%   \caption{DOM Structure of YouTube's Home Buttons in 2023\add{.}}
%   \vspace{-3pt}
% \end{figure}

% For instance, Figure \ref{fig:element_merge_example} shows the DOM structure of YouTube's home button in 2023 and its simplified HTML code (Figure~\ref{fig:youtube_html}).
% This simple button contains 12 elements as labeled in Figure~\ref{fig:youtube_html}.
% By deeply analyzing this HTML code snippet and its DOM structure, we observed this button is composed of three main components (1) button \delete{frame }\add{region} (elements 1--3), (2) button icon (elements 4--7), and (3) button text (element 8).
% From the user's viewpoint, elements 9--12 are not visible, e.g., the size of element 10 is 0, and the test case could not execute the event in these elements.
% However, the invisible elements and duplicated elements cause the number of elements on the HTML page to exceed the actual number of visible components, which affects the matching results.
% %increases the matching complexity and affect the matching result.
% %or duplicated elements
% To solve this problem, we filter invisible and merge duplicated elements into a group using the steps below:
% %The \cluster{} is described as follows:
% \begin{description}[leftmargin=*]
%     \item[1) Filter invisible elements:] If an element has (1) width or height less than 5 (too small to be visible) or (2) \texttt{isDisplayed=false}.
%     \item[2) Merge elements:] If an element has only one visible child element, the child element will be merged into its parent element. 
%     \item[3) Merge properties:] After merging, the parent element will have all properties of the merged child element. If the parent element has neither id nor text, it will use the id/text of the child element.
% %     \item Rebuild a new tree using the remaining elements.
%     \end{description}
% % \yz{To improve calculate the text similarity, if an element has no text but has a value attribute, we will set its text to value attribute.}
% %Moreover, when an element does not have any text attribute, we use its value attribute (\texttt{value=``text''}) to represent its text. %attribute.
% %Moreover, we treat the text and the value attribute (\texttt{value=``text''}) of an element as interchangeable.
% After \cluster{}, we rebuild a new tree using the remaining elements.
% In \add{F}igure \ref{fig:element_merge_example},  element\add{s} 1, 4, and 8 \add{are} eventually saved, where element\add{s} 4 and 8 are saved as children of element 1.





% %The node type in rebuilt tree is set as one of the following type: $\mathtt{T_{NL}}$, $\mathtt{T_{LT}}$, and $\mathtt{T_{LWT}}$, where type $\mathtt{T_{NL}}$ represents non-leaf node, $\mathtt{T_{LT}}$ is the leaf node with text, while $\mathtt{T_{LWT}}$ represents left node without text.

% % Set the DOM node type.
% %     There are three types of non-leaf type, image type, and text type.
% %     Non-leaf type: non-leaf node.
% %     Text type: Leaf node element with text.
% %     Image type: Leaf node element without text.


% % \subsection{PreMatching\todo{merge section}}

% \subsection{Similarity Metrics}

% In this subsection, we define the similarity metrics used to compute the similarity between the old and new elements.
% % Based on our research, the id attribute is less likely to change.

% Given two DOM trees $\mathcal{T}_o$ and $\mathcal{T}_n$, representing the old and new versions of Webpages, we denote the element list of $\mathcal{T}_o$ as $\mathcal{E}_o$=\{$e_o^1, e_o^2, \dots$\}, and element list of $\mathcal{T}_n$ as $\mathcal{E}_n$ = \{$e_n^1, e_n^2, \dots$\}.
% The attribute of a node $e$ is denoted as $e.\mathtt{id}$, $e.\mathtt{class}$, $e.\mathtt{text}$, etc.
% % For a certain element $e$, the region of $e$ is defined as its ancestor nodes, i.e., taking $e$'s ancestor nodes as the region where it is located.
% If $e_o^i$ and $e_n^j$ is determined as match, $e_o^i \mapsto{} e_n^j$ will be saved to matching list $\mathcal{M}$.


% \vspace{5pt}
% \noindent\textbf{1) Id similarity.} The most straightforward similarity metric is the exact matching of $n.\mathtt{id}$.
% Since the id attribute of elements is usually unique in Webpages, we define elements $e_o^i$ and $e_n^j$ match if (1) $e_o^i.\mathtt{id}$ is exactly the same as $e_n^j.\mathtt{id}$, and (2) $e_o^i.\mathtt{id}$ is a unique id among $\mathcal{E}^o$, and $e_n^j.\mathtt{id}$ is a unique id among $\mathcal{E}^n$.
% %\yz{and $n_o^i \mapsto{} n_n^j$ will not change in the iteration phase}.

% % \todo{define sure match?} The matching result is stored in sure match, which will not change during subsequent iterations. \todo{not convincing. id still changes according to Figure 1. May be changed to cite paper?}

% %Based on our study, we found that elements are rarely transformed between container type and leaf node type. \todo{not convincing. which RQ shows this?}
% % But in fact, separating the container elements and leaf-node elements also caused some errors.
% % To reduce the number of comparisons, we separate the calculation of non-leaf node elements and leaf node elements. \todo{efficiency? find a reason?}
% % Therefore, two similarity matrices are constructed, namely the non-leaf node similarity metrics and the leaf node similarity metrics.

% Besides id similarity, we also used two existing similarity metrics:
% % is constructed according to the similarity between elements. 
% % \begin{itemize}[leftmargin=*]
%     % \item [
    
%     \noindent\textbf{2)} \textbf{Property similarity ($S_{prop}$).}
%     TF-IDF (Term Frequency–Inverse Document Frequency) is a widely used text similarity metric~\cite {sparck1972statistical}.
%     As some words in properties appear in many elements, these repeated words will not be able to distinguish elements (e.g., \texttt{div}).
%     Therefore, TF-IDF can effectively use words with important meanings to calculate similarity.
%     Compared to SFTM~\cite{brisset2020sftm}, which uses IDF, we use TF-IDF to incorporate the term frequency (TF). 
%     Using TF to normalize the final similarity helps to combine the property similarity with other similarities, and avoiding that the property similarity \delete{is}\add{being} large enough to cover other similarities.
%     % \yuanzhang{reason.}
%     %to avoid that the value of property similarity being too high and the values of text similarity and structural similarity are masked.
%     % This idea has been used in SFTM, but it just uses IDF.\xiang{I do not understand this}
%     Moreover, SFTM~\cite{brisset2020sftm} considers XPath, tag, and attribute as properties.
%     According to our observation, text is more stable than XPath during page evolution.
%     Hence, we use text, tag, and attribute to calculate $S_{prop}$ (i.e., we replace XPath with text). %. instead of XPath as a token.
    
%     \noindent\textbf{3)} \textbf{Text similarity ($S_{text}$).}
%     To calculate the similarity of text properties, we use Levenshtein distance~\cite{levenshteinEditDistance}, which perform\add{s} well in existing tool \webevotool~\cite{shao2021webevo} when texts have small changes. %\yz{Note that the design of SFTM did not consider text properties to allow it to match pages in different languages~\cite{brisset2020sftm}.}
%     If the texts of elements are empty, text similarity will be left as 0. 
%     Otherwise, the text similarity is calculated as \add{follows}:
%     \begin{equation*}
%     \label{equ:text-similarity}
%     \begin{aligned}
%    % \vspace{-0.5cm}
%           S_{text}(e_o^i, e_n^j) = edit\_distance(e_o^i.text, e_n^j.text)
%     \end{aligned}
%     % \vspace{-0.5cm}
%     \end{equation*}
% % \end{itemize}
% % Given two nodes $n_o^i$ and $n_n^j$, $n_o^i \mapsto{} n_n^j$ will be saved to matching list $\mathcal{M}$ if their attribute similarity or text similarity is greater than a threshold.
% % They will be used as a reference for the similarity in the iteration phase and will not change in the iteration phase.


% Apart from the above three metrics, we propose two new metrics: \textit{region similarity} and \textit{path similarity}.
% These two metrics allow us to better utilize structural information for matching elements. %are defined with the goal of stably using structural information to help match elements.
% % We expect to use the following insights.



% \noindent\textbf{4) Path similarity.} 
% Based on the first \delete{insight} \add{idea} \textbf{I1}, if two elements exist in the same region, they should have a higher similarity.

% All ancestor nodes of $n$ form a path from the root node to $n$.
% Given two nodes $n_o^i$ and $n_n^j$, the closer the common ancestor in the path they have, the higher similarity they share.
% This is because a closer common ancestor indicates they are located in the same smaller region.
% The common ancestor of the two elements is determined according to the current matching results stored in $\mathcal{M}$.
% Note that the path similarity changes along with the change of $\mathcal{M}$ in the iteration phases, which will be explained in Section~\ref{sec:iterative_optimization}.

% % Considering that the ancestor nodes of a element are non-leaf node, which can be considered as the area where the element is located.
% % And all ancestor nodes are on the path from the root node to the current node.
% % So the deeper the common ancestor of the two elements, the higher the similarity.
% % We use the elements that have been matched to determine the common ancestor of the two elements.
% % So we propose \emph{path similarity $S_p$}, which uses the length from the root node to the deepest matching element as the similarity and normalizes with the total path length.
% % The path similarity calculation method is defined as the formula \ref{equ:path-similarity}.

% Formally, given two elements $e_o^i$ and $e_n^j$, their \emph{path similarity $S_p$} is defined as the length from the root node element to the deepest matching element, normalized with the total path length.
% Formally,
% \begin{equation*}
% \label{equ:path-similarity}
% \begin{aligned}
%       S_p(e_o^i, e_n^j, \mathcal{M}) 
%     = min(\frac{path(M_d(e_o^i))}{path(e_o^i)-1},\frac{path(M_d(e_n^j))}{path(e_n^j)-1})  
% \end{aligned}
% \end{equation*}
% where $path(e)$ is the length of the path from the root node element to $e$, and $M_d(e_o^i) \mapsto M_d(e_n^j) \in \mathcal{M}$ is the deepest matched element in the paths of $e_o^i$ and $e_n^j$, respectively.

% % \xiang{The path similarity changes along with the current matching results in the iteration phases.}\yz{Yes, that's why the matching results are optimized during iterations.}

% \vspace{5pt}
% \noindent\textbf{5) Region similarity.}
% For non-leaf node elements, we can use the second \delete{insight} \add{idea} \textbf{I2} to improve its correct matching rate.
% % Since the non-leaf node can be consider as a region and the meaning of the non-leaf node is defined by the leaf node elements in this region, such as buttons on the navigation bar.
% The non-leaf node element can be considered as a region, and the similarity of two regions can be measured by the similarity of elements located in those two regions.
% %Actually, this is bottom-up measurement.
% Hence, we propose region similarity $S_r$, which calculates the similarity of regions (non-leaf node elements) using the matching result of leaf node elements in two regions, normalized by the total number of leaf node elements.
% Given two non-leaf node elements $e_o^i$ and $e_n^j$, their region similarity is defined as:
% \begin{equation*}
% \label{equ:region-similarity}
%     % S_r(e_o^i, e_n^j) = \frac{C(e_o^i) \cap C(e_n^j)}{max(C(e_o^i), C(e_n^j))}
%     S_r(e_o^i, e_n^j, \mathcal{M}){=}\frac{|\{(e_1, e_2) | e_1 {\in} C(e_o^i){\wedge}e_2 {\in} C(e_n^j){\wedge}e_1 {\mapsto} e_2 {\in} \mathcal{M} \}|}{max(|C(e_o^i)|, |C(e_n^j)|)}
% \end{equation*}
% where $C(e)$ is the list of child {leaf} nodes of $e$.
% Similar to the path similarity, the region similarity also changes along with the change of $\mathcal{M}$ in the iteration phases.
% % where $E \cap E'$ is the matching leaf nodes in region $E$ and $E'$ and 
% % $max(E,E')$ is the maximum number of leaf nodes on the subtree of element $E$ and element $E'$.


% \subsection{Iterative Matching}
% \label{sec:iterative_optimization}
% % In \ref{sec:study-RQ1}, we study how web UI elements evolve.
% % Although after preprocessing, which can alleviate structural changes, the DOM structural may still change greatly.

% % \begin{algorithm}
% % 	\caption{Iterative optimization.}
% % 	\label{alg:iterative_optimization}
% %     \LinesNumbered 
% % 	\KwIn{$\mathcal{N}_o$, $\mathcal{N}_n$: node list of old and new Webpage \\
% % 	\ \ \ \ \ \ \ \ \ \ \ \ \ $t$: maximum number of iterations.}
% % 	\KwOut{$\mathcal{M}$: the matching results}
% %     update = true;\\
% %     \For{$i = 1$ to $t$}{
% % 		\If{ !update}{
% %   %\If{ notupdate}{
% % 		break
% % 			}

% %         \tcc{Update the similarities.}

% %     \For{ $e$ in $N-L$ }{
% %         \For{$e'$ in $N-L'$}{
% %             Similarity($e$,$e'$)=
% %             getInitSimilarity($e$,$e'$)+
% %             S\_r($e$,$e'$)+$\alpha \times$ $ S\_p$ ($c$,$c'$)
% %         }
% %     }
% %     \For{ $l$ in $L$ }{
% %         \For{$l'$ in $L'$}{
% %             Similarity($l$,$l'$)=
% %             getInitSmilarity($l$,$l'$)+$\beta \times$ $S_p$ ($l$,$l'$)
% %         }
% %     }
% %     \tcc{Update the matching result.}
% %   update=updateMatch()\\
% %     }
% % \end{algorithm}



% % The similarity calculation depends on the existing matching result and is used to obtain a new matching result.
% % Therefore, we use an iterative process to optimize the matching results.
% % In each iteration, the algorithm updates the similarity between non-leaf nodes and leaf nodes, and updates the matching result.
% \begin{algorithm}[!tb]
% \footnotesize
% 	\caption{Iterative matching.}
% 	\label{alg:iterative_optimization}
%     \LinesNumbered 
% 	\KwIn{${E}_o$, ${E}_n$: element lists of old and new Webpage \\
%  	\ \ \ \ \ \ \ \ \ \ \ \ \ $t$: maximum number of iterations.}
% 	\KwOut{$\mathcal{M}$: the matching results}
%     $\mathcal{M}$=\{\ \};\\
%     InitialS=$\mathtt{EmptyMap}$;\\
%     % $\mathcal{M}_t$=\{\ \};\\
%     \tcc{initial similarity.}
%     \For{ $e_1$ in ${E}_o$ }{\label{line:init_start}
%         \For{$e_2$ in ${E}_n$}{
%            \If{$e_1.\mathtt{id} == e_2.\mathtt{id}$}{ 
%                 $\mathcal{M} = \mathcal{M}\cup \{e_1 \mapsto e_2\}$;\\
%                 ${E}_o$ = ${E}_o-e_1$;\ \ \ ${E}_n$ = ${E}_n-e_2$;\\
%                 \textbf{break}
%             }
%             InitialS[($e_1$, $e_2$)] = $\alpha{*}S_\mathit{prop}$($e_1$, $e_2$){+} $S_\mathit{text}$($e_1$, $e_2$);\label{line:text}\\
%         }
%     }\label{line:init_end}
    
%     $\mathcal{M}_{w}$=$\mathcal{M}$;~\label{line:ite_start}\\
%     \tcc{iterative match.}
%     \For{$i = 1$ to $t$}{
%         $S$=$\mathtt{EmptyMatrix}$;\\
%        % $\mathcal{M}_t$= $\mathcal{M}_w $;\\
%        \tcc{Update similarity.}
%         \For{ $e_1$ in ${E}_o$ }{
%             \For{$e_2$ in ${E}_n$}{
%                 S[($e_1$, $e_2$)] {=} InitialS[($e_1$, $e_2$)]{+}$\beta{*}S_p(e_1, e_2, \mathcal{M}_w)$;\label{line:path}\\
%                 \If{$\mathit{IsNonLeaf}(e_1) \wedge \mathit{IsNonLeaf}(e_2)$}{\label{line:region_start}
%                     S[($e_1$, $e_2$)] += $\gamma*S_r(e_1, e_2, \mathcal{M}_w)$;
%                 } \label{line:region_end}
%                 % \If{ S[$n_1$, $n_2$] $\ge$ $\theta$ }{
%                 %     \yz{$E$ = $E$ $\cup$ \{ $n_1$,$n_2$,S[$n_1$, $n_2$]\}  }
%                 % }
%             }
%         }
        
%         % \yz{DescendingSimilaritySort($E$);}\\
%         % $E$  $\leftarrow$ \textit{getUniqTopNMatches}($S$, $\theta$);~\label{line:select}\\
%         % $\mathcal{M}_w = \{e_o \mapsto e_n\ |\ (e_o, e_n) \in E.keyset\} \cup \mathcal{M}$; ~\label{line:ite_end}\\
%         $\mathcal{M}_w  = \mathcal{M} $;\\
%         \tcc{Update match result.}
%         $E$ $\leftarrow$ $\{( e_i,e_j,S [( e_i,e_j )])\ |\ S[(e_i,e_j)] \geq \theta\};$~\label{line:select}~\label{line:top}\\
%         \For{$e \in E$}{
%             $\{ e_x \mapsto e_y\}$ = getMatchedPair($e$);\\
%             $\mathcal{M}_w  = \{e_x \mapsto e_y\} \cup \mathcal{M}_w $;~\label{line:save}\\
%         }
%         %\While{!E.isEmpty()}{
%         %    $\{ e_x \mapsto e_y\}$ = Top(E);\\
%         %    $\mathcal{M}_w  = \{e_x \mapsto e_y\} \cup \mathcal{M}_w $;~\label{line:save}\\
%         %    E $\leftarrow$ E $\cap \{ e_i \mapsto e_j \ |\ i \neq x, j \neq y \}$~\label{line:remove}; 
%         % \While{!E.isEmpty()}{
%         %     $\{ e_x \mapsto e_y\}$ = Top(E);\\
%         %     $\mathcal{M}_w  = \{e_x \mapsto e_y\} \cup \mathcal{M}_w $;~\label{line:save}\\
%         %     E $\leftarrow$ E $\cap \{ e_i \mapsto e_j \ |\ i \neq x, j \neq y \}$~\label{line:remove}; 
%         % }
%         %\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $\wedge (n_o, \_)\notin \mathcal{M}  \wedge (\_, n_n)\notin \mathcal{M}\}$;\\
%         % \While{\yz{IsNotEmpty($E$)}}{
%         % \For{($n_o, n_n$) $\in$ $E$}{    
%             % \yz{$E$ = $E - ( n_1, \forall)  -  ( \forall, n_2)$ ;}\\
%             % $\mathcal{M} = \mathcal{M} \cup \{n_o \mapsto n_n\}$;\\
%             % $\mathcal{N}_o$ = $\mathcal{N}_o-n_o$;\ \ \ $\mathcal{N}_n$ = $\mathcal{N}_n-n_n$;
%         % }
%     }~\label{line:ite_end}
%     \Return $\mathcal{M}_w$;
% \end{algorithm}

% Based on similarity metrics, we then present our iterative approach for optimizing the matching results.
% Algorithm \ref{alg:iterative_optimization} shows our iterative matching algorithm.
% The algorithm takes as inputs the element lists of the old and new version Webpages and outputs the matching result.
% Firstly, our tool initializes the similarity for each pair of elements according to id, attribute and text similarity (lines~\ref{line:init_start}-\ref{line:init_end}).
% Specifically, if the ids of two nodes are exactly the same, we are confident of adding them to \textit{sure} matching list $\mathcal{M}$, which will not be modified in the later stage.
% Otherwise, their initial similarity will be calculated based on attribute and text similarity (line~\ref{line:text}).

% %\yz{Iterative matching mainly consists of updating similarity and updating matching results. }
% \add{The} \delete{I}\add{i}terative matching algorithm mainly updates the similarity, and then update\add{s} the matching results iteractively.
% In $t$ iterations (lines~\ref{line:ite_start}-\ref{line:ite_end}), the similarity of each pair is continuously updated according to path similarity at line~\ref{line:path}.
% For non-leaf node elements, their similarity is also updated using region similarity (lines~\ref{line:region_start}-\ref{line:region_end}).
% As mentioned before, path and region similarity values are determined by current matching results (i.e., $\mathcal{M}_w$).
% In each iteration, after updating the similarities, all candidate matching pairs whose similarity is greater or equal to the threshold $\theta$ are selected and saved in $E$ at line~\ref{line:select}.
% % In each iteration, after updating the similarities, all candidate matching pairs whose similarity is greater than the threshold $\theta$ are selected using the function \textit{getUniqTopNMatches} at line~\ref{line:select}.
% We choose to only consider one-to-one matching and use a greedy method to match them.
% In each iteration, we select the matching pair $\{ e_x \mapsto e_y \}$ with the highest similarity from $E$ at line~\ref{line:top} and add it to the matching result $\mathcal{M}$ at line~\ref{line:save}.
% % Delete matching pairs which is related with $e_x$ and $e_y$ in $E$ at line~\ref{line:remove}.
% At the end of the loop, the matching results for this iteration are generated.
% % Moreover, \textit{getUniqTopNMatches} only choose one match with higher similarity for each node in $\mathcal{E}_o$ and $\mathcal{E}_n$ to avoid duplicated matches.
% % The candidate matches combined with sure match ($\mathcal{M}$) will be used to update similarity in the next iteration at line ~\ref{line:ite_end}.
% The iteration terminates when the number of iterations reaches limit $t$ or when the matching results will no longer change.


% % \todo{change the algorithm, currently the condition for converging is not clear (how many rounds of matching will be performed)}

% % The similarity of non-leaf nodes is updated (Lines 5--9) with the initial similarity, path similarity, and region similarity. 
% % And the similarity of leaf nodes is updated (Lines 10--14) with the initial similarity, path similarity.

% % Any one of the old version elements and the new version elements can be considered as a candidate matching pair.
% % In the update matching process (Line 16), all candidate matching pairs whose similarity is greater than the threshold $\theta$ are added to the candidate matching pair list.
% % These matching pairs are sorted by similarity.
% % Each time, the matching pair with the highest similarity is added to the mapping $M$, and the matched elements are deleted from the list of candidate matching pairs.
% % When the candidate matching pair list is empty, the update will be terminated.
% % After iterative optimization, mapping from old elements to new elements will be output as result. 

% Note that the initial outputs of the matching algorithm are matching between element groups (refer to Section~\ref{sec:preprocess}).
% % some actions can only be executed on elements with specific tags, such as input action can only executed on element with ``input'' tags.
% To get the real element matching, the concrete elements are selected from the group according to the following rules: (1) if there is an element in the group with the same tag as the old version element, then that element is selected, (2) otherwise, the outermost element is selected.


% \subsection{Dynamic repair}
% Based on the generated matching results between the old and new versions, \toolName then produces patches for fixing the broken UI tests. 
% Specifically, for each test, \toolName only works when UI actions are triggered.
% For each UI action performed on element $e_o$ that fails to be executed, \toolName will search for the matched element $e_n$ by querying the matching result.
% % and \yz{select element from the matched groups according to the following rules: (1) an element with the same tag as the original element, and (2) elements with other tags.}.
% If \toolName finds $e_o$'s matched \delete{node}\add{element} $e_n$, it will then executes the action on $e_n$.
% \delete{the element found by the repaired locator.}
% Otherwise, \toolName terminates the test execution because the element may have been deleted or not exist on this page anymore.
% The repaired test cases are then validated by executing it again on the new version of the Webpage.
% Finally, \toolName produces the repaired test cases.

% % When an old locator cannot locate the target element, \toolName uses the above method to match the elements on the old page and new page and obtains the mapping of matching result.
% % Because the mapping of matching result is actually a mapping between clusters, \toolName first looks for the old cluster to which the old locator belongs and finds the new cluster to which the old cluster matches.
% % If the mapping does not contain this old cluster, \toolName terminates the execution of the test case because the element may have been deleted or may not be on this page.
% % If the mapping contains this old cluster, \toolName will be relocate to an element in the matched cluster according at the tag of old element.
% % If the tag is \textit{input}, \textit{a} or \textit{button}, which are often related to ``input'', ``redirect'', and ``click'', \toolName will try to output an element with these tags preferentially.
% % Otherwise, the topmost element in the matched cluster will be outputted.

% % the innermost element in the matched new cluster if the old element with tags \textit{input}, \textit{a} or \textit{button}, which are often related to ``input'', ``redirect'', and ``click'', or the outermost element in the matched new cluster.

% % When \toolName catch an target exception thrown by an action, \toolName use the .
% % When the execution of the matched locator is successful, \toolName analyzes the call graph based on the crashed code line and uses JavaParser~\footnote{https://github.com/javaparser/javaparser} to find which element should be modified.
% % \toolName will generate the patch according to the elements definition mode, such as \textit{findElement}.
% % Screenshots of each events during execution are used to help test personnel determine the automatic repair result and modify test cases.
% % The tags \textit{input}, \textit{a}, \textit{button} are related to actions \textit{click} and \textit{input}.
% % When the tag of original element is one of these types, the element with the same tag in the matched cluster is returned.
% % Otherwise, the matched element is returned.
% % replaces the locator with the locator of matched element

==> sections/sections/motivation.tex <==
\section{Motivating Examples}

We show two examples where the combination of ChatGPT helps to improve the matching and test repair results.

\noindent\textbf{Without self-correction.}
% Table \ref{table:motivation_example} shows a target element to be matched by \watertool{} in the old version of MantisBT app, and the list of candidate elements returned by \watertool{}. Initially, \watertool{} incorrectly ranked ``Candidate 1'' as the top element as its priority largely ignores the ``text'' attribute (as shown in Table~\ref{tab:attribute}). %\todo{Reviewer comment: Give a more detailed description in the motivating examples section. Based on the description, WATER prioritizes five attributes (id, XPath, class, linkText, name) with a bias towards XPath. However, as shown in Table 1, Candidate 6 appears to have a higher similarity in these five attributes compared to the target element. So why wouldn't WATER select Candidate 6? Perhaps a more detailed explanation would make it easier for the reader to understand the inadequacies of WATER. Shin Hwei: I added the because ...Please check if text attribute is the only attribute that was the reason behind the ranking or there are other attributes?} 
% However, ChatGPT can correctly select ``Candidate 6'' as the matching result from this ranked list. ChatGPT also explains that it selects the element because ``they share the most similar attributes: xpath, text'' (its explanation consistency is equal to 1). After matching, our approach feeds ChatGPT with the repair prompt, and it successfully repairs the broken statement by updating the locator with XPath from ``Candidate 6''. In this example, as the explanation generated by ChatGPT is consistent, the further matching step by ChatGPT helps to select the lower ranked candidate, leading to the correct element being matched and subsequent correct repair being generated.
Table \ref{table:motivation_example} shows a target element to be matched by \watertool{} in the old version of the MRBS app, and key candidates from the returned list by \watertool{}. Initially, \watertool{} identifies elements with the same text as the target and returns the first match. However, in this case, two elements share the same value for the ``text'' attribute as the target element, and the second one has more similar XPath, position, and size to the target element than the first match, and 
ChatGPT correctly selected ``Candidate 2'' as the matching result from this ranked list. ChatGPT also explained that it chose this element ``Because they share the most similar attributes: xpath, text, tagName, x, y, width, height.'' (its explanation consistency is 0.8, because all attributes except for XPath are consistent with the selection, and the most similar XPath is ``/html[1]/body[1]'' from another candidate). After matching, our approach fed ChatGPT with the repair prompt, and it successfully repaired the broken statement by updating the locator with XPath from ``Candidate 2''. In this example, with ChatGPT's explanation being 80\% consistent, the subsequent matching step by ChatGPT helps select the correct but lower-ranked candidate, leading to successful repair.

% in  Figure~\ref{listing:repair}. The generated fix uses (1) a different locator (\texttt{By.xpath} instead of \texttt{By.name}), and (2) the XPath from ``Candidate 6'' for updating the broken statement.


% \begin{figure}[!th]
% \vspace{-6pt}

% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.name("category")).sendKeys("Category1");
% + driver.findElement(By.xpath("/html[1]/body[1]/div[3]/form[1]/table[1]/tbody[1]/tr[2]/td[2]/input[1]")).sendKeys
% + ("Category1");
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in MantisBT that replaces with different locators.}% (\texttt{By.xpath} instead of \texttt{By.name}).}
% \label{listing:repair}
% \vspace{-6pt}
% \end{figure}

% \begin{figure*}[!t]
% \vspace{-6pt}
% \centering
% \begin{minipage}{\textwidth}
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.name("category")).sendKeys("Category1");
% + driver.findElement(By.xpath("/html[1]/body[1]/div[3]/form[1]/table[1]/tbody[1]/tr[2]/td[2]/input[1]")).sendKeys
% + ("Category1");
% \end{lstlisting}
% \end{minipage}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in MantisBT that replaces with different locators.}% (\texttt{By.xpath} instead of \texttt{By.name}).}
% \label{listing:repair}
% \vspace{-6pt}
% \end{figure*}

\noindent\textbf{With self-correction.}  Figure~\ref{self correct example} shows the matched elements for another target element (\textcircled{\raisebox{-0.9pt}{1}}) selected by \watertool+ChatGPT before and after self-correction. Initially, \watertool+ChatGPT selected (\textcircled{\raisebox{-0.9pt}{2}}) with the explanation ``Because they share the most similar attributes: xpath, text, tagName, linkText.''.
However, our explanation validator detects inconsistencies in the attributes \emph{text} and \emph{linkText} (Explanation Consistency=0.5) and provided this feedback via the self-correction prompt. Guided by this, \watertool+ChatGPT revised its selection to (\textcircled{\raisebox{-0.9pt}{3}}) correctly, with a new explanation ``Because they share the most similar attributes: xpath, text, tagName, linkText.'' (Explanation Consistency=0.75 as all attributes except XPath were consistent with the selection). This example highlights how the self-correction mechanism, supported by the explanation validator, guides ChatGPT to identify and fix its inconsistencies to improve matching results.
%AddAndRemoveMultipleTasksTest_36, MRBS, WATER
% , and the most similar XPath is ``/html[1]/body[1]/div[1]/div[2]/div[1]/ul[1]/li[1]/a[1]'' from another candidate
% \noindent\textbf{With self-correction.}  Figure~\ref{self correct example} shows the fix generated by \watertool+ChatGPT before ($result1$) and after self-correction ($result2$). The explanation provided by ChatGPT for $result1$ is ``Because they share the most similar attributes: xpath, text, tagName, linkText.''.
% Our explanation validator detects that the explanation of the attributes \emph{text} and \emph{linkText} are inconsistent with the selection (Explanation Consistency=0.5). After self-correction, \watertool+ChatGPT repair this broken statement correctly and the result is represented as $result2$. The explanation for $results2$ is ``Because they share the most similar attributes: xpath, text, tagName, linkText.'' (Explanation Consistency=0.75 because all attributes except for XPath are consistent with the selection).

%After self-correction, WATER+ChatGPT selected the correct element. The explanation is ``Because they share the most similar attributes: xpath, text, tagName, linkText.'' and consistency is 0.75. Only the explanation of XPath is consistent with the selection.

%the result 1 is the repair result before self-correctness. After self-correct, WATER+ChatGPT repair this broken statement successfully and the result is represented as result 2.



% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.xpath("//*[@id=\"content 
% - wrapper\"]/div[1]/ul/li[3]/a")).click();
% //result1: before self-correction
% + driver.findElement(By.xpath("/html[1]/body[1]/d
% + iv[1]/div[2]/div[1]/ul[1]/li[1]/a[1]")).click();
% //result2: after self-correction 
% + driver.findElement(By.xpath("/html[1]/body[1]/
% + div[1]/div[2]/div[2]/div[1]/div[4]/div[1]/h2[1]
% + /a[1]")).click();
% \end{lstlisting}
% \vspace{-6pt}
% \caption{ChatGPT fixes for the broken statement in Collabtive that shows the effectiveness of self-correction.}
% \label{listing:sc_example}
% \vspace{-6pt}
% \end{figure}
% water1, AddAndRemoveMultipleTasksTest_36, ec1=0.5, ec2=0.75



%in \watertool's ranked list as the most similar element wrongly. However, the element ranked 6th in \watertool's ranked list is the matching element. Table \ref{table:motivation_example} shows the detailed information of these two elements and the target element. Combining \watertool with ChatGPT can make correct matching.
% \begin{table*}[ht]
% %\caption{The detailed examples of Web Ul elements}
% \caption{An example that shows the target element to be matched, and a list of candidate elements returned by \watertool}
% \label{table:motivation_example}
% \footnotesize
% \centering
% \begin{adjustbox}
% %\resizebox{center}{!}
% %{!}%{%
% %\small
% \begin{tabular}{l|l}
% \hline
% Target Element  & \begin{tabular}[c]{@{}l@{}}\{numericId=70, id=`', name=`new\_category', class=`', \\xpath=`/html{[}1{]}/body{[}1{]}/div{[}4{]}/form{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}2{]}/td{[}2{]}/input{[}1{]}', \\ text=`Category1', tagName=`input', linkText=`', x=363, y=278, width=261, height=21, isLeaf=true\}\end{tabular} \\ \hline
% Candidate 1 & \begin{tabular}[c]{@{}l@{}}\{numericId=20, id=`', name=`', class=`button-small', \\xpath=`/html{[}1{]}/body{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}1{]}/td{[}3{]}/form{[}1{]}/input{[}1{]}', \\ text=`Switch', tagName=`input', linkText=`', x=951, y=121, width=51, height=20, isLeaf=true\}\end{tabular}                 \\
% ...             & ...                                                                                                                                                                                                                                                                                                                     \\
% Candidate 6 & \begin{tabular}[c]{@{}l@{}}\{numericId=70, id=`', name=`name', class=`', \\\textbf{xpath=`/html{[}1{]}/body{[}1{]}/div{[}3{]}/form{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}2{]}/td{[}2{]}/input{[}1{]}'}, \\ \textbf{text=`Category1'}, tagName=`input', linkText=`', x=403, y=295, width=261, height=21, isLeaf=true\}\end{tabular}    \\     
% %\\...             & ...                                                                                                                                                                                                                                                                                                                     \\ 
% \hline
% \end{tabular}
% \end{adjustbox}
% \end{table*}

\begin{table*}
\caption{An example that shows the target element to be matched, and a list of candidate elements returned by \watertool}
\label{table:motivation_example}
\centering
\begin{tabular}{l|l} 
\hline
Target Element & \begin{tabular}[c]{@{}l@{}}\{numericId=96, id='', name='', class='', xpath='/html[1]/body[1]/p[1]', text='Unknown user', tagName='p', linkText='', x=8, y=90,\\ width=1018, height=15, isLeaf=true\}\end{tabular}                                                          \\ 
\hline
Candidate 1    & \begin{tabular}[c]{@{}l@{}}\{numericId=40, id='', name='', class='', xpath='/html[1]/body[1]/div[1]/table[1]/tbody[1]/tr[1]/td[7]/div[1]/a[1]', text='Unknown user',\\ tagName='a', linkText='Unknown user', x=917, y=6, width=111, height=23, isLeaf=true\}\end{tabular}  \\
Candidate 2    & \begin{tabular}[c]{@{}l@{}}\{numericId=47, id='', name='', class='', xpath='\textbf{/html[1]/body[1]/div[2]/p[1]}', text='Unknown user', tagName='p', linkText='', \textbf{x=26, }\\\textbf{y=69, width=982, height=15}, isLeaf=true\}\end{tabular}                        \\
....           & ...                                                                                                                                                                                                                                                                        \\
\hline
\end{tabular}
\end{table*}


\begin{figure}[!t]
    \centering
    %\includegraphics[width=5.5in, height=2.7in]
    \includegraphics[width=0.9\linewidth]{figures/content/sc_example_new.pdf}
    \caption{Generated fixes for the broken statement in Collabtive that shows the effectiveness of self-correction.}
    \label{self correct example}
    \vspace{-6pt}
\end{figure}
% \begin{table}[]
% \begin{tabular}{l|l}
% \hline
% Target Element  & \{numericId=70, id='', name='new\_category', class='', xpath='/html{[}1{]}/body{[}1{]}/div{[}4{]}/form{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}2{]}/td{[}2{]}/input{[}1{]}', text='Category1', tagName='input', linkText='', x=363, y=278, width=261, height=21, isLeaf=true\}                                   \\ \hline
% Candidate No. 1 & \begin{tabular}[c]{@{}l@{}}\{numericId=20, id='', name='', class='button-small', xpath='/html{[}1{]}/body{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}1{]}/td{[}3{]}/form{[}1{]}/input{[}1{]}', \\ text='Switch', tagName='input', linkText='', x=951, y=121, width=51, height=20, isLeaf=true\}\end{tabular}        \\
% ...             & ...                                                                                                                                                                                                                                                                                                            \\
% Candidate No. 6 & \begin{tabular}[c]{@{}l@{}}\{numericId=70, id='', name='name', class='', xpath='/html{[}1{]}/body{[}1{]}/div{[}3{]}/form{[}1{]}/table{[}1{]}/tbody{[}1{]}/tr{[}2{]}/td{[}2{]}/input{[}1{]}', \\ text='Category1', tagName='input', linkText='', x=403, y=295, width=261, height=21, isLeaf=true\}\end{tabular} \\
% ...             & ...                                                                                                                                                                                                                                                                                                            \\ \hline
% \end{tabular}
% \end{table}

% AssignCategoryToUser_51, ranked 6 in water, only modify locator value, correct matching 3 times in 4 times

% Code reuse has well-known benefits on code quality, coding efficiency and maintenance which is one of the reason for the popularity of open source culture (i.e. code sharing). Social programming platforms like Github, Gitlab etc have normalized code foraging via their public platforms, enabling code search and reuse across different projects. Developers prefer removing project borders that enables efficient code foraging and subsequently faster development~\cite{Gharehyazie2017}. Even though searching for code across project takes longer, even more challenging is to tailor to ones' needs. When porting code from one context to another, semantics of the ported code often change due to differences in the surrounding contexts. Developers may overlook such subtle differences, inadvertently creating a porting error~\cite{Ray2013}. Ray et al. shows in their study of the BSD product family ~\cite{Ray2012} ~that around 15\% of lines in BSD release patches consist of ported edits while 26.12\% to 58.85\% of active developers participate in cross-system porting per release on average. The results together indicate that cross-system porting is an essential technique in development and the cost of porting is significant. Ported changes are likely to be more reliable, showing the benefit of selectively porting well-tested edits, hence the popularity of such activity among open source developers~\cite{Gharehyazie2017}. Furthermore, their study concludes that over 50\% of ported changes propagate to other projects within 3 releases,  while some changes take a very long time to propagate.  Currently, cross-system porting in the BSD community seems to heavily depend on developers doing their porting job on time~\cite{Ray2012}.

% In the context of software security, patching vulnerabilities is time critical and many implementations rely on an upstream patch which can be ported efficiently.  Each time a vulnerability is disclosed in a free and open source software (FOSS) component, a software vendor must decide whether to update the FOSS component, patch the application itself, or just do nothing as the vulnerability is not applicable to the old deployed version. This is particularly challenging for enterprise software vendors that consume thousands of FOSS components and offer more than a decade of support and security fixes for their applications. For instance consider the example of the KRACK vulnerability, which affected almost all devices that implement the WPA2 protocol~\cite{krack-site}. During the initial research, it was discovered that Android, Linux, Apple, Windows, OpenBSD, MediaTek,
% Linksys, and others, are all affected by some variant of the
% attacks. Even though the original patch was released on September 2017, it took couple of weeks for many vendors to integrate the patch into their stack~\cite{krack-info}.  The results of the study~\cite{Piantadosi2019} indicate the importance of testing security patches for verification. Mitigating partial patches or introducing new vulnerabilities need to be considered when applying patches for security vulnerabilities, thus one of the reasons for security fixes taking years to be published even though the fix is available. 

% The results of above studies open interesting and novel research directions. For instance testing security patches is not always easy, thus an approach able to automatically understand when a patch is partial by generating test cases is particularly useful to mitigate the danger of partial patches. Addressing some of the above issues is part of our propose work, where a small and much more experienced development team can benefit from an end-to-end automated code transfer system. 



==> sections/sections/overview.tex <==
\section{Motivating Example}

TODO

% \label{sec:overview}


% \begin{figure}
% \begin{subfigure}[t]{0.45\textwidth}
% \centering
% \includegraphics[width=\textwidth]{images/matchexample2.pdf}
% \caption{MRBS Web apps of version 1.2.6.1 and 1.4.9, and part of the broken DeleteNegativeAreaTest.}
% \label{fig:picMRNS}
% \end{subfigure}
% \lstset{escapeinside={!@}{@!}}
% \begin{subfigure}[t]{0.45\textwidth}
% \begin{lstlisting}
% <tr>
%   <td !@\textcolor{red}{class="banner" bgcolor="\#C0E0FF" align="CENTER"}@!>
%         <a href="admin.php?day=28;month=01">Admin</a>
%    </td>... </tr>
% \end{lstlisting}
% \caption{The simplified HTML code of the banner in version 1.2.6.1\add{.}}
% \label{fig:old_version_MRBS}
% \end{subfigure}
% \lstset{escapeinside={!@}{@!}}
% \begin{subfigure}[t]{0.48\textwidth}
% \begin{lstlisting}
% <tr>
%  <td>
%     <a href="admin.php?day=28;month=01;!@\textcolor{blue}{area=888;room=409}@!">Rooms</a>
%  </td>...</tr>
% \end{lstlisting}
% \caption{The simplified HTML code of banner in version 1.4.9\add{.}}
% \label{fig:new_version_MRBS}
% \end{subfigure}
% \caption{Motivating example of MRBS webpage\add{.}}
% \label{fig:match-example}
% \end{figure}

% In this section, we use an example of \add{an} open-source app MRBS in the test 
%  cases dataset~\cite{imtiaz2021automated} 
% % \st{ (we did not use the industrial app to remain anonymous) }
%  to explain the shortcomings of existing approaches~\cite{choudhary2011water,stocco2018vista,shao2021webevo,brisset2020sftm}, and how \toolName fix\add{es} the broken test by matching elements.


% Figure \ref{fig:match-example} shows the screenshots of the MRBS app for version\add{s} 1.2.6.1 and 1.4.9, the simplified HTML code, and one simplified test.
% The broken test (\textit{DeleteNegativeAreaTest}) was manually translated to the Selenium test by the authors of prior work~\cite{imtiaz2021automated}. It contains three events: \circled{1} \textit{click} \add{the} ``Log in'' button, \circled{2} \textit{sleep}, and \circled{3} \textit{click} \add{the} ``Admin'' button.
% In Figure \ref{fig:old_version_MRBS}, we use $e_o^{Admin}$ to denote the old element with text \textit{Admin} and $e_o^{ban}$ to represent the old element with tag \textit{tr}, which is a banner. 
% Similarly, in Figure \ref{fig:new_version_MRBS}, we use $e_n^{Rooms}$ to represent the element with text \textit{Rooms} and $e_n^{ban}$ to represent the element with tag \textit{tr}.
% When \add{MRBS} evolved from 1.2.6.1 to 1.4.9, its view and attributes of elements changed drastically.
% For instance, the text of $e_o^{Admin}$ changed from ``\textit{Admin}'' to ``\textit{Rooms}'', 
% the background color of $e_o^{Admin}$ was changed from blue to dark blue, which caused the visual change, 
% % none of its attribute tokens is unique, 
% the attribute of $e_o^{Admin}$ was extended with ``\texttt{area=888;room=409}'',
% and all the attributes of the ancestors of $e_o^{Admin}$ (i.e., $e_o^{ban}$) were removed.
% % In the version 1.4.9, the locator of ``Log in'' button is ``//*[@id=``logon\_submit'']/input'' and the locator of ``Admin'' button is ``//a[text()=`Admin']''.
% The changes cause \textit{DeleteNegativeAreaTest} to fail in the new version.
% From the motivation example, we can obtain the following observations:
% %does not work anymore on the new version.

% % Most of exist matched methods\cite{stocco2018vista,choudhary2011water,shao2021webevo} failed in the action1, because there are two button with text \textit{Log In} and only SFTM\cite{brisset2020sftm} can use structural information to distinguish them.
% % Let us focus on the element of action 3 as an example.
% % Note that, the webpages that the $O_{Admin}$ and $N_{Rooms}$ jumps to have the same funtion, which contain four functions, \textit{Area}, \textit{Rooms}, \textit{Add Area} and \textit{Add Rooms}.


% %\noindent\textbf{Observation1: A element matching depends on other elements being matched first.} \yz{
% Existing approaches usually match elements by matching either their attributes~\cite{choudhary2011water}, visual information~\cite{stocco2018vista}, or both~\cite{shao2021webevo}. 
% % The significant changes on $e_o^{Admin}$ cause existing approaches to produce incorrect matching results.
% Due to the changes in the attributes and visual information, the similarity between $e^{Admin}_o$ and $e^{Rooms}_n$ is low. 
% Algorithms based on text information~\cite{choudhary2011water}, visual information~\cite{stocco2018vista}, or both~\cite{shao2021webevo} fail to match \add{$e_o^{Admin}$ with $e_n^{Rooms}$}.
% % these algorithms cannot correctly match elements $e_o^{Admin}$ and $e_n^{Rooms}$.
% % Specifically, as the text and attribute changes, matching strategies that rely solely on text or attribute matching~\cite{choudhary2011water} fail to match $e^o_{Admin}$ with $e^n_{Rooms}$.
% % Due to the visual changes, matching strategies relying on visual information (e.g., \vistatool~\cite{stocco2018vista}) also fail to match $e^o_{Admin}$ and $e^n_{Rooms}$.
% The SFTM algorithm~\cite{brisset2020sftm}, which matches attributes of the parent nodes and child nodes for similarity propagation, also fails to match $e_o^{Admin}$ with $e_n^{Rooms}$ because (1) the similarity score based on attribute matching is quite low due to the changes in attributes, and (2) the parent node of $e_o^{Admin}$ do not share common attribute tokens with the parent nodes of $e_n^{Rooms}$.

% By investigating this example, we have the following observation: \textit{an element matching could depend on its neighboring elements that have been matched.}
% In this example, there are multiple elements located in the banner $e_o^{ban}$, including the ``Help'' button, ``Admin'' button, ``Report'' button\delete{ and etc}.
% % so similar to the surrounding elements, they are used to jump to a target page. 
% % The shared attribute ``admin.php'' of $e_o^{Admin}$ and $e_n^{Rooms}$ implies that the target pages is consistent.
% Through the word ``admin.php'' also appears elsewhere on the page, %$e_o^{ban}$ and $e_n^{ban}$ can 
% the elements around $e_n^{Admin}$, e.g., the ``Help'' button of the old and new version which can be easily matched, can be used to distinguish $e_n^{Admin}$ with the ``admin.php'' elements located somewhere else. 
% %and help $e_o^{Admin}$ and $e_n^{Rooms}$ match correctly.
% % the matching of $e_o^{Admin}$ and $e_n^{Rooms}$ will depend on their parent elements $e_o^{ban}$ and $e_n^{ban}$ being able to match correctly and assist in their matching.
% It indicates that element matching could also be guided by the matching results of other elements.

% % \textbf{Observation2: Different types of elements have different meanings.} 

% % \yz{
% % Since the webpage is actually a DOM tree, functional elements such as the buttons that users usually contact are mainly elements at the bottom of the tree.
% % Other elements are used as containers of these functional elements and displayed to users in the form of regions.
% % Elements can therefore be divided into functional type elements and region type elements.
% % In Figure 1, elements with the ``tr'' tag represent the banner region, while elements with the ``td'' and ``a'' tags represent the ``Admin'' button.
% % The meaning of these two types of elements affects each other.
% % The meaning of the banner element depends on the meaning of the buttons located in it.
% % The meaning of the button is also limited by the region it locates in.
% % The similar element may express different meanings in different regions.
% % Existing tools simply calculate similarity based on text or visual information, ignoring the true meanings of elements of different types.
% % }


%  % The first step of fixing the given test is identifying the matched elements in the old and new versions.
% % parts of simplified DOM structures of \textit{Xfinity} home page in version 2018 and version 2020.
% % In this example, some representative elements are marked with blue labels, i.e., \texttt{O1}, \texttt{O2}, \texttt{O3} for version 2018, and \texttt{N1}, \texttt{N2}, \texttt{N3} for version 2020.
% % Let us take element \texttt{O3} as an example.
% % When \textit{Xfinity} evolved from 2018 to 2020, (1) the text of element \texttt{O3} was changed from ``\textit{TV}'' to ``\textit{TV \& Streaming}'', which also caused the visual changes, (2) the attribute of \texttt{O3} has also changed from \textit{"class": "shop-deals\_\_lob-name"} to \textit{"class": "x-heading-group3"}, (3) the DOM structure around \texttt{O3} was also changed, and there are no similar attributes between its parents.
% %First of all, its text has changed from \textit{TV} to \textit{TV\&Streaming}, which also caused the visual changes.
% %Second, its attribute has also changed from \textit{"class": "shop-deals\_\_lob-name"} to \textit{"class": "x-heading-group3"}.
% %Finally, the DOM structure around it also has obvious changes, and there are no similar attributes between its parents.
% % Specifically, changes in attributes and visual changes affect the accuracy of existing approaches.

% % The content in the red label means that the element is matched in \textit{ith} iteration by \toolName.

% %The DOM structure changes, and the fact that parent node does not share similar attributes make it difficult for approaches based on SFTM~\cite{brisset2020sftm} to use the attributes of the parent nodes for similarity propagation.
% %difficult for SFTM~\cite{brisset2020sftm} hard to use the attributes of their parent nodes for similarity propagation.
% %Therefore, none of these methods correctly matches $O7$.

% From the observations, we could measure the similarity of elements based on the following ideas.
% \begin{itemize}[leftmargin=*]
%     \item \textbf{\add{I1:} Elements with closer matched ancestor\add{s} are more similar.}
%     For any element $e_o$ in the old version and any node $e_n$ in the new version, if they have the matched ancestor (e.g., banner), we consider $e_o$ and $e_n$ to be structurally similar.
%     If the matched ancestor is closer to $e_o$ and $e_n$ (e.g., the \delete{right side} \add{child element} of the banner), $e_o$ and $e_n$ are more likely to match due to higher structural similarity.
    
%     \item \textbf{\add{I2:} Ancestors with more common leaf elements are more similar.}
%     For two ancestors (non-leaf elements), if most of their leaf elements match, they are likely to be matched.
%     For example, if most of the buttons in the banner before and after the version updates match, these banners tend to be matched.
    
%     \item \textbf{\add{I3:} Matching element\add{s} by multiple iterations.}
%     Different from existing approaches that rely on pre-defined similarity metrics in one single step, we could perform an iterative approach for matching.
%     In each iteration, a matching result is calculated.
%     The next iteration will recalculate the similarity based on the matching result and also update the matching result.
%     % we could perform matching via multiple iterations.
%     During the iterations, the higher-confident matching results could help to increase the similarity of the lower-confident matched elements through multiple iterations of matching.
% \end{itemize}



% % \noindent\textbf{Key Idea 2. Design similarity based on the type of elements.}
% % From observation 2, we have designed new similarities according to the features of different types elements.
% % Specifically, they are designed based on the two insights below:

% % Our main intuitions are (1) when the webpage evolves, certain elements are very likely to remain in the same region, e.g., $e^o_{Admin}$ remains in the same location (the middle banner); (2) the higher-confident matching results could help to increase the matching score for the lower-confident matched elements through multiple iterations of matching.
% % In other words, the matching result of subsequent iterations is determined by existing matching results.

% \emph{How does \toolName match these elements?}
% In the first iteration, \toolName{} has matched elements with high initial similarities (e.g., the element with text \textit{Help}). 
% % guide \toolName to match the correct elements.
% In the second iteration, the structural similarities of $e_o^{ban}$ and $e_n^{ban}$ are increased because the leaf nodes in the region represented by $e_o^{ban}$, i.e., the element with text \add{``}Help\add{''}, are matched in the first iteration.
% Then, in the third iteration, because the $e_o^{Admin}$ is contained in $e_o^{ban}$ and $e_n^{Rooms}$ is contained in $e_n^{ban}$, and $e_o^{ban}$ are matched with $e_n^{ban}$, the structural similarity between $e_o^{Admin}$ and $e_n^{Rooms}$ are increased.
% After the three iterations, the similarity between $e_o^{Admin}$ and $e_n^{Rooms}$ is larger than the threshold $\theta$, so they can be matched.
% This example shows the advantages of \toolName:
% (1) when attributes change significantly, using the matching results to calculate the structural similarity can enhance the accuracy of the matching;
% (2) in the process of multiple iterations, the elements in the previous iteration could guide the matching of the remaining elements.
% In some cases, the wrongly matched elements can even be corrected during the iterative process (not shown in this example). 

% % For instance, \watertool wrongly match the element of action 1 in above example\todo{modify} and match action 3 in wrong page. 
% %Sometimes the wrong matched elements are corrected during the iteration process, which is not shown in this example.
% With the matching results, \toolName will then repair the broken UI test by changing the locators of event \circled{1} and event \circled{3}.
% Specifically, \toolName updates the locator of the ``Log in'' button from ``/html/body/form/input[3]'' to ``//*[@id=``logon\_submit'']/input'', and the locator of ``Admin'' button from ``//a[text()=`Admin']'' to ``//a[text()=`Rooms']''.
% %Incorrect matching leads to propagated errors due the repair phase.\todo{this is strange}
% %For instance, the MRBS has two ``Log in'' buttons in the \textit{Login} page and \watertool incorrectly match the ``Log in'' button related to event 1 with another ``Log in'' button, which results in incorrect fix.


% % (1) Before execution, \toolName will instrument the test case, and will complete the information gathering and repairing in the instrumented code.
% % (2) In the version 1.2.6.1, \toolName will processing and save the webpage DOM infomation before each action executed.
% % (2) In the version 1.4.9, \toolName will try to check whether the element exist in this webpage, and use the matched locator to replace the original locator if the element is not exist. 

% % The XPath path of these elements and text of partial elements has changed.
% % These elements have only a small amount of attributes.
% % To describe elements more simply, we use $o5$ to represent element 5 in version 2018 and $n5$ to represent element 5 in version 2022, the same to other elements.
% % $o5$ is an element used to display data, and it is difficult to match the corresponding element.
% % The data of this type of element is likely to change during the version change process, which causes both the visual and text information of the element to change.
% % Unfortunately, $o5$ has only the attribute \textit{dir="Itr"} in addition to the text.
% % And $o4$, which is the parent element of $o5$, has only one text attribute that changes.
% % This makes $o5$ potentially difficult to match by itself or its parent.

% % When manually matching these elements, the following steps are usually taken.
% % First, the matching results of $o2$ and $o4$ are obtained, because they have a high degree of similarity with the $n2$ and $n4$.
% % Next, we can infer that the areas where the $o2$ and $o4$ are located match the areas where the $n2$ and $n4$ are located.
% % In fact, we knows that $o1$ matches element $n1$ and element $o4$ matches element $n4$ in this step.
% % Finally, both $o5$ and $n5$ are in the matching area and them have similar text styles, so it is judged that the $o5$ and $n5$ match.

% % How does \toolName match these elements?
% % First, match $o1$ and $n1$ through the equality of id attributes.
% % In the first round of iteration, $o2$ matches $n2$ and $o4$ matches $n4$ because the element's own similar attribute and the structural similarity enhanced by the match of $o1$ and $n1$.
% % In the second round of iteration, $o3$ and $n3$ are matched because their structural similarity is enhanced by the match result in the previous iteration.
% % During the third iteration, $o5$ and $n5$ are matched because the match of $o3$ and $n3$ enhances the structural similarity of o5 and n5.




% % \begin{figure}[!t]
% % \begin{subfigure}{0.43\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{images/structrue-example-left3.pdf}
% % \caption{DOM tree of v2018.} 
% %  \label{img:structrue-example-left}
% % \end{subfigure}
% % \begin{subfigure}{0.55\linewidth}
% % \centering
% % \includegraphics[width=\textwidth]{images/structrue-example-right3.pdf}
% % \caption{DOM tree of v2020.} 
% %  \label{img:structrue-example-right}
% % \end{subfigure}
% % \caption{Element matching example for \textit{Xfinity} home page.}
% %   \label{fig:matching-example-Xfinity}
% % \end{figure}
% % \begin{figure}[htbp]
% % \centering

% % \begin{minipage}{0.24\textwidth}
% % \centering
% % \includegraphics[width=1\textwidth]{images/structrue-example-left.jpg}
% % \caption{
% %  .} 
% %  \label{img:structrue-example-left}
% % \end{minipage}1

% % \begin{minipage}{0.24\textwidth}
% % \centering
% % \includegraphics[width=1\textwidth]{images/structure-example-right.jpg}
% % \caption{11} 
% % \label{img:structrue-example-right}
% % \end{minipage}

% % \end{figure}


% % \begin{figure*}[!th]
% % \vspace{-5pt}
% %   \centering
% %       \centering
% %       \includegraphics[width=0.9\textwidth]{images/ourapproach.jpg}
% %   \vspace{-5pt}
% %   \caption{Overview of our approach}
% %   \label{fig:overview}
% % \vspace{-5pt}
% % \end{figure*}
% % Our match method generally follows the following steps
% % \begin{enumerate}
% %     \item Preprocessing. Filtering non-displayable elements and  merging elements representing a function.
% %     \item Pre-matching. Match the elements with id first, and the matched elements will not change in the subsequent process.
% %     \item Similarity initialization. Construct the initial similarity matrix by attribute. 
% %     \item Iterative optimization. 
% %     In each iteration, our method will use the current matching result to recalculate a new similarity, and then use the new similarity to obtain an optimized matching result.
% % \end{enumerate}


% % After we get the matching result, we can verify the repaired result through the difference-based intent verification stage.



==> sections/sections/reflection.tex <==
\section{Implications and Discussions}
Our study identifies several key implications and suggestions for future test repair and ChatGPT research.

\noindent \textbf{Prioritization of attributes by Web UI test repair tools.} Table~\ref{tab:attribute} shows varying attribute prioritization in element matching among prior test repair tools  (e.g., \watertool{} prioritizes XPath similarity, whereas \vistatool{} uses the position and the size information for visual matching). Our study shows that further matching with ChatGPT can improve over prior approaches (Finding 1) by mitigating their bias, leading to more accurate matching. In fact, our study of the frequently mentioned attributes in ChatGPT's explanation also reveals that ChatGPT has preferences towards certain attributes, e.g., \emph{XPath} and \emph{text} (Finding 5). 
Although this paper only studies the prioritization of attributes in two traditional Web test repair approaches, similar biases may exist in other UI matching techniques. In the future, it is worthwhile to study (1) the characteristics of the selected prioritization in other tasks where UI matching algorithms are used (e.g., compatibility testing~\cite{CdDiff}), and (2) improving the effectiveness of other UI matching techniques via subsequent matching using LLMs.  %Compared to a recent approach that shows that performing iterative matching algorithm over attributes~\cite{UITESTFIX}.   


\noindent\textbf{Test repair techniques used for element pre-selection.} %candidates elements.} 
Our study that compares three approaches (\watertool{},\vistatool{}, and \edtool{}) for the pre-selection of candidate elements shows that a simplified version of \watertool{} (i.e., \edtool{}) combines well with ChatGPT where \edtool{}+ChatGPT outperforms all the evaluated approaches (Finding 2). Compared to \watertool{} that matches multiple attributes (e.g., \emph{id}, \emph{XPath}) and \vistatool{} that uses visual information for matching, %\todo{may need to change this if you change table III about location} (position information when extracting visual information), 
\edtool{} that solely relies on \emph{XPath} is less effective as a standalone matching algorithm (it performs worst among all individual baselines). However, our study shows that by using only XPath similarity, \edtool{} delegates the responsibility of matching using other attributes to ChatGPT which later performs subsequent matching. Intuitively, one may think that \watertool{} that performs the best among the individual baselines would lead to the best results when combining with ChatGPT. \emph{As the best individual baseline may not be the most effective combination with ChatGPT}, our study urges researchers to perform thorough evaluation to choose appropriate baseline to combine with ChatGPT for solving other software maintenance tasks. %Hence, our study encourages thorough investigation of candidate selection approaches instead of choosing the best approach . %provides an interesting perspective of performing pre-selecting using only XPath similarity to give ChatGPT more freedom to perform further matching using other attributes. %In future, we urge tool developers that use ChatGPT  %In future, when designing a combination with ChatGPT, it is worthwhile to study a simplified variant to allow for 


% \section{Discussion}

% %\xiang{remove this para if we submit a technical paper.}
% %\shinhwei{TODO: need to add this section for experience report paper. The current Discussion section does not have suitable contents}
%\noindent \textbf{Open labeled dataset for Web UI test repair.} To facilitate future research in Web UI test repair, we have made our ground truth dataset with manually labeled correct UI elements to be publicly available. %It would be beneficial to have a community-driven dataset and more analysis of the defects within the dataset to facilitate future improvement of the auto-generated programs. We propose the  dataset as an initiative towards this direction. 

%push the limits of the code generation capability of a large language model like Codex, we believe that our systematic investigation of the mistakes made by language models is an important initial step. It would be beneficial to have a community-driven dataset and more analysis of the defects within the dataset to facilitate future improvement of the auto-generated programs. We propose the  dataset as an initiative towards this direction. 

%\noindent\textbf{Using LLM in test repair.} Our study includes \industryteststudy{} industrial Web UI tests with \totcommit{} commits containing  \totdiff{} diff chunks that are related to updating UI tests. The sheer number of UI tests that require manual updates shows that \emph{the need to automate the time-consuming task of fixing broken tests}. Compared to open-source apps, our study also shows that the complexity of UI tests in the industrial app is higher with more lines of code and more events (RQ2). Given the results, we observe that \emph{updating broken UI tests in an industrial setting remains a challenge}. 
\noindent \textbf{LLM-based test repair and robust locators generation.} Our study shows promising results in using LLMs like ChatGPT for Web test repair (Finding 3).
Our manual analysis shows that it can generate correct repairs for the broken statements. Currently, the generated fixes mainly modifies and generate assertions, showing the promises of LLM-based test repair. In future, it is worthwhile to study using LLM for improving test repair technique that fixes broken assertions~\cite{daniel2011reassert}~\cite{yaraghi2024automated}. Another worthwhile future work is to use LLMs like ChatGPT to improve the locator robustness and incorporated into prior techniques like \emph{Robula+} ~\cite{robula2}. For robust locators generation, ChatGPT may be instructed to select different locators, prioritizing locators that are less fragile. %using a diverse set of fix patterns, including modifications and generations of assertions. 
%This shows the promises of using LLM for improving general purpose test repair technique that fixes broken assertions~\cite{daniel2011reassert}~\cite{yaraghi2024automated}. %Although there are several prior tests generation techniques that use LLM,

%\noindent\textbf{ChatGPT's preference towards certain attributes.} Similar to prior approaches that have certain preferences prefer certain attribute (XPath and text) but not always correct (e.g., text is more accurate). 




\noindent \textbf{Improving reliability of ChatGPT output.} Prior study has expressed concerns regarding the tendency of ChatGPT to ``hallucinate'' when solving specific tasks~\cite{Feldt2023aa}, our workflow (that checks whether the explanations provided by ChatGPT are consistent along with the selected elements) %aims to improve the reliability of ChatGPT generated outputs 
shows promising results for improving the matching accuracy for certain combinations (Finding 7). %to combat hallucination. %Our experiments show that the explanation consistency (EC) of ChatGPT correlates well with the accuracy of its matching results (higher EC leads to more correct matching and repair). 
Although our study are limited to Web UI test maintenance, we believe that our proposed way of checking for explanation consistencies is general and can be applied to improve the reliability of ChatGPT for other software maintenance tasks (e.g., test generation). %and automated program repair). %In future, it would be worthwhile to study %To push the limits of the code generation capability of a large language model like Codex, we believe that our systematic investigation of the mistakes made by language models is an important initial step. It would be beneficial to have a community-driven dataset and more analysis of the defects within the dataset to facilitate future improvement of the auto-generated programs. We propose the  dataset as an initiative towards this direction. 

%~\cite{Feldt2023aa}
% %

% % \noindent\textbf{Prevalence of UI test repairs related to event loading.}
% % Our study of \totdiff{} diff chunks in the industrial app shows that \emph{Type-VI: Events related to page loading} are the most common repair type (51.16). This indicates that developers need to add or modify \texttt{sleep} or \texttt{refresh} to ensure the reliability of UI tests. The prevalence of this repair type is consistent with prior studies of flaky tests~\cite{thorve2018empirical,romano2021empirical,luo2014empirical}. Moreover, as required by \company{}, \texttt{sleep} calls were added to improve the stability of the tests, whereas sleep calls were deleted to speed up the test execution. This indicates that developers of industrial apps often consider the \emph{trade-off between the reliability of test outcomes and the efficiency of UI test executions}. Although we focus on repairing broken locators in this paper, our study of an industrial app shows that the prevalence of UI tests update related to event loading provides empirical motivation for future work on the automatic repair of flaky Web UI tests. While there exist several techniques that repair flaky tests~\cite{li2022repairing,zhang2021domain}, we observe there is \emph{little to no approach that specializes in fixing flaky Web UI tests}.
% %This requirement may not generalize to other industrial applications.


% % \noindent\textbf{Types of repairs in broken UI tests.} Our study of \totdiff{} diff chunks shows that developers often need to modify the locator to fix broken UI tests (17\% in our study). As most prior techniques focus on fixing broken locators, this further motivates us to improve over existing techniques by designing \toolName, a more accurate technique for fixing broken locators in Web UI tests. Apart from motivating existing techniques that repair broken assertions~\cite{daniel2011reassert}, Table~\ref{table:modify-type-distribute} shows that there are other types of repair involving adding, deleting and modifying events that are common in the developers' commits. It is worthwhile to design techniques that specialize in repairing broken UI events in the future.


% %Our study also shows that events related to 
% % Our empirical study indicates that backporting patches may involve complex changes beyond copy-and-paste. Although most backporting tasks involve patches in Type-I and Type-II, existing tools such as GNU \texttt{patch} that rely on comparing and merging files cannot address many of them (Table~\ref{table:experiment-comparison-quantitative}). In fact, although Type-II patches seem trivial to backport since no adaptation to the code is required, finding the correct location is nontrivial because (1) the order of the code modifications could be different for the backport (e.g., 
% %the original patch may change $func_A$ and then $func\_B$, but the backporting would have to change $func_B$ and then $func_A$
% % the affected functions appear in a different order); (2) although it may seem that only the line number is different in the target version, the surrounding context may also be vastly different, and simple find-and-replace cannot locate such places; (3) some of the patch locations cannot be easily found by referring to Git commit history, and either need expert knowledge of the file changes or some other semantic methods to find the correct place to insert the patch.
% %

% \noindent\textbf{Open dataset for \delete{W}\add{w}eb UI maintenance.} 
% % Although many techniques have been proposed for repairing broken UI tests in the past decade, we still need help finding an open dataset containing developer-written Web UI tests. 
% % Web UI test maintenance researchers often need to manually write or translate test cases into Selenium tests to evaluate their approach.
% % Having a community-driven dataset is an important direction to encourage future research in studying and automating the repair of broken Web UI tests. 
% % Although we could not share our industrial dataset due to the policy in \company{}, we have manually labelled prior UI webpage datasets (\testDatasetB\cite{leotta2014visual} and \testDatasetA\cite{imtiaz2021automated}) as an initiative towards this direction.
% Although many techniques have been proposed for UI element matching and repairing broken UI tests in the past decade, we notice that there is still a lack of labelled \delete{W}\add{w}eb UI open dataset. 
% Having a community-driven dataset is an important direction to encourage future research in studying and automating the repair of broken \delete{W}\add{w}eb UI tests. 
% Although we could not share our industrial dataset due to the policy in \company{}, we have manually labelled the UI \delete{W}\add{w}eb page dataset (the expanded WebEvo~\cite{shao2021webevo} dataset), and released it as an open dataset as an initiative towards this direction.
% %and the webpages from five web apps) as an initiative towards this direction.



% % fails to backport some patches of Types III, IV, and V when the surrounding context is drastically different in the target version. This raises the question of whether context information helps in backporting in general. Indeed, we learned from our results in Table~\ref{table:experiment-comparison-qualitative} that context information is useful in guiding both \texttt{patch$^c$} and \toolName{} in generating more correct patches for most types of backporting.
% %This scenario is similar to the failure in automated program repair techniques in locating the correct fix location, which results in generating incorrect patches. Research in automated program repair that 
% %Despite having the same transformation with no adaptation in Type-I and Type-II, due to the context difference, 
% %

% \noindent\textbf{Types of repairs in broken UI test cases.}
% % Our study of \totdiff{} diff chunks shows that developers often need to modify the locator to fix broken UI tests (17\% in our study). 
% As most prior techniques focus on fixing broken locators, this further motivates us to improve over existing techniques by designing \toolName, a more accurate technique for fixing broken locators in \delete{W}\add{w}eb UI tests. 
% Although as shown in \add{F}igure \ref{fig:evluation-error-analysis}, there are still 120 out of 166 test cases \delete{that} can be fixed through relocation, \add{of} which \toolName currently cannot fix \add{7}. 
% However, the remaining 46 test cases involving actions such as addition, deletion, propagation of crashes, and branch statements are worth further investigation.
% % Apart from motivating existing techniques that repair broken assertions~\cite{daniel2011reassert}, Table~\ref{table:modify-type-distribute} shows that there are other types of repair involving adding, deleting and modifying events that are common in the developers' commits. 
% It is worthwhile to design techniques that specialize in repairing broken UI events in the future.



% % \noindent\textbf{Match.}


% \noindent\textbf{Importance of DOM structure information.}
% Prior techniques in matching UI elements usually use (1) attribute information (e.g., \watertool~\cite{choudhary2011water}), (2) visual information (i.e., \vistatool~\cite{stocco2018vista}), and (3) structure information (i.e., \sftmtool~\cite{brisset2020sftm}). Our evaluation shows that approaches that use structural information for repairing broken locators are more accurate than those that do not. This indicates the importance of structural information in improving the accuracy of matching UI elements. Although our approach uses textual information (e.g., id) for matching UI elements, relying merely on textual information leads to inaccurate results as textual information is often subject to changes. Compared to using structural information, our results show that \vistatool that relies on visual information takes the longest time due to the overhead in matching elements via image processing and computer vision. Meanwhile, matching using visual information also relies heavily on the accuracy of image processing and computer vision, which is less mature than textual matching used in structural and textural information. For example, in Figure~\ref{fig:picMRNS}, although the general structures of the old and new MRBS pages are similar, \vistatool{} fails to match correctly due to visual changes.
% %(e.g., changes in background color). 
% %For example, during manual inspection of the produced matching results, we realized that \vistatool has wrongly matched an empty picture\todo{ give one example: has wrongly matched an empty picture/ an greyscale picture?} due to inaccurate cropping of the image.  %To correctly match elements, we learned that it is important for an automated UI test repair technique to strike a balance in the generalization such that the context is not over-generalized and the transformation is not over-specific
% %Finding the proper generalization of transformation rules is important in ensuring the quality of automatically backported patches. 
% %In terms of the level of generalizations, SYDIT is the most abstract among all evaluated approaches because it generalizes the transformation by abstracting the context, whereas GNU \texttt{patch} is the least abstract because it merely compares and merges files at the line level. The level of generalization affects the precision and recall of each technique. For example, since \toolName{} over-generalizes more compared to \texttt{patch$^c$}, \texttt{patch$^c$} has higher precision for Type II backporting than \toolName{}. Meanwhile, as under-generalizing could lead to an increase in false negatives,  the recall for Type II is higher in \toolName{} than the recall for \texttt{patch$^c$}. To correctly backport patches, we learned that it is important for an automated backporting technique to strike a balance in the generalization such that the context is not over-generalized and the transformation is not over-specific.  
% %We designed \toolName{} such that it strikes a balance in the generalization to ensure that the context is not over-generalized and the transformation is not over-specific.Based on  
% %Techniques like SYDIT~\cite{sydit} generalize the transformation by abstracting the context. Our evaluation results show that context information helps in producing more correctly backported patches. Although such techniques can reduce the false negatives, they lead to many false positives as the abstraction can match to many other non-related locations in the source code. To correctly backport patches, a balance is needed in the generalization such that the context is not over-generalized and the transformation is not over-specific. Our evaluation 

% \noindent\textbf{Iterative matching.} 
% The key idea behind \toolName{} is an iterative approach that performs multiple rounds of matching to increase the similarities of weakly matched elements. As our experiment shows that our matching algorithm leads to improved matching accuracy, and the algorithm can be theoretically applied for any task that requires matching of UI elements, \delete{it is worthwhile to study in future}\add{in the future, it is worthwhile to study} using an iterative matching approach for tasks beyond the repair of broken tests (i.e., compatibility testing~\cite{CdDiff}). 

% % \yuanzhang{add discussion about the limitation of existing tool}


% %\paragraph{Impact of propagated errors in matching.} 

% % \paragraph{Backporting security patches.} To reduce the exposure to known vulnerabilities, automatically backporting security patches is an important application of \toolName{}. Our evaluation shows that \toolName{} is effective in backporting security patches (i.e., successfully backported $21/30$, that is, 70\% of the evaluated CVEs). Although we only evaluate on the Linux kernel, Table 3 shows that \toolName{} can backport patches for various types of vulnerabilities. Instead of generating patches from scratch, future research on automated repair of security vulnerabilities could look into deriving fixes by referring to existing patches (i.e., patch transplantation~\cite{PatchWeave}). 
% %


% %Linux kernel includes  such as the Linux kernel is an interesting benchmark to evaluate program repair and transformation techniques. The sheer complexity of the patches (with diverse types of transformations) and the absence of test cases for specification should form interesting challenges for the program repair community.

% \noindent \textbf{Threats to Validity.}
% \add{
% Internal threats arise primarily from potential errors in labeling and variations in element change definitions. To address this concern, two authors independently checked and confirmed the accuracy of the annotations, ensuring a higher level of reliability.}
% \add{External threats originate from two main sources. 
% Firstly, the flakiness of test cases can lead to unstable repair results. 
% To minimize the impact of flakiness on the algorithm's repairs, we closely monitor the execution process by capturing screenshots of the executed elements.
% If any issues arise due to external factors, such as network instability, we reprocess the repair procedure accordingly.
% Another concern is the generalization of experimental results.
% We conducted evaluations on limited webpages and test cases.
% However, our datasets consist of both open-source and industrial applications.
% We extensively tested changed elements across various types of famous pages.
% These measures contribute to the reliability and credibility of our experimental findings.
% }




==> sections/sections/related.tex <==
% \section{Related Work}

% \noindent \textbf{UI element matching.}
% UI element matching has important applications, such as test reuse~\cite{10.1145/3460319.3464827}, automated compatibility testing~\cite{CdDiff}, and automated maintenance of test cases.
% There are also various techniques for UI element matching, but few of them are suitable for our evaluation.
% For example, COLOR~\cite{COLOR} and GUIDER~\cite{xu2021guider} uses a combination of attribute and visual information to match elements.
% However, COLOR only recommends updated locators to testers instead of repairing broken test cases directly while GUIDER focused on Android test repair. 
% \yz{\watertool{} and \vistatool{} match elements according to attribute information and visual information individually.}
% % , we select them as representative web UI test repair tools as our baselines.
% \yz{Differently from these prior approaches, we explore the feasibility of using edit distance to obtain an initial ranked list of elements and use ChatGPT to perform global view matching.}
% \yuanzhang{UI element matching in android.}

% \noindent \textbf{Automatic UI test case repair.}
% Recently, many techniques have been proposed that enable testers to maintain UI test cases more efficiently~\cite{repairtech2}.
% % Of these existing methods, most have taken the approach of replacing outdated locators to repair broken tests as in this article.
% % Their successful repairs are also based on correct matching.
% Juyeon Yoon~\cite{repairtech1} 
% % focused on repairing Android GUI tests instead of web UI tests, which break due to changed view ids.
% % They also 
% proposes a tool which found matched elements through similarity and then repair the tests by updating the locator.
% % Some discuss the breakages that are not caused by locator changes.
% % In their study, 这个their study 是谁的study？Yoon的吗？为啥突然说的their study。
% Hang et al.~\cite{theory_repair} focus on the issue of mending dysfunctional workflows in GUI applications,
% % Workflows, defined as a series of activities aimed at accomplishing specific tasks, are the target of their repair method.
% but their approach does not specifically target the repair of actual tests and we do so.
% % Hammoudi et al. proposed an incremental approach known as WATERFALL for test repair in their study~\cite{waterfull}. 
% % This method involves the iterative application of WATER across multiple fine-grained versions of a web application. 
% % Although these approaches share similarities with general program repair techniques~\cite{semantic}~\cite{bibliography}, t
% These approaches typically build a model (e.g., an event flow graph) to finish the task. 
% However, obtaining an accurate application model and the information it needs in the real world is not easy, so we did not consider these tools as baselines in this paper.

% % In the field of web test repair, 
% \yz{Another main approach to solve web UI test failure is to improve the robustness of the element.} 
% % prevent the element locator from failing after web applications update.
% Leotta et al. developed 
% % \emph{Robula}~\cite{robula1} and \emph{Robula+}~\cite{robula2}, which aim to generate robust locators. 
% % They compared the tool's results with other locator generators (\emph{FirePath}, \emph{Selenium IDE}, \emph{Montoto}) and showed that the locators generated by \emph{Robula+} were the most robust. 
% % The idea behind 
% \emph{Robula+}~\yuanzhang{cite?}, which generating locators is to see if an attribute uniquely locates an element based on a predefined attribute priority.
% % Some attributes were also blacklisted because the authors pointed out that they could not be found after the changes were made on the page. 
% They also study how to use multiple locator generators to get more robust locators~\cite{robula3}. 
% They decide the final result by having different locator generators vote, where they give higher weight to more reliable locator generators like \emph{Robula+}. 
% % Experimental results show that this multi-locator voting results in 29.5\% less corrupt locators than using only \emph{Robula+}. 
% Our design of the experiment is inspired by this, letting ChatGPT make a selection among multiple candidates.
% However, we have not considered making the repaired locators more robust now, which may be a part of our future work.


% \noindent \textbf{ChatGPT in software maintenance.} Several studies have used large language models like ChatGPT to assist in several software maintenance tasks (e.g., testing ~\cite{Feldt2023aa,tang2023chatgpt} and repair~\cite{sobania2023analysis,fan2023automated}). %xia2023keep,
% %As a large language model, ChatGPT has high potential for repairing program bugs.
% %A series of work~\cite{xia2023keep,sobania2023analysis} has emerged to investigate the performance of ChatGPT in program repair or use ChatGPT development tools to fix program bugs.
% A recent study revealed that the bug fixing performance of ChatGPT is competitive with existing program repair approaches and providing hints in form of the expected output for a certain input or an observed error message can further increase the bug fixing performance~\cite{sobania2023analysis}. 
% %In order to use ChatGPT to repair tools, Xia et al~\cite{xia2023keep} proposed ChatRepair, which generate a patch by automated conversation-driven approach. 
% Different from all these existing studies, our study focus on the Web UI test repair problem that aims to perform UI test update by fixing broken locators. To the best of our knowledge, we are the first to investigate the quality of  explanations provided by ChatGPT and used matching rules to verify the reliability of the explanation to further improve the test repair performance. %existing studies performance of ChatGPT in testing and repair 
% %Since the repair of Web UI test cases strongly depends on changes in related webpage versions, existing work~\cite{xia2023keep} cannot be directly used in the repair of Web UI test cases.





% % while Yoon et al. 
% % use word and layout embedding to match elements [35].







% % Several model-based approaches to repair broken UI tests are proposed for Java applications [24,37], Web applications [8,14], and Android applications [7,11,21]. 





% %Large Language Models are Few-shot Testers: Exploring LLM-based General Bug Reproduction, test reproduction
% %Fill in the Blank: Context-aware Automated Text Input Generation for Mobile GUI Testing 

% % %There are many existing techniques that can automatically generate patches. We will discuss the relevance and differences between those techniques and \toolName in this section.

% % %Improving Locators Robustness,Automatic Test Case Repair, Automatic Page Objects Generation,Automatic Migration between Approaches


% % % To help developers backport patches, several approaches have been proposed~\cite{Ray2013,tian2012identifying}.
% % % Tian et al.~\cite{tian2012identifying} proposed an approach to automatically identify bug-fixing patches, that should be backported to old versions.
% % % Ray et al.~\cite{Ray2013} proposed to detect and characterize porting errors to help developers avoid them.
% % % In contrast, we directly backport patches and provide patch suggestions for developers.
% % % Another line of relevant work is the Backports Project~\cite{backport}, which enables old Linux kernels to run the latest drivers.
% % % The Backports Project develops a set of tools to automate the backporting process for Linux drivers~\cite{coccinelle, ferdian2016} to make them compilable with old kernel versions.
% % % The Backports Project uses the program matching and transformation tool Coccinelle~\cite{lawall2018coccinelle} to allow developers to express backporting transformation in a generic way that is expected to be applicable to many versions.
% % % In contrast, \toolName is fully automated and does not require manually created transformation rules.
% % % A prior approach by Thung et al.~\cite{ferdian2016} automatically extracts code transformation rules.
% % % However, this approach requires guidance from compilation errors, and it can only transform patches that affect a single line of code.

% % \noindent \textbf{Studies on \delete{W}\add{w}eb UI test maintenance.} 
% % Several studies investigated the characteristics of UI test maintenance for industrial \delete{W}\add{w}eb apps~\cite{leotta2013repairing, leotta2013improving,industry2}.
% % Prior studies of an industrial app (i.e., the Learning Content Management System) revealed that ID-based tests required less maintenance effort than the XPath-based ones~\cite{leotta2013repairing}, and recommended using page object pattern for improving test maintenance~\cite{leotta2013improving}. 
% % Meanwhile, IBM researchers described their experience of using ATA, an approach based on natural-language processing and backtracking exploration to automatically convert manual test steps in one enterprise web app to test cases for improving test automation~\cite{industry2}. 
% % We have analyzed the reasons why the \toolName cannot repair some test cases, and these reasons will guide future improvements in automated program repair.
% %     % Although our paper focuses on industrial apps, it differs from existing studies in several key aspects: (1) we focus on how to improve techniques for the automated repair of broken Web UI tests instead of other test maintenance tasks (e.g., test automation), (2) the characteristics of our industrial apps is different (our selected industrial apps are enterprise-level Web platforms for ICT and data analytic which are pretty complex), and (3) we include more industrial apps (we use one app for the study and \industryevalapp{} apps for our evaluation, whereas prior studies only use one app).

% % %
% % \noindent \textbf{Automatic UI Test Case Repair.}
% % In recent years, automated program repair~\cite{semfix, genprog, relifix, droix, fix2fit, extractfix, mechtaev2018test} has been widely explored to fix many kinds of bugs.
% % Meanwhile, to help testers fix broken UI test cases, many techniques have been proposed~\cite{choudhary2011water,waterfull,ATOM,CHATEM,sitar,stocco2018vista,xu2021guider,imtiaz2021automated,brisset2022erratum,Vifer,METER,10.1007/978-3-030-74296-6_29_WTSR,COLOR}. 
% % Most existing approaches fix broken tests by replacing outdated locators~\cite{choudhary2011water,stocco2018vista,xu2021guider,brisset2022erratum,Vifer,METER}. 
% % The number of successful repairs usually depends on the correct matching rate and can only fix crashes caused by locator changes.
% % Several model-based approaches are proposed for fixing broken UI tests for Java apps~\cite{memon2008automatically,ZhangLE2013}, \delete{W}\add{w}eb apps~\cite{10.1007/978-3-030-74296-6_29_WTSR,imtiaz2021automated}, and Android apps~\cite{sitar,ATOM,CHATEM}. 
% % To repair crashes in broken tests, these approaches usually rely on building a model (e.g., Event Flow Graph) and then picking a new path from the model to replace.
% % However, it is not easy to obtain accurate app models in real-world situations. 
% % Our experiment did not compare with any model-based approaches as they either fail to run~\cite{imtiaz2021automated} or are not publicly available~\cite{10.1007/978-3-030-74296-6_29_WTSR}. 
% % Instead of fixing broken locators, a multi-locator was proposed to strengthen test cases by selecting the best locator to use~\cite{multilocator}.
% % Our technique is inspired by the newly proposed \sftmtool~\cite{brisset2020sftm} matching algorithm, and our repair framework is adapted from the framework in \vistatool~\cite{stocco2018vista}.
% % Compared to these approaches, our approach improves the accuracy of matching UI elements, leading to more correct repairs. 
% % %GUIDER~\cite{xu2021guider} uses proposed an intent-based repair method to locate better where the error occurred. %For the restoration of new event types, Andrea Stocco et al.~\cite{stocco2018vista} used Crawljax to explore new events.
% % %android, Sitar,ATOM,CHATEM
% % %web ATOM

% % \noindent \textbf{Matching UI elements.} 
% % UI element matching are used for automated maintenance of test cases~\cite{xu2021guider,shao2021webevo,choudhary2011water,stocco2018vista}, automated compatibility testing~\cite{CdDiff}, and test reuse~\cite{10.1145/3460319.3464827}.
% % \watertool~\cite{choudhary2011water} relies on attribute information for matching . 
% % Meanwhile, more recent approach approaches~\cite{CdDiff,COLOR,shao2021webevo,METER,xu2021guider} use a combination of attributes and visual information to match elements. 
% % \vistatool~\cite{stocco2018vista} is a representative tool that focuses on matching elements using visual information, whereas Yoon et al. leverage word and layout embedding for matching elements~\cite{Vifer}.
% % Our iterative matching algorithm is most closely related to the \sftmtool algorithm~\cite{brisset2020sftm}, which utilizes structural information and attributes for matching. 
% % Nevertheless, our experiments %that compare four matching algorithms
% % show that \toolName{} outperforms all existing tools in matching accuracy.
% % % \paragraph{UI test augmentation.} 
% % %Leveraging existing tests in automated test generation for web applications



% % %\noindent \textbf{Improving Locators Robustness.} 
% % %Robust locator
% % %multi locator~\cite{multilocator}
% % %While algorithms exist to produce robust web element locators to be used in web test cases, no algorithm is perfect and different algorithms are exposed to different fragilities when the software evolves. Based on such observation, we propose a new type of locator, named multi-locator, which selects the best locator among a candidate set of locators produced by different algorithms. Such selection is based on a voting procedure that assigns different voting weights to different locator generation algorithms.




% % %\paragraph{Program Transformation.} Program transformation techniques infer transformation rules from human-written patches and transfer patches to another codebase by applying the inferred rules. Program transformation has been applied to many software maintenance tasks, including automating repetitive code edits~\cite{refazer, sydit, lase, molderez2017mining, nguyen2019graph}, intelligent refactoring~\cite{bluepencil, gao2020feedback} and fixing software bugs~\cite{phoenix, genesis, getafix}. Those approaches solve problems similar to \toolName, but there are key differences. Most existing works infer transformation rules from multiple human patches, while \toolName synthesizes rules from only one patch. Although \genpat~\cite{genpat} and \sydittool~\cite{sydit} also rely on only one example, they either require a large codebase to provide statistical information or synthesize rules by simply generalizing all identifiers, which results in many false positives, as also confirmed by our experiments on Linux.
% % %Second, some existing transformation techniques~\cite{phoenix, genesis, getafix} transform patches across different projects, and the others~\cite{bluepencil, gao2020feedback, lase, sydit} transform patches within the same codebase.
% % %In contrast, \toolName transforms patches across different versions of the same project. In contrast, \toolName leverages the similarity between Linux kernel versions to synthesize properly generalized transformation rules.

% % %\paragraph{Program Synthesis.} Program synthesis has been applied in many domains (e.g., string manipulation~\cite{flashfill}, fixing vulnerabilities~\cite{yu2016optimal}, and program transformation~\cite{refazer, bluepencil}). Syntax guided synthesis~\cite{alur2013syntax} (SyGuS) unifies synthesis tasks from different domains by specifying the domain-specific syntax and semantics of the desired program. SyGuS constructs programs using the given syntax and semantics with reference to given input-output examples. Sketching~\cite{solar2008sketching, solar2005programming} allows programmers to express their insight about an implementation as a partial program. %The synthesizer automatically completes the sketch to produce an implementation to match the given specification. These techniques have been used in many domains but they require detailed specifications given by multiple examples. In our setting, however, only one example is available. 
% % %Our partial synthesis allows us to synthesize high-quality transformation rule by considering the context where the synthesized program is applied.

% % %\paragraph{Program Repair.} Automated program repair approaches~\cite{apr} automatically fix software errors. Existing repair systems usually generate a patch space according to predefined templates~\cite{kim2013automatic,liu2019tbar,ghanbari2019practical,tan2018repairing}, then search for (or synthesize) the correct patch guided by a correctness specification given via test cases~\cite{le2011genprog,semfix13,prophet16,gao2019crash}. \toolName is not concerned with searching for, or generating a patch, but rather adapting a patch that is already available. %More importantly, \toolName does not rely on test cases, hence, it does not suffer from the test overfitting problem found in test-guided program repair~\cite{issta2015,smith2015cure}.  To patch Linux code, we cannot assume the existence of tests, and thus none of the test-based repair approaches are directly applicable.


==> sections/sections/replication.tex <==
\section*{Data Availability} 
To ensure reproducibility and advance future research in test repair, we made the dataset, scripts and experimental data publicly available on Github under an MIT license \cite{reproducibility}.
% https://anonymous.4open.science/r/ChatGPTWebUITestRepair-0D95/
% https://github.com/xuzhi2021/ChatGPTWebUITestRepair. \todo{need to update this to annonymous github}
% https://anonymous.4open.science/r/ChatGPTUITestRepair-7169.


==> sections/sections/rq1.tex <==
\section{RQ1: Effectiveness of UI Matching}
We evaluate the effectiveness of UI matching by calculating (1) the number of correct matches, and (2) ranking performance of the baselines. %(Section~\ref{sec:matchresult})
% , and (2) ranking performance of the baselines.  To compare the effectiveness  our approaches, we also evaluate two recent UI matching approaches (WebEvo and SFTM). \noindent\textbf{WebEvo:} \webevotool finishes element matching in three stages. First, nodes are considered similar if they share at least one attribute from id, class, or tag, with 70\% of their child nodes also matching. Next, WebEvo checks if the matched nodes have the same structure, tag names, text, and image URLs through comparing multiple historical web versions. Finally, for nodes filtered out from the second stage, it calculates text similarity using edit distance, followed by image similarity. In our experiments, we used the version of WebEvo implemented by \cite{uitestfix}, which includes only the third stage.
 %between nodes. Due to limited budget, we did not combine recent approaches with ChatGPT.%(Section~\ref{sec:rankresult}).

%can be used for guiding repair but
%we exclude these tools as we focus on UI test repair approaches. Moreover, WebEvo and SFTM already contain rematching processes that iteratively enhance their matching result, so we chose not to combine ChatGPT with them for additional matching refinements.
%\todo{add reasons for not comparing with WebEvo and SFTM: I have added some} 
%Specifically, WebEvo employs Dom tree based change detaction, history based semantic structure change detection, and semantics-based visual search to iteratively match elements.
%SFTM uses similarity-based approach and propagated the similarity scores iterat

\subsubsection{Matching Result and Analysis}
\label{sec:matchresult}


%\todo{add "application" column}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[]
% \caption{The matching and repair result of different methods}
% \label{table:matching_repair_result}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccccccc}
% \hline
% Method   & VISTA & VISTA+ChatGPT & WATER & WATER+ChatGPT & Edit Distance & Edit Distance+ChatGPT & Total \\ \hline
% Matching & 68& 97& 81& 86& 43& 122& 139\\
% Repair   & 67& 97& 81& 86& 43& 121& 139\\ \hline
% \end{tabular}%
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \label{table:matching_repair_result}
% \vspace{-6pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|rr|rr|rr|rr|rr|rr}
% \hline
% \multirow{2}{*}{Applications} & \multicolumn{2}{c|}{\vistatool}                                 & \multicolumn{2}{c|}{\vistatool+ChatGPT}                         & \multicolumn{2}{c|}{\watertool}                                 & \multicolumn{2}{c|}{\watertool+ChatGPT}                         & \multicolumn{2}{c|}{\edtool}                         & \multicolumn{2}{c}{\edtool+ChatGPT}                 \\ \cline{2-13} 
%                         & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r|}{Repair} & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r|}{Repair} & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r|}{Repair} & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r|}{Repair} & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r|}{Repair} & \multicolumn{1}{r}{Matching} & \multicolumn{1}{r}{Repair} \\ \hline
% AddressBook             & 1                            &                             1& 1                            & 1                           & 2                            &                             2& 2                            & 2                           & 0                            &                             0& 2                            & 2                           \\
% Claroline               & 48                           &                             47& \textbf{51}                           & \textbf{51}                          & 18                           &                             18& 18                           & 18                          & 1                            &                             1& 47                           & 47                          \\
% Collabtive              & 1&                             1& 1                            & 1                           & \textbf{10}                           &                             \textbf{10} & 7                            & 7                           & 8                            &                             8& 8                            & 8                           \\
% MantisBT                & 11                           &                             11& 37                           & 37                          & 50                           &                             50& 56                           & 56                          & 34                           &                             34& \textbf{63}                           & \textbf{62}                          \\
% MRBS                    & \textbf{7}                            &                             \textbf{7} & \textbf{7}                            & \textbf{7}                           & 1&                             1& 3                            & 3                           & 0                            &                             0& 2                            & 2                           \\ \hline
% Total                   & 68&                             67& 97                           & 97                          & 81                           &                             81& 86                           & 86                          & 43                           &                             43& \textbf{122}                          & \textbf{121}                         \\ \hline
% \end{tabular}
% }
% \end{table*}

% \todo{change order of the table}
% done

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \label{table:matching_repair_result}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|rr|rr|rr|rr|rr|rr|rr}
% \hline
% \multicolumn{1}{l|}{\multirow{2}{*}{Applications}} &
%   \multicolumn{2}{c|}{ChatGPT only} &
%   \multicolumn{2}{c|}{VISTA} &
%   \multicolumn{2}{c|}{VISTA+ChatGPT} &
%   \multicolumn{2}{c|}{WATER} &
%   \multicolumn{2}{c|}{WATER+ChatGPT} &
%   \multicolumn{2}{c|}{EDIT DISTANCE} &
%   \multicolumn{2}{c}{EDIT DISTANCE+ChatGPT} \\ \cline{2-15} 
% \multicolumn{1}{l|}{} &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair \\ \hline
% AddressBook & Error & N/A & 1          & 1          & 1           & 1           & 2           & 2           & 2  & 2  & 0  & 0  & 2            & 2            \\
% Claroline   & Error & N/A & 48         & 48         & \textbf{51} & \textbf{51} & 18          & 18          & 18 & 18 & 1  & 1  & 47           & 47           \\
% Collabtive  & Error & N/A & 1          & 1          & 1           & 1           & \textbf{10} & \textbf{10} & 7  & 7  & 8  & 8  & 8            & 8            \\
% MantisBT    & Error & N/A & 11         & 11         & 37          & 37          & 50          & 50          & 56 & 56 & 34 & 34 & \textbf{63}  & \textbf{62}  \\
% MRBS        & Error & N/A & \textbf{7} & \textbf{7} & \textbf{7}  & \textbf{7}  & 1           & 1           & 3  & 3  & 0  & 0  & 2            & 2            \\ \hline
% Total       & Error & N/A & 68         & 68         & 97          & 97          & 81          & 81          & 86 & 86 & 43 & 43 & \textbf{122} & \textbf{121} \\ \hline
% \end{tabular}%
% }
% \begin{tablenotes}
% \footnotesize
% \item{1} ``Error'' means all experiments fail due to exceeding the token limit. 
% \item{2} ``N/A'' indicates that experiment is not conducted due to no valid matching result.
% \end{tablenotes}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

%commented on 2024.9.22
% \begin{table*}[!htbp]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \setlength{\tabcolsep}{2pt}
% \label{table:matching_repair_result}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|rr|rr|rr|rr|rr|rr}
% \hline
% \multicolumn{1}{l|}{\multirow{2}{*}{Application}} &
%   \multicolumn{2}{c|}{VISTA} &
%   \multicolumn{2}{c|}{VISTA+ChatGPT} &
%   \multicolumn{2}{c|}{WATER} &
%   \multicolumn{2}{c|}{WATER+ChatGPT} &
%   \multicolumn{2}{c|}{EDIT DISTANCE} &
% %  \multicolumn{2}{c}{EDIT DISTANCE+ChatGPT} \\ \cline{2-13} 
%     \multicolumn{2}{c}{EDIT+ChatGPT} \\ \cline{2-13} 
% \multicolumn{1}{l|}{} &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair &
%   Matching &
%   Repair \\ \hline
% AddressBook & 1          & 1          & 1           & 1           & 2           & 2           & 2  & 2  & 0  & 0  & 2            & 2            \\
% Claroline   & 48         & 47         & \textbf{51} & \textbf{51} & 18          & 18          & 18 & 18 & 1  & 1  & 47           & 47           \\
% Collabtive  & 1          & 1          & 1           & 1           & \textbf{10} & \textbf{10} & 7  & 7  & 8  & 8  & 8            & 8            \\
% MantisBT    & 11         & 11         & 37          & 37          & 50          & 50          & 56 & 56 & 34 & 34 & \textbf{63}  & \textbf{62}  \\
% MRBS        & \textbf{7} & \textbf{7} & \textbf{7}  & \textbf{7}  & 1           & 1           & 3  & 3  & 0  & 0  & 2            & 2            \\ \hline
% Total       & 68         & 67         & 97          & 97          & 81          & 81          & 86 & 86 & 43 & 43 & \textbf{122} & \textbf{121} \\ \hline
% \end{tabular}%
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \setlength{\tabcolsep}{2pt}
% \label{table:matching_repair_result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{r|r|r||r|r|r|r|r|rr}
% \hline
% &\multicolumn{2}{c||}{Re-matching Approaches} & \multicolumn{7}{c}{Baselines and Combination Approaches} \\\hline
% %& WebEvo                & SFTM               &  &  &  \\
% \multirow{2}{*}{Applications} & \multicolumn{1}{c|}{WebEvo} & \multicolumn{1}{c||}{SFTM} & \multicolumn{1}{c|}{VISTA} & \multicolumn{1}{c|}{VISTA+ChatGPT} & \multicolumn{1}{c|}{WATER} & \multicolumn{1}{c|}{WATER+ChatGPT} & \multicolumn{1}{c|}{EDIT DISTANCE} & \multicolumn{2}{c}{EDIT DIS+ChatGPT} \\
%                               & Matching            & Matching         & Matching / Repair          & Matching / Repair                  & Matching / Repair          & Matching / Repair                  & Matching / Repair                  & Matching          & Repair           \\ \hline
% AddressBook                   & 0                           & 2                         & 1                          & 1                                  & 2                          & 2                                  & 0                                  & 2                 & 2                \\
% Claroline                     & 14                          & 15                        & 48                         & \textbf{51}                        & 18                         & 18                                 & 1                                  & 47                & 47               \\
% Collabtive                    & 5                           & 5                         & 1                          & 1                                  & \textbf{10}                & 7                                  & 8                                  & 8                 & 8                \\
% MantisBT                      & 53                          & 44                        & 11                         & 37                                 & 50                         & 56                                 & 34                                 & \textbf{63}       & \textbf{62}      \\
% MRBS                          & 2                           & 5                         & \textbf{7}                 & \textbf{7}                         & 1                          & 3                                  & 0                                  & 2                 & 2                \\\hline
% Total                         & 74                          & 71                        & 68                         & 97                                 & 81                         & 86                                 & 43                                 & \textbf{122}      & \textbf{121}     \\ \hline
% \end{tabular}
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \setlength{\tabcolsep}{2pt}
% \label{table:matching_repair_result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{r|rr|rrrrrrrrrrrr}
% \hline
% \multicolumn{1}{l|}{\multirow{3}{*}{Applications}} & \multicolumn{2}{l|}{Recent Tools}                   & \multicolumn{12}{c}{Baselines and Combination Approaches (with self-correction)}                                                                                                                                                                                                                                                                                                                                \\ \cline{2-15} 
% \multicolumn{1}{l|}{}                              & \multicolumn{1}{c|}{WebEvo}   & \multicolumn{1}{c|}{SFTM}     & \multicolumn{2}{c|}{VISTA}                                     & \multicolumn{2}{c|}{VISTA+ChatGPT}                              & \multicolumn{2}{c|}{WATER}                                      & \multicolumn{2}{c|}{WATER+ChatGPT}                         & \multicolumn{2}{c|}{EDIT DIS}                              & \multicolumn{2}{c}{EDIT DIS+ChatGPT}                      \\
% \multicolumn{1}{l|}{}                              & \multicolumn{1}{c|}{Matching} & \multicolumn{1}{c|}{Matching} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Repair}     & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Repair}      & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Repair}      & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Repair} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Repair} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c}{Repair} \\ \hline
% AddressBook                                        & \multicolumn{1}{r|}{0}        & 2                             & 1                            & \multicolumn{1}{r|}{1}          & 1                            & \multicolumn{1}{r|}{1}           & 2                            & \multicolumn{1}{r|}{2}           & 2                            & \multicolumn{1}{r|}{2}      & 0                            & \multicolumn{1}{r|}{0}      & 2                            & 2                          \\
% Claroline                                          & \multicolumn{1}{r|}{14}       & 15                            & 48                           & \multicolumn{1}{r|}{48}         & \textbf{51}                  & \multicolumn{1}{r|}{\textbf{51}} & 18                           & \multicolumn{1}{r|}{18}          & 18                           & \multicolumn{1}{r|}{18}     & 1                            & \multicolumn{1}{r|}{1}      & 47                           & 47                         \\
% Collabtive                                         & \multicolumn{1}{r|}{5}        & 5                             & 1                            & \multicolumn{1}{r|}{1}          & 1                            & \multicolumn{1}{r|}{1}           & {10}                  & \multicolumn{1}{r|}{10} & {\textbf{11}}                            & \multicolumn{1}{r|}{\textbf{11}}      & 8                            & \multicolumn{1}{r|}{8}      & 8                            & 8                          \\
% MantisBT                                           & \multicolumn{1}{r|}{53}       & 44                            & 11                           & \multicolumn{1}{r|}{11}         & 37                           & \multicolumn{1}{r|}{37}          & 50                           & \multicolumn{1}{r|}{50}          & 56                           & \multicolumn{1}{r|}{56}     & 34                           & \multicolumn{1}{r|}{34}     & \textbf{64}                  & \textbf{63}                \\
% MRBS                                               & \multicolumn{1}{r|}{2}        & 5                             & \textbf{7}                   & \multicolumn{1}{r|}{\textbf{7}} & \textbf{7}                   & \multicolumn{1}{r|}{\textbf{7}}  & 1                            & \multicolumn{1}{r|}{1}           & 4                            & \multicolumn{1}{r|}{4}      & 0                            & \multicolumn{1}{r|}{0}      & 2                            & 2                          \\\hline
% Total                                              & \multicolumn{1}{r|}{74}       & 71                            & 68                           & \multicolumn{1}{r|}{68}         & 97                           & \multicolumn{1}{r|}{97}          & 81                           & \multicolumn{1}{r|}{81}          & 91                           & \multicolumn{1}{r|}{91}     & 43                           & \multicolumn{1}{r|}{43}     & \textbf{123}                 & \textbf{122}               \\ \hline
% \end{tabular}
% }
% \end{table*}





% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \setlength{\tabcolsep}{2pt}
% \label{table:matching_repair_result}
% \resizebox{1\linewidth}{!}{
% \centering
% \begin{tabular}{c|cccc|cccccccccccc}
% \hline
% \multirow{3}{*}{Applications} & \multicolumn{4}{c|}{Recent Approaches}                             & \multicolumn{12}{c}{Baselines and Combination Approaches (with self-correction)}                                                                                                                                                                  \\ \cline{2-17} 
%                               & \multicolumn{2}{c|}{WebEvo}            & \multicolumn{2}{c|}{SFTM} & \multicolumn{2}{c|}{VISTA}             & \multicolumn{2}{c|}{VISTA+ChatGPT}     & \multicolumn{2}{c|}{WATER}             & \multicolumn{2}{c|}{WATER+ChatGPT}     & \multicolumn{2}{c|}{EDIT DIS}          & \multicolumn{2}{c}{EDIT DIS+ChatGPT} \\
%                               & Matching & \multicolumn{1}{c|}{Repair} & Matching     & Repair     & Matching & \multicolumn{1}{c|}{Repair} & Matching & \multicolumn{1}{c|}{Repair} & Matching & \multicolumn{1}{c|}{Repair} & Matching & \multicolumn{1}{c|}{Repair} & Matching & \multicolumn{1}{c|}{Repair} & Matching           & Repair          \\ \hline
% AddressBook                   & 0        & \multicolumn{1}{c|}{0}      & 2            & 2          & 1        & \multicolumn{1}{c|}{1}      & 1        & \multicolumn{1}{c|}{1}      & 2        & \multicolumn{1}{c|}{2}      & 2        & \multicolumn{1}{c|}{2}      & 0        & \multicolumn{1}{c|}{0}      & 2                  & 2               \\
% Claroline                     & 14       & \multicolumn{1}{c|}{14}     & 15           & 15         & 48       & \multicolumn{1}{c|}{48}     & 51       & \multicolumn{1}{c|}{51}     & 18       & \multicolumn{1}{c|}{18}     & 18       & \multicolumn{1}{c|}{18}     & 1        & \multicolumn{1}{c|}{1}      & 47                 & 47              \\
% Collabtive                    & 5        & \multicolumn{1}{c|}{5}      & 5            & 5          & 1        & \multicolumn{1}{c|}{1}      & 1        & \multicolumn{1}{c|}{1}      & 10       & \multicolumn{1}{c|}{10}     & 11       & \multicolumn{1}{c|}{11}     & 8        & \multicolumn{1}{c|}{8}      & 8                  & 8               \\
% MantisBT                      & 53       & \multicolumn{1}{c|}{53}     & 44           & 44         & 11       & \multicolumn{1}{c|}{11}     & 37       & \multicolumn{1}{c|}{37}     & 50       & \multicolumn{1}{c|}{50}     & 56       & \multicolumn{1}{c|}{56}     & 34       & \multicolumn{1}{c|}{34}     & 64                 & 63              \\
% MRBS                          & 2        & \multicolumn{1}{c|}{2}      & 5            & 5          & 7        & \multicolumn{1}{c|}{7}      & 7        & \multicolumn{1}{c|}{7}      & 1        & \multicolumn{1}{c|}{1}      & 4        & \multicolumn{1}{c|}{4}      & 0        & \multicolumn{1}{c|}{0}      & 2                  & 2               \\ \hline
% Total                         & 74       & \multicolumn{1}{c|}{74}     & 71           & 71         & 68       & \multicolumn{1}{c|}{68}     & 97       & \multicolumn{1}{c|}{97}     & 81       & \multicolumn{1}{c|}{81}     & 91       & \multicolumn{1}{c|}{91}     & 43       & \multicolumn{1}{c|}{43}     & 123                & 122             \\ \hline
% \end{tabular}
% }
% \end{table*}



% \begin{table*}[]
% \caption{The number of correct matching and the number of correct repairs of different approaches}
% \setlength{\tabcolsep}{2pt}
% \label{table:matching_repair_result}
% \resizebox{1\linewidth}{!}{
% \centering
% \begin{tabular}{c|cccc|cccccccccccc}
% \hline
% \multirow{3}{*}{Applications} & \multicolumn{4}{c|}{Recent Approaches}                          & \multicolumn{12}{c}{Baselines and Combination Approaches (with self-correction)}                                                                                                                                                                                  \\ \cline{2-17} 
%                               & \multicolumn{2}{c|}{WebEvo}         & \multicolumn{2}{c|}{SFTM} & \multicolumn{2}{c|}{VISTA}                   & \multicolumn{2}{c|}{VISTA+ChatGPT}             & \multicolumn{2}{c|}{WATER}          & \multicolumn{2}{c|}{WATER+ChatGPT}             & \multicolumn{2}{c|}{EDIT DIS}       & \multicolumn{2}{c}{EDIT DIS+ChatGPT} \\
%                               & Matching & \multicolumn{1}{c|}{Fix} & Matching       & Fix      & Matching  & \multicolumn{1}{c|}{Fix}        & Matching    & \multicolumn{1}{c|}{Fix}         & Matching & \multicolumn{1}{c|}{Fix} & Matching    & \multicolumn{1}{c|}{Fix}         & Matching & \multicolumn{1}{c|}{Fix} & Matching          & Fix              \\ \hline
% AddressBook                   & 0        & \multicolumn{1}{c|}{0}   & 2              & 2        & 1          & \multicolumn{1}{c|}{1}          & 1           & \multicolumn{1}{c|}{1}           & 2        & \multicolumn{1}{c|}{2}   & 2           & \multicolumn{1}{c|}{2}           & 0        & \multicolumn{1}{c|}{0}   & 2                 & 2                \\
% Claroline                     & 14       & \multicolumn{1}{c|}{14}  & 15             & 15       & 48         & \multicolumn{1}{c|}{48}         & \textbf{51} & \multicolumn{1}{c|}{\textbf{51}} & 18       & \multicolumn{1}{c|}{18}  & 18          & \multicolumn{1}{c|}{18}          & 1        & \multicolumn{1}{c|}{1}   & 47                & 47               \\
% Collabtive                    & 5        & \multicolumn{1}{c|}{5}   & 5              & 5        & 1          & \multicolumn{1}{c|}{1}          & 1           & \multicolumn{1}{c|}{1}           & 10       & \multicolumn{1}{c|}{10}  & \textbf{11} & \multicolumn{1}{c|}{\textbf{11}} & 8        & \multicolumn{1}{c|}{8}   & 8                 & 8                \\
% MantisBT                      & 53       & \multicolumn{1}{c|}{53}  & 44             & 44       & 11         & \multicolumn{1}{c|}{11}         & 37          & \multicolumn{1}{c|}{37}          & 50       & \multicolumn{1}{c|}{50}  & 56          & \multicolumn{1}{c|}{56}          & 34       & \multicolumn{1}{c|}{34}  & \textbf{64}       & \textbf{63}      \\
% MRBS                          & 2        & \multicolumn{1}{c|}{2}   & 5              & 5        & \textbf{7} & \multicolumn{1}{c|}{\textbf{7}} & \textbf{7}  & \multicolumn{1}{c|}{\textbf{7}}  & 1        & \multicolumn{1}{c|}{1}   & 4           & \multicolumn{1}{c|}{4}           & 0        & \multicolumn{1}{c|}{0}   & 2                 & 2                \\ \hline
% Total                         & 74       & \multicolumn{1}{c|}{74}  & 71             & 71       & 68         & \multicolumn{1}{c|}{68}         & 97          & \multicolumn{1}{c|}{97}          & 81       & \multicolumn{1}{c|}{81}  & 91          & \multicolumn{1}{c|}{91}          & 43       & \multicolumn{1}{c|}{43}  & \textbf{123}      & \textbf{122}     \\ \hline
% \end{tabular}
% }
% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{The number of correct matching and repairs of different approaches. Bold values indicate the best performance.}
\setlength{\tabcolsep}{2pt}
\label{table:matching_repair_result}
\resizebox{1\linewidth}{!}{
\centering
\begin{tabular}{l|rrrr|rrrrrrrrrrrr}
\hline
\multirow{3}{*}{Applications} & \multicolumn{4}{c|}{Recent Approaches}                                                                            & \multicolumn{12}{c}{Baselines and Combination Approaches (with self-correction)}                                                                                                                                                                                                                                                                                                       \\ \cline{2-17} 
                              & \multicolumn{2}{c|}{WebEvo}                             & \multicolumn{2}{c|}{SFTM}                               & \multicolumn{2}{c|}{VISTA}                                     & \multicolumn{2}{c|}{VISTA+ChatGPT}                              & \multicolumn{2}{c|}{WATER}                                     & \multicolumn{2}{c|}{WATER+ChatGPT}                              & \multicolumn{2}{c|}{EDIT DIS}                           & \multicolumn{2}{c}{EDIT DIS+ChatGPT}                   \\
                              & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix}        & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix}         & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix}        & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix}         & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c|}{Fix} & \multicolumn{1}{c}{Matching} & \multicolumn{1}{c}{Fix} \\ \hline
AddressBook                   & 0                            & \multicolumn{1}{r|}{0}   & \textbf{2}                   & \textbf{2}               & 1                            & \multicolumn{1}{r|}{1}          & 1                            & \multicolumn{1}{r|}{1}           & \textbf{2}                   & \multicolumn{1}{r|}{\textbf{2}} & \textbf{2}                   & \multicolumn{1}{r|}{\textbf{2}}  & 0                            & \multicolumn{1}{r|}{0}   & \textbf{2}                   & \textbf{2}              \\
Claroline                     & 14                           & \multicolumn{1}{r|}{14}  & 15                           & 15                       & 48                           & \multicolumn{1}{r|}{48}         & \textbf{51}                  & \multicolumn{1}{r|}{\textbf{51}} & 18                           & \multicolumn{1}{r|}{18}         & 18                           & \multicolumn{1}{r|}{18}          & 1                            & \multicolumn{1}{r|}{1}   & 47                           & 47                      \\
Collabtive                    & 5                            & \multicolumn{1}{r|}{5}   & 5                            & 5                        & 1                            & \multicolumn{1}{r|}{1}          & 1                            & \multicolumn{1}{r|}{1}           & 10                           & \multicolumn{1}{r|}{10}         & \textbf{11}                  & \multicolumn{1}{r|}{\textbf{11}} & 8                            & \multicolumn{1}{r|}{8}   & 8                            & 8                       \\
MantisBT                      & 53                           & \multicolumn{1}{r|}{53}  & 44                           & 44                       & 11                           & \multicolumn{1}{r|}{11}         & 37                           & \multicolumn{1}{r|}{37}          & 50                           & \multicolumn{1}{r|}{50}         & 56                           & \multicolumn{1}{r|}{56}          & 34                           & \multicolumn{1}{r|}{34}  & \textbf{64}                  & \textbf{63}             \\
MRBS                          & 2                            & \multicolumn{1}{r|}{2}   & 5                            & 5                        & \textbf{7}                   & \multicolumn{1}{r|}{\textbf{7}} & \textbf{7}                   & \multicolumn{1}{r|}{\textbf{7}}  & 1                            & \multicolumn{1}{r|}{1}          & 4                            & \multicolumn{1}{r|}{4}           & 0                            & \multicolumn{1}{r|}{0}   & 2                            & 2                       \\ \hline
Total                         & 74                           & \multicolumn{1}{r|}{74}  & 71                           & 71                       & 68                           & \multicolumn{1}{r|}{68}         & 97                           & \multicolumn{1}{r|}{97}          & 81                           & \multicolumn{1}{r|}{81}         & 91                           & \multicolumn{1}{r|}{91}          & 43                           & \multicolumn{1}{r|}{43}  & \textbf{123}                 & \textbf{122}            \\ \hline
\end{tabular}
}
\end{table*}


% \todo{refer to the blog about not using more syllabus than you should, change "as well as"} 
We evaluate a total of eight matching
% \todo{change this number and the description if want to add webevo and sftm}
approaches, including individual baselines (\vistatool, \watertool, \edtool), their combinations with ChatGPT, and two recent approaches. For each approach, we recorded its abilities to correctly match the ground truth elements of the broken statements in our dataset. 
The ``Matching'' columns in Table~\ref{table:matching_repair_result} show the results on the evaluated applications. 
% All results of ChatGPT only are marked as ``Error'' due to matching prompts exceeding the token limit (averaging around 21733 tokens), resulting in the error message ``This model's maximum context length is 4097 tokens. However, your messages resulted in x tokens. Please reduce the length of the messages.'' 
Comparing the overall matching results of individual baselines with their combination with ChatGPT (with self-correction), we observe that all combinations outperform the individual baseline (i.e., 97 versus 68 for \vistatool, 91 versus 81 for \watertool, and 123 versus 43 for \edtool{}). This result confirms our hypothesis that combining prior test repair approaches with ChatGPT help improve the UI matching results. 
% Although adding ChatGPT does not improve for some cases, there is only one project (Collabtive) where \watertool+ChatGPT performed worse than \watertool\todo{can you check why this case happen and add an explanation}. 
Across projects, the improvement is greatest in MantisBT with \vistatool+ChatGPT and \watertool+ChatGPT, in Claroline with \edtool{}. Meanwhile, \edtool{}+ChatGPT outperformed \edtool{} in most projects, including AddressBook, Caroline, and MRBS. For the recent approaches, Table~\ref{table:matching_repair_result} shows that the \webevotool and \sftmtool{} give similar matching results (74 and 71) that are slightly better than the two individual baselines (\vistatool{} and \edtool{}). However, both recent approaches perform worse than all the combination approaches, indicating that the combination with LLMs like ChatGPT can further enhance the matching accuracy of traditional approaches (\watertool{} and \vistatool{}). 
%\todo{Add one sentence: Meanwhile, we notice that the two iterative matching tools perform similarly with \vistatool{}}
%(AddressBook, Caroline (47 versus 1), and MRBS).



%For \vistatool, the performance is better when combined with ChatGPT. After combining with ChatGPT, it matches 30 broken statements that originally could not be matched and 67 broken statements that could originally be matched, without matching any originally matchable broken statements incorrectly.
% It  misses 3 originally matchable broken statements, with 64 broken statements still correctly matched. These matching failures are due to similar candidates confuse ChatGPT and ChatGPT select a similar one but not the most similar one. The selected elements are parent or ancestor elements of the most similar element, which means the ChatGPT just may not match accurately when there are multiple elements that are very similar to the target. The reason why \vistatool{} combined with ChatGPT fail to increase the correct matching is due to the limitation of the \vistatool's candidates selection method, which will be introduced in the next subsection.

%For WATER, combining with ChatGPT has both advantages and disadvantages. Combining with ChatGPT results in matching 8 additional broken statements, with 78 broken statements still correctly matched, but 3 originally matchable broken statements are now missed. 
%\todo{xzl: add the the failure reason}

\begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]

\textbf{Finding 1:} All combinations of prior Web test repair approaches with ChatGPT performs generally better than the corresponding standalone approach (without ChatGPT). %helps to improve the UI matching results for all the evaluated approaches. 

\textbf{Implication 1:} Our suggested workflow of using prior repair tools for selecting candidate elements and then ChatGPT for subsequent matching help improve the matching accuracy. %of UI matching.

\end{tcolorbox}
We notice that \vistatool{}'s matching algorithm using visual information is effective for certain apps (e.g., Claroline and MRBS). However, \edtool{}+ChatGPT performs the best among all approaches, fixing 122 out of a total of 139 broken statements. 
Specifically, \edtool{}+ChatGPT yields the greatest improvement (186\%) over the individual \edtool{} approach. After combining with ChatGPT, it correctly matches 80 elements that were originally mismatched and ensures that nearly all initially correctly matched statements remain correct (42).
Given that the individual \edtool{} performs the worst among all baselines,
we think this result is counterintuitive as one would select the tool that performs well individually (i.e., \watertool) to combine with ChatGPT to get more improvement.  %surprising improvement compared to Edit Distance. 

% \todo{xzl: add the description about cases that only ED+ChatGPT can match correctly}
%  no case can only be matched correctly by ed+chatgpt

\begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]
\textbf{Finding 2:} Although the individual \edtool{} approach performs the worst among all individual baselines, its combination with ChatGPT outperforms all evaluated approaches. %helps to improve the UI matching results for all the evaluated approaches. 

\textbf{Implication 2:} \edtool{} %, a simplified variant of \watertool, 
combines well with ChatGPT. %compared to other combinations. 
By prioritizing only XPath similarity, it is more effective in guiding ChatGPT for subsequent matching. %using other attributes. %delegates responsibility of matching other attributes to ChatGPT for subsequent matching. %its pre-trained data.    
\end{tcolorbox}

\noindent\textbf{Effectiveness of the standalone ChatGPT (ChatGPT only).} 
Another natural baseline approach will be to use the standalone ChatGPT for performing all the matching and repair steps. Hence, we also check the effectiveness of standalone ChatGPT by providing all UI elements as candidates instead of using a selection algorithm to choose 10 of them. However, all the prompts throw errors due to the token limit being exceeded for all cases. This is expected as for a Webpage in our dataset, there are an average of 224 UI elements to be matched where attribute information for each element occupies around 101 tokens. The average number of tokens (224*101=21733) also shows the high cost of the standalone ChatGPT.

\subsubsection{Ranking performance of the baselines}
\label{sec:rankresult}
As the combination of \edtool{}+ChatGPT outperforms all other approaches, we investigate the reasons behind the improvement. Specifically, as \watertool{} and \vistatool{} originally return only one element as the best matching result, we analyze the ranking performance of each baseline approach.
Given a selected element $s_e$ by a tool $t$ and the correct element $t_e$ (i.e., the corresponding element in the ground truth), we consider $t$ \emph{hits} if $s_e$ is exactly the same as $t_e$. 
%The prerequisite for ChatGPT to select the matched element correctly is that the given candidate lists contain ground truth elements. Therefore, we analyzed whether each candidate list contain the ground truth. If the ground truth is included in the candidate list, 
If one of the elements in ranked list produced by a tool $t$ hits, 
we record its ranking to evaluate the ranking performance.
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/content/Method_Comparison_Hit_Rates.pdf}
    
     \caption{Comparison of Hit Ratios for the three baselines}
   % \caption{Comparison of ground truth Hit Ratios for the three baselines}$
    \label{Hit Rates}
\end{figure}
We employ metrics commonly used in evaluating top-N recommendation task~\cite{Hit_Ratio_old}: Top-K Hit Ratio (HR, or Recall, in this study, the proportion of experimental instances in which the top N candidates selected by each baseline contain ground truth in the candidate list). Figure ~\ref{Hit Rates} depicts the variation of Hit Ratio with increasing values of N for the three baselines. %each of the three candidate selection methods. %are illustrated (Figure ~\ref{Hit Rates}).
% \todo{change everything to "hits" instead of covering ground truth}
% done
We observe several interesting trends in Figure~\ref{Hit Rates}:  1) When N=1, the Hit Ratio for \vistatool{} and \watertool{} is already around 50\%, while \edtool{}'s is only 30.9\%. This indicates that the top candidate of \vistatool{} and \watertool{} already effectively hits ground truth, whereas \edtool's advantage is less evident. 2) As N increases, the Hit Ratios for \vistatool{} and \watertool{} increase slowly. Even at N=10, their Hit Ratios only increase by less than 25\% compared to when N is 1. In contrast, \edtool{}'s Hit Ratio gradually increases, reaching 68.3\%, 84.2\%, and 90.1\% when N is 5, 9, and 10, respectively. Hence, if expanding the number of selected candidates to the top 10 in the candidate list, \edtool{} is more likely to hit the ground truth element compared to \vistatool{} and \watertool{}, leading to more potential improvement when combined with ChatGPT.


\section{RQ2: Effectiveness and Efficiency of Repair}
Before checking for the repair correctness of each repaired statement, we first check if ChatGPT has the correct matching result for the broken statement because a correct repair can only be generated after a correct matching. %.element information. 
%If the element matching is correct, we further validate the repair correctness. %evaluate the chosen locator and the corresponding element information to confirm the correctness of the repair.  
 

\noindent\textbf{Repair Correctness.} As the ground truth repaired statements written by developers of the Web apps are unavailable in our dataset, and the repaired statements generated by ChatGPT may have diverse but semantically-equivalent fixes, we need to manually validate the correctness of all generated repaired statements. To reduce the manual effort in validation, we use a semi-automated approach. Specifically, given the original broken statement $o$, the repaired statement $r$, and the ground truth element $e$, we design a parser that automatically parses the locator type (e.g., \texttt{By.name} and \texttt{By.xpath}), and the expression within the locator (e.g., the XPath value) in the repaired statement $r$ to verify their correctness with respect to the ground truth element $e$. For example, if ChatGPT uses \texttt{By.xpath} as the locator, it should use the XPath information of $e$ rather than the value of other attributes. Our parser also identifies cases requiring manual analysis where more substantial changes have been introduced by ChatGPT, including (1) different types of locators between $o$ and $r$, and (2) additional statements added to the repaired statement $r$. %Then, we manually validate the repair correctness. 

%is valid (syntax and values if it is correct), update assertion if update.    check validity of locator expression, other modifications manually check and value.  
%\todo{how to check repair}
The ``Fix'' columns in
Table \ref{table:matching_repair_result} shows the repair results for all approaches. The results of the combination approaches (with self-correction) are not only the best results 
across the four runs, on average, \vistatool{}+ChatGPT, \watertool{}+ChatGPT, and \edtool+ChatGPT achieve success in 2.17, 2.01, and 2.89 runs out of 4, respectively, indicating consistent performance across different runs.
From Table \ref{table:matching_repair_result}, we can observe that the number of correct repair is almost equal to the number of correct matching, except for one case in \edtool+ChatGPT. 
% \vistatool{} fails to repair one statement in Claroline after correctly matching the element as it currently does not support the repair of assertion values~\cite{vista}.
For MantisBT, \edtool+ChatGPT correctly matches a element but generates a repair that modifies the original intention of the broken statement. Specifically, the broken statement sends an empty text input ``'' to the element, but \edtool's repaired statement sends ``Test'' to the element. %The case that \edtool matched correctly but repair incorrectly is because originally the broken statement sends ``'' to the element, but \edtool's repaired statement sends ``Test'' to the element, which change the intent of original test statement.
Nevertheless, \edtool+ChatGPT still excels with the best performance (122 correct repairs).

\noindent\textbf{Repair Efficiency.} 
% As ChatGPT has been used to perform subsequent matching, one concern may be that it may incur overhead and increase the overall time taken for finding the repair. Hence, we measure the \emph{repair efficiency} by measuring the overall time taken for the entire matching and repair workflow. 
To assess potential delays from using ChatGPT, we measured the total time for matching and repair for each broken statement.
 On average, \webevotool takes \SI{45.73}{s}, \sftmtool{} takes \SI{47.98}{s}, \vistatool{} takes \SI{36.91}{s}, \vistatool{}+ChatGPT \SI{41.44}{s}, \watertool{} takes \SI{30.22}{s}, \watertool+ChatGPT \SI{35.11}{s}, \edtool{} \SI{24.02}{s}, and \edtool{}+ChatGPT \SI{28.17}{s} per broken statement. Approaches involving \vistatool{} and \webevotool are more time-consuming because \vistatool{} uses computer vision techniques for matching, which takes more time than matching textual information. \sftmtool{} takes more time because it iteratively propagates and refines the similarity scores during matching process. Overall, ChatGPT adds minimal overhead.


\begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]

\textbf{Finding 3:} The repair effectiveness is mostly similar to the matching effectiveness (except for one incorrect repair). %with one exception of incorrect repair. %due to the limitation of the tool (i.e., \vistatool) and repair that modify the original intention of the statements (i.e., \edtool{}+ChatGPT). %helps to improve the UI matching results for all the evaluated approaches. 

% \textbf{Implication 3:} With correct matching elements, most approaches could repair correctly. For one case, we identify some limitations of evaluated approaches, including lack of diverse fix patterns (\vistatool) and introducing non-intention perserving changes (\edtool{}+ChatGPT).   
\textbf{Implication 3:} Using correctly matched elements, most approaches could repair correctly. %For one case, we identify the limitation of introducing non-intention preserving changes (\edtool{}+ChatGPT). 
%\edtool{}, a simplified variant of a prior test repair approach (\watertool) integrates well with ChatGPT compared to other combinations. By ranking elements using only XPath similarity, \edtool{} delegates the responsibility of matching using other attributes to ChatGPT which can later perform better global view matching. %its pre-trained data.    

\end{tcolorbox}

%\vistatool repairs wrongly on one broken statement with correct matching result because \vistatool does not support repair of assertion values~\cite{vista}.
%\yuanzhang{Why do some methods have different results?Why would one test case not be fixed correctly?}

% \noindent\textbf{Fix Patterns used by ChatGPT.}
% Our prompt directs ChatGPT to only modify the locator and outdated assertion in the broken statement based on the matching elements for preserving the original intention of the test.
% For example, actions like changing a click operation to entering text on the element should not happen.
% During the manual validation of the repair result, we examine both the correctness of the repaired locator and the content outside the locator. To investigate the diversity of the generated repairs, we manually analyze and derive some common fix patterns used by ChatGPT. %through delving into some instances.\yuanzhang{Choose another reason.
% Overall, we found five fix patterns in the repair of ChatGPT, described below: %only modify locator values, use different locating methods, add statements, modify assertions values, modify assertion method and values. All repairs should contain modify locator values.








% \noindent\textbf{Single statement change: Modify locator values .} 73.61\% of correct repairs share this fix pattern. Figure~\ref{listing:repairs1} shows an example of ChatGPT generated repair where it modifies the value of the locator for updating the values of the XPath. 

% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.xpath("//*[@id=\"content\"]
% - /form[2]/div[4]/input")).click();
% + driver.findElement(By.xpath("/html[1]/body[1]/div
% + [1]/div[4]/form[2]/div[3]/input[1]")).click();  
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in AddressBook that only modifies the value of locator.}
% \label{listing:repairs1}
% \vspace{-6pt}
% \end{figure}
% % water2, TestAssignGroup_44, Addressbook, only modify locator value

% \noindent\textbf{Single statement change: Modify assertion values.} Figure~\ref{listing:repairs2} shows an example of ChatGPT generated repair where it modifies the value of the assertion for updating the values of the XPath. 
% % As \vistatool{} does not currently support update of assertion values, 
% % ChatGPT could help \vistatool{} in generating repaired statement that use more diverse fix patterns in this case. 
% We observe that 13.82\% correct repairs involve assertion. In 7.79\% of these cases, ChatGPT modified assertion values to update outdated expected values. 


% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - assertEquals(driver.findElement(By.xpath("//div[
% - @id='claroBody']/div[2]/div")).getText(),  
% - "This username is already taken");
% + assertEquals(driver.findElement(By.xpath("/html
% + [1]/body[1]/div[1]/div[2]/div[1]/div[2]")). 
% + getText(), "This user name is already taken");
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in Claroline that changes the assertion value for XPath update.}
% \label{listing:repairs2}
% \vspace{-6pt}
% \end{figure}
% % vista2, TestAddUserTwice_86, claroline, modify assertion value


% \noindent\textbf{Single statement change: Use different assertions and values.} Figure~\ref{listing:repairs3} shows an example of ChatGPT generated repair where it uses a different type of assertion (replacing \texttt{assertEquals} with \texttt{assertTrue}) and assertion value (update the XPath). In this case, the statement that replaces \texttt{assertTrue} with \texttt{assertEquals} preserves the semantic of assertion as the original statement still invoke \texttt{.equals()} within the assertion. %We think that ChatGPT suggested this repair because \texttt{assertEquals}  
% In 10.39\% of correct repairs that involve assertions, ChatGPT used different assertions. %from the broken statements.


% % There are 18 cases where broken statement is an assertion. Considering all the repair results of three approaches and each approach containing 4 results, we have 216 cases where broken statement is an assertion.

% % ChatGPT uses different assertions in 23 cases out of them (10.65\%).
% % out of all repair results

% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - Assert.assertTrue(driver.findElement(By.xpath("//
% - *[@id=\"loginBox\"]/h3")).getText().equals
% - ("Authentication"));
% + Assert.assertEquals("Authentication",driver.
% + findElement(By.xpath("/html[1]/body[1]/div[1]/div
% + [2]/div[1]/div[1]/div[1]/div[1]")).getText());
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in Claroline that uses different assertions (replacing \texttt{assertEquals} with \texttt{assertTrue}) and assertion value (update XPath).}
% \label{listing:repairs3}
% \vspace{-6pt}
% \end{figure}
% % water0, TestLoginLogout_35, claroline, modify assertion method and value


% \noindent\textbf{Single statement change: Use different locators and values.} Figure~\ref{listing:repair} shows an example of ChatGPT generated repair where it uses a different type of locator (replacing \texttt{By.name} with \texttt{By.xpath}) and locator value (update the XPath). 
% Compared to other locators (\texttt{By.name} and \texttt{By.className}), we observe that most broken statements tend to use \texttt{By.xpath} locators (70.50\%). Among the generated correct repair, we observed that ChatGPT often use ``By.xpath'' when updating the broken locator (99.82\%).  
%  %70.50\% of locators are \texttt{By.xpath}
% %Moreover, ChatGPT also used \texttt{By.name} and \texttt{By.className} once separately (0.09\% and 0.09\%). 
% % 3 kinds of locators are used by ChatGPT, not considering whether the locator is different from that of broken statement. The next paragraph is about changing the locator
% In 26.39\% correct repair, ChatGPT changed the locators and values. Among these cases, we only observe one case where ChatGPT changes \texttt{By.xpath} into another locator (\texttt{By.className}). For the remaining cases, ChatGPT replaces other locators with \texttt{By.xpath}.

% % regardless of the original locator of the broken statement (70.50\% of the broken statements\todo{this may be outdated information, check if this is correct}   in the dataset were initially located by ``By.xpath''). ChatGPT also uses \texttt{By.id}, \texttt{By.name}, \texttt{By.className}, \texttt{By.linkText} methods when repairing, with frequency of 1.69\%, 0.24\%, 0.18\% and 0.006\%.
% %\sh{TODO: check if this is correct}.  %In this case, the statement that replaces \texttt{assertTrue} with \texttt{assertEquals} preserves the semantic of assertion as the original statement still invoke \texttt{.equals()} within the assertion.

% % ChatGPT uses different types of locator in 29.65\% cases.
% % out of all repair result

% \noindent\textbf{Multi-statements change: Add statements and modify locators.} 1.26\% of correct repairs have multi-statements changes. Figure~\ref{listing:repairs6} shows an example of ChatGPT generated repair where (1) it stores the element into a temporary variable \texttt{element}, (2) performs the click action on the variable, and (3) add an assertion to check for the validity of the text of the element. Since the test where the broken statement is located has other assertion that serves as test oracle, adding the assertions is unnecessary in this example. However, this example demonstrates the ability of ChatGPT in generating assertions which could be helpful for test case generation.   %\todo{use the old example for addition of statement as this example is a bit trivial}



% % ChatGPT generates multiple statements in 16 cases (0.97\%).
% % out of all repair results


% % \begin{figure}[!th]
% % \centering
% % \begin{lstlisting}[style=mystyle, escapechar=^]
% % - driver.findElement(By.xpath("/html/body/div[7]/a[1]
% % -   /table/tbody/tr[2]/td/form/input[4]")).click();
% % + WebElement element = driver.findElement(By.xpath("/html/
% % +   body/div[6]/a[1]/table/tbody/tr[2]/td/form/input[4]"));
% % + element.click();
% % \end{lstlisting}
% % \vspace{-6pt}
% % \caption{A ChatGPT generated repair for the broken statement in MantisBT that adds an additional statement that stores the element in a temporary variable.}
% % \label{listing:repairs4}
% % \vspace{-6pt}
% % \end{figure}
% % % xpath0, UpdateCategoryEmptyTest_46, mantisbt, add statement

% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.xpath("//div[@id='claroBody
% - ']/div[2]/div")).click();
% + WebElement element = driver.findElement(By.xpath(
% + "/html[1]/body[1]/div[1]/div[2]/div[1]/div[1]"));
% + element.click();
% + String actualText = element.getText();
% + String expectedText = "The new user has been 
% + sucessfully created";
% + assertEquals(expectedText, actualText);
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT generated fix for the broken statement in Claroline that adds statements.}
% \label{listing:repairs6}
% \vspace{-6pt}
% \end{figure}
% % TestAddAdmin66, water0



%Our findings indicate that ChatGPT successfully repairs all the locator with the correct element information when the element matching is accurate. Notably, we observed that ChatGPT often use ``By.xpath'' when updating the broken locator, regardless of the original locator of the broken statement (70.5\% of the broken statements in the dataset were initially located by ``By.xpath''). Figure~\ref{listing:repair} shows the example for the repair result where ChatGPT uses ``By.name'' as the locator\todo{modify the code listing to add a code example}, which is the same as that of the original broken statement. \sh{TODO: check if this is correct}. 

%\subsubsection{Repair Patterns for Other Parts of the Statement}



% In exploring ChatGPT's performance in preserving the original test intent of test statements, we found two kinds of surprising modification. 

% The first case that ChatGPT modifies the part outside the locator is updating expected values in assertions based on matching element's information. 
% This modification is not universal; among the 139 broken statements, 17 are assertion-related, all tasked with validating whether the text of selected element aligns with the anticipated value.
% The methods VISTA+ChatGPT, WATER+ChatGPT, and Edit Distance+ChatGPT yield four instances of this case.
% In three of these instances, all the methods rectify the expected value of the broken statement in line 48 of Claroline's test cases ``TestEditZone'' by changing ``The changes have been carried out correctly\textbackslash n + textzone\_top.inc.html'' to ``The changes have been carried out correctly textzone\_top.inc.htm''. Although the changed text equals to the text information of the matching element, this repaired statement still fails. The problem occurs in extracting element information with Jsoup. Even though the documentation says Jsoup will add ``\textbackslash n`` before <br> tag which is adding two new lines in the final text and we try Jsoup's new version on it, we still cannot get the ``\textbackslash n`` in this case. Consequently, the number of successful fixes for WATER+ChatGPT is one less than the number of accurate matches.

% For VISTA+ChatGPT and Edit Distance+ChatGPT, they fail to achieve a correct match since they did not accurately match the correct element in the previous step, even though the text and ground truth of the matched element are the same. In these cases, the number of correct matching and correct repair are not different because of this assertion modification.

% Another instance of altering the assertion's expected value occurs when Edit Distance+ChatGPT transforms "This username is already taken" into "This user name is already taken." This modification aligns with the information of matching element as well, rendering the change reasonable and successful.

% However, the one case that Edit Distance+ChatGPT successfully matches the element but fail to repair the broken statement happens when ChatGPT neglects to update the assertion's expected value where such an update is warranted. Specifically, "New users will receive an e-mail with their username and password" should have been updated to "New users will receive an e-mail with their user name and password," but ChatGPT did not effect this change based on the text of the matching element. Because our prompt only direct ChatGPT to update the locator, ChatGPT did not check all assertion's expected value. It also turns out that only 2 of 17 assertions have outdated expected values that need to be updated. However, if testers desire such modification, they can add corresponding instructions to upate the expected value of assertions.


% In the other case of changing the original test statement intent, ChatGPT repaired ``driver.findElement(...).click();'' with ``driver.switchTo().frame(driver.findElement(...));''. But this is reasonable because it incorrectly selects an iframe element as the result of element match and the iframe element itself doesn't support the ``.click()'' action. Ifram element is a container instead of an interactable object. If ChatGPT only change the locator to click on this iframe element, the repaired statement would throw NoSuchElementException~\cite{selenium-docs}. To operate on an element inside an iframe, we need to switch to the context of the iframe first, i.e., execute ``driver.switchTo(iframe element);'' in a similar way to switch windows, and then driver can find the specific element inside the iframe and and manipulate it. However, ChatGPT only has the selected iframe element so it can only generate the repair statement that switch to this iframe. ChatGPT does not have the element information which should be operated on insider the iframe so it only generate the switch statement as repaired result. 

==> sections/sections/rq2.tex <==
\section{RQ3: Quality of ChatGPT's Explanation}% on Matching Result}
%\todo{modify table according to 4 answers, EC should be changed to correct rate because it is different from explanation consistency. Is it the latest one?}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[ht]
% \centering
% \setlength{\tabcolsep}{1.4pt}
% \small
% \caption{Effectiveness of SC Mechanism: ``M'' represents the number of times an attribute is mentioned and ``C'' denotes the number of times where the mentioned attribute is consistent in the generated explanation for each approach}
% \label{table:explanation}
% \resizebox{0.9\linewidth}{!}{%
% \small
% \begin{tabular}{c|rr|rr|rr|rr|rr|rr|rr|rr|rr|rr}
% \hline
% \multirow{2}{*}{Approach} &
%   \multicolumn{2}{c|}{id} &
%   \multicolumn{2}{c|}{name} &
%   \multicolumn{2}{c|}{class} &
%   \multicolumn{2}{c|}{XPath} &
%   \multicolumn{2}{c|}{text} &
%   \multicolumn{2}{c|}{tagName} & 
%   \multicolumn{2}{c|}{linkText} &
%   \multicolumn{2}{c|}{position} &
%   \multicolumn{2}{c|}{size} &
%   \multicolumn{2}{c}{isLeaf} \\ \cline{2-21} 
%  &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} & 
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c|}{M} &
%   \multicolumn{1}{c}{C} &
%   \multicolumn{1}{c}{M} \\ \hline
% \vistatool{}         & 1& 16& 11& 30& 98& 111& 304& 542& 392& 498& 390& 412& 111&122& 74& 201& 113& 201& 164& 169
% \\
% \watertool{}         & 12& 122& 28& 55& 148& 161& 254& 555& 346& 484& 299& 410& 176&192& 154& 221& 213& 221& 201& 201
% \\
% \edtool{} & 121& 121& 23& 131& 159& 164& 291& 556& 452& 510& 316& 347& 126&149& 128& 306& 179& 304& 178& 179
% \\ \hline
% Total& 134& 259& 62& 216& 405& 436& 849& \textbf{1653}& \textbf{1190}& 1492& 1005& 1169& 413&463& 356& 728& 505& 726& 543& 549\\ \hline
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[ht]
% \centering
% \setlength{\tabcolsep}{1.4pt}
% \small
% \caption{Effectiveness of SC Mechanism: ``M'' represents the number of times an attribute is mentioned and ``C'' denotes the number of times where the mentioned attribute is consistent in the generated explanation for each approach}
% \label{table:explanation}
% \resizebox{1\linewidth}{!}{%
% \small
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \hline
% \multirow{2}{*}{Approach} & \multicolumn{2}{c|}{id} & \multicolumn{2}{c|}{name} & \multicolumn{2}{c|}{class} & \multicolumn{2}{c|}{XPath} & \multicolumn{2}{c|}{text} & \multicolumn{2}{c|}{tagName} & \multicolumn{2}{c|}{linkText} & \multicolumn{2}{c|}{position} & \multicolumn{2}{c|}{size} & \multicolumn{2}{c}{isLeaf} \\ \cline{2-21} 
%                           & C          & M          & C           & M           & C            & M           & C       & M                & C                & M      & C            & M             & C             & M             & C             & M             & C           & M           & C            & M           \\ \hline
% VISTA+ChatGPT             & 10         & 35         & 21          & 50          & 112          & 146         & 393     & 590              & 302              & 497    & 368          & 424           & 115           & 135           & 85            & 217           & 131         & 218         & 175          & 188         \\
% WATER+ChatGPT             & 14         & 25         & 40          & 75          & 116          & 152         & 276     & 547              & 362              & 498    & 360          & 367           & 180           & 203           & 157           & 241           & 226         & 241         & 212          & 215         \\
% EDIT DIS+ChatGPT          & 25         & 28         & 24          & 29          & 123          & 144         & 326     & 523              & 362              & 467    & 267          & 309           & 126           & 160           & 137           & 251           & 186         & 249         & 191          & 197         \\ \hline
% Total                     & 49         & 88         & 85          & 154         & 351          & 442         & 995     & \textbf{1660}    & \textbf{1026}    & 1462   & 995          & 1100          & 421           & 498           & 379           & 709           & 543         & 708         & 578          & 600         \\ \hline
% \end{tabular}
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{1.4pt}
\small
\caption{Effectiveness of SC Mechanism: ``M'' represents the number of times an attribute is mentioned and ``C'' denotes the number of times where the mentioned attribute is consistent in the generated explanation for each approach}
\label{table:explanation}
\resizebox{1\linewidth}{!}{%
\small
\begin{tabular}{l|rr|rr|rr|rr|rr|rr|rr|rr|rr|rr}
\hline
\multirow{2}{*}{Approach} & \multicolumn{2}{c|}{id}                        & \multicolumn{2}{c|}{name}                      & \multicolumn{2}{c|}{class}                     & \multicolumn{2}{c|}{XPath}                     & \multicolumn{2}{c|}{text}                      & \multicolumn{2}{c|}{tagName}                   & \multicolumn{2}{c|}{linkText}                  & \multicolumn{2}{c|}{position}                  & \multicolumn{2}{c|}{size}                      & \multicolumn{2}{c}{isLeaf}                    \\ \cline{2-21} 
                          & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{M} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{M} \\ \hline
VISTA+ChatGPT             & 10                    & 35                     & 21                    & 50                     & 112                   & 146                    & 393                   & 590                    & 302                   & 497                    & 368                   & 424                    & 115                   & 135                    & 85                    & 217                    & 131                   & 218                    & 175                   & 188                   \\
WATER+ChatGPT             & 14                    & 25                     & 40                    & 75                     & 116                   & 152                    & 276                   & 547                    & 362                   & 498                    & 360                   & 367                    & 180                   & 203                    & 157                   & 241                    & 226                   & 241                    & 212                   & 215                   \\
EDIT DIS+ChatGPT          & 25                    & 28                     & 24                    & 29                     & 123                   & 144                    & 326                   & 523                    & 362                   & 467                    & 267                   & 309                    & 126                   & 160                    & 137                   & 251                    & 186                   & 249                    & 191                   & 197                   \\ \hline
Total                     & 49                    & 88                     & 85                    & 154                    & 351                   & 442                    & 995                   & \textbf{1660}          & \textbf{1026}         & 1462                   & 995                   & 1100                   & 421                   & 498                    & 379                   & 709                    & 543                   & 708                    & 578                   & 600                   \\ \hline
\end{tabular}
}
\end{table*}


% To assess the quality of ChatGPT's explanations for element matching results, we employ two metrics: 
% \[
% Mention \ Rate(a)=\frac{mention(a)}{|explanations|}
% \]

% \[
% Explanation\ Reliability (a)=\frac{mention_{correct}(a)}{\sum_{n=1} ^{explanation} \ mention(a)}
% \]

% the \textbf{mention rate} (the number of times ChatGPT mentions a certain attribute in its explanations divided by the total number of experiments) and the \textbf{correct rate} (the number of times ChatGPT mentions a certain attribute in its explanations and the selected element's attribute is indeed similar to the target element, divided by the total number of times ChatGPT mentions that attribute). These metrics are used to evaluate ChatGPT's tendency to mention various attributes during element matching and the degree of alignment between ChatGPT's explanations and the actual circumstances.
As our study uses explanation to overcome hallucination, it is important to investigate its quality.
To assess the quality of ChatGPT's explanations for element matching results, we use two metrics: (1) \emph{mention frequency} (the number of times where an attribute $a$ has been mentioned $M$), and (2) \emph{mention consistency} (the number of times where an attribute $a$ has been consistently mentioned $C$ where the consistency is determined by our explanation validator described in Section~\ref{sec:evalidate}). These two metrics helps in answering the research questions below:
%We denote the explanation as $e$ and attribute as $a$.

\begin{description}[leftmargin=*]
\item[RQ3a:] What are the frequently mentioned attributes in ChatGPT's explanation?
\item[RQ3b:] What are the mentioned attributes that are consistent in ChatGPT's explanation?
\end{description}

%The first metric $M$ (number of times where an attribute has been mentioned in ChatGPT's generated explanation) will help us to understand the attributes that are frequently used by ChatGPT for matching, whereas the second metric $C$ will  %we define mention rate $M$ as the number of times ChatGPT mentions a attribute in its explanations divided by the total number of explanations. Formally, for given a attribute $a$

%To assess the quality of ChatGPT's explanations for element matching results, we use two metrics: (1) Mention Rate $MR$, and (2) Explanation consistency $EC$. We denote the explanation as $e$ and attribute as $a$. To understand which attributes are frequently used by ChatGPT for matching, we define mention rate $MR$ as the number of times ChatGPT mentions a attribute in its explanations divided by the total number of explanations.
%Formally, for given a attribute $a$
%\begin{equation*}
%\label{equ:mention-rate}
%\begin{aligned}
%MR(a)=\frac{|\{e|a \in e\}|}{|\{e\}|}
%\end{aligned}
%\end{equation*}

%Furthermore, to evaluate the degree of consistency between ChatGPT’s explanations and the actual circumstances, explanation consistency $EC$\todo{change to correct rate/attribute correctness} is used to evaluate the correctness of ChatGPT's explanation. 
%$EC$ is defined as:
%\begin{equation*}
%\label{equ:explanation-rate}
%CR(a)=\frac{|\{e|a \in e \wedge  %cons(a)\}|}{|\{e| a \in e\}|}
%\end{equation*}
%where cons() means the explanation about attribute $a$ is consistent with the actual circumstances.
%\yuanzhang{It seems that there is no explanation on how to judge whether it is consistent (correct).}



Table~\ref{table:explanation} presents the mention frequency and mention consistency of ChatGPT for each attribute. Table~\ref{table:explanation} shows that ChatGPT mentions two attributes most frequently: \emph{XPath} (1660) and \emph{text} (1462), whereas the least mentioned attribute is \emph{id} (88). Compared to the priority imposed by prior test repair approaches (shown in Table~\ref{tab:attribute}), this result shows that ChatGPT has certain preferences towards particular attributes since it often mention the \emph{XPath} and \emph{text} attributes regardless of the baseline used for selecting the list of candidate elements.
\vspace{-0.1cm}
\begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]
%\vspace{-0.1cm}
\textbf{Finding 4:} ChatGPT frequently mentions the  the \emph{XPath} and \emph{text} attributes in the provided explanations.

\textbf{Implication 4:} Similar to other approaches that have certain priority, ChatGPT %has preferences towards the 
prioritizes
\emph{XPath} and \emph{text} attributes. 
%\vspace{-0.1cm}
\end{tcolorbox}


%\vspace{-0.6cm}
Table~\ref{table:explanation} also shows the attributes with the greatest mention consistency are \emph{text} (1026), \emph{XPath} (995), and \emph{tagName} (995). 
Although ChatGPT prefers using \emph{XPath} (1660) and \emph{text} (1462) for matching, our results show that
prioritizing the \emph{text} attribute over the \emph{XPath} attribute will lead to better matching results (as the \emph{text} attribute is mentioned more consistently).
%\vspace{-0.5cm}

\begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]

\textbf{Finding 5:} The most frequently mentioned attribute by ChatGPT (i.e., XPath) tends to lead to incorrect matching (low mentioned consistency). In contrast, the \emph{text} attribute is high in mention frequency and mention consistency.

\textbf{Implication 5:} Prioritizing the \emph{text} attribute over \emph{XPath} attribute is better for ChatGPT as it will be more accurate. %matching.
%\vspace{-0.1cm}
\end{tcolorbox} 
%Conversely, the attribute \emph{name} (62)
% \yz{href}
% linkTex
%shows the least accurate correspondence (53\%). %\textit{XPath} (99\%) and text (85\%), while the least mentioned attribute is name (13\%). The three attributes that ChatGPT's explanations most accurately correspond to the actual situation are isLeaf (97\%), class (93\%), and linkText (93\%). Conversely, the attribute id 
% \yz{href}
% linkTextshows the least accurate correspondence (53\%). 

%\textit{XPath} is the attribute most frequently mentioned in ChatGPT's explanations, being referenced in almost every explanation. However, upon examination, the accuracy of such explanations is not high, reaching only 57\%. In contrast, the attributes class, linkText, size and isLeaf are seldom mentioned by ChatGPT (about 30\%), but their explanation correct rates reach about 90\%. Attributes text and tagName, despite being frequently mentioned (85\% and 67\%, respectively), exhibit relatively high explanation accuracy (above 80\%). On the other hand, attributes id and name 
% \yz{href} 
%\todo{lqs: change all the "href" into "linktext"?}are rarely mentioned by ChatGPT (less than 15\%), and their explanation correct rates are also not high (53\% and 54\%, respectively). 



\noindent\textbf{Correlation between EC and correctness of the matching.} 
% Our explanation validator measures the explanation consistency (EC) to check and improve the reliability of the matching results of ChatGPT. 
Our explanation validator measures the explanation consistency (EC) as a mechanism to check and improve the reliability of ChatGPT's matching results. However, even if our explanation validator can accurately assess EC, it does not guarantee correct matching (i.e., retrieving the target element in the labeled ground truth). To investigate the correlation between our proposed EC and the \emph{correctness of the final matching result} (i.e., whether it selects the ground truth element), we measure the correlation between these two variables. 
%it is essential to verify the correlation between EC and ``whether the element in ground truth is selected'' for each explanation. 
As the two variables are binary (correctness) and continuous (EC between 0 and 1) categories respectively, we compute the Point-Biserial Correlation Coefficient ($r_{pbi}$)~\cite{tate1954correlation} for all explanations. As this is a special case of the Pearson Correlation, we assess the strength of the relationship by %evaluating the numerical value of 
calculating
the correlation coefficient. 

For the three combinations with ChatGPT, the values for the Point-Biserial Correlation Coefficient are: $r_{pbi}$=0.51 for \vistatool{}+ChatGPT, $r_{pbi}$=0.84 for \watertool{}+ChatGPT, and $r_{pbi}$=0.49 for \edtool{}+ChatGPT. These values indicate that EC and the matching correctness for \vistatool{}+ChatGPT and \edtool{}+ChatGPT are only moderately correlated but \emph{strongly correlated for the \watertool{}+ChatGPT combination}. %The strong correlation between EC and \watertool{}+ChatGPT's correctness of the matching implies that our explanation validator will be the most effective in improving the matching results for the \watertool{}+ChatGPT combination among all evaluated combinations.
%We think that the strong correlation between EC and \watertool{}+ChatGPT's correctness of the matching is due to the design of \watertool{}'s UI matching algorithm that considers more diverse set of attributes compared to \vistatool{} and \edtool{} (as shown in Table~\ref{tab:attribute}) and these attributes may be mentioned in the explanation provided by ChatGPT. 

%can be attributed to the results that the combination of \watertool{}+ChatGPT gives the least improvement over the vanilla \watertool{}.  

%\todo{Add a table or figure to include the correlations. what is the correlation value and what does the value indicate?}
%经统计，VISTA, WATER, and Edit Distance各自的相关性为0.32, 0.85, and 0.48.

 \begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]

\textbf{Finding 6:} %Among all combinations, 
EC for \watertool{}+ChatGPT strongly correlates with matching correctness among all combinations.

\textbf{Implication 6:}
The strong correlation shows that our explanation validator %and generated self-correction prompt
is the most effective for \watertool{}+ChatGPT to improve its matching correctness.

\end{tcolorbox}
% \begin{table*}[]
% \caption{The mention rate of each attributes and candidate list}
% \label{table:mention rate}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccccccllll}
% \hline
% Candidates List&
%   \multicolumn{1}{l}{id} &
%   \multicolumn{1}{l}{name} &
%   \multicolumn{1}{l}{text} &
%   \multicolumn{1}{l}{tagName} &
%   \multicolumn{1}{l}{linkText} &
%   \multicolumn{1}{l}{size} &  XPath& location&isLeaf &Average\\ \hline
% VISTA& 0.02 & 0.04 & 0.83 & 0.71 & 0.04 & 0.13 & 0.98 & 0.13 & 0.37 &0.36 
% \\
% WATER& 0.23 & 0.10 & 0.79 & 0.67 & 0.22 & 0.16 & 1.00 & 0.16 & 0.16 &0.39 
% \\
% XPath& 0.22 & 0.21 & 0.93 & 0.58 & 0.17 & 0.14 & 1.00 & 0.14 & 0.16 &0.39 
% \\ \hline
% Average& 0.16 & 0.12 & 0.85 & 0.65 & 0.15 & 0.14 & 0.99 & 0.14 & 0.23 &0.38 \\ \hline
% \end{tabular}%
% }
% \end{table*}



% \begin{table*}[]
% \caption{The correct rate of each attributes and candidate list}
% \label{table:correct rate}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccccccllll}
% \hline
% Candidates List&
%   \multicolumn{1}{l}{id} &
%   \multicolumn{1}{l}{name} &
%   \multicolumn{1}{l}{text} &
%   \multicolumn{1}{l}{tagName} &
%   \multicolumn{1}{l}{linkText} &
%   \multicolumn{1}{l}{size} &  XPath& location&isLeaf &Average\\ \hline
% VISTA& 0.33 & 0.17 & 0.68 & 0.70 & 0.67 & 0.94 & 0.49 & 0.39 & 0.76 &0.57 
% \\
% WATER& 0.09 & 0.64 & 0.58 & 0.47 & 1.00 & 0.59 & 0.44 & 1.00 & 0.86 &0.63 
% \\
% XPath& 1.00 & 0.07 & 0.66 & 0.82 & 1.00 & 0.63 & 0.58 & 0.79 & 0.82 &0.71 
% \\ \hline
% Average& 0.48 & 0.29 & 0.64 & 0.67 & 0.89 & 0.72 & 0.50 & 0.73 & 0.82 &0.64 \\ \hline
% \end{tabular}%
% }
% \end{table*}



==> sections/sections/rq3.tex <==
% \section{RQ3: ChatGPT's Effectiveness on Repair}
\section{RQ4: Ablation study for the SC mechanism}%Improving reliability of ChatGPT's generated explanation}


% \begin{table}[h!]
% \setlength{\tabcolsep}{1.2pt}
% \caption{The results before and after self-correction (SC)}
% %\caption{The matching and repair results before and after self-correction (SC)}
% \label{table:scr_result}
% \small
%  \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|cc|cc|cc|}
% \hline
% \multirow{2}{*}{Approach} & \multicolumn{2}{c|}{\vistatool{}+ChatGPT} & \multicolumn{2}{c|}{\watertool{}+ChatGPT} & \multicolumn{2}{c|}{\edtool{}+ChatGPT} \\ \cline{2-7} 
%                  & before SC & after SC & before SC & after SC & before SC & after SC \\ \hline
% Matching & 97        & 97       & 86        & 91       & 122       & 123      \\
% % Average EC       &           &          &           &          &           &          \\
% Repair           & 97        & 97       & 86        & 91       & 121       & 122      \\ \hline
% \end{tabular}%
%  }
% %\vspace{-0.5cm}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\setlength{\tabcolsep}{1.2pt}
\caption{The results before and after self-correction (SC)}
%\caption{The matching and repair results before and after self-correction (SC)}
\label{table:scr_result}
\small
 \resizebox{\linewidth}{!}{%
\begin{tabular}{|l|cr|cr|cr|}
\hline
\multirow{2}{*}{Approach} & \multicolumn{2}{c|}{\vistatool{}+ChatGPT} & \multicolumn{2}{c|}{\watertool{}+ChatGPT} & \multicolumn{2}{c|}{\edtool{}+ChatGPT} \\ \cline{2-7} 
                          & before SC                & \multicolumn{1}{c|}{after SC}   & before SC                & \multicolumn{1}{c|}{after SC}   & before SC               & \multicolumn{1}{c|}{after SC} \\ \hline
Matching                  & \multicolumn{1}{r}{97}   & 97                              & \multicolumn{1}{r}{86}   & 91                              & \multicolumn{1}{r}{122} & 123                           \\
Repair                    & \multicolumn{1}{r}{97}   & 97                              & \multicolumn{1}{r}{86}   & 91                              & \multicolumn{1}{r}{121} & 122                           \\ \hline
\end{tabular}
}
\end{table}


% \begin{figure}[!th]
% \centering
% \begin{lstlisting}[style=mystyle, escapechar=^]
% - driver.findElement(By.xpath("/html/body/form/input[3]"))
% -   .click();
% + driver.findElement(By.xpath("/html[1]/body[1]/div[2]/
% +   form[1]/fieldset[1]/input[3]")).click(); //result 1
% + driver.findElement(By.xpath("/html/body/div[2]/form
% +   /fieldset/div[3]/input")).click();  //result 2 
% \end{lstlisting}
% \vspace{-6pt}
% \caption{A ChatGPT fix for the broken statement in MRBS that shows the effectiveness of self-correction.}
% \label{listing:sc_example}
% \vspace{-6pt}
% \end{figure}
% water0, HelpTest_33, MRBS, only modify locator value




% ``Because they share the most similar attributes: xpath, text, tagName, linkText, x, y, width, height, isLeaf.''. The explanation of attributes text, linkText and location are inconsistent with the selection and the EC value is 0.57.

% After self-correction, the explanation of selection is ``Because they share the most similar attributes: xpath, text, tagName, linkText, location, size, isLeaf.'' and EC value is



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \caption{The matching results and explanation consistency before and after self-correct}
% \label{table:scr_result}
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{|c|cc|cc|cc|}
% \hline
% \multirow{2}{*}{Approach} & \multicolumn{2}{c|}{VISTA+ChatGPT} & \multicolumn{2}{c|}{WATER+ChatGPT} & \multicolumn{2}{c|}{XPath+ChatGPT} \\ \cline{2-7} 
%                           & before SC        & after SC        & before SC        & after SC        & before SC        & after SC        \\ \hline
% Matching          & 64               & 66              & 86               & 87              & 122              & 120             \\ 
% Average EC                & 0.73             & 0.80            & 0.73             & 0.75            & 0.80             & 0.82            \\ \hline
% \end{tabular}}
% \end{table}
%表X显示了VISTA, WATER, XPath三种工具结合ChatGPT后，分别进行self correct (SC)前后的正确匹配与平均explanation consistency (EC)的结果对比。在计算EC平均值时，是先计算出每个broken statement的EC，然后对所有broken statement的EC取平均值。可以看出，经过SC，所有approach的平均EC都有了提升，而除了XPath+ChatGPT之外的approach的正确匹配数量也有了提升。之所以XPath+ChatGPT在SC后的平均EC的升高没有伴随着正确匹配数量的升高，可能是因为根据SC前的计算结果，二者的相关性本来就只是接近moderate positive correlation （0.48）。

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}


As the self-correction (SC) mechanism was the key in the design of our proposed combination, we conduct an ablation study in RQ4 to evaluate the effectiveness of this mechanism. %whether this mechanism leads to improvement of the matching and repair results. 
Specifically, we count and compare the number of correct matches and repairs before and after the self-correction.
%When computing the average EC, we first calculate the EC for each broken statement and then determine the mean across all broken statements.
%We can observe that after SC, the average EC for all approaches has improved. 
Table \ref{table:scr_result} presents the results of the three approaches combined with ChatGPT before and after self-correction (SC), comparing the correct matches and average explanation consistency (EC). %The ``M'' columns in the table represents the number of times an attribute is mentioned, whereas ``C'' columns denotes the number of times where the mentioned attribute is consistent in the generated explanation for each approach.
Except for \edtool+ChatGPT, the number of correct matches has increased for the other approaches. Notably, \watertool{}+ChatGPT shows the most significant improvement, gaining 5 more correct matches and repairs after self-correction (SC). Meanwhile, we think that \edtool+ChatGPT does not show any improvement due to the moderately positive correlation between EC and matching accuracy (0.49). %observed based on the pre-SC computation results. %We think that \edtool+ChatGPT does not show an increase in the number of correct matches despite the rise in average EC after SC might be attributed to the moderate positive correlation (0.48) observed based on the pre-SC computation results.

\ignorespaces

\ignorespaces
  \begin{tcolorbox}[left=0pt,right=0pt,top=0pt,bottom=0pt]

\textbf{Finding 7:} The improvement given by self-correction varies across tools. Among the three combinations, \watertool{} benefits the most (5 more correct matching after correction).

\textbf{Implication 7:}
Our proposed workflow of %explanation consistency and 
guiding ChatGPT via self-correct prompt %as hints to ChatGPT %to improve the reliability of its explanation 
improves the effectiveness of certain combinations (e.g., \watertool{}+ChatGPT). %benefit approach like \watertool{}+ChatGPT.

\end{tcolorbox}




==> sections/sections/threats.tex <==
\section{threats to validity}
% We didn't try all possible configurations, the performance of codex model and repair tools may varies in different settings, e.g., larger max tokens

\noindent \textbf{External Threats.} During the ground truth construction and evaluating our way of calculating EC, we mitigate potential bias by asking two annotators to manually construct and cross-validate the ``ground truth target element and patch''. The two annotators met to resolve any disagreement during the annotation, and further discussed until a consensus was reached. To reduce bias in selection of Web applications, we evaluate on a widely used dataset. As with prior evaluations, our findings may not generalize beyond the selected applications and tests in the dataset. 
 To encourage future research in Web UI element matching and repair, we also release our dataset. Due to limited resources and budget, we use the cost-effective GPT 3.5-Turbo model which may be less effective than newer models in Web test repair. Nevertheless, the extended input of a ChatGPT with a larger token limit (e.g., ChatGPT-16k) may still be insufficient for representing UI elements because for a Webpage, there are an average of 224 elements to be matched where the attribute information for each element occupies 101 tokens, 224*101=22624 tokens. %(exceed 16k). 
 As ChatGPT performance may vary across settings, our experiments may not generalize beyond the studied settings, and fixing other forms of UI tests (we focus on Java Selenium Web UI tests~\cite{shariff2019improving}).
% \todo{check if we are only limited to Java Selenium Web UI tests} 
% done
We mitigate this threat by reusing settings and suggestions in prior work (e.g., referring to OpenAI documentation for prompt design and using temperature 0.8 as in prior work ~\cite{fan2023automated}), and evaluating several test repair tools that use different algorithms (e.g., text-based and visual-based). As our study only evaluates the test repair capability of ChatGPT, the findings may not apply for other LLMs. Nevertheless, our suggested workflow of using LLMs to perform subsequent matching and rematching based on inconsistent explanations are still generally applicable. %as the proposed workflow is orthogonal to any LLMs.  %As the underlying algorithm used in Codex-e has not been documented, we only use it as a black-box APR tool that produces patches by editing existing programs. To ensure that the training data does not overlap with the evaluated tasks, we have confirmed with the developer of Codex-e that Codex and Codex-e use the same dataset for training. Nevertheless, our experiments show that Codex-e is able to generate fixes for many incorrect solutions. %e.g., larger max tokens

\noindent\textbf{Internal Threats.} Our experimental scripts may have bugs that can affect our results. To mitigate this threat, we made our scripts and results publicly available \cite{reproducibility}.
% \url{https://github.com/xuzhi2021/ChatGPTUITestRepair}.
% \url{https://anonymous.4open.science/r/ChatGPTWebUITestRepair-0D95/}.


%\noindent\textbf{Construct Threats.} Construct threats may arise when our evaluation metric of the number of correctly fixed solutions/tasks may be too coarse-grained to reflect the effectiveness of APR. Nevertheless, we followed the same metrics used by APR research and recent code generation research. 
%(we also check the dataset to ensure only the old UI tests are available in GitHub) \todo{check if the ground updated test is in GItHub
\noindent\textbf{Conclusion Threats.} Conclusion threats of our study include (1) overfitting of our dataset and (2) subjectivity of ground truth construction. To ensure that the matching and repair tasks do not overlap with the training dataset of ChatGPT to minimize the possibility of overfitting, we manually analyze the updated UI tests, and we have manually labeled and created a ground truth dataset that can be used to support future research in Web UI test repair. We mitigate the subjectivity of ground truth construction by cross-validating between two annotators during ground truth construction.  %We minimize (1) by constructing a new dataset that does not overlap with the training set of the Codex model. In the experiment, the program generation, and program repair procedure are all automated, while the ground truth construction involves subjective opinions, we minimize it by cross-validating between two annotators.

%and our data (initial solutions produced by Codex and all patches produced by APR tools) is publicly available at \url{https://github.com/apr4codex/ase2022}.

==> sections/sigproc.tex <==
% \documentclass{article}
% \begin{document}
% \nocite{*}
% \bibliography{sigproc}
% \bibliographystyle{plain}
% \end{document}

==> sigproc.tex <==
% \documentclass{article}
% \begin{document}
% \nocite{*}
% \bibliography{sigproc}
% \bibliographystyle{plain}
% \end{document}
